Building Machine Translation Systems for the Next Thousand Languages

In this paper we share findings from our effort to build practical machine translation (MT) systems capable of translating across over one thousand languages. We describe results in three research domains: (i) Building clean, web-mined datasets for 1500+ languages by leveraging semi-supervised pre-training for language identification and developing data-driven filtering techniques; (ii) Developing practical MT models for under-served languages by leveraging massively multilingual models trained with supervised parallel data for over 100 high-resource languages and monolingual datasets for an additional 1000+ languages; and (iii) Studying the limitations of evaluation metrics for these languages and conducting qualitative analysis of the outputs from our MT models, highlighting several frequent error modes of these types of models. We hope that our work provides useful insights to practitioners working towards building MT systems for currently understudied languages, and highlights research directions that can complement the weaknesses of massively multilingual models in data-sparse settings.

==> Next Thousand Languages/langid_results_tables.tex <==
\newcommand{\inserttfiifkappa}{
\begin{table*}
\centering
\begin{tabular}{ll|lllll}
\hline
\hline
 $\kappa$ &  $\tau$ & mean recall & median recall & mean $\delta_l$ & median $\delta_l$ & $\delta_l > 10$ \\
 \hline
 5000 & 1000 & 94.3 & 98.9 & 8.6 & 1.2 & 20 \\
 10000 & 1000 &  94.2 & 98.9 & 7.3 & 0.7 & 16 \\
 20000 & 1000 & 94.1 & 98.7 & 5.7 & 0.4 & 14 \\
 80000 & 1000 & 93.4 & 98.5 & 2.9 & 0.1 & 8 \\
 80000 & 2000 & 94.9 & 99.3 & 6.8 &  0.4 &  21  \\
\hline
\end{tabular}

\caption{Investigating the effect of varying the IIF-thresholding parameter $\kappa$ on the recall and distractibility ($\delta_l$) of \tfiif{} filtering, over 1598 languages. As we increase $\kappa$, the distractibility steadily trends down, with only small losses in recall. Increasing $\tau$ recoups lost recall but increases distractibility.}
\label{tab:tfiif_kappa}
\end{table*}
}

\newcommand{\insertdocumentconsistency}{
\begin{table*}
\centering
\begin{tabular}{l|r}
\hline
\hline
 range & \% of sentences \\
 \hline
$[0\%,  10\%)$   & 86.31\% \\
$[10\%, 20\%)$   & 6.55\% \\
$[20\%, 30\%)$   & 2.66\% \\
$[30\%, 40\%)$   & 1.55\% \\
$[40\%, 50\%)$   & 0.97\% \\
$[50\%, 60\%)$   & 0.67\% \\
$[60\%, 70\%)$   & 0.34\% \\
$[70\%, 80\%)$   & 0.21\% \\
$[80\%, 90\%)$   & 0.21\% \\
$[90\%, 100\%)$    & 0.25\% \\
$100\%$  & 0.30\% \\
\hline
\end{tabular}

\caption{Histogram of document-consistency scores, using a 1745-language CLD3 LangID model, on web text.}
\label{tab:documentconsistency}
\end{table*}
}

==> Next Thousand Languages/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Next Thousand Languages/mt_results_tables.tex <==


\newcommand{\insertmtcapacity}{\begin{table}[t]
\centering
\begin{tabular}{lcccccccccc}
\toprule
                   & \multicolumn{2}{c}{en-mfa}    & \multicolumn{2}{c}{en-ff}     & \multicolumn{2}{c}{en-mni}    & \multicolumn{2}{c}{en-kri}    & \multicolumn{2}{c}{en-mad} \\
Mono Size          & \multicolumn{2}{c}{7k}      & \multicolumn{2}{c}{86k}     & \multicolumn{2}{c}{106k}    & \multicolumn{2}{c}{129k}   & \multicolumn{2}{c}{138k} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
                   \midrule
1.5B  & 57.8 &	\textbf{26.0} & 33.7 &	\textbf{31.1} & 54.8 &	\textbf{35.7} & 48.7 &	\textbf{32.7} & 44.9 &	\textbf{29.8}\\
6B & \textbf{62.1} & 	17.9 & \textbf{34.3} & 	25.0  & 55.1 & 	31.9  & \textbf{54.8} & 	28.2 &  \textbf{52.0} & 	25.9 \\
\midrule
\midrule
                       & \multicolumn{2}{c}{en-doi}     & \multicolumn{2}{c}{en-bm}    & \multicolumn{2}{c}{en-ban}     & \multicolumn{2}{c}{en-quc}    & \multicolumn{2}{c}{en-ady}\\
Mono Size          & \multicolumn{2}{c}{179k}     & \multicolumn{2}{c}{187k}      & \multicolumn{2}{c}{188k}     & \multicolumn{2}{c}{250k}    & \multicolumn{2}{c}{296k} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
      \midrule
1.5B  & 57.4 &	\textbf{29.9} & 27.6 &	28.7 & 32.2 &	\textbf{31.8} & 24.4 &	\textbf{22.8} & 53.7 &	\textbf{21.8} \\
6B &  \textbf{60.4} & 	24.4  & \textbf{33.4} & 	28.5 &  \textbf{35.5} & 	29.4 &  \textbf{27.5} & 	22.2 &  \textbf{56.0} & 	21.4 \\
\midrule
\midrule     & \multicolumn{2}{c}{en-av} 
                      & \multicolumn{2}{c}{en-gom*}     & \multicolumn{2}{c}{en-iso*}    & \multicolumn{2}{c}{en-yua}     & \multicolumn{2}{c}{en-min}      \\
Mono Size           & \multicolumn{2}{c}{301k}  & \multicolumn{2}{c}{311k}     & \multicolumn{2}{c}{409k}      & \multicolumn{2}{c}{419k}     & \multicolumn{2}{c}{533k} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1.5B   & 48.1 &	26.1 & 50.7 &	1.1 &
17.9 &	16.5  &34.6 &	30.6 &
58.8 &	51.8 \\
6B &  \textbf{50.5} & 	\textbf{27.3} &  \textbf{53.3} & 	0.9 &  \textbf{19.3} & 	16.8 &  \textbf{39.3} & 	\textbf{31.3} &  \textbf{62.6} & 	\textbf{54.1} \\
\midrule
\midrule     & \multicolumn{2}{c}{en-bho}    & \multicolumn{2}{c}{en-kl*} & \multicolumn{2}{c}{en-qu}    & \multicolumn{2}{c}{en-gn}
                      & \multicolumn{2}{c}{en-bbc}      \\
Mono Size               & \multicolumn{2}{c}{734k}    & \multicolumn{2}{c}{741k}  & \multicolumn{2}{c}{842k}   & \multicolumn{2}{c}{861k} & \multicolumn{2}{c}{923k}    \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1.5B &
54.8&	38.9&
18.4&	12.5  &
29.9 &	29.8 &
26.7 &	24.3 &
40.9 &	34.9\\
6B&  
\textbf{56.9}&	38.8&
\textbf{20.0}&	\textbf{13.0} & \textbf{32.7} & 	30.2 &  \textbf{35.6} & 	\textbf{28.8} &  \textbf{43.9} & 	\textbf{35.6}  \\
\midrule
\midrule      & \multicolumn{2}{c}{en-skr}    & \multicolumn{2}{c}{en-ak}    & \multicolumn{2}{c}{en-ts*}    & \multicolumn{2}{c}{en-mai}    & \multicolumn{2}{c}{en-ce}
                          \\
Mono Size           & \multicolumn{2}{c}{974k}      & \multicolumn{2}{c}{1.29m}     & \multicolumn{2}{c}{1.3m}    & \multicolumn{2}{c}{1.35m}   & \multicolumn{2}{c}{1.36m}   \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1.5B   &
44.4 &	\textbf{32.8} &
31.7 &	32.1 &
25.5 &	17.4 &
57.8 &	\textbf{34.1} &
44.6 &	23.5 \\
6B&  \textbf{46.1} & 	28.5 &  \textbf{34.6} & 	\textbf{32.8} &  \textbf{28.3} & 	17.5 &  \textbf{59.9} & 	32.5 &  \textbf{48.1} & 	\textbf{24.4} \\
\midrule
\midrule     & \multicolumn{2}{c}{en-pcm}     & \multicolumn{2}{c}{en-nso}   & \multicolumn{2}{c}{en-ilo}     & \multicolumn{2}{c}{en-cv}    & \multicolumn{2}{c}{en-ti} \\
Mono Size          & \multicolumn{2}{c}{1.59m}     & \multicolumn{2}{c}{1.87m}    & \multicolumn{2}{c}{2.6m}     & \multicolumn{2}{c}{2.9m}    & \multicolumn{2}{c}{3.9m} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1.5B   &
\textbf{54.9} &	\textbf{54.7} &
45.8 &	45  &
\textbf{50.8} &	\textbf{49.7} &
39.9 &	\textbf{28.1} &
37.9	 &19.9\\
6B  &  52.5 & 	52.4 &  \textbf{49.1} & 	\textbf{46.9} &  
39.9 & 	47.8 &
\textbf{44.4} & 	27.5 &  
\textbf{40.9} & 	20.0\\
\midrule
\midrule       & \multicolumn{2}{c}{en-om}
                      & \multicolumn{2}{c}{en-sa}  & \multicolumn{2}{c}{en-dv}    & \multicolumn{2}{c}{en-lus*}     & \multicolumn{2}{c}{en-as}    \\
Mono Size              & \multicolumn{2}{c}{5.6m}  & \multicolumn{2}{c}{6.2m}  & \multicolumn{2}{c}{7.9m}     & \multicolumn{2}{c}{8.3m}    & \multicolumn{2}{c}{9.3m}  \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1.5B &
32.1	 &36 &
43.5 &	\textbf{26.9}   &
\textbf{37} &	\textbf{43.2} &
22.6 &	16.9 &
\textbf{52.9} &	36.3\\
6B &  
\textbf{37.0} & 	\textbf{36.7} &  
\textbf{45.8} & 	24.7&  35.8 & 	39.2 &  \textbf{33.0} & 	\textbf{19.1} &  49.6 & 	36.2   \\
\midrule         & \multicolumn{2}{c}{en-mzn}    & \multicolumn{2}{c}{en-bew}  & \multicolumn{2}{c}{en-ckb*}    & & & \multicolumn{2}{c}{\textbf{Average}} \\

Mono Size       & \multicolumn{2}{c}{11.6m}   & \multicolumn{2}{c}{33.3m}  & \multicolumn{2}{c}{76.9m}    &  & \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ && &$\leftarrow$  & $\rightarrow$  \\
         \midrule

1.5B &
50 &	\textbf{41.3} &
49.8 &	\textbf{45.7}  &
46.6 & 40.8\\
6B  &  \textbf{53.3} & 	40.2 &  \textbf{51.6} & 	44.0 &  
\textbf{51.7} & \textbf{41.6}&
&&
\textbf{+2.7} & \textbf{-1.0}\\
\bottomrule
\end{tabular}
\caption{Comparison of our 206-language 1.5B and 6B models trained on supervised data from 112 languages to and from English and monolingual data from 206 languages. Languages marked with * weren't included in the set of 206 languages, so monolingual data was not used for these languages in this experiment.}
\label{tab:mtcapacity}
\end{table}
}







\newcommand{\insertmtmultilinguality}{\begin{table}[t]
\centering
\begin{tabular}{lcccccccccc}
\toprule
                   & \multicolumn{2}{c}{en-mfa}    & \multicolumn{2}{c}{en-ff}     & \multicolumn{2}{c}{en-mni}    & \multicolumn{2}{c}{en-kri}    & \multicolumn{2}{c}{en-mad} \\
Mono Size          & \multicolumn{2}{c}{7k}      & \multicolumn{2}{c}{86k}     & \multicolumn{2}{c}{106k}    & \multicolumn{2}{c}{129k}   & \multicolumn{2}{c}{138k} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
                   \midrule
200L & 62.1 & 	17.9 & 34.3 & 	25.0  & 55.1 & 	31.9  & 54.8 & 	28.2 &  \textbf{52.0} & 	25.9 \\
1000L&
\textbf{65.4}&	\textbf{27.5}&
\textbf{41.2}&	\textbf{32.3}&
\textbf{56.4}&	\textbf{38.2}&
\textbf{56.5}&	\textbf{34.9}&
50.5&	\textbf{30.2}\\
\midrule
\midrule
                       & \multicolumn{2}{c}{en-doi}     & \multicolumn{2}{c}{en-bm}    & \multicolumn{2}{c}{en-ban}     & \multicolumn{2}{c}{en-quc}    & \multicolumn{2}{c}{en-ady}\\
Mono Size          & \multicolumn{2}{c}{179k}     & \multicolumn{2}{c}{187k}      & \multicolumn{2}{c}{188k}     & \multicolumn{2}{c}{250k}    & \multicolumn{2}{c}{296k} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
      \midrule
200L &  60.4 & 	24.4  & 33.4 & 	28.5 &  35.5 & 	29.4 &  \textbf{27.5} & 	22.2 & \textbf{56.0} & 	21.4 \\
1000L&
\textbf{63.1}&	\textbf{25.5}&
\textbf{36.3}&	\textbf{34.3}&
35.4&	\textbf{33.1}&
26.7&	\textbf{22.9}&
54.8&	\textbf{28.2}\\
\midrule
\midrule     & \multicolumn{2}{c}{en-av} 
                      & \multicolumn{2}{c}{en-gom*}     & \multicolumn{2}{c}{en-iso*}    & \multicolumn{2}{c}{en-yua}     & \multicolumn{2}{c}{en-min}      \\
Mono Size           & \multicolumn{2}{c}{301k}  & \multicolumn{2}{c}{311k}     & \multicolumn{2}{c}{409k}      & \multicolumn{2}{c}{419k}     & \multicolumn{2}{c}{533k} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

200L &  \textbf{50.5} & 	27.3 &  53.3 & 	0.9 &  19.3 & 	16.8 &  39.3 & 	31.3 &  62.6 & 	54.1 \\
1000L &
48.1&	\textbf{28.1}&
\textbf{55.5}&	\textbf{39.1}&
\textbf{29.4}&	\textbf{30.5}&
\textbf{40.7}&	31.6&
62.4&	\textbf{56.1}\\
\midrule
\midrule     & \multicolumn{2}{c}{en-bho}    & \multicolumn{2}{c}{en-kl*} & \multicolumn{2}{c}{en-qu}    & \multicolumn{2}{c}{en-gn}
                      & \multicolumn{2}{c}{en-bbc}      \\
Mono Size               & \multicolumn{2}{c}{734k}    & \multicolumn{2}{c}{741k}  & \multicolumn{2}{c}{842k}   & \multicolumn{2}{c}{861k} & \multicolumn{2}{c}{923k}    \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

200L &  
56.9&	38.8&
20.0&	13.0& 32.7 & 	30.2 &  35.6 & 	28.8 &  43.9 & 	35.6 \\
1000L &  
\textbf{58.3}&	\textbf{40.6}&
\textbf{29.7}&	\textbf{23.1}&
32.5&	\textbf{33.1}&
\textbf{38.9}&	\textbf{32.2}&
44.0	&35.4\\
\midrule
\midrule      & \multicolumn{2}{c}{en-skr}    & \multicolumn{2}{c}{en-ak}    & \multicolumn{2}{c}{en-ts*}    & \multicolumn{2}{c}{en-mai}    & \multicolumn{2}{c}{en-ce}
                          \\
Mono Size           & \multicolumn{2}{c}{974k}      & \multicolumn{2}{c}{1.29m}     & \multicolumn{2}{c}{1.3m}    & \multicolumn{2}{c}{1.35m}   & \multicolumn{2}{c}{1.36m}   \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

200L  &  46.1 & 	28.5 &  34.6 & 	32.8&  28.3 & 	17.5 &  59.9 & 	32.5 &  \textbf{48.1} & 	\textbf{24.4} \\
1000L &
\textbf{48.4}&	\textbf{31.3}&
\textbf{36.3}&	\textbf{34.3}&
\textbf{43.0}	&\textbf{45.5}&
\textbf{61.6}&	\textbf{37.6}&
44.9&	23.7\\
\midrule
\midrule     & \multicolumn{2}{c}{en-pcm}     & \multicolumn{2}{c}{en-nso}   & \multicolumn{2}{c}{en-ilo}     & \multicolumn{2}{c}{en-cv}    & \multicolumn{2}{c}{en-ti} \\
Mono Size          & \multicolumn{2}{c}{1.59m}     & \multicolumn{2}{c}{1.87m}    & \multicolumn{2}{c}{2.6m}     & \multicolumn{2}{c}{2.9m}    & \multicolumn{2}{c}{3.9m} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

200L &  \textbf{52.5} & 	52.4 &  49.1 & 	\textbf{46.9} &
39.9 & 	47.8 &
44.4 & 	27.5 &
40.9 & 	20.0\\
1000L &
51.2&	\textbf{53.5}&
\textbf{51.3}&	41.6&
\textbf{43.4}&	\textbf{52.4}&
\textbf{46.3}&	\textbf{32.1}&
\textbf{44.2}&	\textbf{21.1}\\
\midrule
\midrule       & \multicolumn{2}{c}{en-om}
                      & \multicolumn{2}{c}{en-sa}  & \multicolumn{2}{c}{en-dv}    & \multicolumn{2}{c}{en-lus}     & \multicolumn{2}{c}{en-as}    \\
Mono Size              & \multicolumn{2}{c}{5.6m}  & \multicolumn{2}{c}{6.2m}  & \multicolumn{2}{c}{7.9m}     & \multicolumn{2}{c}{8.3m}    & \multicolumn{2}{c}{9.3m}  \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

200L  &  
37.0 & 	36.7 &
45.8 & 	24.7 &  
35.8 & 	39.2 &  
33.0 & 	19.1 &  
49.6 & 	36.2\\
1000L&
\textbf{38.1}&	\textbf{39.1}&
\textbf{46.3}&	\textbf{28.4}&
\textbf{45.2}&	\textbf{43.7}&
\textbf{34.5}&	\textbf{39.3}&
\textbf{58.6}&	\textbf{36.7}\\
\midrule         & \multicolumn{2}{c}{en-mzn}    & \multicolumn{2}{c}{en-bew}  & \multicolumn{2}{c}{en-ckb*}    & & & \multicolumn{2}{c}{\textbf{Average}} \\

Mono Size       & \multicolumn{2}{c}{11.6m}   & \multicolumn{2}{c}{33.3m}  & \multicolumn{2}{c}{25.1m}    &  & \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ && &$\leftarrow$  & $\rightarrow$  \\
         \midrule

200L  & 
53.3 & 	40.2 & 
51.6 & 	44.0 &  
51.7 & 41.6\\
1000L &
\textbf{55.2}&	\textbf{41.4}&
51.8&	\textbf{46.0} &
\textbf{54.4}&	41.6
&&&
\textbf{+2.5} & \textbf{+5.3}\\
\bottomrule
\end{tabular}
\caption{Comparison of our 206-language 6B and 1000-language 6B models trained on monolingual data from 206 languages and 1000 languages respectively, while sharing supervised data from 112 languages. Languages marked with * weren't included in the set of 206 languages, so monolingual data was not used for these languages in the baseline model, and the 1000-language model consequently sees larger performance improvements.}
\label{tab:mtmultilinguality}
\end{table}
}







\newcommand{\insertmtfinetuning}{\begin{table}[t]
\centering
\begin{tabular}{lcccccccccc}
\toprule
                       & \multicolumn{2}{c}{en-ff}     & \multicolumn{2}{c}{en-mni}    & \multicolumn{2}{c}{en-kri}& \multicolumn{2}{c}{en-doi}     & \multicolumn{2}{c}{en-bm}     \\
Mono Size          & \multicolumn{2}{c}{86k}     & \multicolumn{2}{c}{106k}    & \multicolumn{2}{c}{129k} & \multicolumn{2}{c}{179k}     & \multicolumn{2}{c}{187k}   \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
                   \midrule
1000L&
41.2&	32.3&
56.4&	38.2&
56.5&	34.9&
63.1&	25.5&
36.3&	34.3\\
Finetuned&
\textbf{44.5}&	\textbf{35.7}&
\textbf{60.5}&	\textbf{40.8}&
\textbf{62.2}&	\textbf{36.8}&
\textbf{64.6}&	\textbf{37.2}&
\textbf{37.9}&	34.7\\
\midrule
\midrule
                            & \multicolumn{2}{c}{en-quc}
                      & \multicolumn{2}{c}{en-gom}     & \multicolumn{2}{c}{en-yua}& \multicolumn{2}{c}{en-bho}    & \multicolumn{2}{c}{en-kl}\\
Mono Size             & \multicolumn{2}{c}{250k}     &  \multicolumn{2}{c}{311k}     &  \multicolumn{2}{c}{419k}  & \multicolumn{2}{c}{734k}    & \multicolumn{2}{c}{741k} \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
      \midrule
1000L&
26.7&	22.9 &
55.5&	39.1&
40.7&	31.6 &  
58.3&	40.6&
29.7&	23.1\\
Finetuned&
\textbf{29.2}&	\textbf{23.5}&
\textbf{57.5}&	\textbf{40.0}&
\textbf{43.0}&   31.8 &  
\textbf{60.5}&	\textbf{41.4}&
\textbf{39.1}&	\textbf{27.8}\\
\midrule
\midrule
                          & \multicolumn{2}{c}{en-qu}    & \multicolumn{2}{c}{en-gn} & \multicolumn{2}{c}{en-ak} & \multicolumn{2}{c}{en-ts}    & \multicolumn{2}{c}{en-mai}      \\
Mono Size            & \multicolumn{2}{c}{842k}   & \multicolumn{2}{c}{861k}    & \multicolumn{2}{c}{1.29m}& \multicolumn{2}{c}{1.3m}    & \multicolumn{2}{c}{1.35m}   \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1000L&
32.5&	33.1&
38.9&	32.2&
36.3&	34.3&
43.0	&45.5&
61.6&	37.6\\
Finetuned&
\textbf{35.3}&	\textbf{36.1}&
\textbf{42.7}&	32.3&
\textbf{38.6}&	34.1&
\textbf{46.2}&	\textbf{46.5}&
\textbf{64.3}&	\textbf{39.2}\\
\midrule
\midrule       & \multicolumn{2}{c}{en-pcm}     & \multicolumn{2}{c}{en-nso}    & \multicolumn{2}{c}{en-ilo}     & \multicolumn{2}{c}{en-ti}    & \multicolumn{2}{c}{en-om} \\
Mono Size           & \multicolumn{2}{c}{1.59m}     & \multicolumn{2}{c}{1.87m}      & \multicolumn{2}{c}{2.6m}     & \multicolumn{2}{c}{3.9m}   & \multicolumn{2}{c}{5.6m} \\
            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1000L &
51.2&	53.5&
51.3&	41.6&
43.4&	52.4&
44.2&	21.1&
38.1&	39.1\\
Finetuned&
\textbf{59.3}&	\textbf{54.5}&
\textbf{52.2}&	\textbf{45.4}&
\textbf{61.7}&	\textbf{53.4}&
\textbf{46.0}&	21.0&
\textbf{41.2}&	\textbf{39.9}\\
\midrule
\midrule   
                      & \multicolumn{2}{c}{en-sa}       & \multicolumn{2}{c}{en-dv}   & \multicolumn{2}{c}{en-lus}     & \multicolumn{2}{c}{en-as}  & \multicolumn{2}{c}{en-ckb} \\
Mono Size            & \multicolumn{2}{c}{6.2m}    & \multicolumn{2}{c}{7.9m}  & \multicolumn{2}{c}{8.3m}    & \multicolumn{2}{c}{9.3m}  & \multicolumn{2}{c}{25.1m}\\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

1000L&
46.3&	28.4 &
45.2&	43.7&
34.5&	39.3&
58.6&	36.7&
54.4&	41.6\\
Finetuned&
\textbf{49.0}	&\textbf{30.9}&
\textbf{47.3}&	43.8&
\textbf{40.0}	&\textbf{40.3}&
\textbf{59.8}&	\textbf{39.0} &  
54.7&	\textbf{42.7}\\
\bottomrule
\end{tabular}
\caption{Comparison of our 1000-language 6B models against the 30-language version fine-tuned from this model. Scores are shown for the languages that were fine-tuned on.}
\label{tab:mtfinetuning}
\end{table}
}







\newcommand{\insertmtfiltering}{\begin{table}[t]
\centering
\begin{tabular}{lcccccccccc}
\toprule
                       & \multicolumn{2}{c}{en-ff}     & \multicolumn{2}{c}{en-mni}    & \multicolumn{2}{c}{en-kri}& \multicolumn{2}{c}{en-doi}     & \multicolumn{2}{c}{en-bm}     \\
Mono Size          & \multicolumn{2}{c}{86k}     & \multicolumn{2}{c}{106k}    & \multicolumn{2}{c}{129k} & \multicolumn{2}{c}{179k}     & \multicolumn{2}{c}{187k}   \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
                   \midrule
Finetuned&
44.5&	35.7&
60.5&	40.8&
62.2&	\textbf{36.8}&
64.6&	37.2&
37.9&	34.7\\
Filtered&
\textbf{45.3}&	35.3&
\textbf{62.1}&	40.8&
\textbf{64.2}&	35.4&
\textbf{65.5}&	36.9&
\textbf{38.4}&	34.7\\
\midrule
\midrule
                            & \multicolumn{2}{c}{en-quc}
                      & \multicolumn{2}{c}{en-gom}     & \multicolumn{2}{c}{en-yua} & \multicolumn{2}{c}{en-bho}    & \multicolumn{2}{c}{en-kl}\\
Mono Size             & \multicolumn{2}{c}{250k}     &  \multicolumn{2}{c}{311k}     &  \multicolumn{2}{c}{419k}  & \multicolumn{2}{c}{734k}    & \multicolumn{2}{c}{741k}  \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
      \midrule
Finetuned&
29.2&	23.5&
57.5&	40&
43	&31.8 &  
60.5&	41.4&
39.1&	27.8\\
Filtered&
\textbf{29.8}&	23.5&
57.9&	\textbf{40.8}&
\textbf{43.7}&	32.0 &  
60.9&	41.2&
39.0&	\textbf{35.8}\\

\midrule
\midrule
                        &   \multicolumn{2}{c}{en-qu}    & \multicolumn{2}{c}{en-gn}& \multicolumn{2}{c}{en-ak} & \multicolumn{2}{c}{en-ts}    & \multicolumn{2}{c}{en-mai}        \\
Mono Size            & \multicolumn{2}{c}{842k}   & \multicolumn{2}{c}{861k}    & \multicolumn{2}{c}{1.29m}& \multicolumn{2}{c}{1.3m}    & \multicolumn{2}{c}{1.35m}   \\

            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

Finetuned&
35.3&	36.1&
42.7&	32.3&
38.6&	34.1&
46.2&	46.5&
64.3&	39.2\\
Filtered&
35.3&	35.7&
43.0&	32.1&
38.6&	34.3&
\textbf{47.5}&	46.5&
\textbf{65.5}&	39.2\\
\midrule
\midrule      & \multicolumn{2}{c}{en-pcm}     & \multicolumn{2}{c}{en-nso}  & \multicolumn{2}{c}{en-ilo}     & \multicolumn{2}{c}{en-ti}    & \multicolumn{2}{c}{en-om} \\
Mono Size              & \multicolumn{2}{c}{1.59m}     & \multicolumn{2}{c}{1.87m}  & \multicolumn{2}{c}{2.6m}     & \multicolumn{2}{c}{3.9m}   & \multicolumn{2}{c}{5.6m} \\
            Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\
         \midrule

Finetuned&
59.3&	54.5&
52.2&	45.4&
61.7&	53.4&
46.0&	21.0&
\textbf{41.2}&	39.9\\
Filtered &
\textbf{64.6}&	\textbf{57.2}&
52.5&	\textbf{47.1}&
\textbf{62.7}&	\textbf{54.1}&
46.1&	21.5&
40.7&	40.0\\
\midrule
\midrule   
                      & \multicolumn{2}{c}{en-sa}       & \multicolumn{2}{c}{en-dv}   & \multicolumn{2}{c}{en-lus}     & \multicolumn{2}{c}{en-as}  & \multicolumn{2}{c}{en-ckb} \\
Mono Size            & \multicolumn{2}{c}{6.2m}    & \multicolumn{2}{c}{7.9m}  & \multicolumn{2}{c}{8.3m}    & \multicolumn{2}{c}{9.3m}  & \multicolumn{2}{c}{25.1m}\\
         \midrule

Finetuned&
49.0	&30.9&
47.3&	43.8&
40.0	&\textbf{40.3}&
59.8&	39.0 &  
54.7&	42.7\\
Filtered&
49.2&	31.0&
\textbf{48.4}&	\textbf{45.0}&
\textbf{42.1}&	39.7&
\textbf{60.6}&	\textbf{39.6} &  
\textbf{55.3}&	42.6\\
\bottomrule
\end{tabular}
\caption{Comparison of our 30-language fine-tuned model against one fine-tuned with RTT and LangID filtered data.}
\label{tab:mtfiltering}
\end{table}
}










\newcommand{\insertdistilledperf}{\begin{table}[t]

\centering
\small
\begin{tabular}{l|r:rrrrrrr:r:r}
LP & avg & 0 & 1 & 2 & 3 & 4 & 5 & 6 & entropy & \chrf{} \\
\hline
% en & 	ti & 	5.4 & 	0 & 	0 & 	1 & 	4 & 	11 & 	18 & 	66 & 	0.45 & 	22.0 \\ 
% en & 	ay & 	5.1 & 	0 & 	0 & 	2 & 	5 & 	17 & 	36 & 	40 & 	0.56 & 	33.3 \\ 
% en & 	bm & 	5 & 	0 & 	1 & 	1 & 	3 & 	22 & 	40 & 	34 & 	0.55 & 	36.6 \\ 
% en & 	ts & 	4.9 & 	1 & 	0 & 	2 & 	6 & 	24 & 	32 & 	37 & 	0.59 & 	46.5 \\ 
% en & 	lus & 	4.9 & 	3 & 	0 & 	5 & 	0 & 	33 & 	13 & 	47 & 	0.55 & 	41.1 \\ 
% en & 	ilo & 	4.7 & 	0 & 	0 & 	3 & 	2 & 	25 & 	64 & 	7 & 	0.44 & 	54.8 \\ 
% en & 	ff & 	4.6 & 	1 & 	1 & 	4 & 	7 & 	24 & 	45 & 	18 & 	0.61 & 	37.2 \\ 
% en & 	ln & 	4.6 & 	0 & 	0 & 	3 & 	10 & 	28 & 	41 & 	18 & 	0.61 & 	34.9 \\ 
% en & 	doi & 	4.5 & 	0 & 	0 & 	2 & 	3 & 	38 & 	50 & 	6 & 	0.49 & 	40.9 \\ 
% en & 	kri & 	4.4 & 	0 & 	2 & 	9 & 	14 & 	26 & 	23 & 	27 & 	0.71 & 	36.6 \\ 
% en & 	om & 	4.4 & 	0 & 	0 & 	3 & 	10 & 	42 & 	37 & 	8 & 	0.56 & 	40.3 \\ 
% en & 	dv & 	4.1 & 	2 & 	2 & 	8 & 	12 & 	33 & 	29 & 	14 & 	0.71 & 	45.6 \\ 
% en & 	sa & 	4.1 & 	4 & 	1 & 	3 & 	7 & 	52 & 	30 & 	4 & 	0.57 & 	33.3 \\ 
% en & 	as & 	4 & 	0 & 	0 & 	4 & 	12 & 	60 & 	23 & 	0 & 	0.47 & 	40.8 \\ 
% en & 	gom & 	4 & 	4 & 	1 & 	14 & 	11 & 	38 & 	12 & 	21 & 	0.71 & 	41.5 \\ 
% en & 	lg & 	3.9 & 	0 & 	8 & 	11 & 	18 & 	22 & 	25 & 	16 & 	0.76 & 	39.7 \\ 
% en & 	ak & 	3.8 & 	0 & 	0 & 	19 & 	0 & 	69 & 	0 & 	12 & 	0.39 & 	34.6 \\ 
% en & 	ckb & 	3.6 & 	1 & 	2 & 	14 & 	32 & 	30 & 	13 & 	9 & 	0.7 & 	44.3 \\ 
% en & 	nso & 	3.4 & 	7 & 	13 & 	13 & 	16 & 	19 & 	19 & 	14 & 	0.83 & 	47.6 \\ 
% en & 	kl & 	3.2 & 	13 & 	3 & 	19 & 	13 & 	29 & 	10 & 	13 & 	0.79 & 	40.7 \\ 
% en & 	mni-Mtei & 	3.2 & 	0 & 	0 & 	24 & 	32 & 	43 & 	1 & 	0 & 	0.51 & 	47.7 \\ 
% en & 	gn & 	3.1 & 	0 & 	8 & 	30 & 	18 & 	35 & 	8 & 	2 & 	0.66 & 	32.2 \\ 
% en & 	qu & 	3.1 & 	4 & 	4 & 	20 & 	30 & 	36 & 	6 & 	0 & 	0.65 & 	37.2 \\ 
% en & 	ee & 	3 & 	7 & 	14 & 	18 & 	21 & 	19 & 	12 & 	9 & 	0.82 & 	39.9 \\ 
% en & 	mai & 	3 & 	8 & 	1 & 	30 & 	20 & 	30 & 	8 & 	4 & 	0.71 & 	40.2 \\ 
% en & 	pcm & 	2.7 & 	20 & 	9 & 	22 & 	4 & 	27 & 	10 & 	9 & 	0.78 & 	57.5 \\ 
% en & 	bho & 	2.3 & 	0 & 	6 & 	70 & 	14 & 	8 & 	1 & 	0 & 	0.44 & 	42.4 \\ 
% en & 	yua & 	2.1 & 	0 & 	30 & 	42 & 	17 & 	8 & 	2 & 	1 & 	0.59 & 	32.8 \\ 
% \hdashline											
% ti & 	en & 	4.6 & 	0 & 	0 & 	3 & 	9 & 	31 & 	37 & 	21 & 	0.62 & 	45.8 \\ 
% ay & 	en & 	4.8 & 	2 & 	1 & 	5 & 	6 & 	12 & 	48 & 	27 & 	0.61 & 	38.8 \\ 
% ln & 	en & 	4.8 & 	0 & 	1 & 	1 & 	6 & 	25 & 	46 & 	22 & 	0.58 & 	32.3 \\ 
% lg & 	en & 	5.6 & 	0 & 	1 & 	2 & 	3 & 	4 & 	8 & 	82 & 	0.34 & 	41.1 \\ 
% mni-Mtei & 	en & 	3.5 & 	0 & 	1 & 	20 & 	14 & 	65 & 	1 & 	0 & 	0.44 & 	62.9 \\ 
% bm & 	en & 	5.1 & 	0 & 	0 & 	0 & 	4 & 	12 & 	52 & 	32 & 	0.5 & 	38.7 \\ 
% ts & 	en & 	4.3 & 	1 & 	1 & 	8 & 	14 & 	27 & 	33 & 	17 & 	0.68 & 	47.5 \\ 
% lus & 	en & 	4.6 & 	4 & 	4 & 	5 & 	4 & 	13 & 	40 & 	31 & 	0.66 & 	41.7 \\ 
% ilo & 	en & 	4.6 & 	0 & 	0 & 	3 & 	3 & 	30 & 	59 & 	6 & 	0.47 & 	62.4 \\ 
% ff & 	en & 	4.6 & 	7 & 	1 & 	10 & 	4 & 	13 & 	11 & 	54 & 	0.63 & 	45.8 \\ 
% doi & 	en & 	4.6 & 	1 & 	0 & 	1 & 	4 & 	41 & 	33 & 	20 & 	0.56 & 	65.8 \\ 
% kri & 	en & 	5 & 	0 & 	1 & 	6 & 	8 & 	13 & 	18 & 	53 & 	0.59 & 	64.8 \\ 
% om & 	en & 	4.6 & 	0 & 	0 & 	1 & 	7 & 	37 & 	50 & 	7 & 	0.5 & 	41.9 \\ 
% dv & 	en & 	3.4 & 	0 & 	2 & 	19 & 	33 & 	33 & 	14 & 	0 & 	0.61 & 	48.7 \\ 
% sa & 	en & 	4.4 & 	0 & 	1 & 	1 & 	4 & 	55 & 	33 & 	6 & 	0.48 & 	48.9 \\ 
% as & 	en & 	5.2 & 	0 & 	2 & 	8 & 	2 & 	10 & 	15 & 	64 & 	0.51 & 	60.4 \\ 
% gom & 	en & 	5.5 & 	0 & 	0 & 	2 & 	1 & 	5 & 	30 & 	62 & 	0.43 & 	57.2 \\ 
% ak & 	en & 	4.8 & 	0 & 	1 & 	4 & 	9 & 	19 & 	31 & 	37 & 	0.64 & 	39.4 \\ 
% ckb & 	en & 	2.9 & 	4 & 	12 & 	27 & 	14 & 	36 & 	7 & 	0 & 	0.69 & 	56.4 \\ 
% nso & 	en & 	3.4 & 	2 & 	12 & 	14 & 	18 & 	34 & 	9 & 	12 & 	0.76 & 	52.8 \\ 
% kl & 	en & 	4.6 & 	2 & 	3 & 	11 & 	5 & 	25 & 	9 & 	46 & 	0.65 & 	39.6 \\ 
% gn & 	en & 	3.5 & 	0 & 	0 & 	12 & 	31 & 	49 & 	7 & 	1 & 	0.54 & 	43.6 \\ 
% qu & 	en & 	2.9 & 	0 & 	4 & 	28 & 	47 & 	18 & 	5 & 	0 & 	0.57 & 	35.6 \\ 
% ee & 	en & 	4.5 & 	3 & 	3 & 	8 & 	12 & 	13 & 	22 & 	39 & 	0.71 & 	37.3 \\ 
% mai & 	en & 	3.2 & 	0 & 	2 & 	38 & 	15 & 	25 & 	19 & 	0 & 	0.62 & 	65.4 \\ 
% pcm & 	en & 	4.6 & 	1 & 	0 & 	3 & 	7 & 	31 & 	39 & 	20 & 	0.61 & 	65.4 \\ 
% bho & 	en & 	3.4 & 	0 & 	0 & 	15 & 	44 & 	31 & 	10 & 	0 & 	0.56 & 	61.7 \\ 
% yua & 	en & 	3.4 & 	0 & 	1 & 	20 & 	36 & 	29 & 	13 & 	2 & 	0.63 & 	42.1 \\ 

en$\rightarrow$ti &     5.4 &   0 &     0 &     1 &     4 &     11 &    18 &    66 &    0.45 &  22.0 \\ 
en$\rightarrow$ay &     5.1 &   0 &     0 &     2 &     5 &     17 &    36 &    40 &    0.56 &  33.3 \\ 
en$\rightarrow$bm &     5.0 &   0 &     1 &     1 &     3 &     22 &    40 &    34 &    0.55 &  36.6 \\ 
en$\rightarrow$ts &     4.9 &   1 &     0 &     2 &     6 &     24 &    32 &    37 &    0.59 &  46.5 \\ 
en$\rightarrow$lus &    4.9 &   3 &     0 &     5 &     0 &     33 &    13 &    47 &    0.55 &  41.1 \\ 
en$\rightarrow$ilo &    4.7 &   0 &     0 &     3 &     2 &     25 &    64 &    7 &     0.44 &  54.8 \\ 
en$\rightarrow$ff &     4.6 &   1 &     1 &     4 &     7 &     24 &    45 &    18 &    0.61 &  37.2 \\ 
en$\rightarrow$ln &     4.6 &   0 &     0 &     3 &     10 &    28 &    41 &    18 &    0.61 &  34.9 \\ 
en$\rightarrow$doi &    4.5 &   0 &     0 &     2 &     3 &     38 &    50 &    6 &     0.49 &  40.9 \\ 
en$\rightarrow$kri &    4.4 &   0 &     2 &     9 &     14 &    26 &    23 &    27 &    0.71 &  36.6 \\ 
en$\rightarrow$om &     4.4 &   0 &     0 &     3 &     10 &    42 &    37 &    8 &     0.56 &  40.3 \\ 
en$\rightarrow$dv &     4.1 &   2 &     2 &     8 &     12 &    33 &    29 &    14 &    0.71 &  45.6 \\ 
en$\rightarrow$sa &     4.1 &   4 &     1 &     3 &     7 &     52 &    30 &    4 &     0.57 &  33.3 \\ 
en$\rightarrow$as &     4.0 &   0 &     0 &     4 &     12 &    60 &    23 &    0 &     0.47 &  40.8 \\ 
en$\rightarrow$gom &    4.0 &   4 &     1 &     14 &    11 &    38 &    12 &    21 &    0.71 &  41.5 \\ 
en$\rightarrow$lg &     3.9 &   0 &     8 &     11 &    18 &    22 &    25 &    16 &    0.76 &  39.7 \\ 
en$\rightarrow$ak &     3.8 &   0 &     0 &     19 &    0 &     69 &    0 &     12 &    0.39 &  34.6 \\ 
en$\rightarrow$ckb &    3.6 &   1 &     2 &     14 &    32 &    30 &    13 &    9 &     0.70 &  44.3 \\ 
en$\rightarrow$nso &    3.4 &   7 &     13 &    13 &    16 &    19 &    19 &    14 &    0.83 &  47.6 \\ 
en$\rightarrow$kl &     3.2 &   13 &    3 &     19 &    13 &    29 &    10 &    13 &    0.79 &  40.7 \\ 
en$\rightarrow$mni-Mtei &       3.2 &   0 &     0 &     24 &    32 &    43 &    1 &     0 &     0.51 &  47.7 \\ 
en$\rightarrow$gn &     3.1 &   0 &     8 &     30 &    18 &    35 &    8 &     2 &     0.66 &  32.2 \\ 
en$\rightarrow$qu &     3.1 &   4 &     4 &     20 &    30 &    36 &    6 &     0 &     0.65 &  37.2 \\ 
en$\rightarrow$ee &     3.0 &   7 &     14 &    18 &    21 &    19 &    12 &    9 &     0.82 &  39.9 \\ 
en$\rightarrow$mai &    3.0 &   8 &     1 &     30 &    20 &    30 &    8 &     4 &     0.71 &  40.2 \\ 
en$\rightarrow$pcm &    2.7 &   20 &    9 &     22 &    4 &     27 &    10 &    9 &     0.78 &  57.5 \\ 
en$\rightarrow$bho &    2.3 &   0 &     6 &     70 &    14 &    8 &     1 &     0 &     0.44 &  42.4 \\ 
en$\rightarrow$yua &    2.1 &   0 &     30 &    42 &    17 &    8 &     2 &     1 &     0.59 &  32.8 \\ 
\hdashline                                                                                      
ti$\rightarrow$en &     4.6 &   0 &     0 &     3 &     9 &     31 &    37 &    21 &    0.62 &  45.8 \\ 
ay$\rightarrow$en &     4.8 &   2 &     1 &     5 &     6 &     12 &    48 &    27 &    0.61 &  38.8 \\ 
ln$\rightarrow$en &     4.8 &   0 &     1 &     1 &     6 &     25 &    46 &    22 &    0.58 &  32.3 \\ 
lg$\rightarrow$en &     5.6 &   0 &     1 &     2 &     3 &     4 &     8 &     82 &    0.34 &  41.1 \\ 
mni-Mtei$\rightarrow$en &       3.5 &   0 &     1 &     20 &    14 &    65 &    1 &     0 &     0.44 &  62.9 \\ 
bm$\rightarrow$en &     5.1 &   0 &     0 &     0 &     4 &     12 &    52 &    32 &    0.50 &  38.7 \\ 
ts$\rightarrow$en &     4.3 &   1 &     1 &     8 &     14 &    27 &    33 &    17 &    0.68 &  47.5 \\ 
lus$\rightarrow$en &    4.6 &   4 &     4 &     5 &     4 &     13 &    40 &    31 &    0.66 &  41.7 \\ 
ilo$\rightarrow$en &    4.6 &   0 &     0 &     3 &     3 &     30 &    59 &    6 &     0.47 &  62.4 \\ 
ff$\rightarrow$en &     4.6 &   7 &     1 &     10 &    4 &     13 &    11 &    54 &    0.63 &  45.8 \\ 
doi$\rightarrow$en &    4.6 &   1 &     0 &     1 &     4 &     41 &    33 &    20 &    0.56 &  65.8 \\ 
kri$\rightarrow$en &    5.0 &   0 &     1 &     6 &     8 &     13 &    18 &    53 &    0.59 &  64.8 \\ 
om$\rightarrow$en &     4.6 &   0 &     0 &     1 &     7 &     37 &    50 &    7 &     0.50 &  41.9 \\ 
dv$\rightarrow$en &     3.4 &   0 &     2 &     19 &    33 &    33 &    14 &    0 &     0.61 &  48.7 \\ 
sa$\rightarrow$en &     4.4 &   0 &     1 &     1 &     4 &     55 &    33 &    6 &     0.48 &  48.9 \\ 
as$\rightarrow$en &     5.2 &   0 &     2 &     8 &     2 &     10 &    15 &    64 &    0.51 &  60.4 \\ 
gom$\rightarrow$en &    5.5 &   0 &     0 &     2 &     1 &     5 &     30 &    62 &    0.43 &  57.2 \\ 
ak$\rightarrow$en &     4.8 &   0 &     1 &     4 &     9 &     19 &    31 &    37 &    0.64 &  39.4 \\ 
ckb$\rightarrow$en &    2.9 &   4 &     12 &    27 &    14 &    36 &    7 &     0 &     0.69 &  56.4 \\ 
nso$\rightarrow$en &    3.4 &   2 &     12 &    14 &    18 &    34 &    9 &     12 &    0.76 &  52.8 \\ 
kl$\rightarrow$en &     4.6 &   2 &     3 &     11 &    5 &     25 &    9 &     46 &    0.65 &  39.6 \\ 
gn$\rightarrow$en &     3.5 &   0 &     0 &     12 &    31 &    49 &    7 &     1 &     0.54 &  43.6 \\ 
qu$\rightarrow$en &     2.9 &   0 &     4 &     28 &    47 &    18 &    5 &     0 &     0.57 &  35.6 \\ 
ee$\rightarrow$en &     4.5 &   3 &     3 &     8 &     12 &    13 &    22 &    39 &    0.71 &  37.3 \\ 
mai$\rightarrow$en &    3.2 &   0 &     2 &     38 &    15 &    25 &    19 &    0 &     0.62 &  65.4 \\ 
pcm$\rightarrow$en &    4.6 &   1 &     0 &     3 &     7 &     31 &    39 &    20 &    0.61 &  65.4 \\ 
bho$\rightarrow$en &    3.4 &   0 &     0 &     15 &    44 &    31 &    10 &    0 &     0.56 &  61.7 \\ 
yua$\rightarrow$en &    3.4 &   0 &     1 &     20 &    36 &    29 &    13 &    2 &     0.63 &  42.1 \\ 
\bottomrule
\end{tabular}
\caption{Performance of the distilled student model in \chrf{} and human evaluation, on a scale from 0 (nonsense/wrong language) to 6 (perfect). The value in the ``avg'' column reports the weighted average score across all sentences. The value under each of the numbers from 0 to 6 is the percent of sentences that were given that rating. The entropy is included to flag suspicious rating patterns: a low entropy may mean that most raters are assigning the same score to all sentences.}
\label{tab:distilledperf}
\end{table}
}

==> Next Thousand Languages/table_audit_instructions.tex <==



\newcommand{\insertauditinstructions}{\begin{table*}[ht]
% \small
\centering
\begin{tabular}{l|rp{0.8\linewidth}}
Code & Weight & 	Description \\ 
\hline
CC &  100	& Natural in-language sentence. It's ok if it has a few small issues, like spelling errors or a few words from another language, or if it's a sentence fragment of reasonable length (about 5 words or more) \\ 
\hdashline
CB & 	50 & In-language, but low-quality. This could be ungrammatical text, boilerplate, or very short fragments. \\ 
\hdashline
CA &  30 &	Correct but ambiguous whether it's in the correct language. This code is only applicable for dialects that are closely related to a major language. For instance, many short sentences in Gulf Arabic may also be valid in MSA, and many written Cantonese sentences might also be valid in Mandarin. \\ 
\hdashline
WD & 	20 & This sentence is in a related but different dialect to the language it's supposed to be in.  This code is only applicable for dialects that are closely related to a similar dialect. For instance, it's supposed to be in Sa'idi Arabic but it's in Egyptian Arabic. \\ 
\hdashline
WL &  0 &	Wrong Language, but still linguistic content \\ 
\hdashline
NL &  0 &	Not a language -- any sort of non-linguistic content. Proper nouns like ``Ibuprofin'', ``Calvin Klein'', or ``Washington DC'' also count as NL. \\ 
\hdashline


\end{tabular}
\caption{Instructions descriptions of the error codes we used to rate samples of our datasets, along with the weight each one is given in the combined quality score.
 \label{tab:audit_instructions}}
\end{table*}
}

==> Next Thousand Languages/table_bleu_vs_chrf.tex <==

% https://docs.google.com/spreadsheets/d/1L0k4YtK3dQ1sSmR7N0sLHb_Q5YSH18FRrJ3y5PxEm4Y/edit?resourcekey=0-vluzCspbPwsV7QXKmYNnfg#gid=789359841
\newcommand{\insertbleuvschrf}{
\begin{table*}
\centering
\small
\begin{tabular}{lrrr||lrrr}
\hline
\hline
% sl & tl &	bleu & 	chrf & 	ratio \\ 
lp &	\bleu{} & 	\chrf{} & 	ratio & lp &	\bleu{} & 	\chrf{} & 	ratio \\ 
\hline
% en & om & 	3.8 & 	40.1 & 	4.0 \\ 
% en & lg & 	3.7 & 	39.8 & 	4.0 \\ 
% en & dv & 	5.4 & 	45.5 & 	3.5 \\ 
% en & sa & 	2.8 & 	33.1 & 	3.5 \\ 
% en & qu & 	3.6 & 	36.2 & 	3.4 \\ 
% en & ln & 	3.5 & 	34.9 & 	3.2 \\ 
% en & kl & 	5.3 & 	40.6 & 	2.9 \\ 
% en & ay & 	4.6 & 	34.3 & 	2.4 \\ 
% en & ckb & 	9.4 & 	44.2 & 	1.9 \\ 
% en & gn & 	5.2 & 	32.1 & 	1.7 \\ 
% en & mai & 	8.6 & 	39.8 & 	1.7 \\ 
% en & as & 	9.6 & 	40.6 & 	1.6 \\ 
% en & mni-Mtei & 	12.9 & 	47.1 & 	1.6 \\ 
% en & ts & 	12.8 & 	46.7 & 	1.6 \\ 
% en & gom & 	10.8 & 	42.3 & 	1.6 \\ 
% en & ee & 	11.9 & 	40.5 & 	1.3 \\ 
% en & ff & 	9.9 & 	37.2 & 	1.3 \\ 
% en & bm & 	9.5 & 	36.4 & 	1.3 \\ 
% en & lus & 	13.2 & 	41.5 & 	1.2 \\ 
% en & kri & 	10.6 & 	36.2 & 	1.1 \\ 
% en & ilo & 	24.2 & 	54.9 & 	1.1 \\ 
% en & ak & 	10.4 & 	34.6 & 	1.0 \\ 
% en & nso & 	20.3 & 	47.6 & 	1.0 \\ 
% en & bho & 	16.7 & 	42.7 & 	1.0 \\ 
% en & doi & 	15.3 & 	40.7 & 	1.0 \\ 
% en & ti & 	3.7 & 	22.1 & 	0.4 \\ 

en$\rightarrow$om &     3.8 &   40.1 &  4.0  & en$\rightarrow$ts &      12.8 &  46.7 &  1.6 \\ 
en$\rightarrow$lg &     3.7 &   39.8 &  4.0  & en$\rightarrow$gom &     10.8 &  42.3 &  1.6 \\ 
en$\rightarrow$dv &     5.4 &   45.5 &  3.5  & en$\rightarrow$ee &      11.9 &  40.5 &  1.3 \\ 
en$\rightarrow$sa &     2.8 &   33.1 &  3.5  & en$\rightarrow$ff &      9.9 &   37.2 &  1.3 \\ 
en$\rightarrow$qu &     3.6 &   36.2 &  3.4  & en$\rightarrow$bm &      9.5 &   36.4 &  1.3 \\ 
en$\rightarrow$ln &     3.5 &   34.9 &  3.2  & en$\rightarrow$lus &     13.2 &  41.5 &  1.2 \\ 
en$\rightarrow$kl &     5.3 &   40.6 &  2.9  & en$\rightarrow$kri &     10.6 &  36.2 &  1.1 \\ 
en$\rightarrow$ay &     4.6 &   34.3 &  2.4  & en$\rightarrow$ilo &     24.2 &  54.9 &  1.1 \\ 
en$\rightarrow$ckb &    9.4 &   44.2 &  1.9  & en$\rightarrow$ak &      10.4 &  34.6 &  1.0 \\ 
en$\rightarrow$gn &     5.2 &   32.1 &  1.7  & en$\rightarrow$nso &     20.3 &  47.6 &  1.0 \\ 
en$\rightarrow$mai &    8.6 &   39.8 &  1.7  & en$\rightarrow$bho &     16.7 &  42.7 &  1.0 \\ 
en$\rightarrow$as &     9.6 &   40.6 &  1.6  & en$\rightarrow$doi &     15.3 &  40.7 &  1.0 \\ 
en$\rightarrow$mni-Mtei &       12.9 &  47.1 &  1.6  & en$\rightarrow$ti &      3.7 &   22.1 &  0.4 \\ 

\hline
\end{tabular}

\caption{\chrf{} versus \bleu{} scores on \enxx language pairs in the distilled model. Although it is almost impossible to compare these scores directly, as explained for a variety of reasons in the text, it is still clear that they give a very different picture of the performance on the languages. In order to make an approximate comparison between the two, we have included the ratio of the \scaledchrf{} score to the \bleu{} score. Language pairs in this table are sorted from the highest ratio (where \bleu{} underestimates performance) on the top to the lowest ratio on the bottom. As expected, polysynthetic and agglutinative languages are misjudged my \bleu{}.}
\label{tab:chrfvsbleu}
\end{table*}
}

% https://docs.google.com/document/d/1rFpb2RIzpmUtbak4_4NWOrCvx5A7q4L_pDhyw-r0C_A/edit#


==> Next Thousand Languages/table_clusters.tex <==

\begin{table*}
% \centering
\small
\begin{tabular}{l p{0.45\linewidth} | l p{0.45\linewidth}}
\hline
\hline
i & languages in cluster &  i & languages in cluster    \\
\hline

     1 & kfq,bns,bjj,lmn-Deva,hif-Deva,en-Deva,gom,hlb,kok,bhb,mai,ks-Deva,awa,bfy  & 2 & doi,gbm,myi,wry,xnr,mwr,raj,rwr,hoj,mtr,kfy,gdx, gju-Deva-IN,bfz,sd-Deva \\
     3 & sat-Deva,sjp,hne,dty,bho,sa,sck,sgj,unr-Deva-IN,mai-Latn,mag,hoc,rkt-Deva-IN  & 4 & vah,noe,bgc,wbr,ahr,swv,gon-Deva,vas,kru,bgq,brx,mjl,new \\
     5 & gwc,trw,hno,mki,scl,bal,hnd,phr,bft,dcc,plk,gjk, bgp-Arab & 6 & pa-Arab,gju,skr,doi-Arab,ks \\
     7 & tbc,aau,wos,kbq,buk,emi,tif,kew,nas,akh,nop,tlf, kjs,yby & 8 & dad,mmo,apz,mpt,amp,sny,omw,tbg,yuj,yuw,roo,wnu \\
     9 & gdr,aon,hla,lbb,ape,mlh,mhl,sll,dah,myw,gvf,ptp, kpw & 10 & btz,mui,bew,jax,gay,max,mfb,vkt,pmy,mkn,abs,xmm,mqy \\
    11 & meo,msi,min,cjm-Latn,kge,bss,ace,bbc,trp,kac,kha,prk & 12 & mdr,bgz,bug,ha,amo,iba,mhy \\
    13 & qxq,psi,kmz,tks,luz,fay,wne,psh,haz,lrl,hac,sdh,tly-IR,mvy & 14 & krj,ceb,bkd,hil,clu,hnn,mel,msb,abx,tsg,bik \\
    15 & mrw,cyo,bto,mdh,msk,pam,kqe,pag,ilo,agn,bku,bts, iry,kmk & 16 & sim,rro,bzh,gai,lcm,rai,ksd,leu,apb,sps,sgz,swp,kqw \\
    17 & iws,bef,enq,kyz,zia,kpf,kyg,avt,kyc,sue,mmx,kwj & 18 & sn,ngl,kri,kdn,co,seh,nyu,cjk,tum,ts,lon, ndc-ZW,pih,ny \\
    19 & tpz,aii,syc,arc,cr-Latn,hsb,pap,ach,syr-Syrn,syr & 20 & gng,knk,kno,sef,bm,fon,ada,dnj,dyu,msc,dga,bci,yre \\
    21 & fan,bbj,bum,bas,bsp,bba,tem,yal,sus,gso,sba & 22 & kv,av,ady,koi,kbd,mdf,udm,myv,dar \\
    23 & sah,mrj,tly-Cyrl-RU,kaa,chm,crh,kum,krc,xal,ba, az-RU,en-Cyrl,cv & 24 & cpb,mcb,cpu,vmw,cbu,cni,eko,apu,tsz,shp,mgh,cpy,pua \\
    25 & cax,guh,hub,ycn,mfi,cui,acu,ign & 26 & en-Arab,acx,apc,abv,acw,ber-Arab,acq,aeb,aec,afb \\
    27 & mde,mey,ar-MA,acm,apd-SD,gdq,ayl,arq,shu & 28 & kn-Latn,hi-Latn,te-Latn,ntp,sd-Latn,ta-Latn, mr-Latn,bgp,mbj,hif,gu-Latn,ml-Latn,gom-Latn \\
    29 & syl-Latn,bn-Latn,jiv,rhg-Latn,fo,se & 30 & cwe,kde,nym,vid,ngp,ziw,kdc,suk,zaj,ruf \\
    31 & dov,fip,kmb,mgw,kki,heh,ndj,poy,uli & 32 & otm,cuc,cnt,ctu,cle,chz,cpa,mzk,maq \\
    33 & maa,ots,mxb,ote,maj,kcg,otn,trs,trq & 34 & acf,gcf,frp,gcr,crs,rcf,oc,mfe,wa,io \\
    35 & pis,kl,vec,jbo,tpi,bi & 36 & mhi,nin,ajg,atg,iso,igb,ijc,lgg \\
    37 & ikw,eza,izz,anw,ibb,btt,mgd,pad & 38 & beo,knv,bmq,gor,bco,gur,kao,kus \\
    39 & knj,zpt,lgl,kwd,mor,pls,snp,udu & 40 & za,zh-Latn,zyj,mmr,cqd,mww-CN,ium,ii-Latn \\
    41 & lhu,tlh,mic,tob,poh,hni,mlp,pcc & 42 & luy,jaa,lg,sxb,nyn,cgg,xog,haq,nyo,rn,nnb,lsm,hay,myx,gwr \\
    43 & sbe,viv,wat,ssx,khs,dob,mox,tte,kud,tbo,bdd,bxh, mpx,aui & 44 & fuf,so,fub-Latn,fuv,ffm,snk,ymm,fue,srr,wlx,aa,ff,fuq \\
    45 & igl,ikk,kaa-Latn,ndz,nog,luc,dgr,yo,gkn, bcq-Latn,blh,bmv & 46 & soq,mcq,acn,bbr,bmh,byx,wer,mbh,wrs,agd,gfk \\
    47 & gag,kmz-Latn,zza,ar-Latn,bgx-Latn,wo, mde-Latn,tzo,brh-Latn,aly,aeb-Latn & 48 & kmu,spl,mva,snc,haw,meu,gah,npy,ho,mvn,khz \\
    49 & lua,quy,pri,gog,ae-Latn,quf,qul,quh,ay-PE,qu & 50 & wsk,bxg,bhg,aom,btd,nou,kpr,hvn,wuv,okv \\
    51 & gdn,asg,kqf,wed,tsw,brx-Latn,kdl,pwg,bbb,mwc & 52 & bch,gnn,myu,wro,cab,ssd,bnp,irk,djr,nak \\
    53 & rmo,kaq,smt,ctd-Latn,mkj,pon,bgs,pck,war & 54 & row,llg,txq,rgu,otd,bhw,twu,urb,nfa \\
    55 & wes,hwc,cmr,jam,kgp,icr,gyn,bzj,ury & 56 & faa,kpx,stn,stq,mzn,apr,lrc,bgn \\
    57 & ifk,xnn,ifa,bnc,ebk,kne,ifu,ifb & 58 & cce,st,toh,ve,tsc,led,tn,nso \\
    59 & hdy-Latn,gof,kbr,gmv-Latn,dwr,drs-Latn, ktb-Latn,wal & 60 & mih,gaw,tvk,vep,ssg,lid,ltg,os \\
    61 & rwo,ubu,tlb,wiu,mux,gbi,tby,ipi & 62 & stv,gez,kqy,ti,ktb,hdy,kxc,sgw \\
    63 & nys,xh,jid,nd,ss-SZ,nr,gup,zu & 64 & lef,kg,yaf,jbu,lu,ln,ktu,mkw \\
    65 & sxu,dje,got,ang,gsw,kr,mir & 66 & bzc,mg,tdx,bmm,skg,rkb,apy \\
    67 & nch,azz,ngu,ttc,ncl,nhe,nhw & 68 & tuv,dln,wap,teo,ik,kwi,bla \\
    69 & yka,bpr,ewo,caf,pez,bps,tbl & 70 & brx-Beng,syl,bpy,rkt,dv,ctg,grt \\
    71 & qvh,qvw,qxn,qub,qxo,qvm,qxh & 72 & unr-Latn,sat-Latn,gil,aoz,aaz,na \\
    73 & bhl,aey,jae,urt,azd,hot & 74 & agt,mpg,kue,nga,eri,zne \\
    75 & amf,nmz,om,hae,bud,lob & 76 & tzh,mbl,klt,arn,hlt,zyp \\
    77 & cao,ay,zsr,zar,zac,auc & 78 & lus,cbl,cnh,cfm,bgr,cdf \\
    79 & mna,tuc,geb,dnw,kvg,bmu & 80 & stv-Latn,itv,twb,fai,bnj,cuk \\
    81 & kmg,mpp,ded,bru,shj,yap & 82 & zpl,cbr,ztg,stp,kjb,zao \\
    83 & sri,noa,cbv,emp,tnc,cto & 84 & yua,chd,mam,hus,mop,chf \\
    85 & muy,dgc,due,prf,duo,xsb & 86 & pbb,pah,gun,gn,kgk,gyr \\
    87 & nna,ntj,wbp,mpj,gvn,wmt & 88 & nij,mvp,kje,lex,sda,mqj \\
    89 & wob,ktj,nwb,wwa,ted,nko & 90 & ak,acd,gub,abr,bkq \\
    91 & kkc,laj,kdi,alz,adh & 92 & ghs,agg,ian,nup,opm \\
    93 & uvl,ino,mee,mnb,ata & 94 & rop,ru-Latn,bg-Latn,el-Latn,tcs \\
\end{tabular}
\caption{Complete list of clusters used for the web crawl, based on the False Negative Rate of our n-gram CLD3 model. All singleton clusters are omitted from this table. Order of clusters is from largest to smallest, but reflects the superclusters that were broken by hand.
 \label{tab:clusters}}
\end{table*}



\begin{table*}
% \centering
\small
\begin{tabular}{l p{0.2\linewidth} | l p{0.2\linewidth} | l p{0.2\linewidth} | l p{0.2\linewidth} |}
\hline
\hline
i & languages in cluster &  i & languages in cluster &  i & languages in cluster  &  i & languages in cluster    \\
\hline
    95 & big,lww,bki,mas,bsn & 96 & cjv,tim,kgr,bom,yss &    97 & cdo,mnp,nan-Latn-TW,cnk,hak & 98 & nia,mej,ceg,kos,tet \\
    99 & hag,maw,dag,xed,cko & 100 & dts,oku,nhu,mur,cme &   101 & trc,zav,zpq,kia,cut & 102 & dgz,nvm,rap,mti,ja-Latn \\
   103 & dzg,gqr,mcn,ig,gvl & 104 & rim,mwe,tll,ng,kj &   105 & ksr,mh,kpj,kyq,myb & 106 & tnp,tnn,nwi,tly,tnk \\
   107 & qvo,quw,qvz,qvi,qxr & 108 & zpo,zaa,zap,zca,zpi &   109 & aby,amk,tqo,yrb & 110 & quc,usp,cak,acr \\
   111 & tgo,mad,aoi,ade & 112 & rug,tgp,rnl,akb &   113 & bus,bqp,akp,bqc & 114 & ood,alq,ber-Latn,gd \\
   115 & apw,atb,auy,kze & 116 & obo,msm,atd,mbd &   117 & for,usa,awb,mog & 118 & pko,awk,niq,sgc \\
   119 & jac,ayo,ch,zos & 120 & azg,zpc,chj,snn &   121 & bav,bfd,kyf,las & 122 & wmw,dug,nyf,bep \\
   123 & kvx,sd,mve,bgq-Arab & 124 & nsn,nho,nlg,bgt &   125 & gud,nfr,kma,biv & 126 & blz,loe,bjp,mwv \\
   127 & bjr,kup,nhi,ncj & 128 & bqj,klv,kto,bkv &   129 & blt-Latn,tyz,nut,mtq & 130 & boj,syb,suc,lnd \\
   131 & nzi,xrb,iri,bov & 132 & smk,br,kw,ivv &   133 & kwf,far,bvd,bvc & 134 & sua,mav,pss,bwu \\
   135 & izr,tiy,cjp,gum & 136 & mio,cta,mxt,mjc &   137 & zpu,zad,ixl,ctp & 138 & kms,med,upv,cwt \\
   139 & des,pir,gvc,tav & 140 & kmh,yut,dtb,dtp &   141 & ter,enx,sg,kkj & 142 & nyy,ess,jmc,nim \\
   143 & mek,yml,ksj,fj & 144 & gej,mkl,tbz,grb &   145 & unr-Orya,kxu,hlb-Orya,jun & 146 & tnr,ons,kgf,nca \\
   147 & mtp,sbl,sgb,kqp & 148 & xla,ktm,nss,pma &   149 & sm,tvl,mi,to & 150 & mzi,miz,mix,poe \\
   151 & xtd,mza,sja,mpm & 152 & vun,pkb,nnq,old &   153 & zpv,zab,zaw,toj & 154 & aak,cav,huu \\
   155 & kmo,dww,abt & 156 & bvz,kqc,adz &   157 & gwi,oj,agr & 158 & bjv,amx,nif \\
   159 & ann,mtj,otq & 160 & eka,apn,txu &   161 & neb,ee,avn & 162 & plw,ban,btx \\
   163 & bwq,bbo,bex & 164 & hig,bcw,pbi &   165 & kfr,bhb-Gujr,vas-Gujr & 166 & ndy,tiv,bim \\
   167 & ura,bmr,cof & 168 & box,lem,sld &   169 & tab,inh,ce & 170 & lwo,chq,pao \\
   171 & mcf,con,gdg & 172 & oj-Cans,iu,crm &   173 & enb,kln,cro & 174 & yaz,csk,tlj \\
   175 & xon,gux,daa & 176 & nus,dip,din &   177 & srm,srn,djk & 178 & dyo,mxp,mco \\
   179 & tpt,kbm,gam & 180 & yi,gv,ztq &   181 & hmn,zpm,ntu & 182 & ljp,hui,met \\
   183 & jic,maz,zas & 184 & niy,vut,ken &   185 & mnw,ksw,shn & 186 & kub,taq,mda \\
   187 & lew,kzf,mqn & 188 & xsm,sig,lia &   189 & mbi,mbs,mbb & 190 & miy,meh,tuo \\
   191 & mfk,mif,meq & 192 & ms-Arab-BN,ms-Arab,mfa &   193 & nlc,mps,nbq & 194 & tna,qwh,nhg \\
   195 & npl,nsu,nhy & 196 & rmc,zae,rom &   197 & sil,tpm,vag & 198 & zam,srq,zpz \\
   199 & toc,top,tos & 200 & yva,yon,wnc &   201 & tac,alp & 202 & kkl,amn \\
   203 & atq,ptu & 204 & awx,iou &   205 & ayp,su-Arab & 206 & beu,wim \\
   207 & bfo,dgi & 208 & bib,yle &   209 & mqb,blw & 210 & bm-Nkoo,nqo \\
   211 & dz,bo & 212 & bua,dng &   213 & cbc,tue & 214 & mcd,cbt \\
   215 & cgc,mmn & 216 & chk,xbi &   217 & ug,ckb & 218 & cok,crn \\
   219 & cot,not & 220 & myy,cub &   221 & mfy,ese & 222 & kbc,etr \\
   223 & gon,lmn & 224 & kvn,guo &   225 & hrx,mca & 226 & kbp,ntr \\
   227 & kdj,keo & 228 & mau,kek &   229 & mfz,ker & 230 & xsi,kij \\
   231 & lo,kjg & 232 & knf,nuj &   233 & kpz,ong & 234 & tmc,lme \\
   235 & nkf,lmk & 236 & tcy,lmn-Knda &   237 & lsi,mhx & 238 & mcu,ozm \\
   239 & mil,mib & 240 & naf,miq &   241 & moa,tod & 242 & ulk,msy \\
   243 & nuy,mwp & 244 & nhr,vmy &   245 & tew,nv & 246 & pab,ppo \\
   247 & pmf,ppk & 248 & yam,pny &   249 & pxm,tfr & 250 & qvs,qup \\
   251 & sat-Beng,unr & 252 & sty,tyv &   253 & taj,xsr & 254 & tpp,tee \\
   255 & tih,txa & 256 & tku,too \\
\end{tabular}
\caption{Clusters part 2
 \label{tab:clusters2}}
\end{table*}


==> Next Thousand Languages/table_datasize_all.tex <==
\newcommand{\insertgianttable}{
\begin{footnotesize}
\begin{longtable}{p{0.09\linewidth}|p{0.07\linewidth}p{0.17\linewidth}p{0.07\linewidth}p{0.09\linewidth}lp{0.09\linewidth}p{0.03\linewidth}l}

% \centering
% \begin{tabular}{l|llllll}
BCP-47  & 	Mono  & 	Language Name  & 	Speak.  & Cont.  &  Script  & 	Clust.  & 	F1  & 	RTT  \\
\hline
\endhead
% {\tablename\ \thetable\ -- \textit{Continued from previous page}} \\
\hline
en  &	7388M  &	English  &	550M  &	Europe  &	Latn  &	en  &	98.2  &	NA \\
es  &	1751M  &	Spanish  &	490M  &	Europe  &	Latn  &	es  &	98.8  &	77.8 \\
de  &	1693M  &	German  &	83M  &	Europe  &	Latn  &	de  &	98.4  &	78.2 \\
id  &	950M  &	Indonesian  &	200M  &	Asia  &	Latn  &	id  &	97.3  &	76.9 \\
hu  &	724M  &	Hungarian  &	13M  &	Europe  &	Latn  &	hu  &	98.8  &	68.1 \\
pl  &	687M  &	Polish  &	38M  &	Europe  &	Latn  &	pl  &	98.0  &	72.8 \\
zh  &	676M  &	Chinese  &	1000M  &	Asia  &	Hans  &	zh  &	99.1  &	64.0 \\
ko  &	672M  &	Korean  &	52M  &	Asia  &	Kore  &	ko  &	99.9  &	64.0 \\
ja  &	652M  &	Japanese  &	130M  &	Asia  &	Jpan  &	ja  &	99.6  &	65.2 \\
ru  &	570M  &	Russian  &	150M  &	Europe  &	Cyrl  &	ru  &	97.3  &	74.0 \\
tr  &	565M  &	Turkish  &	82M  &	Europe  &	Latn  &	tr  &	99.0  &	70.9 \\
th  &	531M  &	Thai  &	20M  &	Asia  &	Thai  &	th  &	98.9  &	67.9 \\
it  &	491M  &	Italian  &	61M  &	Europe  &	Latn  &	it  &	98.9  &	77.3 \\
pt  &	485M  &	Portuguese  &	220M  &	Europe  &	Latn  &	pt  &	98.0  &	80.0 \\
vi  &	477M  &	Vietnamese  &	96M  &	Asia  &	Latn  &	vi  &	99.7  &	73.8 \\
fr  &	450M  &	French  &	75M  &	Europe  &	Latn  &	fr  &	97.6  &	77.7 \\
ms  &	394M  &	Malay  &	80M  &	Asia  &	Latn  &	ms  &	92.3  &	77.5 \\
nl  &	320M  &	Dutch  &	21M  &	Europe  &	Latn  &	nl  &	99.2  &	79.8 \\
uk  &	320M  &	Ukrainian  &	32M  &	Europe  &	Cyrl  &	uk  &	99.2  &	72.1 \\
sv  &	311M  &	Swedish  &	8M  &	Europe  &	Latn  &	sv  &	98.7  &	79.0 \\
ro  &	301M  &	Romanian  &	19M  &	Europe  &	Latn  &	ro  &	96.8  &	75.1 \\
cs  &	300M  &	Czech  &	10M  &	Europe  &	Latn  &	cs  &	98.9  &	73.0 \\
fa  &	275M  &	Persian  &	40M  &	Asia  &	Arab  &	fa  &	95.0  &	70.3 \\
lv  &	260M  &	Standard Latvian  &	2M  &	Europe  &	Latn  &	lv  &	98.5  &	75.5 \\
ar  &	258M  &	Arabic  &	180M  &	Africa  &	Arab  &	ar  &	97.9  &	71.8 \\
no  &	231M  &	Norwegian  &	5M  &	Europe  &	Latn  &	no  &	87.1  &	79.9 \\
ta  &	220M  &	Tamil  &	76M  &	Asia  &	Taml  &	ta  &	100  &	67.9 \\
el  &	173M  &	Modern Greek  &	13M  &	Europe  &	Grek  &	el  &	99.4  &	75.8 \\
fi  &	171M  &	Finnish  &	5M  &	Europe  &	Latn  &	fi  &	97.0  &	72.3 \\
hi  &	165M  &	Hindi  &	320M  &	Asia  &	Deva  &	hi  &	97.9  &	75.5 \\
mr  &	156M  &	Marathi  &	83M  &	Asia  &	Deva  &	mr  &	99.5  &	69.8 \\
sk  &	156M  &	Slovak  &	4M  &	Europe  &	Latn  &	sk  &	99.5  &	72.6 \\
hy  &	154M  &	Eastern Armenian  &	6M  &	Europe  &	Armn  &	hy  &	100  &	70.5 \\
kk  &	153M  &	Kazakh  &	11M  &	Europe  &	Cyrl  &	kk  &	99.6  &	60.6 \\
da  &	152M  &	Danish  &	5M  &	Europe  &	Latn  &	da  &	97.0  &	79.3 \\
mk  &	150M  &	Macedonian  &	1M  &	Europe  &	Cyrl  &	mk  &	98.8  &	77.6 \\
bg  &	149M  &	Bulgarian  &	7M  &	Europe  &	Cyrl  &	bg  &	98.3  &	74.4 \\
sr  &	141M  &	Serbian Standard  &	6M  &	Europe  &	Cyrl  &	sr  &	98.4  &	- \\
ml  &	139M  &	Malayalam  &	35M  &	Asia  &	Mlym  &	ml  &	100  &	62.5 \\
az  &	135M  &	Azerbaijani  &	18M  &	Asia  &	Latn  &	az  &	98.3  &	70.9 \\
is  &	134M  &	Icelandic  &	300K  &	Europe  &	Latn  &	is  &	97.5  &	78.6 \\
te  &	127M  &	Telugu  &	82M  &	Asia  &	Telu  &	te  &	100  &	72.8 \\
ne  &	116M  &	Nepali  &	16M  &	Asia  &	Deva  &	ne  &	99.3  &	65.6 \\
et  &	112M  &	Estonian  &	1M  &	Europe  &	Latn  &	et  &	99.4  &	73.5 \\
he  &	108M  &	Modern Hebrew  &	4M  &	Europe  &	Hebr  &	he  &	100  &	- \\
mn  &	100M  &	Mongolian  &	5M  &	Asia  &	Cyrl  &	mn  &	97.3  &	61.5 \\
ur  &	99M  &	Urdu  &	120M  &	Asia  &	Arab  &	ur  &	98.4  &	75.5 \\
hr  &	97M  &	Croatian Standard  &	4M  &	Europe  &	Latn  &	hr  &	79.4  &	75.3 \\
fil  &	95M  &	Filipino  &	22M  &	Asia  &	Latn  &	fil  &	97.3  &	80.6 \\
lt  &	86M  &	Lithuanian  &	2M  &	Europe  &	Latn  &	lt  &	99.9  &	72.8 \\
msi  &	84M  &	Brunei-Sabah Malay  &	3M  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	94.3  &	69.6 \\
be  &	83M  &	Belarusian  &	3M  &	Europe  &	Cyrl  &	be  &	99.2  &	73.9 \\
kn  &	80M  &	Kannada  &	43M  &	Asia  &	Knda  &	kn  &	100  &	71.5 \\
my  &	78M  &	Burmese  &	33M  &	Asia  &	Mymr  &	my  &	99.7  &	53.3 \\
bn  &	73M  &	Bengali  &	260M  &	Asia  &	Beng  &	bn  &	98.0  &	70.4 \\
af  &	71M  &	Afrikaans  &	17M  &	Africa  &	Latn  &	af  &	97.7  &	82.1 \\
eu  &	70M  &	Basque  &	500K  &	Europe  &	Latn  &	eu  &	99.9  &	72.9 \\
gu  &	69M  &	Gujarati  &	56M  &	Asia  &	Gujr  &	gu  &	98.0  &	75.2 \\
mi  &	67M  &	Maori  &	200K  &	Oceania  &	Latn  &	\scriptsize{mi-4l}  &	99.6  &	67.2 \\
gdx  &	67M  &	Godwari  &	3M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	70.5  &	74.2 \\
gl  &	64M  &	Galician  &	2M  &	Europe  &	Latn  &	gl  &	94.2  &	76.9 \\
sl  &	59M  &	Slovenian  &	2M  &	Europe  &	Latn  &	sl  &	97.9  &	72.7 \\
lo  &	59M  &	Lao  &	20M  &	Asia  &	Laoo  &	\scriptsize{kjg-2l}  &	100  &	72.0 \\
gd  &	57M  &	Scottish Gaelic  &	50K  &	Europe  &	Latn  &	\scriptsize{alq-4l}  &	99.4  &	74.5 \\
so  &	56M  &	Somali  &	24M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	99.7  &	67.4 \\
si  &	56M  &	Sinhala  &	16M  &	Asia  &	Sinh  &	si  &	100  &	61.3 \\
uz  &	53M  &	Uzbek  &	57M  &	Europe  &	Latn  &	uz  &	99.8  &	62.2 \\
sw  &	52M  &	Swahili  &	24M  &	Africa  &	Latn  &	sw  &	99.3  &	78.1 \\
km  &	51M  &	Central Khmer  &	16M  &	Asia  &	Khmr  &	km  &	99.9  &	69.4 \\
ha  &	51M  &	Hausa  &	70M  &	Africa  &	Latn  &	\scriptsize{amo-7l}  &	99.4  &	70.5 \\
wry  &	50M  &	Merwari  &	8M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	68.2  &	- \\
ky  &	49M  &	Kirghiz  &	8M  &	Europe  &	Cyrl  &	ky  &	99.8  &	56.7 \\
am  &	47M  &	Amharic  &	22M  &	Africa  &	Ethi  &	am  &	95.1  &	58.0 \\
ca  &	44M  &	Catalan  &	4M  &	Europe  &	Latn  &	ca  &	99.5  &	75.0 \\
ceb  &	44M  &	Cebuano  &	16M  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	99.1  &	73.9 \\
yo  &	43M  &	Yoruba  &	21M  &	Africa  &	Latn  &	\scriptsize{bcq-Latn-12l}  &	99.6  &	73.7 \\
sd  &	42M  &	Sindhi  &	68M  &	Asia  &	Arab  &	\scriptsize{bgq-Arab-4l}  &	99.0  &	67.3 \\
gju-Deva-IN  &	41M  &	Gujari  &	1M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	68.6  &	- \\
co  &	41M  &	Corsican  &	50K  &	Europe  &	Latn  &	\scriptsize{cjk-14l}  &	97.5  &	75.2 \\
mg  &	40M  &	Malagasy  &	18M  &	Africa  &	Latn  &	\scriptsize{apy-7l}  &	99.9  &	65.4 \\
pa  &	37M  &	Eastern Punjabi  &	28M  &	Asia  &	Guru  &	pa  &	99.7  &	71.9 \\
ar-MA  &	36M  &	Arabic  &	180M  &	Africa  &	Arab  &	\scriptsize{acm-9l}  &	46.1  &	69.0 \\
bew  &	33M  &	Betawi  &	5M  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	93.8  &	67.2 \\
ny  &	33M  &	Chichewa  &	12M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	98.8  &	66.1 \\
sq  &	32M  &	Albanian  &	5M  &	Europe  &	Latn  &	sq  &	99.3  &	79.0 \\
ka  &	30M  &	Georgian  &	4M  &	Europe  &	Geor  &	ka  &	99.9  &	71.9 \\
haw  &	30M  &	Hawaiian  &	50K  &	Americas  &	Latn  &	\scriptsize{gah-11l}  &	99.7  &	58.3 \\
hmn  &	28M  &	Hmong  &	3M  &	Europe  &	Latn  &	\scriptsize{hmn-3l}  &	99.7  &	71.5 \\
yi  &	28M  &	Yiddish  &	2M  &	Europe  &	Hebr  &	\scriptsize{gv-3l}  &	100  &	84.8 \\
ig  &	27M  &	Igbo  &	18M  &	Africa  &	Latn  &	\scriptsize{dzg-5l}  &	99.0  &	68.6 \\
ckb  &	25M  &	Central Kurdish  &	7M  &	Europe  &	Arab  &	\scriptsize{ckb-2l}  &	99.3  &	60.0 \\
tt  &	25M  &	Tatar  &	4M  &	Europe  &	Cyrl  &	tt  &	97.0  &	52.5 \\
gsw  &	25M  &	Central Alemannic  &	5M  &	Europe  &	Latn  &	\scriptsize{ang-7l}  &	93.2  &	73.3 \\
arq  &	24M  &	Algerian Arabic  &	27M  &	Africa  &	Arab  &	\scriptsize{acm-9l}  &	79.0  &	66.0 \\
sm  &	24M  &	Samoan  &	500K  &	Oceania  &	Latn  &	\scriptsize{mi-4l}  &	99.9  &	67.6 \\
eo  &	24M  &	Esperanto  &	2M  &	Europe  &	Latn  &	eo  &	99.7  &	78.4 \\
zu  &	23M  &	Zulu  &	11M  &	Africa  &	Latn  &	\scriptsize{gup-8l}  &	96.3  &	71.3 \\
st  &	23M  &	Southern Sotho  &	14M  &	Africa  &	Latn  &	\scriptsize{cce-8l}  &	98.8  &	69.2 \\
ru-Latn  &	23M  &	Russian  &	150M  &	Europe  &	Latn  &	\scriptsize{bg-Latn-5l}  &	97.2  &	51.4 \\
cy  &	22M  &	Welsh  &	700K  &	Europe  &	Latn  &	cy  &	99.7  &	79.4 \\
la  &	22M  &	Latin  &	0K  &	Europe  &	Latn  &	la  &	93.2  &	67.9 \\
or  &	21M  &	Odia  &	35M  &	Asia  &	Orya  &	or  &	100  &	63.2 \\
mt  &	21M  &	Maltese  &	500K  &	Europe  &	Latn  &	mt  &	99.5  &	84.2 \\
rkt  &	20M  &	Rangpuri  &	15M  &	Asia  &	Beng  &	\scriptsize{bpy-7l}  &	98.8  &	59.2 \\
ht  &	20M  &	Haitian  &	10M  &	Americas  &	Latn  &	ht  &	99.9  &	79.3 \\
sn  &	18M  &	Shona  &	9M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	99.6  &	68.6 \\
bo  &	18M  &	Tibetan  &	1M  &	Asia  &	Tibt  &	\scriptsize{bo-2l}  &	99.9  &	28.5 \\
ps  &	18M  &	Nuclear Pashto  &	13M  &	Asia  &	Arab  &	ps  &	98.9  &	59.7 \\
ga  &	17M  &	Irish  &	200K  &	Europe  &	Latn  &	ga  &	98.8  &	80.9 \\
shu  &	16M  &	Chadian Arabic  &	1M  &	Africa  &	Arab  &	\scriptsize{acm-9l}  &	89.5  &	- \\
xh  &	16M  &	Xhosa  &	19M  &	Africa  &	Latn  &	\scriptsize{gup-8l}  &	97.8  &	69.0 \\
lb  &	15M  &	Moselle Franconian  &	400K  &	Europe  &	Latn  &	lb  &	96.7  &	63.7 \\
ku  &	15M  &	Kurdish  &	32M  &	Europe  &	Latn  &	ku  &	98.2  &	57.7 \\
tg  &	14M  &	Tajik  &	8M  &	Europe  &	Cyrl  &	tg  &	99.9  &	64.9 \\
hi-Latn  &	14M  &	Hindi  &	320M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	98.1  &	71.7 \\
jv  &	13M  &	Javanese  &	85M  &	Asia  &	Latn  &	jv  &	99.4  &	77.0 \\
apd-SD  &	13M  &	Sudanese Arabic  &	17M  &	Africa  &	Arab  &	\scriptsize{acm-9l}  &	74.2  &	69.1 \\
su  &	12M  &	Sundanese  &	39M  &	Asia  &	Latn  &	su  &	99.1  &	71.1 \\
mzn  &	12M  &	Mazanderani  &	6M  &	Asia  &	Arab  &	\scriptsize{apr-8l}  &	52.4  &	64.8 \\
meo  &	11M  &	Kedah Malay  &	3M  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	94.4  &	66.7 \\
fy  &	11M  &	Western Frisian  &	800K  &	Europe  &	Latn  &	fy  &	99.7  &	71.7 \\
mrw  &	10M  &	Maranao  &	800K  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	98.0  &	69.2 \\
rw  &	10M  &	Kinyarwanda  &	11M  &	Africa  &	Latn  &	rw  &	98.6  &	47.7 \\
apc  &	10M  &	North Levantine Arabic  &	15M  &	Europe  &	Arab  &	\scriptsize{abv-10l}  &	40.4  &	67.7 \\
as  &	9M  &	Assamese  &	13M  &	Asia  &	Beng  &	as  &	99.7  &	63.7 \\
aec  &	9M  &	Saidi Arabic  &	19M  &	Africa  &	Arab  &	\scriptsize{abv-10l}  &	78.0  &	64.3 \\
fo  &	9M  &	Faroese  &	50K  &	Europe  &	Latn  &	\scriptsize{bn-Latn-6l}  &	98.0  &	71.6 \\
pap  &	9M  &	Papiamento  &	600K  &	Americas  &	Latn  &	\scriptsize{ach-10l}  &	94.8  &	61.4 \\
sah  &	9M  &	Sakha  &	500K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	97.7  &	43.4 \\
acm  &	9M  &	Gilit Mesopotamian Arabic  &	26M  &	Europe  &	Arab  &	\scriptsize{acm-9l}  &	35.2  &	64.2 \\
lus  &	8M  &	Mizo  &	700K  &	Asia  &	Latn  &	\scriptsize{bgr-6l}  &	100  &	35.9 \\
grc  &	8M  &	Ancient Greek (to 1453)  &	0K  &	Europe  &	Grek  &	grc  &	99.9  &	- \\
dv  &	8M  &	Dhivehi  &	300K  &	Asia  &	Thaa  &	\scriptsize{bpy-7l}  &	100  &	53.6 \\
oc  &	7M  &	Occitan  &	500K  &	Europe  &	Latn  &	\scriptsize{acf-10l}  &	96.7  &	73.4 \\
luz  &	7M  &	Southern Luri  &	900K  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	68.4  &	64.2 \\
sa  &	6M  &	Sanskrit  &	100K  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	97.8  &	57.6 \\
bgp-Arab  &	6M  &	Eastern Balochi  &	2M  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	55.1  &	- \\
ug  &	6M  &	Uyghur  &	10M  &	Asia  &	Arab  &	\scriptsize{ckb-2l}  &	100  &	50.5 \\
ba  &	6M  &	Bashkir  &	1M  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	98.0  &	58.2 \\
om  &	6M  &	Oromo  &	24M  &	Africa  &	Latn  &	\scriptsize{amf-6l}  &	99.7  &	56.0 \\
zza  &	5M  &	Zaza  &	2M  &	Europe  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	71.7  &	- \\
zh-Latn  &	5M  &	Chinese  &	1000M  &	Asia  &	Latn  &	\scriptsize{cqd-8l}  &	99.2  &	22.2 \\
vas-Gujr  &	4M  &	Vasavi  &	1M  &	Asia  &	Gujr  &	\scriptsize{bhb-Gujr-3l}  &	78.7  &	68.5 \\
vec  &	4M  &	Venetian  &	4M  &	Europe  &	Latn  &	\scriptsize{bi-6l}  &	94.5  &	73.5 \\
tk  &	4M  &	Turkmen  &	8M  &	Europe  &	Latn  &	tk  &	99.9  &	57.5 \\
hil  &	4M  &	Hiligaynon  &	6M  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	99.3  &	70.8 \\
ti  &	4M  &	Tigrinya  &	9M  &	Africa  &	Ethi  &	\scriptsize{gez-8l}  &	99.9  &	57.0 \\
syl  &	4M  &	Sylheti  &	23M  &	Asia  &	Beng  &	\scriptsize{bpy-7l}  &	86.9  &	65.8 \\
phr  &	4M  &	Pahari Potwari  &	2M  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	54.5  &	73.6 \\
ayl  &	4M  &	Libyan Arabic  &	5M  &	Africa  &	Arab  &	\scriptsize{acm-9l}  &	86.3  &	65.0 \\
el-Latn  &	3M  &	Modern Greek  &	13M  &	Europe  &	Latn  &	\scriptsize{bg-Latn-5l}  &	98.9  &	26.0 \\
kaa  &	3M  &	Kara-Kalpak  &	600K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	99.3  &	61.8 \\
bs  &	3M  &	Bosnian Standard  &	9M  &	Europe  &	Cyrl  &	bs  &	70.8  &	74.1 \\
bgp  &	3M  &	Eastern Balochi  &	2M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	91.1  &	70.0 \\
br  &	3M  &	Breton  &	200K  &	Europe  &	Latn  &	\scriptsize{br-4l}  &	82.8  &	42.8 \\
gdq  &	3M  &	Mehri  &	100K  &	Europe  &	Arab  &	\scriptsize{acm-9l}  &	51.7  &	- \\
tet  &	3M  &	Tetum  &	500K  &	Asia  &	Latn  &	\scriptsize{ceg-5l}  &	98.4  &	53.5 \\
to  &	3M  &	Tonga (Tonga Islands)  &	200K  &	Oceania  &	Latn  &	\scriptsize{mi-4l}  &	100  &	57.5 \\
cv  &	3M  &	Chuvash  &	1M  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	92.9  &	48.6 \\
kfr  &	3M  &	Kachchi  &	900K  &	Asia  &	Gujr  &	\scriptsize{bhb-Gujr-3l}  &	82.5  &	63.4 \\
ilo  &	3M  &	Ilocano  &	9M  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	93.4  &	47.6 \\
bg-Latn  &	3M  &	Bulgarian  &	7M  &	Europe  &	Latn  &	\scriptsize{bg-Latn-5l}  &	97.2  &	65.0 \\
bal  &	3M  &	Balochi  &	8M  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	23.0  &	61.8 \\
hif  &	2M  &	Fiji Hindi  &	500K  &	Oceania  &	Latn  &	\scriptsize{bgp-13l}  &	99.6  &	69.4 \\
mey  &	2M  &	Hassaniyya  &	3M  &	Africa  &	Arab  &	\scriptsize{acm-9l}  &	69.5  &	- \\
dz  &	2M  &	Dzongkha  &	200K  &	Asia  &	Tibt  &	\scriptsize{bo-2l}  &	98.2  &	39.5 \\
tn  &	2M  &	Tswana  &	8M  &	Africa  &	Latn  &	\scriptsize{cce-8l}  &	90.5  &	66.5 \\
bn-Latn  &	2M  &	Bengali  &	260M  &	Asia  &	Latn  &	\scriptsize{bn-Latn-6l}  &	98.5  &	57.5 \\
lg  &	2M  &	Ganda  &	4M  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	98.7  &	58.2 \\
te-Latn  &	2M  &	Telugu  &	82M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	98.6  &	59.3 \\
mde  &	2M  &	Maba (Chad)  &	300K  &	Africa  &	Arab  &	\scriptsize{acm-9l}  &	48.5  &	- \\
nso  &	2M  &	Pedi  &	14M  &	Africa  &	Latn  &	\scriptsize{cce-8l}  &	98.6  &	68.0 \\
rm  &	2M  &	Romansh  &	50K  &	Europe  &	Latn  &	rm  &	99.9  &	61.7 \\
za  &	2M  &	Northern Daic  &	15M  &	Asia  &	Latn  &	\scriptsize{cqd-8l}  &	98.7  &	27.3 \\
tpi  &	2M  &	Tok Pisin  &	4M  &	Oceania  &	Latn  &	\scriptsize{bi-6l}  &	99.3  &	61.3 \\
pcm  &	2M  &	Nigerian Pidgin  &	30M  &	Africa  &	Latn  &	pcm  &	97.9  &	71.1 \\
mtq  &	2M  &	Muong  &	1M  &	Asia  &	Latn  &	\scriptsize{blt-Latn-4l}  &	96.3  &	- \\
cnh  &	2M  &	Haka Chin  &	100K  &	Asia  &	Latn  &	\scriptsize{bgr-6l}  &	99.9  &	37.2 \\
iba  &	2M  &	Iban  &	2M  &	Asia  &	Latn  &	\scriptsize{amo-7l}  &	99.8  &	54.8 \\
ja-Latn  &	2M  &	Japanese  &	130M  &	Asia  &	Latn  &	\scriptsize{dgz-5l}  &	98.6  &	20.9 \\
ium  &	2M  &	Iu Mien  &	800K  &	Asia  &	Latn  &	\scriptsize{cqd-8l}  &	98.9  &	18.9 \\
crs  &	2M  &	Seselwa Creole French  &	50K  &	Africa  &	Latn  &	\scriptsize{acf-10l}  &	99.8  &	72.9 \\
se  &	1.5M  &	North Saami  &	50K  &	Europe  &	Latn  &	\scriptsize{bn-Latn-6l}  &	90.2  &	- \\
kha  &	1.4M  &	Khasi  &	800K  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	99.9  &	38.3 \\
ln  &	1.4M  &	Kinshasa Lingala  &	15M  &	Africa  &	Latn  &	\scriptsize{jbu-8l}  &	96.4  &	56.1 \\
tyv  &	1.4M  &	Tuvinian  &	300K  &	Europe  &	Cyrl  &	\scriptsize{sty-2l}  &	99.4  &	47.4 \\
ce  &	1.4M  &	Chechen  &	1M  &	Europe  &	Cyrl  &	\scriptsize{ce-3l}  &	99.9  &	41.6 \\
mai  &	1.3M  &	Maithili  &	17M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	98.6  &	60.8 \\
nr  &	1.3M  &	South Transvaal Ndebele  &	1M  &	Africa  &	Latn  &	\scriptsize{gup-8l}  &	86.3  &	- \\
dty  &	1.3M  &	Dotyali  &	800K  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	77.6  &	57.8 \\
ts  &	1.3M  &	Tsonga  &	13M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	72.9  &	55.0 \\
fj  &	1.3M  &	Fijian  &	300K  &	Oceania  &	Latn  &	\scriptsize{fj-4l}  &	98.8  &	37.5 \\
ak  &	1.3M  &	Akan  &	13M  &	Africa  &	Latn  &	\scriptsize{abr-5l}  &	93.8  &	49.5 \\
kaa-Latn  &	1.3M  &	Kara-Kalpak  &	600K  &	Europe  &	Latn  &	\scriptsize{bcq-Latn-12l}  &	86.7  &	55.9 \\
os  &	1.3M  &	Iron Ossetian  &	600K  &	Europe  &	Cyrl  &	\scriptsize{gaw-8l}  &	93.5  &	55.2 \\
bik  &	1.2M  &	Bikol  &	2M  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	94.4  &	68.7 \\
ber-Latn  &	1.2M  &	Berber  &	2M  &	Africa  &	Latn  &	\scriptsize{alq-4l}  &	99.7  &	32.9 \\
ctd-Latn  &	1.2M  &	Tedim Chin  &	300K  &	Asia  &	Latn  &	\scriptsize{bgs-9l}  &	99.5  &	23.5 \\
tly-IR  &	1.2M  &	North-Central Talysh  &	900K  &	Europe  &	Arab  &	\scriptsize{fay-14l}  &	88.7  &	63.1 \\
plk  &	1.1M  &	Kohistani Shina  &	200K  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	65.1  &	- \\
tks  &	1.1M  &	Takestani  &	200K  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	88.9  &	- \\
kmz  &	1.1M  &	Khorasan Turkic  &	400K  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	60.7  &	64.4 \\
mnw  &	1.1M  &	Mon  &	900K  &	Asia  &	Mymr  &	\scriptsize{ksw-3l}  &	99.9  &	24.4 \\
scl  &	1M  &	Shina  &	400K  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	30.1  &	- \\
ml-Latn  &	1M  &	Malayalam  &	35M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	98.7  &	58.2 \\
el-CY  &	1M  &	Modern Greek  &	13M  &	Europe  &	Grek  &	el-CY  &	99.6  &	71.0 \\
skr  &	1M  &	Saraiki  &	26M  &	Asia  &	Arab  &	\scriptsize{doi-Arab-5l}  &	99.8  &	65.1 \\
udm  &	1M  &	Udmurt  &	300K  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	98.1  &	45.6 \\
bbc  &	900K  &	Batak Toba  &	2M  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	98.3  &	47.9 \\
war  &	900K  &	Waray (Philippines)  &	3M  &	Asia  &	Latn  &	\scriptsize{bgs-9l}  &	98.3  &	70.8 \\
mki  &	900K  &	Dhatki  &	200K  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	26.8  &	- \\
srn  &	900K  &	Sranan Tongo  &	100K  &	Americas  &	Latn  &	\scriptsize{djk-3l}  &	98.4  &	56.9 \\
pck  &	900K  &	Paite Chin  &	50K  &	Asia  &	Latn  &	\scriptsize{bgs-9l}  &	99.5  &	32.3 \\
gn  &	900K  &	Guarani  &	5M  &	Americas  &	Latn  &	\scriptsize{gn-6l}  &	98.8  &	50.3 \\
qu  &	800K  &	Quechua  &	9M  &	Americas  &	Latn  &	\scriptsize{ae-Latn-10l}  &	98.3  &	48.8 \\
kj  &	800K  &	Kuanyama  &	600K  &	Africa  &	Latn  &	\scriptsize{kj-5l}  &	98.5  &	39.9 \\
bug  &	800K  &	Buginese  &	5M  &	Asia  &	Latn  &	\scriptsize{amo-7l}  &	83.5  &	- \\
ee  &	800K  &	Ewe  &	4M  &	Africa  &	Latn  &	\scriptsize{avn-3l}  &	99.5  &	49.6 \\
ltg  &	800K  &	East Latvian  &	200K  &	Europe  &	Latn  &	\scriptsize{gaw-8l}  &	94.9  &	63.7 \\
hsb  &	800K  &	Upper Sorbian  &	5K  &	Europe  &	Latn  &	\scriptsize{ach-10l}  &	59.6  &	- \\
kl  &	700K  &	Kalaallisut  &	50K  &	Americas  &	Latn  &	\scriptsize{bi-6l}  &	87.7  &	34.1 \\
bho  &	700K  &	Bhojpuri  &	51M  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	96.6  &	56.2 \\
ta-Latn  &	700K  &	Tamil  &	76M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	99.1  &	53.8 \\
ve  &	700K  &	Venda  &	2M  &	Africa  &	Latn  &	\scriptsize{cce-8l}  &	99.9  &	52.9 \\
bi  &	700K  &	Bislama  &	200K  &	Oceania  &	Latn  &	\scriptsize{bi-6l}  &	99.1  &	- \\
az-RU  &	700K  &	Azerbaijani  &	18M  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	99.7  &	58.1 \\
kbd  &	700K  &	Kabardian  &	2M  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	87.7  &	46.1 \\
nut  &	600K  &	Nung (Viet Nam)  &	1M  &	Asia  &	Latn  &	\scriptsize{blt-Latn-4l}  &	97.9  &	- \\
hif-Deva  &	600K  &	Fiji Hindi  &	500K  &	Oceania  &	Deva  &	\scriptsize{awa-14l}  &	89.5  &	69.9 \\
ar-Latn  &	600K  &	Arabic  &	180M  &	Europe  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	95.2  &	29.5 \\
krc  &	600K  &	Karachay-Balkar  &	300K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	98.5  &	52.7 \\
chm  &	600K  &	Mari  &	500K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	99.5  &	44.5 \\
pag  &	600K  &	Pangasinan  &	1M  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	92.0  &	48.9 \\
mui  &	600K  &	Musi  &	3M  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	90.4  &	62.5 \\
shn  &	600K  &	Shan  &	3M  &	Asia  &	Mymr  &	\scriptsize{ksw-3l}  &	100  &	40.3 \\
gom-Latn  &	500K  &	Goan Konkani  &	2M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	99.0  &	56.0 \\
noe  &	500K  &	Nimadi  &	2M  &	Asia  &	Deva  &	\scriptsize{ahr-13l}  &	99.2  &	62.8 \\
mh  &	500K  &	Marshallese  &	50K  &	Oceania  &	Latn  &	\scriptsize{kpj-5l}  &	100  &	31.4 \\
min  &	500K  &	Minangkabau  &	6M  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	100  &	59.1 \\
yue  &	500K  &	Yue Chinese  &	84M  &	Asia  &	Hant  &	yue  &	99.1  &	55.4 \\
new  &	500K  &	Kathmandu Valley Newari  &	900K  &	Asia  &	Deva  &	\scriptsize{ahr-13l}  &	98.3  &	51.4 \\
cjk  &	500K  &	Chokwe  &	1M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	98.7  &	43.7 \\
jax  &	500K  &	Jambi Malay  &	1M  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	85.8  &	69.1 \\
bft  &	500K  &	Balti  &	300K  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	13.7  &	- \\
dov  &	500K  &	Dombe  &	2M  &	Africa  &	Latn  &	\scriptsize{dov-9l}  &	100  &	44.8 \\
kv  &	500K  &	Komi  &	200K  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	95.2  &	44.0 \\
cfm  &	500K  &	Falam Chin  &	100K  &	Asia  &	Latn  &	\scriptsize{bgr-6l}  &	99.9  &	36.7 \\
fay  &	500K  &	Fars Dialects  &	50K  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	60.9  &	62.3 \\
mr-Latn  &	500K  &	Marathi  &	83M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	98.0  &	64.5 \\
lu  &	400K  &	Luba-Katanga  &	2M  &	Africa  &	Latn  &	\scriptsize{jbu-8l}  &	98.3  &	39.1 \\
wa  &	400K  &	Walloon  &	600K  &	Europe  &	Latn  &	\scriptsize{acf-10l}  &	91.2  &	54.1 \\
yua  &	400K  &	Yucatec Maya  &	800K  &	Americas  &	Latn  &	\scriptsize{chd-6l}  &	99.3  &	57.9 \\
abv  &	400K  &	Baharna Arabic  &	300K  &	Europe  &	Arab  &	\scriptsize{abv-10l}  &	8.1  &	- \\
sg  &	400K  &	Sango  &	2M  &	Africa  &	Latn  &	\scriptsize{enx-4l}  &	99.7  &	31.0 \\
iso  &	400K  &	Isoko  &	400K  &	Africa  &	Latn  &	\scriptsize{ajg-8l}  &	99.9  &	35.1 \\
kac  &	400K  &	Southern Jinghpaw  &	900K  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	100  &	38.4 \\
syr  &	400K  &	Syriac  &	1M  &	Europe  &	Syrc  &	\scriptsize{ach-10l}  &	99.9  &	40.4 \\
pam  &	400K  &	Pampanga  &	2M  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	99.5  &	52.5 \\
afb  &	400K  &	Gulf Arabic  &	5M  &	Europe  &	Arab  &	\scriptsize{abv-10l}  &	4.1  &	- \\
qxq  &	400K  &	Qashqa'i  &	2M  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	61.8  &	61.0 \\
ada  &	400K  &	Adangme  &	800K  &	Africa  &	Latn  &	\scriptsize{ada-13l}  &	99.7  &	44.1 \\
ctg  &	400K  &	Chittagonian  &	15M  &	Asia  &	Beng  &	\scriptsize{bpy-7l}  &	90.9  &	65.2 \\
kg  &	400K  &	Kongo  &	6M  &	Africa  &	Latn  &	\scriptsize{jbu-8l}  &	93.8  &	- \\
mtr  &	400K  &	Mewari  &	5M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	89.2  &	44.8 \\
io  &	400K  &	Ido  &	5K  &	Europe  &	Latn  &	\scriptsize{acf-10l}  &	84.6  &	- \\
pmy  &	400K  &	Papuan Malay  &	500K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	88.3  &	68.3 \\
ss-SZ  &	400K  &	Swati  &	3M  &	Africa  &	Latn  &	\scriptsize{gup-8l}  &	87.3  &	64.7 \\
mwr  &	400K  &	Marwari  &	8M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	97.3  &	- \\
ktu  &	400K  &	Kituba (DRC)  &	5M  &	Africa  &	Latn  &	\scriptsize{jbu-8l}  &	99.8  &	43.6 \\
nd  &	300K  &	Zimbabwean Ndebele  &	2M  &	Africa  &	Latn  &	\scriptsize{gup-8l}  &	98.6  &	69.1 \\
kek  &	300K  &	Kekchí  &	800K  &	Americas  &	Latn  &	\scriptsize{kek-2l}  &	100  &	35.1 \\
mfe  &	300K  &	Morisyen  &	1M  &	Africa  &	Latn  &	\scriptsize{acf-10l}  &	100  &	66.0 \\
bua  &	300K  &	Buriat  &	400K  &	Europe  &	Cyrl  &	\scriptsize{bua-2l}  &	96.9  &	44.5 \\
tvl  &	300K  &	Tuvalu  &	50K  &	Oceania  &	Latn  &	\scriptsize{mi-4l}  &	99.6  &	- \\
chk  &	300K  &	Chuukese  &	50K  &	Oceania  &	Latn  &	\scriptsize{chk-2l}  &	100  &	34.4 \\
dcc  &	300K  &	Deccan  &	13M  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	89.2  &	61.2 \\
gom  &	300K  &	Goan Konkani  &	2M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	85.6  &	59.2 \\
pon  &	300K  &	Pohnpeian  &	50K  &	Oceania  &	Latn  &	\scriptsize{bgs-9l}  &	99.7  &	39.9 \\
av  &	300K  &	Avar  &	800K  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	99.1  &	45.8 \\
mfb  &	300K  &	Bangka  &	300K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	91.5  &	66.6 \\
sjp  &	300K  &	Surjapuri  &	1M  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	96.3  &	55.4 \\
tiv  &	300K  &	Tiv  &	2M  &	Africa  &	Latn  &	\scriptsize{bim-3l}  &	100  &	27.7 \\
ady  &	300K  &	Adyghe  &	600K  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	89.2  &	43.2 \\
btx  &	300K  &	Batak Karo  &	600K  &	Asia  &	Latn  &	\scriptsize{ban-3l}  &	100  &	39.1 \\
wo  &	300K  &	Wolof  &	4M  &	Africa  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	99.3  &	50.1 \\
tsc  &	300K  &	Tswa  &	1M  &	Africa  &	Latn  &	\scriptsize{cce-8l}  &	98.6  &	66.9 \\
hne  &	300K  &	Chhattisgarhi  &	18M  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	98.9  &	56.9 \\
ay  &	300K  &	Central-Southern Aymara  &	3M  &	Americas  &	Latn  &	\scriptsize{auc-6l}  &	99.6  &	31.0 \\
pa-Arab  &	300K  &	Eastern Punjabi  &	28M  &	Asia  &	Arab  &	\scriptsize{doi-Arab-5l}  &	96.4  &	64.3 \\
gag  &	300K  &	Gagauz  &	600K  &	Europe  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	99.0  &	61.9 \\
raj  &	300K  &	Rajasthani  &	18M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	88.0  &	47.9 \\
quc  &	200K  &	K'iche'  &	2M  &	Americas  &	Latn  &	\scriptsize{acr-4l}  &	99.9  &	38.8 \\
zyj  &	200K  &	Youjiang Zhuang  &	900K  &	Asia  &	Latn  &	\scriptsize{cqd-8l}  &	99.1  &	26.4 \\
bhb-Gujr  &	200K  &	Bhili  &	3M  &	Asia  &	Gujr  &	\scriptsize{bhb-Gujr-3l}  &	98.2  &	- \\
ho  &	200K  &	Hiri Motu  &	100K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	99.4  &	32.6 \\
zap  &	200K  &	Zapotec  &	400K  &	Americas  &	Latn  &	\scriptsize{zaa-5l}  &	100  &	32.1 \\
crh  &	200K  &	Crimean Tatar  &	500K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	99.7  &	53.1 \\
mam  &	200K  &	Mam  &	500K  &	Americas  &	Latn  &	\scriptsize{chd-6l}  &	99.8  &	28.3 \\
rhg-Latn  &	200K  &	Rohingya  &	2M  &	Asia  &	Latn  &	\scriptsize{bn-Latn-6l}  &	98.7  &	50.0 \\
rom  &	200K  &	Romani  &	4M  &	Europe  &	Latn  &	\scriptsize{rmc-3l}  &	99.1  &	44.0 \\
mgh  &	200K  &	Makhuwa-Meetto  &	7M  &	Africa  &	Latn  &	\scriptsize{apu-13l}  &	99.6  &	30.0 \\
lrc  &	200K  &	Northern Luri  &	2M  &	Asia  &	Arab  &	\scriptsize{apr-8l}  &	67.2  &	- \\
kmz-Latn  &	200K  &	Khorasan Turkic  &	400K  &	Asia  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	93.0  &	54.9 \\
myv  &	200K  &	Erzya  &	400K  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	98.0  &	36.3 \\
ace  &	200K  &	Acehnese  &	4M  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	99.7  &	50.1 \\
bns  &	200K  &	Bundeli  &	3M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	87.8  &	- \\
acw  &	200K  &	Hijazi Arabic  &	14M  &	Europe  &	Arab  &	\scriptsize{abv-10l}  &	6.4  &	- \\
nan-Latn-TW  &	200K  &	Min Nan Chinese  &	59M  &	Asia  &	Latn  &	\scriptsize{cdo-5l}  &	100  &	27.1 \\
quh  &	200K  &	South Bolivian Quechua  &	3M  &	Americas  &	Latn  &	\scriptsize{ae-Latn-10l}  &	99.9  &	39.2 \\
gbm  &	200K  &	Garhwali  &	3M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	95.1  &	53.9 \\
ctu  &	200K  &	Chol  &	200K  &	Americas  &	Latn  &	\scriptsize{chz-9l}  &	100  &	29.8 \\
acq  &	200K  &	Ta'izzi-Adeni Arabic  &	7M  &	Europe  &	Arab  &	\scriptsize{abv-10l}  &	12.3  &	- \\
bfy  &	200K  &	Bagheli  &	8M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	91.5  &	62.0 \\
gv  &	200K  &	Manx  &	5K  &	Europe  &	Latn  &	\scriptsize{gv-3l}  &	98.3  &	36.6 \\
xmm  &	200K  &	Manado Malay  &	800K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	94.5  &	59.7 \\
mel  &	200K  &	Central Melanau  &	100K  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	89.7  &	74.2 \\
ksw  &	200K  &	S'gaw Karen  &	1M  &	Asia  &	Mymr  &	\scriptsize{ksw-3l}  &	100  &	38.0 \\
seh  &	200K  &	Sena  &	2M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	99.5  &	52.5 \\
msb  &	200K  &	Masbatenyo  &	400K  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	99.4  &	57.3 \\
tsg  &	200K  &	Tausug  &	1M  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	98.4  &	54.0 \\
dtp  &	200K  &	Central Dusun  &	100K  &	Asia  &	Latn  &	\scriptsize{dtb-4l}  &	100  &	23.9 \\
yap  &	200K  &	Yapese  &	5K  &	Oceania  &	Latn  &	\scriptsize{bru-6l}  &	99.3  &	- \\
kum  &	200K  &	Kumyk  &	400K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	99.9  &	47.9 \\
fon  &	200K  &	Fon  &	1M  &	Africa  &	Latn  &	\scriptsize{ada-13l}  &	99.9  &	40.9 \\
alt  &	200K  &	Southern Altai  &	50K  &	Europe  &	Cyrl  &	alt  &	100  &	43.4 \\
wal  &	200K  &	Wolaytta  &	2M  &	Africa  &	Latn  &	\scriptsize{drs-Latn-8l}  &	99.7  &	29.6 \\
en-Arab  &	200K  &	English  &	550M  &	Europe  &	Arab  &	\scriptsize{abv-10l}  &	97.4  &	56.5 \\
nzi  &	200K  &	Nzima  &	300K  &	Africa  &	Latn  &	\scriptsize{bov-4l}  &	100  &	40.6 \\
cak  &	200K  &	Kaqchikel  &	400K  &	Americas  &	Latn  &	\scriptsize{acr-4l}  &	100  &	24.1 \\
ban  &	200K  &	Balinese  &	3M  &	Asia  &	Latn  &	\scriptsize{ban-3l}  &	100  &	51.7 \\
zne  &	200K  &	Zande  &	1M  &	Africa  &	Latn  &	\scriptsize{agt-6l}  &	99.5  &	16.9 \\
bm  &	200K  &	Bambara  &	14M  &	Africa  &	Latn  &	\scriptsize{ada-13l}  &	99.1  &	42.1 \\
mdh  &	200K  &	Maguindanao  &	1M  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	96.4  &	43.7 \\
xal  &	200K  &	Oirad-Kalmyk-Darkhat  &	400K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	91.5  &	42.8 \\
abs  &	200K  &	Ambonese Malay  &	2M  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	88.8  &	63.7 \\
tzo  &	200K  &	Tzotzil  &	200K  &	Americas  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	99.9  &	29.5 \\
bgc  &	200K  &	Haryanvi  &	13M  &	Asia  &	Deva  &	\scriptsize{ahr-13l}  &	91.7  &	56.9 \\
vkt  &	200K  &	Tenggarong Kutai Malay  &	200K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	93.6  &	64.8 \\
doi  &	200K  &	Kangri-Dogri  &	2M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	93.5  &	- \\
gez  &	200K  &	Geez  &	0K  &	Africa  &	Ethi  &	\scriptsize{gez-8l}  &	87.6  &	- \\
rwr  &	200K  &	Marwari (India)  &	8M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	84.9  &	44.9 \\
tum  &	200K  &	Tumbuka  &	2M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	47.9  &	- \\
ang  &	200K  &	Old English (ca. 450-1100)  &	0K  &	Europe  &	Latn  &	\scriptsize{ang-7l}  &	97.6  &	- \\
nia  &	200K  &	Nias  &	800K  &	Asia  &	Latn  &	\scriptsize{ceg-5l}  &	100  &	23.1 \\
bts  &	200K  &	Batak Simalungun  &	1M  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	100  &	34.1 \\
ng  &	200K  &	Ndonga  &	800K  &	Africa  &	Latn  &	\scriptsize{kj-5l}  &	95.0  &	35.0 \\
ach  &	200K  &	Acoli  &	1M  &	Africa  &	Latn  &	\scriptsize{ach-10l}  &	99.6  &	21.0 \\
rcf  &	200K  &	Réunion Creole French  &	600K  &	Africa  &	Latn  &	\scriptsize{acf-10l}  &	99.3  &	66.9 \\
kos  &	200K  &	Kosraean  &	5K  &	Oceania  &	Latn  &	\scriptsize{ceg-5l}  &	98.8  &	- \\
skg  &	200K  &	West Malagasy Sakalava  &	1M  &	Africa  &	Latn  &	\scriptsize{apy-7l}  &	93.4  &	57.6 \\
mrj  &	200K  &	Western Mari  &	5K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	94.3  &	45.8 \\
bci  &	200K  &	Baoulé  &	2M  &	Africa  &	Latn  &	\scriptsize{ada-13l}  &	98.9  &	32.1 \\
ch  &	200K  &	Chamorro  &	50K  &	Oceania  &	Latn  &	\scriptsize{ayo-4l}  &	98.9  &	31.9 \\
qvi  &	200K  &	Imbabura Highland Quichua  &	300K  &	Americas  &	Latn  &	\scriptsize{quw-5l}  &	100  &	38.7 \\
gym  &	200K  &	Ngäbere  &	200K  &	Americas  &	Latn  &	gym  &	100  &	19.5 \\
cyo  &	150K  &	Cuyonon  &	100K  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	85.0  &	69.1 \\
stq  &	150K  &	Ems-Weser Frisian  &	5K  &	Europe  &	Latn  &	\scriptsize{apr-8l}  &	89.6  &	- \\
tcy  &	150K  &	Tulu  &	2M  &	Asia  &	Knda  &	\scriptsize{lmn-Knda-2l}  &	100  &	49.4 \\
meu  &	150K  &	Motu  &	50K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	99.1  &	27.4 \\
pau  &	150K  &	Palauan  &	50K  &	Oceania  &	Latn  &	pau  &	100  &	- \\
bas  &	150K  &	Basa (Cameroon)  &	300K  &	Africa  &	Latn  &	\scriptsize{bas-11l}  &	99.4  &	21.0 \\
guc  &	140K  &	Wayuu  &	300K  &	Americas  &	Latn  &	guc  &	100  &	18.5 \\
quy  &	140K  &	Ayacucho Quechua  &	900K  &	Americas  &	Latn  &	\scriptsize{ae-Latn-10l}  &	99.7  &	29.8 \\
gu-Latn  &	140K  &	Gujarati  &	56M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	98.1  &	60.9 \\
mad  &	140K  &	Madurese  &	7M  &	Asia  &	Latn  &	\scriptsize{ade-4l}  &	99.8  &	44.7 \\
cbk  &	140K  &	Chavacano  &	700K  &	Asia  &	Latn  &	cbk  &	100  &	- \\
awa  &	140K  &	Awadhi  &	4M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	98.1  &	61.4 \\
brx  &	130K  &	Bodo-Mech  &	1M  &	Asia  &	Deva  &	\scriptsize{ahr-13l}  &	100  &	32.8 \\
koi  &	130K  &	Komi-Permyak  &	50K  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	93.7  &	40.6 \\
arn  &	130K  &	Mapudungun  &	300K  &	Americas  &	Latn  &	\scriptsize{arn-6l}  &	99.6  &	33.6 \\
nv  &	130K  &	Navajo  &	200K  &	Americas  &	Latn  &	\scriptsize{nv-2l}  &	99.2  &	24.6 \\
nhe  &	130K  &	Eastern Huasteca Nahuatl  &	400K  &	Americas  &	Latn  &	\scriptsize{azz-7l}  &	99.7  &	29.4 \\
fip  &	130K  &	Fipa  &	200K  &	Africa  &	Latn  &	\scriptsize{dov-9l}  &	100  &	32.0 \\
dyu  &	130K  &	Dyula  &	16M  &	Africa  &	Latn  &	\scriptsize{ada-13l}  &	99.8  &	27.8 \\
xnr  &	130K  &	Kangri  &	2M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	96.2  &	57.7 \\
kbp  &	130K  &	Kabiyé  &	1M  &	Africa  &	Latn  &	\scriptsize{kbp-2l}  &	100  &	32.1 \\
kw  &	130K  &	Cornish  &	5K  &	Europe  &	Latn  &	\scriptsize{br-4l}  &	92.6  &	- \\
kri  &	130K  &	Krio  &	4M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	99.6  &	61.0 \\
rn  &	130K  &	Rundi  &	9M  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	97.5  &	- \\
mdf  &	120K  &	Moksha  &	5K  &	Europe  &	Cyrl  &	\scriptsize{ady-9l}  &	84.8  &	- \\
tzh  &	120K  &	Tzeltal  &	400K  &	Americas  &	Latn  &	\scriptsize{arn-6l}  &	99.4  &	30.9 \\
cab  &	120K  &	Garifuna  &	200K  &	Americas  &	Latn  &	\scriptsize{bch-10l}  &	100  &	18.8 \\
trp  &	120K  &	Kok Borok  &	800K  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	99.8  &	38.3 \\
mkn  &	120K  &	Kupang Malay  &	200K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	98.6  &	53.7 \\
rki  &	120K  &	Rakhine  &	2M  &	Asia  &	Mymr  &	rki  &	99.9  &	49.2 \\
gyn  &	120K  &	Guyanese Creole English  &	600K  &	Americas  &	Latn  &	\scriptsize{bzj-9l}  &	99.4  &	71.8 \\
syl-Latn  &	120K  &	Sylheti  &	23M  &	Asia  &	Latn  &	\scriptsize{bn-Latn-6l}  &	99.1  &	- \\
max  &	120K  &	North Moluccan Malay  &	700K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	91.3  &	- \\
izz  &	120K  &	Izi  &	500K  &	Africa  &	Latn  &	\scriptsize{anw-8l}  &	99.7  &	26.6 \\
dje  &	110K  &	Zarma-Kaado  &	2M  &	Africa  &	Latn  &	\scriptsize{ang-7l}  &	99.6  &	22.2 \\
smt  &	110K  &	Simte  &	50K  &	Asia  &	Latn  &	\scriptsize{bgs-9l}  &	99.9  &	- \\
iu  &	110K  &	Inuktitut  &	50K  &	Americas  &	Cans  &	\scriptsize{crm-3l}  &	99.8  &	26.9 \\
bmm  &	110K  &	Northern Betsimisaraka Malagasy  &	1M  &	Africa  &	Latn  &	\scriptsize{apy-7l}  &	91.8  &	- \\
lhu  &	110K  &	Lahu  &	500K  &	Asia  &	Latn  &	\scriptsize{hni-8l}  &	99.9  &	29.3 \\
djk  &	110K  &	Aukan  &	50K  &	Americas  &	Latn  &	\scriptsize{djk-3l}  &	100  &	35.3 \\
cuk  &	110K  &	San Blas Kuna  &	50K  &	Americas  &	Latn  &	\scriptsize{bnj-6l}  &	100  &	12.3 \\
mni  &	110K  &	Manipuri  &	2M  &	Asia  &	Beng  &	mni  &	99.9  &	37.9 \\
mak  &	100K  &	Makasar  &	5M  &	Asia  &	Latn  &	mak  &	100  &	19.2 \\
bto  &	100K  &	Iriga Bicolano  &	200K  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	95.2  &	64.6 \\
tab  &	100K  &	Tabasaran  &	100K  &	Europe  &	Cyrl  &	\scriptsize{ce-3l}  &	100  &	33.4 \\
mps  &	100K  &	Dadibi  &	50K  &	Oceania  &	Latn  &	\scriptsize{mps-3l}  &	99.8  &	- \\
mbt  &	100K  &	Matigsalug Manobo  &	50K  &	Asia  &	Latn  &	mbt  &	100  &	21.5 \\
gui  &	100K  &	Eastern Bolivian Guaraní  &	50K  &	Americas  &	Latn  &	gui  &	100  &	20.6 \\
fan  &	100K  &	Fang (Equatorial Guinea)  &	1M  &	Africa  &	Latn  &	\scriptsize{bas-11l}  &	99.1  &	31.0 \\
ngu  &	100K  &	Central Guerrero Nahuatl  &	200K  &	Americas  &	Latn  &	\scriptsize{azz-7l}  &	99.7  &	28.3 \\
srm  &	100K  &	Saramaccan  &	50K  &	Americas  &	Latn  &	\scriptsize{djk-3l}  &	100  &	- \\
ms-Arab-BN  &	100K  &	Malay  &	80M  &	Asia  &	Arab  &	\scriptsize{mfa-3l}  &	92.7  &	53.9 \\
ndc-ZW  &	100K  &	Ndau  &	2M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	99.0  &	60.5 \\
nnb  &	100K  &	Nande  &	900K  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.7  &	35.7 \\
ber  &	100K  &	Berber  &	2M  &	Africa  &	Tfng  &	ber  &	100  &	26.5 \\
ibb  &	100K  &	Ibibio  &	2M  &	Africa  &	Latn  &	\scriptsize{anw-8l}  &	98.6  &	48.3 \\
nyu  &	90K  &	Nyungwe  &	400K  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	98.0  &	- \\
gub  &	90K  &	Guajajára  &	50K  &	Americas  &	Latn  &	\scriptsize{abr-5l}  &	100  &	- \\
kmb  &	90K  &	Kimbundu  &	4M  &	Africa  &	Latn  &	\scriptsize{dov-9l}  &	100  &	25.0 \\
trw  &	90K  &	Torwali  &	50K  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	88.4  &	43.8 \\
nij  &	90K  &	Ngaju  &	900K  &	Asia  &	Latn  &	\scriptsize{kje-6l}  &	100  &	38.9 \\
cgg  &	90K  &	Chiga  &	2M  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.3  &	50.5 \\
twu  &	90K  &	Termanu  &	50K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	100  &	19.9 \\
kn-Latn  &	90K  &	Kannada  &	43M  &	Asia  &	Latn  &	\scriptsize{bgp-13l}  &	98.6  &	46.0 \\
ms-Arab  &	90K  &	Malay  &	80M  &	Asia  &	Arab  &	\scriptsize{mfa-3l}  &	88.9  &	55.7 \\
oj  &	90K  &	Ojibwe  &	50K  &	Americas  &	Latn  &	\scriptsize{agr-3l}  &	99.9  &	- \\
acf  &	90K  &	Saint Lucian Creole French  &	200K  &	Americas  &	Latn  &	\scriptsize{acf-10l}  &	100  &	48.9 \\
cac  &	90K  &	Chuj  &	50K  &	Americas  &	Latn  &	cac  &	100  &	13.8 \\
jiv  &	90K  &	Shuar  &	50K  &	Americas  &	Latn  &	\scriptsize{bn-Latn-6l}  &	100  &	12.0 \\
alz  &	90K  &	Alur  &	2M  &	Africa  &	Latn  &	\scriptsize{adh-5l}  &	99.6  &	21.3 \\
akb  &	90K  &	Batak Angkola  &	800K  &	Asia  &	Latn  &	\scriptsize{akb-4l}  &	100  &	15.4 \\
ff  &	90K  &	Fula  &	12M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	90.6  &	40.6 \\
aa  &	80K  &	Afar  &	2M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	99.7  &	19.8 \\
miq  &	80K  &	Mískito  &	200K  &	Americas  &	Latn  &	\scriptsize{miq-2l}  &	100  &	19.1 \\
bgz  &	80K  &	Banggai  &	100K  &	Asia  &	Latn  &	\scriptsize{amo-7l}  &	92.7  &	56.2 \\
nyn  &	80K  &	Nyankole  &	2M  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.7  &	37.7 \\
adh  &	80K  &	Adhola  &	400K  &	Africa  &	Latn  &	\scriptsize{adh-5l}  &	100  &	18.5 \\
bzj  &	80K  &	Belize Kriol English  &	200K  &	Americas  &	Latn  &	\scriptsize{bzj-9l}  &	100  &	57.9 \\
nyo  &	80K  &	Nyoro  &	700K  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.3  &	46.7 \\
kfy  &	80K  &	Kumaoni  &	2M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	93.8  &	50.7 \\
kjb  &	80K  &	Q'anjob'al  &	50K  &	Americas  &	Latn  &	\scriptsize{cbr-6l}  &	96.7  &	14.3 \\
frp  &	80K  &	Arpitan  &	100K  &	Europe  &	Latn  &	\scriptsize{acf-10l}  &	90.4  &	- \\
jvn  &	80K  &	Caribbean Javanese  &	50K  &	Americas  &	Latn  &	jvn  &	100  &	26.9 \\
mdy  &	80K  &	Male (Ethiopia)  &	100K  &	Africa  &	Ethi  &	mdy  &	100  &	22.7 \\
hae  &	80K  &	Eastern Oromo  &	4M  &	Africa  &	Latn  &	\scriptsize{amf-6l}  &	99.5  &	48.6 \\
qxr  &	80K  &	Cañar Highland Quichua  &	200K  &	Americas  &	Latn  &	\scriptsize{quw-5l}  &	99.7  &	37.7 \\
noa  &	80K  &	Woun Meu  &	50K  &	Americas  &	Latn  &	\scriptsize{cbv-6l}  &	99.9  &	- \\
krj  &	70K  &	Kinaray-a  &	400K  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	99.5  &	58.9 \\
hui  &	70K  &	Huli  &	200K  &	Oceania  &	Latn  &	\scriptsize{hui-3l}  &	99.9  &	12.0 \\
enq  &	70K  &	Enga  &	200K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	99.5  &	12.1 \\
sgj  &	70K  &	Surgujia  &	1M  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	97.5  &	56.8 \\
lrl  &	70K  &	Larestani  &	200K  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	56.8  &	- \\
gof  &	70K  &	Gofa  &	400K  &	Africa  &	Ethi  &	\scriptsize{drs-Latn-8l}  &	99.6  &	24.1 \\
sxn  &	70K  &	Sangir  &	200K  &	Asia  &	Latn  &	sxn  &	100  &	31.9 \\
hus  &	70K  &	Huastec  &	100K  &	Americas  &	Latn  &	\scriptsize{chd-6l}  &	100  &	19.6 \\
tuc  &	70K  &	Mutu  &	5K  &	Oceania  &	Latn  &	\scriptsize{bmu-6l}  &	100  &	- \\
maz  &	70K  &	Central Mazahua  &	50K  &	Americas  &	Latn  &	\scriptsize{jic-3l}  &	100  &	15.7 \\
hix  &	70K  &	Hixkaryána  &	5K  &	Americas  &	Latn  &	hix  &	99.6  &	- \\
ks  &	70K  &	Kashmiri  &	6M  &	Asia  &	Arab  &	\scriptsize{doi-Arab-5l}  &	96.5  &	47.0 \\
clu  &	70K  &	Caluyanun  &	50K  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	98.9  &	- \\
acx  &	70K  &	Omani Arabic  &	1M  &	Europe  &	Arab  &	\scriptsize{abv-10l}  &	4.9  &	- \\
prk  &	70K  &	South Wa  &	800K  &	Asia  &	Latn  &	\scriptsize{ace-12l}  &	100  &	26.3 \\
mas  &	70K  &	Masai  &	1M  &	Africa  &	Latn  &	\scriptsize{big-5l}  &	99.8  &	16.2 \\
pis  &	70K  &	Pijin  &	400K  &	Oceania  &	Latn  &	\scriptsize{bi-6l}  &	100  &	21.3 \\
amu  &	70K  &	Guerrero Amuzgo  &	50K  &	Americas  &	Latn  &	amu  &	100  &	12.0 \\
myu  &	70K  &	Mundurukú  &	5K  &	Americas  &	Latn  &	\scriptsize{bch-10l}  &	99.9  &	- \\
kjg  &	70K  &	Khmu  &	700K  &	Asia  &	Laoo  &	\scriptsize{kjg-2l}  &	100  &	37.1 \\
sda  &	70K  &	Toraja-Sa'dan  &	800K  &	Asia  &	Latn  &	\scriptsize{kje-6l}  &	98.4  &	20.1 \\
kpg  &	70K  &	Kapingamarangi  &	5K  &	Oceania  &	Latn  &	kpg  &	100  &	- \\
bus  &	70K  &	Bokobaru  &	50K  &	Africa  &	Latn  &	\scriptsize{akp-4l}  &	99.5  &	16.5 \\
mag  &	70K  &	Magahi  &	28M  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	99.6  &	57.7 \\
dwr  &	70K  &	Dawro  &	500K  &	Africa  &	Latn  &	\scriptsize{drs-Latn-8l}  &	100  &	19.8 \\
sja  &	70K  &	Epena  &	5K  &	Americas  &	Latn  &	\scriptsize{mpm-4l}  &	99.1  &	- \\
ahk  &	60K  &	Akha  &	600K  &	Asia  &	Latn  &	ahk  &	100  &	26.2 \\
ffm  &	60K  &	Maasina Fulfulde  &	1M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	98.6  &	29.0 \\
xav  &	60K  &	Xavánte  &	5K  &	Americas  &	Latn  &	xav  &	87.5  &	- \\
chr  &	60K  &	Cherokee  &	50K  &	Americas  &	Cher  &	chr  &	100  &	19.7 \\
kyz  &	60K  &	Kayabí  &	5K  &	Americas  &	Latn  &	\scriptsize{avt-12l}  &	71.1  &	- \\
tll  &	60K  &	Tetela  &	800K  &	Africa  &	Latn  &	\scriptsize{kj-5l}  &	99.9  &	24.8 \\
tee  &	60K  &	Huehuetla Tepehua  &	5K  &	Americas  &	Latn  &	\scriptsize{tee-2l}  &	99.9  &	- \\
niq  &	60K  &	Nandi  &	1M  &	Africa  &	Latn  &	\scriptsize{awk-4l}  &	98.8  &	20.0 \\
din  &	60K  &	Dinka  &	1M  &	Africa  &	Latn  &	\scriptsize{din-3l}  &	99.7  &	27.6 \\
nog  &	60K  &	Nogai  &	50K  &	Europe  &	Cyrl  &	\scriptsize{bcq-Latn-12l}  &	100  &	51.6 \\
tca  &	60K  &	Ticuna  &	50K  &	Americas  &	Latn  &	tca  &	100  &	8.6 \\
abt  &	60K  &	Ambulas  &	50K  &	Oceania  &	Latn  &	\scriptsize{abt-3l}  &	99.8  &	10.3 \\
bhw  &	60K  &	Biak  &	50K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	100  &	20.5 \\
dln  &	60K  &	Darlong  &	5K  &	Asia  &	Latn  &	\scriptsize{bla-7l}  &	99.9  &	- \\
xog  &	60K  &	Soga  &	3M  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.4  &	56.6 \\
cbt  &	60K  &	Shawi  &	5K  &	Americas  &	Latn  &	\scriptsize{cbt-2l}  &	100  &	- \\
vep  &	60K  &	Veps  &	5K  &	Europe  &	Latn  &	\scriptsize{gaw-8l}  &	90.9  &	- \\
gil  &	60K  &	Gilbertese  &	100K  &	Oceania  &	Latn  &	\scriptsize{aaz-6l}  &	100  &	14.3 \\
tyz  &	60K  &	Tày  &	3M  &	Asia  &	Latn  &	\scriptsize{blt-Latn-4l}  &	99.5  &	22.8 \\
bqc  &	60K  &	Boko (Benin)  &	200K  &	Africa  &	Latn  &	\scriptsize{akp-4l}  &	99.8  &	19.0 \\
ksd  &	60K  &	Kuanua  &	50K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	99.2  &	15.4 \\
tob  &	60K  &	Toba  &	50K  &	Americas  &	Latn  &	\scriptsize{hni-8l}  &	100  &	13.3 \\
bru  &	60K  &	Eastern Bru  &	50K  &	Asia  &	Latn  &	\scriptsize{bru-6l}  &	100  &	21.4 \\
sat-Latn  &	60K  &	Santali  &	6M  &	Asia  &	Latn  &	\scriptsize{aaz-6l}  &	98.9  &	40.0 \\
msy  &	60K  &	Aruamu  &	5K  &	Oceania  &	Latn  &	\scriptsize{msy-2l}  &	99.6  &	- \\
cbu  &	60K  &	Candoshi-Shapra  &	5K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	99.1  &	- \\
shp  &	60K  &	Shipibo-Conibo  &	50K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	100  &	- \\
qub  &	60K  &	Huallaga Huánuco Quechua  &	50K  &	Americas  &	Latn  &	\scriptsize{qub-7l}  &	99.5  &	26.0 \\
agr  &	60K  &	Aguaruna  &	50K  &	Americas  &	Latn  &	\scriptsize{agr-3l}  &	100  &	14.6 \\
emp  &	60K  &	Northern Emberá  &	50K  &	Americas  &	Latn  &	\scriptsize{cbv-6l}  &	99.6  &	12.3 \\
suz  &	60K  &	Sunwar  &	50K  &	Asia  &	Deva  &	suz  &	100  &	17.2 \\
maa  &	60K  &	San Jerónimo Tecóatl Mazatec  &	50K  &	Americas  &	Latn  &	\scriptsize{kcg-9l}  &	100  &	- \\
ifk  &	60K  &	Tuwali Ifugao  &	50K  &	Asia  &	Latn  &	\scriptsize{bnc-8l}  &	100  &	19.9 \\
arc  &	50K  &	Official Aramaic (700-300 BCE)  &	0K  &	Europe  &	Syrc  &	\scriptsize{ach-10l}  &	80.0  &	- \\
bim  &	50K  &	Bimoba  &	400K  &	Africa  &	Latn  &	\scriptsize{bim-3l}  &	100  &	15.6 \\
otq  &	50K  &	Querétaro Otomi  &	50K  &	Americas  &	Latn  &	\scriptsize{ann-3l}  &	99.9  &	47.0 \\
tdx  &	50K  &	Tandroy Malagasy  &	1M  &	Africa  &	Latn  &	\scriptsize{apy-7l}  &	99.6  &	48.2 \\
tav  &	50K  &	Tatuyo  &	5K  &	Americas  &	Latn  &	\scriptsize{des-4l}  &	100  &	- \\
pir  &	50K  &	Wa'ikhana  &	5K  &	Americas  &	Latn  &	\scriptsize{des-4l}  &	99.6  &	- \\
ded  &	50K  &	Dedua  &	5K  &	Oceania  &	Latn  &	\scriptsize{bru-6l}  &	99.7  &	- \\
txu  &	50K  &	Kayapó  &	5K  &	Americas  &	Latn  &	\scriptsize{apn-3l}  &	99.2  &	- \\
qvh  &	50K  &	Huamalíes-Dos de Mayo Huánuco Quechua  &	50K  &	Americas  &	Latn  &	\scriptsize{qub-7l}  &	100  &	19.7 \\
mav  &	50K  &	Sateré-Mawé  &	5K  &	Americas  &	Latn  &	\scriptsize{bwu-4l}  &	100  &	- \\
ubu  &	50K  &	Umbu-Ungu  &	50K  &	Oceania  &	Latn  &	\scriptsize{gbi-8l}  &	99.9  &	11.8 \\
toj  &	50K  &	Tojolabal  &	50K  &	Americas  &	Latn  &	\scriptsize{toj-4l}  &	100  &	27.2 \\
inb  &	50K  &	Inga  &	50K  &	Americas  &	Latn  &	inb  &	100  &	- \\
aoj  &	50K  &	Mufian  &	50K  &	Oceania  &	Latn  &	aoj  &	99.6  &	- \\
mbb  &	50K  &	Western Bukidnon Manobo  &	50K  &	Asia  &	Latn  &	\scriptsize{mbb-3l}  &	85.9  &	- \\
acr  &	50K  &	Achi  &	50K  &	Americas  &	Latn  &	\scriptsize{acr-4l}  &	99.9  &	21.1 \\
xtd  &	50K  &	Diuxi-Tilantongo Mixtec  &	5K  &	Americas  &	Latn  &	\scriptsize{mpm-4l}  &	99.9  &	- \\
kjh  &	50K  &	Khakas  &	50K  &	Europe  &	Cyrl  &	kjh  &	100  &	37.9 \\
dyi  &	50K  &	Djimini Senoufo  &	50K  &	Africa  &	Latn  &	dyi  &	100  &	18.5 \\
mpm  &	50K  &	Yosondúa Mixtec  &	50K  &	Americas  &	Latn  &	\scriptsize{mpm-4l}  &	99.7  &	- \\
kwi  &	50K  &	Awa-Cuaiquer  &	50K  &	Americas  &	Latn  &	\scriptsize{bla-7l}  &	100  &	- \\
bjj  &	50K  &	Kanauji  &	10M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	97.8  &	55.4 \\
amn  &	50K  &	Amanab  &	5K  &	Oceania  &	Latn  &	\scriptsize{amn-2l}  &	99.9  &	- \\
plu  &	50K  &	Palikúr  &	5K  &	Americas  &	Latn  &	plu  &	98.7  &	- \\
ood  &	50K  &	Tohono O'odham  &	50K  &	Americas  &	Latn  &	\scriptsize{alq-4l}  &	100  &	- \\
czt  &	50K  &	Zotung Chin  &	50K  &	Asia  &	Latn  &	czt  &	100  &	19.9 \\
tbg  &	50K  &	North Tairora  &	50K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	100  &	- \\
gjk  &	50K  &	Kachi Koli  &	600K  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	77.3  &	59.6 \\
crn  &	50K  &	El Nayar Cora  &	50K  &	Americas  &	Latn  &	\scriptsize{cok-2l}  &	99.7  &	- \\
cni  &	50K  &	Asháninka  &	50K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	100  &	13.0 \\
qup  &	50K  &	Southern Pastaza Quechua  &	1M  &	Americas  &	Latn  &	\scriptsize{qup-2l}  &	99.7  &	- \\
ify  &	50K  &	Keley-i Kallahan  &	50K  &	Asia  &	Latn  &	ify  &	99.9  &	- \\
srq  &	50K  &	Sirionó  &	5K  &	Americas  &	Latn  &	\scriptsize{srq-3l}  &	98.9  &	- \\
tbz  &	50K  &	Ditammari  &	200K  &	Africa  &	Latn  &	\scriptsize{gej-4l}  &	100  &	16.1 \\
aeb  &	50K  &	Tunisian Arabic  &	11M  &	Africa  &	Arab  &	\scriptsize{abv-10l}  &	13.1  &	- \\
sus  &	50K  &	Susu  &	1M  &	Africa  &	Latn  &	\scriptsize{bas-11l}  &	100  &	20.5 \\
itv  &	50K  &	Itawit  &	100K  &	Asia  &	Latn  &	\scriptsize{bnj-6l}  &	99.9  &	28.9 \\
cce  &	50K  &	Chopi  &	800K  &	Africa  &	Latn  &	\scriptsize{cce-8l}  &	99.4  &	33.3 \\
qwh  &	50K  &	Huaylas Ancash Quechua  &	300K  &	Americas  &	Latn  &	\scriptsize{nhg-3l}  &	100  &	25.4 \\
teo  &	50K  &	Teso  &	2M  &	Africa  &	Latn  &	\scriptsize{bla-7l}  &	100  &	14.4 \\
lon  &	50K  &	Malawi Lomwe  &	2M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	99.5  &	- \\
gun  &	50K  &	Mbyá Guaraní  &	50K  &	Americas  &	Latn  &	\scriptsize{gn-6l}  &	99.4  &	- \\
ppk  &	50K  &	Uma  &	50K  &	Asia  &	Latn  &	\scriptsize{pmf-2l}  &	100  &	- \\
ann  &	50K  &	Obolo  &	200K  &	Africa  &	Latn  &	\scriptsize{ann-3l}  &	100  &	26.3 \\
laj  &	50K  &	Lango (Uganda)  &	2M  &	Africa  &	Latn  &	\scriptsize{adh-5l}  &	99.7  &	25.7 \\
eza  &	50K  &	Ezaa  &	600K  &	Africa  &	Latn  &	\scriptsize{anw-8l}  &	99.7  &	29.2 \\
caf  &	50K  &	Southern Carrier  &	5K  &	Americas  &	Latn  &	\scriptsize{bpr-7l}  &	99.9  &	- \\
lex  &	50K  &	Luang  &	50K  &	Asia  &	Latn  &	\scriptsize{kje-6l}  &	100  &	- \\
msm  &	50K  &	Agusan Manobo  &	50K  &	Asia  &	Latn  &	\scriptsize{atd-4l}  &	100  &	24.6 \\
tuf  &	50K  &	Central Tunebo  &	5K  &	Americas  &	Latn  &	tuf  &	100  &	- \\
quf  &	50K  &	Lambayeque Quechua  &	50K  &	Americas  &	Latn  &	\scriptsize{ae-Latn-10l}  &	99.5  &	- \\
bzc  &	50K  &	Southern Betsimisaraka Malagasy  &	2M  &	Africa  &	Latn  &	\scriptsize{apy-7l}  &	96.4  &	61.4 \\
jbo  &	50K  &	Lojban  &	0K  &	Europe  &	Latn  &	\scriptsize{bi-6l}  &	98.0  &	- \\
yss  &	50K  &	Yessan-Mayo  &	5K  &	Oceania  &	Latn  &	\scriptsize{bom-5l}  &	99.9  &	- \\
tzj  &	50K  &	Tz'utujil  &	50K  &	Americas  &	Latn  &	tzj  &	100  &	13.4 \\
qvc  &	40K  &	Cajamarca Quechua  &	50K  &	Americas  &	Latn  &	qvc  &	100  &	16.4 \\
stp  &	40K  &	Southeastern Tepehuan  &	50K  &	Americas  &	Latn  &	\scriptsize{cbr-6l}  &	100  &	- \\
wsk  &	40K  &	Waskia  &	50K  &	Oceania  &	Latn  &	\scriptsize{aom-10l}  &	97.7  &	- \\
knj  &	40K  &	Akateko  &	50K  &	Americas  &	Latn  &	\scriptsize{knj-8l}  &	99.3  &	15.8 \\
qvz  &	40K  &	Northern Pastaza Quichua  &	50K  &	Americas  &	Latn  &	\scriptsize{quw-5l}  &	100  &	- \\
pad  &	40K  &	Paumari  &	5K  &	Americas  &	Latn  &	\scriptsize{anw-8l}  &	100  &	- \\
cbi  &	40K  &	Cha'palaa  &	5K  &	Americas  &	Latn  &	cbi  &	100  &	- \\
tac  &	40K  &	Lowland Tarahumara  &	50K  &	Americas  &	Latn  &	\scriptsize{alp-2l}  &	99.9  &	- \\
ngl  &	40K  &	Mozambique Lomwe  &	2M  &	Africa  &	Latn  &	\scriptsize{cjk-14l}  &	96.2  &	- \\
kaq  &	40K  &	Capanahua  &	50K  &	Americas  &	Latn  &	\scriptsize{bgs-9l}  &	100  &	- \\
jam  &	40K  &	Jamaican Creole English  &	3M  &	Americas  &	Latn  &	\scriptsize{bzj-9l}  &	99.9  &	57.9 \\
cpy  &	40K  &	South Ucayali Ashéninka  &	5K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	99.2  &	15.0 \\
en-Cyrl  &	40K  &	English  &	550M  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	98.0  &	87.3 \\
car  &	40K  &	Galibi Carib  &	5K  &	Americas  &	Latn  &	car  &	100  &	- \\
gju  &	40K  &	Gujari  &	1M  &	Asia  &	Arab  &	\scriptsize{doi-Arab-5l}  &	98.9  &	51.3 \\
pab  &	40K  &	Parecís  &	5K  &	Americas  &	Latn  &	\scriptsize{pab-2l}  &	99.9  &	- \\
yuj  &	40K  &	Karkar-Yuri  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	98.0  &	- \\
jac  &	40K  &	Popti'  &	5K  &	Americas  &	Latn  &	\scriptsize{ayo-4l}  &	98.1  &	- \\
mjc  &	40K  &	San Juan Colorado Mixtec  &	50K  &	Americas  &	Latn  &	\scriptsize{cta-4l}  &	99.6  &	- \\
med  &	40K  &	Melpa  &	100K  &	Oceania  &	Latn  &	\scriptsize{cwt-4l}  &	100  &	13.6 \\
qvs  &	40K  &	San Martín Quechua  &	50K  &	Americas  &	Latn  &	\scriptsize{qup-2l}  &	99.7  &	- \\
urb  &	40K  &	Urubú-Kaapor  &	5K  &	Americas  &	Latn  &	\scriptsize{bhw-9l}  &	99.7  &	- \\
bnp  &	40K  &	Bola  &	50K  &	Oceania  &	Latn  &	\scriptsize{bch-10l}  &	99.0  &	- \\
yle  &	40K  &	Yele  &	5K  &	Oceania  &	Latn  &	\scriptsize{bib-2l}  &	100  &	- \\
acu  &	40K  &	Achuar-Shiwiar  &	5K  &	Americas  &	Latn  &	\scriptsize{acu-8l}  &	99.1  &	- \\
cof  &	40K  &	Tsafiki  &	5K  &	Americas  &	Latn  &	\scriptsize{bmr-3l}  &	100  &	- \\
poh  &	40K  &	Poqomchi'  &	50K  &	Americas  &	Latn  &	\scriptsize{hni-8l}  &	100  &	12.6 \\
gbi  &	40K  &	Galela  &	50K  &	Asia  &	Latn  &	\scriptsize{gbi-8l}  &	100  &	13.6 \\
kto  &	40K  &	Kuot  &	5K  &	Oceania  &	Latn  &	\scriptsize{bkv-4l}  &	99.9  &	- \\
bfz  &	40K  &	Mahasu Pahari  &	1M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	94.4  &	- \\
cao  &	40K  &	Chácobo  &	5K  &	Americas  &	Latn  &	\scriptsize{auc-6l}  &	99.7  &	- \\
myy  &	40K  &	Macuna  &	5K  &	Americas  &	Latn  &	\scriptsize{cub-2l}  &	100  &	- \\
aaz  &	40K  &	Amarasi  &	50K  &	Asia  &	Latn  &	\scriptsize{aaz-6l}  &	100  &	15.3 \\
nch  &	40K  &	Central Huasteca Nahuatl  &	200K  &	Americas  &	Latn  &	\scriptsize{azz-7l}  &	95.7  &	19.2 \\
ixl  &	40K  &	Ixil  &	100K  &	Americas  &	Latn  &	\scriptsize{ctp-4l}  &	100  &	15.1 \\
rwo  &	40K  &	Rawa  &	50K  &	Oceania  &	Latn  &	\scriptsize{gbi-8l}  &	99.9  &	- \\
azg  &	40K  &	San Pedro Amuzgos Amuzgo  &	50K  &	Americas  &	Latn  &	\scriptsize{azg-4l}  &	100  &	- \\
yaq  &	40K  &	Yaqui  &	50K  &	Americas  &	Latn  &	yaq  &	99.6  &	- \\
iou  &	40K  &	Tuma-Irumu  &	5K  &	Oceania  &	Latn  &	\scriptsize{awx-2l}  &	97.0  &	- \\
qvw  &	40K  &	Huaylla Wanca Quechua  &	300K  &	Americas  &	Latn  &	\scriptsize{qub-7l}  &	100  &	16.7 \\
snn  &	40K  &	Siona-Tetete  &	5K  &	Americas  &	Latn  &	\scriptsize{azg-4l}  &	100  &	- \\
sxu  &	40K  &	Central East Middle German  &	2M  &	Europe  &	Latn  &	\scriptsize{ang-7l}  &	99.9  &	64.3 \\
bch  &	40K  &	Bariai  &	5K  &	Oceania  &	Latn  &	\scriptsize{bch-10l}  &	98.8  &	- \\
bud  &	40K  &	Ntcham  &	300K  &	Africa  &	Latn  &	\scriptsize{amf-6l}  &	100  &	17.2 \\
tih  &	40K  &	Timugon Murut  &	5K  &	Asia  &	Latn  &	\scriptsize{tih-2l}  &	99.8  &	- \\
mcd  &	40K  &	Sharanahua  &	5K  &	Americas  &	Latn  &	\scriptsize{cbt-2l}  &	100  &	- \\
apn  &	40K  &	Apinayé  &	5K  &	Americas  &	Latn  &	\scriptsize{apn-3l}  &	91.4  &	- \\
yaa  &	40K  &	Yaminahua  &	5K  &	Americas  &	Latn  &	yaa  &	100  &	- \\
mqy  &	40K  &	Manggarai  &	900K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	97.8  &	48.9 \\
yka  &	40K  &	Yakan  &	100K  &	Asia  &	Latn  &	\scriptsize{bpr-7l}  &	99.8  &	23.6 \\
rmc  &	40K  &	Central Romani  &	100K  &	Europe  &	Latn  &	\scriptsize{rmc-3l}  &	100  &	25.7 \\
tfr  &	40K  &	Teribe  &	5K  &	Americas  &	Latn  &	\scriptsize{pxm-2l}  &	100  &	- \\
tna  &	40K  &	Tacana  &	5K  &	Americas  &	Latn  &	\scriptsize{nhg-3l}  &	100  &	- \\
nhy  &	40K  &	Northern Oaxaca Nahuatl  &	50K  &	Americas  &	Latn  &	\scriptsize{nhy-3l}  &	99.7  &	- \\
nfa  &	40K  &	Dhao  &	5K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	99.1  &	- \\
zos  &	40K  &	Francisco León Zoque  &	50K  &	Americas  &	Latn  &	\scriptsize{ayo-4l}  &	98.4  &	- \\
zpz  &	40K  &	Texmelucan Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{srq-3l}  &	100  &	- \\
mqj  &	40K  &	Mamasa  &	50K  &	Asia  &	Latn  &	\scriptsize{kje-6l}  &	97.9  &	14.5 \\
xsi  &	40K  &	Sio  &	5K  &	Oceania  &	Latn  &	\scriptsize{kij-2l}  &	99.9  &	- \\
srr  &	40K  &	Sereer  &	1M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	81.6  &	21.4 \\
hac  &	40K  &	Gurani  &	400K  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	68.6  &	52.1 \\
yal  &	40K  &	Yalunka  &	100K  &	Africa  &	Latn  &	\scriptsize{bas-11l}  &	100  &	16.4 \\
aey  &	40K  &	Amele  &	5K  &	Oceania  &	Latn  &	\scriptsize{aey-6l}  &	97.3  &	- \\
lep-Tibt  &	40K  &	Lepcha  &	50K  &	Asia  &	Tibt  &	lep-Tibt  &	100  &	9.9 \\
kia  &	40K  &	Kim  &	50K  &	Africa  &	Latn  &	\scriptsize{cut-5l}  &	99.9  &	- \\
sef  &	40K  &	Cebaara Senoufo  &	3M  &	Africa  &	Latn  &	\scriptsize{ada-13l}  &	98.7  &	41.1 \\
lac  &	40K  &	Lacandon  &	5K  &	Americas  &	Latn  &	lac  &	99.8  &	- \\
rro  &	40K  &	Waima  &	50K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	97.7  &	- \\
cav  &	40K  &	Cavineña  &	5K  &	Americas  &	Latn  &	\scriptsize{aak-3l}  &	99.9  &	- \\
bvz  &	40K  &	Bauzi  &	5K  &	Asia  &	Latn  &	\scriptsize{adz-3l}  &	100  &	- \\
qxh  &	40K  &	Panao Huánuco Quechua  &	50K  &	Americas  &	Latn  &	\scriptsize{qub-7l}  &	99.5  &	17.3 \\
mcf  &	40K  &	Matsés  &	5K  &	Americas  &	Latn  &	\scriptsize{con-3l}  &	100  &	- \\
gvl  &	40K  &	Gulay  &	200K  &	Africa  &	Latn  &	\scriptsize{dzg-5l}  &	92.6  &	- \\
alq  &	40K  &	Algonquin  &	5K  &	Americas  &	Latn  &	\scriptsize{alq-4l}  &	99.9  &	- \\
gum  &	40K  &	Guambiano  &	50K  &	Americas  &	Latn  &	\scriptsize{cjp-4l}  &	100  &	- \\
cr-Latn  &	40K  &	Cree  &	200K  &	Americas  &	Latn  &	\scriptsize{ach-10l}  &	24.2  &	- \\
guh  &	40K  &	Guahibo  &	50K  &	Americas  &	Latn  &	\scriptsize{acu-8l}  &	100  &	10.8 \\
sri  &	40K  &	Siriano  &	5K  &	Americas  &	Latn  &	\scriptsize{cbv-6l}  &	99.2  &	- \\
kvn  &	40K  &	Border Kuna  &	50K  &	Americas  &	Latn  &	\scriptsize{guo-2l}  &	100  &	- \\
acn  &	40K  &	Longchuan Achang  &	50K  &	Asia  &	Latn  &	\scriptsize{acn-11l}  &	100  &	14.4 \\
mxb  &	40K  &	Tezoatlán Mixtec  &	50K  &	Americas  &	Latn  &	\scriptsize{kcg-9l}  &	98.9  &	- \\
ppo  &	40K  &	Folopa  &	5K  &	Oceania  &	Latn  &	\scriptsize{pab-2l}  &	98.2  &	- \\
atd  &	40K  &	Ata Manobo  &	50K  &	Asia  &	Latn  &	\scriptsize{atd-4l}  &	70.9  &	- \\
zam  &	40K  &	Cuixtla-Xitla Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{srq-3l}  &	100  &	- \\
mti  &	40K  &	Maiwa (Papua New Guinea)  &	5K  &	Oceania  &	Latn  &	\scriptsize{dgz-5l}  &	99.8  &	- \\
jic  &	40K  &	Tol  &	5K  &	Americas  &	Latn  &	\scriptsize{jic-3l}  &	100  &	- \\
cui  &	40K  &	Cuiba  &	5K  &	Americas  &	Latn  &	\scriptsize{acu-8l}  &	100  &	- \\
ata  &	40K  &	Pele-Ata  &	5K  &	Oceania  &	Latn  &	\scriptsize{ata-5l}  &	98.8  &	- \\
cnk  &	40K  &	Khumi Chin  &	50K  &	Asia  &	Latn  &	\scriptsize{cdo-5l}  &	100  &	16.9 \\
bnc  &	40K  &	Bontok  &	50K  &	Asia  &	Latn  &	\scriptsize{bnc-8l}  &	99.6  &	15.5 \\
con  &	40K  &	Cofán  &	5K  &	Americas  &	Latn  &	\scriptsize{con-3l}  &	100  &	- \\
guo  &	40K  &	Guayabero  &	5K  &	Americas  &	Latn  &	\scriptsize{guo-2l}  &	100  &	- \\
caa  &	40K  &	Chortí  &	50K  &	Americas  &	Latn  &	caa  &	100  &	12.5 \\
toh  &	30K  &	Gitonga  &	400K  &	Africa  &	Latn  &	\scriptsize{cce-8l}  &	99.9  &	29.9 \\
xon  &	30K  &	Konkomba  &	900K  &	Africa  &	Latn  &	\scriptsize{daa-3l}  &	98.6  &	17.3 \\
rug  &	30K  &	Roviana  &	5K  &	Oceania  &	Latn  &	\scriptsize{akb-4l}  &	99.9  &	- \\
bbb  &	30K  &	Barai  &	5K  &	Oceania  &	Latn  &	\scriptsize{asg-10l}  &	99.6  &	- \\
chf  &	30K  &	Tabasco Chontal  &	50K  &	Americas  &	Latn  &	\scriptsize{chd-6l}  &	100  &	20.3 \\
cub  &	30K  &	Cubeo  &	5K  &	Americas  &	Latn  &	\scriptsize{cub-2l}  &	100  &	- \\
tke  &	30K  &	Takwane  &	2M  &	Africa  &	Latn  &	tke  &	97.3  &	- \\
ape  &	30K  &	Bukiyip  &	50K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	69.9  &	- \\
tuo  &	30K  &	Tucano  &	5K  &	Americas  &	Latn  &	\scriptsize{meh-3l}  &	99.3  &	- \\
npl  &	30K  &	Nahuatl, Southeastern Puebla  &	300K  &	Americas  &	Latn  &	\scriptsize{nhy-3l}  &	94.5  &	- \\
mmx  &	30K  &	Madak  &	5K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	98.4  &	- \\
ifa  &	30K  &	Amganad Ifugao  &	50K  &	Asia  &	Latn  &	\scriptsize{bnc-8l}  &	99.7  &	- \\
boj  &	30K  &	Anjam  &	5K  &	Oceania  &	Latn  &	\scriptsize{boj-4l}  &	100  &	- \\
ter  &	30K  &	Terena-Kinikinao-Chane  &	50K  &	Americas  &	Latn  &	\scriptsize{enx-4l}  &	100  &	- \\
mpx  &	30K  &	Misima-Paneati  &	50K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	97.5  &	- \\
msk  &	30K  &	Mansaka  &	50K  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	100  &	34.2 \\
sdh  &	30K  &	Southern Kurdish  &	3M  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	70.2  &	- \\
ber-Arab  &	30K  &	Berber  &	2M  &	Africa  &	Arab  &	\scriptsize{abv-10l}  &	99.5  &	21.1 \\
zia  &	30K  &	Zia  &	5K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	96.2  &	- \\
mna  &	30K  &	Mbula  &	5K  &	Oceania  &	Latn  &	\scriptsize{bmu-6l}  &	99.0  &	- \\
apy  &	30K  &	Apalaí  &	5K  &	Americas  &	Latn  &	\scriptsize{apy-7l}  &	99.2  &	- \\
kdi  &	30K  &	Kumam  &	200K  &	Africa  &	Latn  &	\scriptsize{adh-5l}  &	99.9  &	15.8 \\
aon  &	30K  &	Bumbita Arapesh  &	5K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	76.9  &	- \\
mpg  &	30K  &	Marba  &	200K  &	Africa  &	Latn  &	\scriptsize{agt-6l}  &	100  &	13.1 \\
mlp  &	30K  &	Bargam  &	5K  &	Oceania  &	Latn  &	\scriptsize{hni-8l}  &	98.4  &	- \\
kyc  &	30K  &	Kyaka  &	50K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	99.2  &	- \\
huu  &	30K  &	Murui Huitoto  &	5K  &	Americas  &	Latn  &	\scriptsize{aak-3l}  &	100  &	- \\
sll  &	30K  &	Salt-Yui  &	5K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	97.6  &	- \\
quw  &	30K  &	Tena Lowland Quichua  &	1M  &	Americas  &	Latn  &	\scriptsize{quw-5l}  &	99.9  &	- \\
bkq  &	30K  &	Bakairí  &	5K  &	Americas  &	Latn  &	\scriptsize{abr-5l}  &	99.2  &	- \\
yaf  &	30K  &	Yaka-Pelende-Lonzo  &	900K  &	Africa  &	Latn  &	\scriptsize{jbu-8l}  &	99.6  &	27.3 \\
ncl  &	30K  &	Michoacán Nahuatl  &	5K  &	Americas  &	Latn  &	\scriptsize{azz-7l}  &	98.8  &	- \\
sgb  &	30K  &	Mag-Anchi Ayta  &	5K  &	Asia  &	Latn  &	\scriptsize{kqp-4l}  &	100  &	- \\
rop  &	30K  &	Kriol  &	5K  &	Oceania  &	Latn  &	\scriptsize{bg-Latn-5l}  &	99.7  &	- \\
rkb  &	30K  &	Rikbaktsa  &	5K  &	Americas  &	Latn  &	\scriptsize{apy-7l}  &	99.2  &	- \\
kqc  &	30K  &	Doromu-Koki  &	5K  &	Oceania  &	Latn  &	\scriptsize{adz-3l}  &	99.5  &	- \\
kew  &	30K  &	West Kewa  &	50K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	95.4  &	11.5 \\
snp  &	30K  &	Siane  &	50K  &	Oceania  &	Latn  &	\scriptsize{knj-8l}  &	100  &	- \\
cjp  &	30K  &	Cabécar  &	5K  &	Americas  &	Latn  &	\scriptsize{cjp-4l}  &	100  &	- \\
viv  &	30K  &	Iduna  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	99.5  &	- \\
sim  &	30K  &	Mende (Papua New Guinea)  &	5K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	98.2  &	- \\
xsm  &	30K  &	Kasem  &	200K  &	Africa  &	Latn  &	\scriptsize{lia-3l}  &	100  &	12.2 \\
iws  &	30K  &	Sepik Iwam  &	5K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	98.8  &	- \\
amm  &	30K  &	Ama (Papua New Guinea)  &	5K  &	Oceania  &	Latn  &	amm  &	99.4  &	- \\
opm  &	30K  &	Oksapmin  &	5K  &	Oceania  &	Latn  &	\scriptsize{agg-5l}  &	98.8  &	- \\
kgk  &	30K  &	Kaiwá  &	50K  &	Americas  &	Latn  &	\scriptsize{gn-6l}  &	98.8  &	- \\
mta  &	30K  &	Cotabato Manobo  &	50K  &	Asia  &	Latn  &	mta  &	100  &	17.0 \\
bef  &	30K  &	Benabena  &	50K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	99.7  &	12.2 \\
ura  &	30K  &	Urarina  &	5K  &	Americas  &	Latn  &	\scriptsize{bmr-3l}  &	100  &	- \\
tim  &	30K  &	Timbe  &	50K  &	Oceania  &	Latn  &	\scriptsize{bom-5l}  &	99.9  &	- \\
ife  &	30K  &	Ifè  &	100K  &	Africa  &	Latn  &	ife  &	99.9  &	18.7 \\
gqr  &	30K  &	Gor  &	50K  &	Africa  &	Latn  &	\scriptsize{dzg-5l}  &	93.0  &	- \\
haz  &	30K  &	Hazaragi  &	2M  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	13.9  &	57.8 \\
row  &	30K  &	Dela-Oenale  &	5K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	98.6  &	- \\
lcm  &	30K  &	Tungag  &	50K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	97.0  &	- \\
wos  &	30K  &	Hanga Hundi  &	5K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	99.5  &	- \\
agn  &	30K  &	Agutaynen  &	50K  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	99.9  &	- \\
lew  &	30K  &	Ledo Kaili  &	400K  &	Asia  &	Latn  &	\scriptsize{kzf-3l}  &	100  &	18.0 \\
mbc  &	30K  &	Macushi  &	50K  &	Americas  &	Latn  &	mbc  &	100  &	- \\
byx  &	30K  &	Qaqet  &	5K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	97.7  &	- \\
apz  &	30K  &	Safeyoka  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	99.2  &	- \\
qxn  &	30K  &	Northern Conchucos Ancash Quechua  &	200K  &	Americas  &	Latn  &	\scriptsize{qub-7l}  &	99.1  &	18.2 \\
rgu  &	30K  &	Ringgou  &	50K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	98.0  &	- \\
for  &	30K  &	Fore  &	50K  &	Oceania  &	Latn  &	\scriptsize{awb-4l}  &	99.7  &	- \\
sny  &	30K  &	Saniyo-Hiyewe  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	97.1  &	- \\
mop  &	30K  &	Mopán Maya  &	5K  &	Americas  &	Latn  &	\scriptsize{chd-6l}  &	100  &	- \\
men  &	30K  &	Mende (Sierra Leone)  &	3M  &	Africa  &	Latn  &	men  &	100  &	20.8 \\
arl  &	30K  &	Arabela  &	5K  &	Americas  &	Latn  &	arl  &	100  &	- \\
hvn  &	30K  &	Hawu  &	100K  &	Asia  &	Latn  &	\scriptsize{aom-10l}  &	100  &	15.8 \\
bba  &	30K  &	Baatonum  &	600K  &	Africa  &	Latn  &	\scriptsize{bas-11l}  &	100  &	17.0 \\
des  &	30K  &	Desano  &	5K  &	Americas  &	Latn  &	\scriptsize{des-4l}  &	99.9  &	- \\
tue  &	30K  &	Tuyuca  &	5K  &	Americas  &	Latn  &	\scriptsize{cbc-2l}  &	100  &	- \\
ino  &	30K  &	Inoke-Yate  &	50K  &	Oceania  &	Latn  &	\scriptsize{ata-5l}  &	100  &	- \\
tod  &	30K  &	Toma  &	200K  &	Africa  &	Latn  &	\scriptsize{moa-2l}  &	100  &	16.9 \\
ots  &	30K  &	Estado de México Otomi  &	50K  &	Americas  &	Latn  &	\scriptsize{kcg-9l}  &	99.9  &	- \\
bpr  &	30K  &	Koronadal Blaan  &	200K  &	Asia  &	Latn  &	\scriptsize{bpr-7l}  &	97.3  &	13.6 \\
aau  &	30K  &	Abau  &	5K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	98.2  &	- \\
khz  &	30K  &	Keapara  &	50K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	97.6  &	- \\
bum  &	30K  &	Bulu (Cameroon)  &	900K  &	Africa  &	Latn  &	\scriptsize{bas-11l}  &	98.6  &	29.9 \\
aer  &	30K  &	Eastern Arrernte  &	5K  &	Oceania  &	Latn  &	aer  &	100  &	- \\
azz  &	30K  &	Highland Puebla Nahuatl  &	200K  &	Americas  &	Latn  &	\scriptsize{azz-7l}  &	99.7  &	13.5 \\
dah  &	30K  &	Gwahatike  &	5K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	97.2  &	- \\
yml  &	30K  &	Iamalele  &	5K  &	Oceania  &	Latn  &	\scriptsize{fj-4l}  &	99.7  &	- \\
bzh  &	30K  &	Mapos Buang  &	50K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	97.5  &	- \\
kgp  &	30K  &	Kaingang  &	50K  &	Americas  &	Latn  &	\scriptsize{bzj-9l}  &	100  &	- \\
tpz  &	30K  &	Tinputz  &	5K  &	Oceania  &	Latn  &	\scriptsize{ach-10l}  &	99.3  &	- \\
bex  &	30K  &	Jur Modo  &	50K  &	Africa  &	Latn  &	\scriptsize{bbo-3l}  &	100  &	11.0 \\
mek  &	30K  &	Mekeo  &	50K  &	Oceania  &	Latn  &	\scriptsize{fj-4l}  &	99.1  &	- \\
sbl  &	30K  &	Botolan Sambal  &	50K  &	Asia  &	Latn  &	\scriptsize{kqp-4l}  &	100  &	23.0 \\
uvl  &	30K  &	Lote  &	5K  &	Oceania  &	Latn  &	\scriptsize{ata-5l}  &	98.4  &	- \\
abx  &	30K  &	Inabaknon  &	50K  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	96.4  &	- \\
ese  &	30K  &	Ese Ejja  &	5K  &	Americas  &	Latn  &	\scriptsize{ese-2l}  &	100  &	- \\
mcb  &	30K  &	Machiguenga  &	5K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	100  &	- \\
pma  &	30K  &	Paama  &	5K  &	Oceania  &	Latn  &	\scriptsize{ktm-4l}  &	99.4  &	- \\
qvm  &	30K  &	M-Y-L Quechua  &	50K  &	Americas  &	Latn  &	\scriptsize{qub-7l}  &	99.6  &	15.6 \\
mbj  &	30K  &	Nadëb  &	5K  &	Americas  &	Latn  &	\scriptsize{bgp-13l}  &	99.2  &	- \\
gso  &	30K  &	Southwest Gbaya  &	200K  &	Africa  &	Latn  &	\scriptsize{bas-11l}  &	100  &	16.8 \\
chd  &	30K  &	Highland Oaxaca Chontal  &	5K  &	Americas  &	Latn  &	\scriptsize{chd-6l}  &	99.6  &	- \\
ssx  &	30K  &	Samberigi  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	99.9  &	- \\
zaa  &	30K  &	Sierra de Juárez Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{zaa-5l}  &	100  &	- \\
bqp  &	30K  &	Busa  &	50K  &	Africa  &	Latn  &	\scriptsize{akp-4l}  &	99.7  &	- \\
kgf  &	30K  &	Kulungtfu-Yuanggeng-Tobo  &	5K  &	Oceania  &	Latn  &	\scriptsize{kgf-4l}  &	99.6  &	- \\
tvk  &	30K  &	Southeast Ambrym  &	5K  &	Oceania  &	Latn  &	\scriptsize{gaw-8l}  &	99.1  &	- \\
pah  &	30K  &	Tenharim-Parintintin-Diahoi  &	5K  &	Americas  &	Latn  &	\scriptsize{gn-6l}  &	99.7  &	- \\
mog  &	30K  &	Mongondow  &	200K  &	Asia  &	Latn  &	\scriptsize{awb-4l}  &	100  &	18.6 \\
zas  &	30K  &	Santo Domingo Albarradas Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{jic-3l}  &	100  &	- \\
zpl  &	30K  &	Lachixío Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{cbr-6l}  &	99.4  &	- \\
pib  &	30K  &	Yine  &	5K  &	Americas  &	Latn  &	pib  &	71.2  &	- \\
omw  &	30K  &	South Tairora  &	50K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	99.9  &	- \\
faa  &	30K  &	Fasu  &	5K  &	Oceania  &	Latn  &	\scriptsize{apr-8l}  &	99.6  &	- \\
dob  &	30K  &	Dobu  &	100K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	99.1  &	13.2 \\
dnw  &	30K  &	Western Dani  &	200K  &	Asia  &	Latn  &	\scriptsize{bmu-6l}  &	100  &	13.5 \\
gor  &	30K  &	Gorontalo  &	1M  &	Asia  &	Latn  &	\scriptsize{bco-8l}  &	100  &	18.4 \\
hak  &	30K  &	Hakka Chinese  &	30M  &	Asia  &	Latn  &	\scriptsize{cdo-5l}  &	91.6  &	28.0 \\
poe  &	30K  &	San Juan Atzingo Popoloca  &	5K  &	Americas  &	Latn  &	\scriptsize{mix-4l}  &	99.5  &	- \\
gwi  &	30K  &	Gwich'in  &	5K  &	Americas  &	Latn  &	\scriptsize{agr-3l}  &	99.9  &	- \\
npy  &	30K  &	Napu  &	5K  &	Asia  &	Latn  &	\scriptsize{gah-11l}  &	100  &	- \\
kpr  &	30K  &	Korafe-Yegha  &	5K  &	Oceania  &	Latn  &	\scriptsize{aom-10l}  &	97.6  &	- \\
vid  &	30K  &	Vidunda  &	50K  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	100  &	17.1 \\
yva  &	30K  &	Yawa  &	50K  &	Asia  &	Latn  &	\scriptsize{wnc-3l}  &	100  &	- \\
llg  &	30K  &	Lole  &	50K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	94.6  &	- \\
sps  &	30K  &	Saposa  &	5K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	97.3  &	- \\
wmw  &	30K  &	Mwani  &	100K  &	Africa  &	Latn  &	\scriptsize{bep-4l}  &	99.5  &	19.9 \\
mif  &	30K  &	Mofu-Gudur  &	50K  &	Africa  &	Latn  &	\scriptsize{meq-3l}  &	100  &	16.1 \\
fuf  &	30K  &	Pular  &	3M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	99.9  &	20.9 \\
kbq  &	30K  &	Kamano  &	50K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	98.8  &	11.8 \\
fuv  &	30K  &	Nigerian Fulfulde  &	12M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	98.1  &	- \\
ptu  &	30K  &	Bambam  &	50K  &	Asia  &	Latn  &	\scriptsize{atq-2l}  &	99.7  &	- \\
pri  &	30K  &	Paicî  &	5K  &	Oceania  &	Latn  &	\scriptsize{ae-Latn-10l}  &	97.2  &	- \\
en-Deva  &	30K  &	English  &	550M  &	Europe  &	Deva  &	\scriptsize{awa-14l}  &	97.1  &	75.9 \\
ymm  &	30K  &	Maay  &	3M  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	99.8  &	- \\
bmh  &	30K  &	Kein  &	5K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	98.1  &	- \\
zpo  &	30K  &	Amatlán Zapotec  &	50K  &	Americas  &	Latn  &	\scriptsize{zaa-5l}  &	88.4  &	- \\
smk  &	30K  &	Bolinao  &	50K  &	Asia  &	Latn  &	\scriptsize{br-4l}  &	99.0  &	28.6 \\
amp  &	30K  &	Alamblak  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	97.6  &	- \\
mic  &	30K  &	Mi'kmaq  &	5K  &	Americas  &	Latn  &	\scriptsize{hni-8l}  &	100  &	- \\
gkn  &	30K  &	Gokana  &	50K  &	Africa  &	Latn  &	\scriptsize{bcq-Latn-12l}  &	100  &	22.4 \\
cbs  &	30K  &	Cashinahua  &	5K  &	Americas  &	Latn  &	cbs  &	100  &	- \\
gvc  &	30K  &	Kotiria  &	5K  &	Americas  &	Latn  &	\scriptsize{des-4l}  &	100  &	- \\
xla  &	30K  &	Kamula  &	5K  &	Oceania  &	Latn  &	\scriptsize{ktm-4l}  &	99.6  &	- \\
sab  &	30K  &	Buglere  &	50K  &	Americas  &	Latn  &	sab  &	100  &	- \\
spp  &	30K  &	Supyire Senoufo  &	500K  &	Africa  &	Latn  &	spp  &	100  &	12.0 \\
gvn  &	30K  &	Kuku-Yalanji  &	5K  &	Oceania  &	Latn  &	\scriptsize{gvn-6l}  &	99.6  &	- \\
trc  &	30K  &	Copala Triqui  &	50K  &	Americas  &	Latn  &	\scriptsize{cut-5l}  &	88.0  &	- \\
thk  &	30K  &	Tharaka  &	200K  &	Africa  &	Latn  &	thk  &	100  &	20.9 \\
poy  &	30K  &	Pogolo  &	200K  &	Africa  &	Latn  &	\scriptsize{dov-9l}  &	100  &	15.7 \\
gej  &	30K  &	Gen  &	300K  &	Africa  &	Latn  &	\scriptsize{gej-4l}  &	100  &	24.1 \\
aak  &	30K  &	Ankave  &	5K  &	Oceania  &	Latn  &	\scriptsize{aak-3l}  &	100  &	- \\
rnl  &	30K  &	Halam  &	5K  &	Asia  &	Latn  &	\scriptsize{akb-4l}  &	100  &	- \\
kpf  &	30K  &	Komba  &	50K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	98.6  &	- \\
ghs  &	30K  &	Guhu-Samane  &	50K  &	Oceania  &	Latn  &	\scriptsize{agg-5l}  &	99.2  &	- \\
ajg  &	30K  &	Aja (Benin)  &	600K  &	Africa  &	Latn  &	\scriptsize{ajg-8l}  &	99.8  &	29.7 \\
bmu  &	30K  &	Burum-Mindik  &	5K  &	Oceania  &	Latn  &	\scriptsize{bmu-6l}  &	97.4  &	- \\
fuq  &	30K  &	Central-Eastern Niger Fulfulde  &	500K  &	Africa  &	Latn  &	\scriptsize{aa-13l}  &	100  &	16.3 \\
gvf  &	30K  &	Golin  &	50K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	98.2  &	12.6 \\
cbv  &	30K  &	Kakua  &	5K  &	Americas  &	Latn  &	\scriptsize{cbv-6l}  &	100  &	- \\
ake  &	30K  &	Akawaio  &	50K  &	Americas  &	Latn  &	ake  &	100  &	- \\
usp  &	30K  &	Uspanteco  &	5K  &	Americas  &	Latn  &	\scriptsize{acr-4l}  &	100  &	- \\
kpj  &	30K  &	Karajá  &	5K  &	Americas  &	Latn  &	\scriptsize{kpj-5l}  &	98.6  &	- \\
mtp  &	30K  &	Wichí Lhamtés Nocten  &	5K  &	Americas  &	Latn  &	\scriptsize{kqp-4l}  &	100  &	- \\
tku  &	30K  &	Upper Necaxa Totonac  &	5K  &	Americas  &	Latn  &	\scriptsize{tku-2l}  &	99.6  &	- \\
wnc  &	30K  &	Wantoat  &	5K  &	Oceania  &	Latn  &	\scriptsize{wnc-3l}  &	99.8  &	- \\
sgw  &	30K  &	Sebat Bet Gurage  &	1M  &	Africa  &	Ethi  &	\scriptsize{gez-8l}  &	99.2  &	35.6 \\
pwg  &	20K  &	Gapapaiwa  &	5K  &	Oceania  &	Latn  &	\scriptsize{asg-10l}  &	97.7  &	- \\
huv  &	20K  &	San Mateo del Mar Huave  &	50K  &	Americas  &	Latn  &	huv  &	100  &	- \\
tly-Cyrl-RU  &	20K  &	North-Central Talysh  &	900K  &	Europe  &	Cyrl  &	\scriptsize{az-RU-13l}  &	99.8  &	28.7 \\
kmu  &	20K  &	Kanite  &	5K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	99.9  &	- \\
bhb  &	20K  &	Bhili  &	3M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	100  &	44.2 \\
ljp  &	20K  &	Lampung Api  &	800K  &	Asia  &	Latn  &	\scriptsize{hui-3l}  &	100  &	25.3 \\
wrs  &	20K  &	Waris  &	5K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	98.7  &	- \\
ttc  &	20K  &	Tektiteko  &	5K  &	Americas  &	Latn  &	\scriptsize{azz-7l}  &	100  &	- \\
myb  &	20K  &	Mbay  &	50K  &	Africa  &	Latn  &	\scriptsize{kpj-5l}  &	99.1  &	14.2 \\
mhx  &	20K  &	Maru  &	50K  &	Asia  &	Latn  &	\scriptsize{lsi-2l}  &	100  &	15.9 \\
knv  &	20K  &	Tabo  &	5K  &	Oceania  &	Latn  &	\scriptsize{bco-8l}  &	99.9  &	- \\
mbl  &	20K  &	Maxakalí  &	5K  &	Americas  &	Latn  &	\scriptsize{arn-6l}  &	99.3  &	- \\
nhi  &	20K  &	Zacatlán-Ahuacatlán-Tepetzintla Nahuatl  &	50K  &	Americas  &	Latn  &	\scriptsize{bjr-4l}  &	98.7  &	- \\
tby  &	20K  &	Tabaru  &	50K  &	Asia  &	Latn  &	\scriptsize{gbi-8l}  &	100  &	- \\
soq  &	20K  &	Kanasi  &	5K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	98.8  &	- \\
agg  &	20K  &	Angor  &	5K  &	Oceania  &	Latn  &	\scriptsize{agg-5l}  &	99.0  &	- \\
kwd  &	20K  &	Kwaio  &	50K  &	Oceania  &	Latn  &	\scriptsize{knj-8l}  &	99.9  &	- \\
ssg  &	20K  &	Seimat  &	5K  &	Oceania  &	Latn  &	\scriptsize{gaw-8l}  &	96.3  &	- \\
zaj  &	20K  &	Zaramo  &	5K  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	99.2  &	- \\
ahr  &	20K  &	Ahirani  &	2M  &	Asia  &	Deva  &	\scriptsize{ahr-13l}  &	99.1  &	32.3 \\
pmf  &	20K  &	Pamona  &	100K  &	Asia  &	Latn  &	\scriptsize{pmf-2l}  &	100  &	14.2 \\
mco  &	20K  &	Coatlán Mixe  &	50K  &	Americas  &	Latn  &	\scriptsize{dyo-3l}  &	100  &	- \\
txq  &	20K  &	Tii  &	50K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	94.5  &	- \\
lif  &	20K  &	Limbu  &	800K  &	Asia  &	Deva  &	lif  &	99.9  &	- \\
ycn  &	20K  &	Yucuna  &	5K  &	Americas  &	Latn  &	\scriptsize{acu-8l}  &	100  &	- \\
kln  &	20K  &	Kalenjin  &	9M  &	Africa  &	Latn  &	\scriptsize{cro-3l}  &	99.9  &	12.5 \\
xsu  &	20K  &	Sanumá  &	5K  &	Americas  &	Latn  &	xsu  &	100  &	- \\
nus  &	20K  &	Nuer  &	900K  &	Africa  &	Latn  &	\scriptsize{din-3l}  &	100  &	22.8 \\
nak  &	20K  &	Nakanai  &	50K  &	Oceania  &	Latn  &	\scriptsize{bch-10l}  &	98.9  &	- \\
lid  &	20K  &	Nyindrou  &	5K  &	Oceania  &	Latn  &	\scriptsize{gaw-8l}  &	99.2  &	- \\
spl  &	20K  &	Selepet  &	5K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	99.5  &	- \\
aom  &	20K  &	Ömie  &	5K  &	Oceania  &	Latn  &	\scriptsize{aom-10l}  &	99.9  &	- \\
nhg  &	20K  &	Tetelcingo Nahuatl  &	5K  &	Americas  &	Latn  &	\scriptsize{nhg-3l}  &	100  &	- \\
cpu  &	20K  &	Pichis Ashéninka  &	50K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	96.9  &	13.3 \\
muh  &	20K  &	Mündü  &	50K  &	Africa  &	Latn  &	muh  &	100  &	- \\
nmz  &	20K  &	Nawdm  &	200K  &	Africa  &	Latn  &	\scriptsize{amf-6l}  &	99.9  &	14.7 \\
taj  &	20K  &	Eastern Tamang  &	300K  &	Asia  &	Deva  &	\scriptsize{taj-2l}  &	100  &	18.3 \\
nca  &	20K  &	Iyo  &	5K  &	Oceania  &	Latn  &	\scriptsize{kgf-4l}  &	99.3  &	- \\
ik  &	20K  &	Alaskan Inupiaq  &	5K  &	Americas  &	Latn  &	\scriptsize{bla-7l}  &	99.6  &	- \\
gam  &	20K  &	Kandawo  &	5K  &	Oceania  &	Latn  &	\scriptsize{gam-3l}  &	99.1  &	- \\
kue  &	20K  &	Kuman  &	100K  &	Oceania  &	Latn  &	\scriptsize{agt-6l}  &	99.1  &	13.1 \\
bbr  &	20K  &	Girawa  &	5K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	96.0  &	- \\
roo  &	20K  &	Rotokas  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	91.7  &	- \\
big  &	20K  &	Biangai  &	50K  &	Oceania  &	Latn  &	\scriptsize{big-5l}  &	100  &	- \\
dip  &	20K  &	Northeastern Dinka  &	5M  &	Africa  &	Latn  &	\scriptsize{din-3l}  &	100  &	14.9 \\
aeb-Latn  &	20K  &	Tunisian Arabic  &	11M  &	Africa  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	76.9  &	15.4 \\
lee  &	20K  &	Lyélé  &	100K  &	Africa  &	Latn  &	lee  &	99.6  &	12.4 \\
bgs  &	20K  &	Tagabawa  &	50K  &	Asia  &	Latn  &	\scriptsize{bgs-9l}  &	92.3  &	- \\
apb  &	20K  &	Sa'a  &	50K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	99.5  &	- \\
kmh  &	20K  &	Kalam  &	50K  &	Oceania  &	Latn  &	\scriptsize{dtb-4l}  &	99.5  &	- \\
soy  &	20K  &	Miyobe  &	50K  &	Africa  &	Latn  &	soy  &	100  &	- \\
gfk  &	20K  &	Patpatar  &	5K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	98.4  &	- \\
nvm  &	20K  &	Namiae  &	5K  &	Oceania  &	Latn  &	\scriptsize{dgz-5l}  &	99.1  &	- \\
bgr  &	20K  &	Bawm Chin  &	50K  &	Asia  &	Latn  &	\scriptsize{bgr-6l}  &	100  &	- \\
gnn  &	20K  &	Gumatj  &	5K  &	Oceania  &	Latn  &	\scriptsize{bch-10l}  &	100  &	- \\
qxo  &	20K  &	Southern Conchucos Ancash Quechua  &	900K  &	Americas  &	Latn  &	\scriptsize{qub-7l}  &	98.9  &	17.1 \\
cbr  &	20K  &	Cashibo-Cacataibo  &	5K  &	Americas  &	Latn  &	\scriptsize{cbr-6l}  &	100  &	- \\
bhl  &	20K  &	Bimin  &	5K  &	Oceania  &	Latn  &	\scriptsize{aey-6l}  &	99.6  &	- \\
amr  &	20K  &	Amarakaeri  &	5K  &	Americas  &	Latn  &	amr  &	100  &	- \\
kde  &	20K  &	Makonde  &	1M  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	98.3  &	24.4 \\
zad  &	20K  &	Cajonos Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{ctp-4l}  &	100  &	- \\
bps  &	20K  &	Sarangani Blaan  &	200K  &	Asia  &	Latn  &	\scriptsize{bpr-7l}  &	97.4  &	15.3 \\
mks  &	20K  &	Silacayoapan Mixtec  &	50K  &	Americas  &	Latn  &	mks  &	99.6  &	- \\
muy  &	20K  &	Muyang  &	50K  &	Africa  &	Latn  &	\scriptsize{dgc-6l}  &	100  &	12.8 \\
ncu  &	20K  &	Chumburung  &	50K  &	Africa  &	Latn  &	ncu  &	100  &	15.0 \\
stn  &	20K  &	Owa  &	5K  &	Oceania  &	Latn  &	\scriptsize{apr-8l}  &	100  &	- \\
sd-Deva  &	20K  &	Sindhi  &	68M  &	Asia  &	Deva  &	\scriptsize{bfz-15l}  &	98.3  &	34.4 \\
hub  &	20K  &	Huambisa  &	5K  &	Americas  &	Latn  &	\scriptsize{acu-8l}  &	98.8  &	- \\
cpb  &	20K  &	Ucayali-Yurúa Ashéninka  &	5K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	97.0  &	14.2 \\
mio  &	20K  &	Pinotepa Nacional Mixtec  &	50K  &	Americas  &	Latn  &	\scriptsize{cta-4l}  &	100  &	- \\
chz  &	20K  &	Ozumacín Chinantec  &	5K  &	Americas  &	Latn  &	\scriptsize{chz-9l}  &	100  &	- \\
aia  &	20K  &	Arosi  &	5K  &	Oceania  &	Latn  &	aia  &	100  &	- \\
ian  &	20K  &	Iatmul  &	5K  &	Oceania  &	Latn  &	\scriptsize{agg-5l}  &	99.9  &	- \\
way  &	20K  &	Wayana  &	5K  &	Americas  &	Latn  &	way  &	100  &	- \\
ndz  &	20K  &	Ndogo  &	50K  &	Africa  &	Latn  &	\scriptsize{bcq-Latn-12l}  &	100  &	- \\
agd  &	20K  &	Agarabi  &	50K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	98.5  &	- \\
mcp  &	20K  &	Makaa  &	50K  &	Africa  &	Latn  &	mcp  &	100  &	15.0 \\
wbp  &	20K  &	Warlpiri  &	5K  &	Oceania  &	Latn  &	\scriptsize{gvn-6l}  &	99.9  &	- \\
mox  &	20K  &	Molima  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	96.2  &	- \\
tbc  &	20K  &	Takia  &	50K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	97.7  &	12.4 \\
sxb  &	20K  &	Suba  &	100K  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.9  &	25.0 \\
kbm  &	20K  &	Iwal  &	5K  &	Oceania  &	Latn  &	\scriptsize{gam-3l}  &	99.8  &	- \\
bon  &	20K  &	Bine  &	5K  &	Oceania  &	Latn  &	bon  &	99.7  &	- \\
pls  &	20K  &	San Marcos Tlalcoyalco Popoloca  &	50K  &	Americas  &	Latn  &	\scriptsize{knj-8l}  &	100  &	- \\
vmy  &	20K  &	Ayautla Mazatec  &	5K  &	Americas  &	Latn  &	\scriptsize{nhr-2l}  &	98.6  &	- \\
nop  &	20K  &	Numanggang  &	5K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	98.7  &	- \\
qvn  &	20K  &	North Junín Quechua  &	50K  &	Americas  &	Latn  &	qvn  &	100  &	17.1 \\
cgc  &	20K  &	Kagayanen  &	50K  &	Asia  &	Latn  &	\scriptsize{cgc-2l}  &	100  &	22.4 \\
kwj  &	20K  &	Kwanga  &	50K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	97.3  &	- \\
kcg  &	20K  &	Tyap  &	100K  &	Africa  &	Latn  &	\scriptsize{kcg-9l}  &	100  &	13.9 \\
enx  &	20K  &	Southern Lengua  &	5K  &	Americas  &	Latn  &	\scriptsize{enx-4l}  &	99.0  &	- \\
mfy  &	20K  &	Mayo  &	50K  &	Americas  &	Latn  &	\scriptsize{ese-2l}  &	99.9  &	- \\
aby  &	20K  &	Aneme Wake  &	5K  &	Oceania  &	Latn  &	\scriptsize{aby-4l}  &	100  &	- \\
cco  &	20K  &	Comaltepec Chinantec  &	50K  &	Americas  &	Latn  &	cco  &	100  &	- \\
boa  &	20K  &	Bora  &	5K  &	Americas  &	Latn  &	boa  &	100  &	- \\
ikw  &	20K  &	Ikwere  &	200K  &	Africa  &	Latn  &	\scriptsize{anw-8l}  &	99.9  &	20.1 \\
lmn-Knda  &	20K  &	Lambadi  &	6M  &	Asia  &	Knda  &	\scriptsize{lmn-Knda-2l}  &	100  &	33.3 \\
rai  &	20K  &	Ramoaaina  &	50K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	95.9  &	- \\
leu  &	20K  &	Kara (Papua New Guinea)  &	5K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	99.1  &	- \\
sue  &	20K  &	Suena  &	5K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	99.6  &	- \\
auc  &	20K  &	Waorani  &	5K  &	Americas  &	Latn  &	\scriptsize{auc-6l}  &	100  &	- \\
kdc  &	20K  &	Kutu  &	50K  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	97.7  &	19.1 \\
awb  &	20K  &	Awa (Papua New Guinea)  &	5K  &	Oceania  &	Latn  &	\scriptsize{awb-4l}  &	99.9  &	- \\
kpw  &	20K  &	Kobon  &	50K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	99.6  &	- \\
mux  &	20K  &	Bo-Ung  &	50K  &	Oceania  &	Latn  &	\scriptsize{gbi-8l}  &	99.5  &	11.2 \\
mqb  &	20K  &	Mbuko  &	50K  &	Africa  &	Latn  &	\scriptsize{blw-2l}  &	100  &	- \\
kne  &	20K  &	Kankanaey  &	200K  &	Asia  &	Latn  &	\scriptsize{bnc-8l}  &	100  &	25.7 \\
blz  &	20K  &	Balantak  &	50K  &	Asia  &	Latn  &	\scriptsize{bjp-4l}  &	100  &	14.2 \\
vmw  &	20K  &	Makhuwa  &	3M  &	Africa  &	Latn  &	\scriptsize{apu-13l}  &	99.9  &	16.2 \\
tcs  &	20K  &	Torres Strait Creole  &	5K  &	Oceania  &	Latn  &	\scriptsize{bg-Latn-5l}  &	99.4  &	- \\
mie  &	20K  &	Ocotepec Mixtec  &	50K  &	Americas  &	Latn  &	mie  &	99.9  &	- \\
mhy  &	20K  &	Ma'anyan  &	200K  &	Asia  &	Latn  &	\scriptsize{amo-7l}  &	99.5  &	34.7 \\
btd  &	20K  &	Batak Dairi  &	1M  &	Asia  &	Latn  &	\scriptsize{aom-10l}  &	100  &	21.5 \\
lem  &	20K  &	Nomaande  &	5K  &	Africa  &	Latn  &	\scriptsize{box-3l}  &	100  &	- \\
hop  &	20K  &	Hopi  &	5K  &	Americas  &	Latn  &	hop  &	99.9  &	- \\
ken  &	20K  &	Kenyang  &	50K  &	Africa  &	Latn  &	\scriptsize{ken-3l}  &	97.3  &	- \\
ssd  &	20K  &	Siroi  &	5K  &	Oceania  &	Latn  &	\scriptsize{bch-10l}  &	99.1  &	- \\
kms  &	20K  &	Kamasau  &	5K  &	Oceania  &	Latn  &	\scriptsize{cwt-4l}  &	97.4  &	- \\
yuw  &	20K  &	Yau (Morobe Province)  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	97.6  &	- \\
agt  &	20K  &	Central Cagayan Agta  &	5K  &	Asia  &	Latn  &	\scriptsize{agt-6l}  &	97.6  &	- \\
maj  &	20K  &	Jalapa De Díaz Mazatec  &	50K  &	Americas  &	Latn  &	\scriptsize{kcg-9l}  &	100  &	- \\
tpm  &	20K  &	Tampulma  &	50K  &	Africa  &	Latn  &	\scriptsize{sil-3l}  &	100  &	- \\
khs  &	20K  &	Kasua  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	99.9  &	- \\
kzf  &	20K  &	Da'a Kaili  &	400K  &	Asia  &	Latn  &	\scriptsize{kzf-3l}  &	100  &	16.6 \\
ign  &	20K  &	Ignaciano  &	50K  &	Americas  &	Latn  &	\scriptsize{acu-8l}  &	100  &	11.3 \\
mwv  &	20K  &	Mentawai  &	50K  &	Asia  &	Latn  &	\scriptsize{bjp-4l}  &	100  &	14.7 \\
cul  &	20K  &	Culina  &	5K  &	Americas  &	Latn  &	cul  &	100  &	- \\
apu  &	20K  &	Apurinã  &	5K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	99.9  &	- \\
ncj  &	20K  &	Northern Puebla Nahuatl  &	50K  &	Americas  &	Latn  &	\scriptsize{bjr-4l}  &	100  &	18.6 \\
xnn  &	20K  &	Northern Kankanay  &	50K  &	Asia  &	Latn  &	\scriptsize{bnc-8l}  &	99.2  &	24.4 \\
bvd  &	20K  &	Baeggu  &	5K  &	Oceania  &	Latn  &	\scriptsize{bvc-4l}  &	99.1  &	- \\
nko  &	20K  &	Nkonya  &	50K  &	Africa  &	Latn  &	\scriptsize{ktj-6l}  &	100  &	- \\
cwe  &	20K  &	Kwere  &	50K  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	97.6  &	21.7 \\
tap  &	20K  &	Taabwa  &	300K  &	Africa  &	Latn  &	tap  &	100  &	23.5 \\
wrk  &	20K  &	Garrwa  &	5K  &	Oceania  &	Latn  &	wrk  &	100  &	- \\
gah  &	20K  &	Alekano  &	50K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	97.6  &	- \\
yam  &	20K  &	Yamba  &	50K  &	Africa  &	Latn  &	\scriptsize{pny-2l}  &	100  &	7.0 \\
geb  &	20K  &	Kire  &	5K  &	Oceania  &	Latn  &	\scriptsize{bmu-6l}  &	100  &	- \\
ctp  &	20K  &	Western Highland Chatino  &	50K  &	Americas  &	Latn  &	\scriptsize{ctp-4l}  &	83.9  &	- \\
mbs  &	20K  &	Sarangani Manobo  &	50K  &	Asia  &	Latn  &	\scriptsize{mbb-3l}  &	99.6  &	16.0 \\
nlg  &	20K  &	Gela  &	50K  &	Oceania  &	Latn  &	\scriptsize{bgt-4l}  &	99.0  &	- \\
nsn  &	20K  &	Nehan  &	5K  &	Oceania  &	Latn  &	\scriptsize{bgt-4l}  &	99.4  &	- \\
bao  &	20K  &	Waimaha  &	5K  &	Americas  &	Latn  &	bao  &	99.7  &	- \\
cle  &	20K  &	Lealao Chinantec  &	5K  &	Americas  &	Latn  &	\scriptsize{chz-9l}  &	100  &	- \\
mvn  &	20K  &	Minaveha  &	5K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	98.2  &	- \\
tpt  &	20K  &	Tlachichilco Tepehua  &	5K  &	Americas  &	Latn  &	\scriptsize{gam-3l}  &	100  &	- \\
zyp  &	20K  &	Zyphe  &	50K  &	Asia  &	Latn  &	\scriptsize{arn-6l}  &	99.9  &	- \\
pio  &	20K  &	Piapoco  &	5K  &	Americas  &	Latn  &	pio  &	100  &	- \\
bgx-Latn  &	20K  &	Rumelian Turkish  &	300K  &	Europe  &	Latn  &	\scriptsize{aeb-Latn-11l}  &	95.6  &	59.5 \\
myx  &	20K  &	Masaaba  &	3M  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.8  &	25.0 \\
tsz  &	20K  &	Purepecha  &	50K  &	Americas  &	Latn  &	\scriptsize{apu-13l}  &	100  &	15.2 \\
dww  &	20K  &	Dawawa  &	5K  &	Oceania  &	Latn  &	\scriptsize{abt-3l}  &	98.3  &	- \\
gnw  &	20K  &	Western Bolivian Guaraní  &	5K  &	Americas  &	Latn  &	gnw  &	100  &	- \\
ksr  &	20K  &	Borong  &	5K  &	Oceania  &	Latn  &	\scriptsize{kpj-5l}  &	98.5  &	- \\
otn  &	20K  &	Tenango Otomi  &	50K  &	Americas  &	Latn  &	\scriptsize{kcg-9l}  &	100  &	15.1 \\
gdn  &	20K  &	Umanakaina  &	5K  &	Oceania  &	Latn  &	\scriptsize{asg-10l}  &	99.5  &	- \\
kmo  &	20K  &	Kwoma  &	5K  &	Oceania  &	Latn  &	\scriptsize{abt-3l}  &	100  &	- \\
nii  &	20K  &	Nii  &	50K  &	Oceania  &	Latn  &	nii  &	100  &	- \\
tsw  &	20K  &	Salka-Tsishingini  &	200K  &	Africa  &	Latn  &	\scriptsize{asg-10l}  &	98.1  &	15.9 \\
not  &	20K  &	Nomatsiguenga  &	5K  &	Americas  &	Latn  &	\scriptsize{cot-2l}  &	100  &	- \\
ury  &	20K  &	Orya  &	5K  &	Asia  &	Latn  &	\scriptsize{bzj-9l}  &	100  &	- \\
anv  &	20K  &	Denya  &	50K  &	Africa  &	Latn  &	anv  &	100  &	- \\
pbc  &	20K  &	Patamona  &	50K  &	Americas  &	Latn  &	pbc  &	100  &	- \\
blt-Latn  &	20K  &	Tai Dam  &	800K  &	Asia  &	Latn  &	\scriptsize{blt-Latn-4l}  &	99.7  &	24.4 \\
aii  &	20K  &	Assyrian Neo-Aramaic  &	800K  &	Europe  &	Syrc  &	\scriptsize{ach-10l}  &	100  &	35.7 \\
mhl  &	20K  &	Mauwake  &	5K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	65.5  &	- \\
myk  &	20K  &	Mamara Senoufo  &	700K  &	Africa  &	Latn  &	myk  &	100  &	13.2 \\
mee  &	20K  &	Mengen  &	5K  &	Oceania  &	Latn  &	\scriptsize{ata-5l}  &	99.8  &	- \\
kpx  &	20K  &	Mountain Koiali  &	5K  &	Oceania  &	Latn  &	\scriptsize{apr-8l}  &	99.1  &	- \\
udu  &	20K  &	Uduk  &	50K  &	Africa  &	Latn  &	\scriptsize{knj-8l}  &	100  &	- \\
mnp  &	20K  &	Min Bei Chinese  &	10M  &	Asia  &	Latn  &	\scriptsize{cdo-5l}  &	99.8  &	16.2 \\
alp  &	20K  &	Alune  &	50K  &	Asia  &	Latn  &	\scriptsize{alp-2l}  &	100  &	- \\
wiu  &	20K  &	Wiru  &	50K  &	Oceania  &	Latn  &	\scriptsize{gbi-8l}  &	99.0  &	- \\
gyr  &	20K  &	Guarayu  &	5K  &	Americas  &	Latn  &	\scriptsize{gn-6l}  &	100  &	- \\
meq  &	20K  &	Merey  &	50K  &	Africa  &	Latn  &	\scriptsize{meq-3l}  &	100  &	- \\
kjs  &	20K  &	East Kewa  &	50K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	95.3  &	11.4 \\
mcq  &	20K  &	Ese  &	50K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	96.7  &	- \\
ong  &	20K  &	Olo  &	50K  &	Oceania  &	Latn  &	\scriptsize{kpz-2l}  &	99.9  &	- \\
tnn  &	20K  &	North Tanna  &	5K  &	Oceania  &	Latn  &	\scriptsize{nwi-5l}  &	99.9  &	- \\
coe  &	20K  &	Koreguaje  &	5K  &	Americas  &	Latn  &	coe  &	99.9  &	- \\
hrx  &	20K  &	Hunsrik  &	3M  &	Americas  &	Latn  &	\scriptsize{hrx-2l}  &	99.6  &	48.8 \\
tte  &	20K  &	Bwanabwana  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	98.3  &	- \\
yut  &	20K  &	Yopno  &	5K  &	Oceania  &	Latn  &	\scriptsize{dtb-4l}  &	99.2  &	- \\
sgz  &	20K  &	Sursurunga  &	5K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	97.7  &	- \\
ceg  &	20K  &	Chamacoco  &	5K  &	Americas  &	Latn  &	\scriptsize{ceg-5l}  &	100  &	- \\
qul  &	20K  &	North Bolivian Quechua  &	100K  &	Americas  &	Latn  &	\scriptsize{ae-Latn-10l}  &	99.6  &	20.9 \\
mvp  &	20K  &	Duri  &	100K  &	Asia  &	Latn  &	\scriptsize{kje-6l}  &	99.7  &	14.4 \\
xed  &	20K  &	Hdi  &	50K  &	Africa  &	Latn  &	\scriptsize{cko-5l}  &	100  &	- \\
bqj  &	20K  &	Bandial  &	50K  &	Africa  &	Latn  &	\scriptsize{bkv-4l}  &	99.6  &	- \\
duo  &	20K  &	Dupaninan Agta  &	5K  &	Asia  &	Latn  &	\scriptsize{dgc-6l}  &	99.5  &	- \\
mza  &	20K  &	Santa María Zacatepec Mixtec  &	5K  &	Americas  &	Latn  &	\scriptsize{mpm-4l}  &	99.6  &	- \\
mva  &	20K  &	Manam  &	5K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	97.7  &	- \\
akh  &	20K  &	Angal Heneng  &	50K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	97.8  &	12.0 \\
blw  &	20K  &	Balangao  &	50K  &	Asia  &	Latn  &	\scriptsize{blw-2l}  &	92.5  &	- \\
luy  &	20K  &	Luhya  &	1M  &	Africa  &	Latn  &	\scriptsize{cgg-15l}  &	99.7  &	20.6 \\
mnb  &	20K  &	Muna  &	300K  &	Asia  &	Latn  &	\scriptsize{ata-5l}  &	100  &	13.5 \\
nou  &	20K  &	Ewage-Notu  &	50K  &	Oceania  &	Latn  &	\scriptsize{aom-10l}  &	99.9  &	- \\
ebk  &	20K  &	Eastern Bontok  &	50K  &	Asia  &	Latn  &	\scriptsize{bnc-8l}  &	97.7  &	- \\
tpp  &	20K  &	Pisaflores Tepehua  &	5K  &	Americas  &	Latn  &	\scriptsize{tee-2l}  &	100  &	- \\
wim  &	20K  &	Wik-Mungkan  &	5K  &	Oceania  &	Latn  &	\scriptsize{beu-2l}  &	99.9  &	- \\
avt  &	20K  &	Au  &	5K  &	Oceania  &	Latn  &	\scriptsize{avt-12l}  &	98.3  &	- \\
blh  &	20K  &	Kuwaa  &	50K  &	Africa  &	Latn  &	\scriptsize{bcq-Latn-12l}  &	100  &	- \\
mfi  &	20K  &	Wandala  &	50K  &	Africa  &	Latn  &	\scriptsize{acu-8l}  &	100  &	13.5 \\
eri  &	20K  &	Ogea  &	5K  &	Oceania  &	Latn  &	\scriptsize{agt-6l}  &	98.3  &	- \\
mpt  &	20K  &	Mian  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	98.1  &	- \\
swp  &	20K  &	Suau  &	5K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	99.4  &	- \\
nho  &	20K  &	Takuu  &	5K  &	Oceania  &	Latn  &	\scriptsize{bgt-4l}  &	96.0  &	- \\
aso  &	20K  &	Dano  &	50K  &	Oceania  &	Latn  &	aso  &	100  &	11.6 \\
wnu  &	20K  &	Usan  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	96.7  &	- \\
zav  &	20K  &	Yatzachi Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{cut-5l}  &	100  &	- \\
bcw  &	20K  &	Bana  &	50K  &	Africa  &	Latn  &	\scriptsize{bcw-3l}  &	100  &	- \\
dgz  &	20K  &	Daga  &	5K  &	Oceania  &	Latn  &	\scriptsize{dgz-5l}  &	99.8  &	- \\
ipi  &	20K  &	Ipili  &	50K  &	Oceania  &	Latn  &	\scriptsize{gbi-8l}  &	99.5  &	- \\
nsu  &	20K  &	Sierra Negra Nahuatl  &	50K  &	Americas  &	Latn  &	\scriptsize{nhy-3l}  &	99.5  &	- \\
urt  &	20K  &	Urat  &	5K  &	Oceania  &	Latn  &	\scriptsize{aey-6l}  &	99.1  &	- \\
obo  &	20K  &	Obo Manobo  &	50K  &	Asia  &	Latn  &	\scriptsize{atd-4l}  &	100  &	16.1 \\
zpi  &	20K  &	Santa María Quiegolani Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{zaa-5l}  &	100  &	- \\
sat-Deva  &	20K  &	Santali  &	6M  &	Asia  &	Deva  &	\scriptsize{bho-13l}  &	98.1  &	- \\
cjv  &	20K  &	Chuave  &	50K  &	Oceania  &	Latn  &	\scriptsize{bom-5l}  &	97.5  &	- \\
ifu  &	20K  &	Mayoyao Ifugao  &	50K  &	Asia  &	Latn  &	\scriptsize{bnc-8l}  &	100  &	- \\
atg  &	20K  &	Ivbie North-Okpela-Arhe  &	50K  &	Africa  &	Latn  &	\scriptsize{ajg-8l}  &	100  &	- \\
icr  &	20K  &	San Andres Creole English  &	50K  &	Americas  &	Latn  &	\scriptsize{bzj-9l}  &	100  &	- \\
neb  &	20K  &	Toura (Côte d'Ivoire)  &	50K  &	Africa  &	Latn  &	\scriptsize{avn-3l}  &	100  &	8.9 \\
apr  &	20K  &	Arop-Lokep  &	5K  &	Oceania  &	Latn  &	\scriptsize{apr-8l}  &	99.2  &	- \\
aoz  &	20K  &	Uab Meto  &	800K  &	Asia  &	Latn  &	\scriptsize{aaz-6l}  &	100  &	15.5 \\
mca  &	20K  &	Maca  &	5K  &	Americas  &	Latn  &	\scriptsize{hrx-2l}  &	100  &	- \\
tiy  &	20K  &	Tiruray  &	50K  &	Asia  &	Latn  &	\scriptsize{cjp-4l}  &	100  &	13.2 \\
gdr  &	20K  &	Wipi  &	5K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	98.4  &	- \\
kqw  &	20K  &	Kandas  &	5K  &	Oceania  &	Latn  &	\scriptsize{apb-13l}  &	93.8  &	- \\
zaw  &	20K  &	Mitla Zapotec  &	50K  &	Americas  &	Latn  &	\scriptsize{toj-4l}  &	100  &	- \\
atq  &	20K  &	Aralle-Tabulahan  &	50K  &	Asia  &	Latn  &	\scriptsize{atq-2l}  &	99.9  &	- \\
ruf  &	20K  &	Luguru  &	700K  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	100  &	17.3 \\
kje  &	20K  &	Kisar  &	50K  &	Asia  &	Latn  &	\scriptsize{kje-6l}  &	100  &	- \\
fai  &	20K  &	Faiwol  &	5K  &	Oceania  &	Latn  &	\scriptsize{bnj-6l}  &	99.8  &	- \\
zpq  &	20K  &	Zoogocho Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{cut-5l}  &	100  &	- \\
mcn  &	20K  &	Masana  &	200K  &	Africa  &	Latn  &	\scriptsize{dzg-5l}  &	50.7  &	47.6 \\
nlc  &	20K  &	Nalca  &	50K  &	Asia  &	Latn  &	\scriptsize{mps-3l}  &	100  &	- \\
yby  &	20K  &	Yaweyuha  &	5K  &	Oceania  &	Latn  &	\scriptsize{aau-14l}  &	97.6  &	- \\
pao  &	20K  &	Northern Paiute  &	5K  &	Americas  &	Latn  &	\scriptsize{chq-3l}  &	99.9  &	- \\
mcu  &	20K  &	Donga Mambila  &	50K  &	Africa  &	Latn  &	\scriptsize{mcu-2l}  &	100  &	7.6 \\
kbc  &	20K  &	Kadiwéu  &	5K  &	Americas  &	Latn  &	\scriptsize{etr-2l}  &	100  &	- \\
djr  &	20K  &	Djambarrpuyngu  &	5K  &	Oceania  &	Latn  &	\scriptsize{bch-10l}  &	100  &	- \\
zae  &	20K  &	Yareni Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{rmc-3l}  &	100  &	- \\
wer  &	20K  &	Weri  &	50K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	99.2  &	- \\
maw  &	20K  &	Mampruli  &	200K  &	Africa  &	Latn  &	\scriptsize{cko-5l}  &	100  &	14.1 \\
kud  &	20K  &	Auhelawa  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	98.0  &	- \\
dad  &	20K  &	Marik  &	5K  &	Oceania  &	Latn  &	\scriptsize{amp-12l}  &	94.4  &	- \\
cax  &	20K  &	Lomeriano-Ignaciano Chiquitano  &	5K  &	Americas  &	Latn  &	\scriptsize{acu-8l}  &	100  &	- \\
ons  &	20K  &	Ono  &	50K  &	Oceania  &	Latn  &	\scriptsize{kgf-4l}  &	100  &	- \\
wuv  &	20K  &	Wuvulu-Aua  &	5K  &	Oceania  &	Latn  &	\scriptsize{aom-10l}  &	98.6  &	- \\
gay  &	20K  &	Gayo  &	300K  &	Asia  &	Latn  &	\scriptsize{abs-13l}  &	97.2  &	31.9 \\
gng  &	20K  &	Ngangam  &	50K  &	Africa  &	Latn  &	\scriptsize{ada-13l}  &	100  &	15.4 \\
nim  &	20K  &	Nilamba  &	700K  &	Africa  &	Latn  &	\scriptsize{ess-4l}  &	100  &	16.5 \\
snc  &	20K  &	Sinaugoro  &	50K  &	Oceania  &	Latn  &	\scriptsize{gah-11l}  &	97.6  &	- \\
nhu  &	20K  &	Noone  &	50K  &	Africa  &	Latn  &	\scriptsize{cme-5l}  &	100  &	10.9 \\
daa  &	20K  &	Dangaleat  &	50K  &	Africa  &	Latn  &	\scriptsize{daa-3l}  &	100  &	12.3 \\
yli  &	20K  &	Angguruk Yali  &	50K  &	Asia  &	Latn  &	yli  &	100  &	- \\
bgq-Arab  &	20K  &	Bagri  &	2M  &	Asia  &	Arab  &	\scriptsize{bgq-Arab-4l}  &	99.7  &	- \\
tnk  &	20K  &	Kwamera  &	5K  &	Oceania  &	Latn  &	\scriptsize{nwi-5l}  &	99.4  &	- \\
knf  &	20K  &	Mankanya  &	50K  &	Africa  &	Latn  &	\scriptsize{knf-2l}  &	100  &	13.5 \\
mbh  &	20K  &	Mangseng  &	5K  &	Oceania  &	Latn  &	\scriptsize{acn-11l}  &	98.3  &	- \\
cme  &	20K  &	Cerma  &	50K  &	Africa  &	Latn  &	\scriptsize{cme-5l}  &	100  &	10.3 \\
dgr  &	20K  &	Dogrib  &	5K  &	Americas  &	Latn  &	\scriptsize{bcq-Latn-12l}  &	99.8  &	- \\
kup  &	20K  &	Kunimaipa  &	50K  &	Oceania  &	Latn  &	\scriptsize{bjr-4l}  &	99.5  &	- \\
lww  &	20K  &	Lewo  &	5K  &	Oceania  &	Latn  &	\scriptsize{big-5l}  &	99.5  &	- \\
ktb  &	20K  &	Kambaata  &	900K  &	Africa  &	Ethi  &	\scriptsize{gez-8l}  &	99.9  &	13.5 \\
dop  &	20K  &	Lukpa  &	50K  &	Africa  &	Latn  &	dop  &	100  &	- \\
kki  &	20K  &	Kagulu  &	200K  &	Africa  &	Latn  &	\scriptsize{dov-9l}  &	100  &	17.3 \\
mpp  &	20K  &	Migabac  &	5K  &	Oceania  &	Latn  &	\scriptsize{bru-6l}  &	99.3  &	- \\
sua  &	20K  &	Sulka  &	5K  &	Oceania  &	Latn  &	\scriptsize{bwu-4l}  &	98.7  &	- \\
yon  &	20K  &	Yonggom  &	5K  &	Oceania  &	Latn  &	\scriptsize{wnc-3l}  &	100  &	- \\
eka  &	15K  &	Ekajuk  &	50K  &	Africa  &	Latn  &	\scriptsize{apn-3l}  &	100  &	12.6 \\
mih  &	15K  &	Chayuco Mixtec  &	50K  &	Americas  &	Latn  &	\scriptsize{gaw-8l}  &	99.5  &	- \\
cux  &	15K  &	Tepeuxila Cuicatec  &	50K  &	Americas  &	Latn  &	cux  &	100  &	- \\
tlb  &	15K  &	Tobelo  &	50K  &	Asia  &	Latn  &	\scriptsize{gbi-8l}  &	100  &	- \\
klv  &	15K  &	Maskelynes  &	5K  &	Oceania  &	Latn  &	\scriptsize{bkv-4l}  &	99.9  &	- \\
due  &	15K  &	Umiray Dumaget Agta  &	5K  &	Asia  &	Latn  &	\scriptsize{dgc-6l}  &	100  &	- \\
lmn-Deva  &	15K  &	Lambadi  &	6M  &	Asia  &	Deva  &	\scriptsize{awa-14l}  &	98.4  &	24.8 \\
xuo  &	15K  &	Kuo  &	50K  &	Africa  &	Latn  &	xuo  &	100  &	- \\
shk  &	15K  &	Shilluk  &	200K  &	Africa  &	Latn  &	shk  &	100  &	- \\
xsb  &	15K  &	Tinà Sambal  &	50K  &	Asia  &	Latn  &	\scriptsize{dgc-6l}  &	100  &	21.8 \\
amk  &	15K  &	Ambai  &	50K  &	Asia  &	Latn  &	\scriptsize{aby-4l}  &	100  &	- \\
zab  &	14K  &	San Juan Guelavía Zapotec  &	50K  &	Americas  &	Latn  &	\scriptsize{toj-4l}  &	99.7  &	- \\
mig  &	14K  &	San Miguel El Grande Mixtec  &	50K  &	Americas  &	Latn  &	mig  &	60.8  &	- \\
hla  &	14K  &	Halia  &	50K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	97.6  &	- \\
dgc  &	14K  &	Casiguran-Nagtipunan Agta  &	5K  &	Asia  &	Latn  &	\scriptsize{dgc-6l}  &	99.1  &	- \\
iry  &	14K  &	Iraya  &	50K  &	Asia  &	Latn  &	\scriptsize{agn-14l}  &	96.8  &	- \\
vun  &	14K  &	Vunjo  &	900K  &	Africa  &	Latn  &	\scriptsize{nnq-4l}  &	99.9  &	15.9 \\
hot  &	14K  &	Hote  &	5K  &	Oceania  &	Latn  &	\scriptsize{aey-6l}  &	93.1  &	- \\
otd  &	14K  &	Ot Danum  &	50K  &	Asia  &	Latn  &	\scriptsize{bhw-9l}  &	100  &	- \\
ade  &	14K  &	Adele  &	50K  &	Africa  &	Latn  &	\scriptsize{ade-4l}  &	100  &	- \\
nin  &	14K  &	Ninzo  &	50K  &	Africa  &	Latn  &	\scriptsize{ajg-8l}  &	100  &	13.4 \\
gaw  &	14K  &	Nobonob  &	5K  &	Oceania  &	Latn  &	\scriptsize{gaw-8l}  &	100  &	- \\
nwi  &	14K  &	Southwest Tanna  &	5K  &	Oceania  &	Latn  &	\scriptsize{nwi-5l}  &	100  &	- \\
naf  &	14K  &	Nabak  &	50K  &	Oceania  &	Latn  &	\scriptsize{miq-2l}  &	98.1  &	- \\
ztq  &	14K  &	Quioquitani-Quieri Zapotec  &	5K  &	Americas  &	Latn  &	\scriptsize{gv-3l}  &	99.7  &	- \\
bkd  &	14K  &	Talaandig-Binukid  &	50K  &	Asia  &	Latn  &	\scriptsize{abx-11l}  &	93.9  &	- \\
mit  &	14K  &	Southern Puebla Mixtec  &	5K  &	Americas  &	Latn  &	mit  &	100  &	- \\
kbr  &	14K  &	Kafa  &	800K  &	Africa  &	Latn  &	\scriptsize{drs-Latn-8l}  &	100  &	12.8 \\
cnt  &	14K  &	Tepetotutla Chinantec  &	5K  &	Americas  &	Latn  &	\scriptsize{chz-9l}  &	100  &	- \\
bdd  &	14K  &	Bunama  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	97.3  &	- \\
bm-Nkoo  &	14K  &	Bambara  &	14M  &	Africa  &	Nkoo  &	\scriptsize{bm-Nkoo-2l}  &	78.3  &	12.1 \\
myw  &	14K  &	Muyuw  &	5K  &	Oceania  &	Latn  &	\scriptsize{aon-13l}  &	97.9  &	- \\
box  &	14K  &	Buamu  &	200K  &	Africa  &	Latn  &	\scriptsize{box-3l}  &	100  &	13.1 \\
prf  &	13K  &	Paranan  &	50K  &	Asia  &	Latn  &	\scriptsize{dgc-6l}  &	99.6  &	- \\
ziw  &	13K  &	Zigula-Mushungulu  &	400K  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	98.3  &	17.6 \\
maq  &	13K  &	Chiquihuitlán Mazatec  &	5K  &	Americas  &	Latn  &	\scriptsize{chz-9l}  &	99.9  &	- \\
yrb  &	13K  &	Yareba  &	5K  &	Oceania  &	Latn  &	\scriptsize{aby-4l}  &	100  &	- \\
lwo  &	13K  &	Luwo  &	50K  &	Africa  &	Latn  &	\scriptsize{chq-3l}  &	100  &	13.2 \\
ozm  &	13K  &	Koonzime  &	50K  &	Africa  &	Latn  &	\scriptsize{mcu-2l}  &	100  &	9.5 \\
csk  &	13K  &	Jola-Esulalu  &	50K  &	Africa  &	Latn  &	\scriptsize{csk-3l}  &	100  &	13.0 \\
kdl  &	13K  &	Tsikimba  &	50K  &	Africa  &	Latn  &	\scriptsize{asg-10l}  &	99.0  &	16.3 \\
hno  &	13K  &	Northern Hindko  &	4M  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	40.5  &	32.3 \\
waj  &	13K  &	Waffa  &	5K  &	Oceania  &	Latn  &	waj  &	99.8  &	- \\
kkc  &	12K  &	Odoodee  &	5K  &	Oceania  &	Latn  &	\scriptsize{adh-5l}  &	99.8  &	- \\
mil  &	12K  &	Peñoles Mixtec  &	50K  &	Americas  &	Latn  &	\scriptsize{mib-2l}  &	100  &	- \\
ndj  &	12K  &	Ndamba  &	50K  &	Africa  &	Latn  &	\scriptsize{dov-9l}  &	100  &	15.9 \\
ngp  &	12K  &	Ngulu  &	100K  &	Africa  &	Latn  &	\scriptsize{cwe-10l}  &	98.3  &	16.3 \\
okv  &	11K  &	Orokaiva  &	50K  &	Oceania  &	Latn  &	\scriptsize{aom-10l}  &	99.1  &	14.6 \\
nnq  &	11K  &	Ngindo  &	200K  &	Africa  &	Latn  &	\scriptsize{nnq-4l}  &	99.9  &	13.9 \\
grt  &	11K  &	Garo  &	1M  &	Asia  &	Beng  &	\scriptsize{bpy-7l}  &	100  &	- \\
psh  &	11K  &	Southwest Pashayi  &	50K  &	Asia  &	Arab  &	\scriptsize{fay-14l}  &	15.5  &	38.0 \\
hnd  &	11K  &	Southern Hindko  &	600K  &	Asia  &	Arab  &	\scriptsize{bal-13l}  &	17.3  &	- \\
tgp  &	11K  &	Movono  &	5K  &	Oceania  &	Latn  &	\scriptsize{akb-4l}  &	100  &	- \\
tbo  &	10K  &	Tawala  &	50K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	98.5  &	- \\
bxh  &	9K  &	Buhutu  &	5K  &	Oceania  &	Latn  &	\scriptsize{aui-14l}  &	93.2  &	- \\
mfa  &	7K  &	Kelantan-Pattani Malay  &	1M  &	Asia  &	Arab  &	\scriptsize{mfa-3l}  &	95.9  &	23.2 \\
 \label{tab:datasize_full}
\end{longtable}
\end{footnotesize}
}



==> Next Thousand Languages/table_datasize_summary.tex <==
\newcommand{\inserttabledatasizesummary}{
\begin{table*}
\centering
\begin{tabular}{l|rrrrr}
 
 dataset & N & total & median &  $>$ 1M &  $>$ 100K \\
\hline
LRL-full & 1503 & 1.7B & 25k & 122 & 322 \\
LRL-train  & 1057 & 1.7B & 38k & 122 & 321 \\
all-train  & 1140 & 28B & 43k & 205 & 404 \\
\end{tabular}
\caption{Summary statistics about monolingual data for 1) the full dataset of low-resource languages; 2) the portion thereof used to train our model; and 3) the full training set including high resource languages. Columns are the number of languages covered, the total number of sentences across all languages, the median number of sentences per language, the number of languages with more than 1 million sentences, and the number of languages with more than 100,000 sentences.
 \label{tab:datasize_summary}}
\end{table*}}

==> Next Thousand Languages/table_direct.tex <==
\begin{table}[htb]%\[!htb\]
    \begin{subtable}[t]{.5\textwidth}
        \raggedright
            \begin{tabular}{l|l|ll|ll}
\hline
 lang. & direct & \multicolumn{2}{c}{close HRL} & \multicolumn{2}{|c}{closer LRL} \\
 
\hline
\multicolumn{6}{c}{}\\
\multicolumn{6}{c}{Native American Languages}\\
\hline
 ay & 33.1 & es & \textbf{34.2} & - &  - \\
 gn & \textbf{31.5} & es & 28.9 & - &  - \\
 kl & \textbf{35.5} & da & 27.5 & - &  - \\
 qu & \textbf{35.3} & es & 29.5 & - &  - \\
 quc & \textbf{24.1} & es & 22.5 & - &  - \\
 yua & \textbf{31.5} & es & 28.4 & - &  - \\
 
\multicolumn{6}{c}{}\\
\multicolumn{6}{c}{Indian Languages (Indo-European)}\\
\hline
 as & 39.2 & hi & \textbf{39.8} & bn & 36.3 \\
 bho & 42.0 & hi & \textbf{43.4} & - &  - \\
 doi & 36.3 & hi & \textbf{39.5} & pa & 33.3 \\
 dv & \textbf{44.4} & hi & 42.0 & si & 39.7 \\
 gom & \textbf{40.2} & hi & 39.3 & mr & 39.7 \\
 ks & 21.9 & hi & 25.7 & ur & \textbf{28.5} \\
 mai & 38.1 & hi & \textbf{44.3 }& - &  - \\
 sa & \textbf{30.5} & hi & 27.3 & - &  - \\
 \multicolumn{6}{c}{}\\
 \multicolumn{6}{c}{}\\
            \end{tabular}
    \end{subtable}%
   \begin{subtable}[t]{.5\textwidth}
        \raggedleft
        \begin{tabular}{l|l|ll|ll}
        \hline
         lang. & direct & \multicolumn{2}{c}{close HRL} & \multicolumn{2}{|c}{closer LRL} \\
 
\hline
\multicolumn{6}{c}{}\\
\multicolumn{6}{c}{Indian Languages (Not Indo-European)}\\
\hline
 brx-Beng & 4.6 &  hi & \textbf{11.5} & my & 3.4 \\
 lus & \textbf{38.6} &      hi & \textbf{38.2} & my & 34.1 \\
 mni & \textbf{40.7} &      hi & 35.5 & my & 29.4 \\
 sat-Latn & \textbf{20.9} & hi & \textbf{20.8} & km & 18.2 \\
 
\multicolumn{6}{c}{}\\
\multicolumn{6}{c}{Bantu Languages}\\
\hline
 lg & \textbf{38.7} &  sw & 34.1 & rw & 33.6 \\
 ln & \textbf{34.4} &  sw & 31.9 & fr & 25.5 \\
 nso & \textbf{45.7} & sw & 33.3 & st & 29.1 \\
 ts & \textbf{46.2} &  sw & 40.0 & zu & 44.0 \\
 
\multicolumn{6}{c}{}\\
\multicolumn{6}{c}{Other}\\
\hline
 bm & \textbf{34.3} & fr & 26.6 & - &  - \\
 ff & \textbf{34.7} & sw & 26.7 & - &  - \\
 ilo & \textbf{54.0} & id & 48.4 & fil & 51.2 \\
 om & \textbf{39.2} & - &  - & so & 30.2 \\
 ti & 21.4 & - &  - & am & \textbf{22.6} \\
 yue & 20.3 & zh & \textbf{21.6} & - &  - \\
        \end{tabular}
    \end{subtable}
    
\caption{Results for bridged translation from English (\chrf{}) on 1200 sentences/language. Bridging seems to improve quality only when the intermediate language is both higher-resource and close to the target language.} 
\label{tab:direct}
\end{table}








==> Next Thousand Languages/table_error_magnification.tex <==


% \begin{wraptable}{r}{5.5cm}
% \centering
% \begin{tabular}{l|ll}
% language  & \% mono & \% synthetic \\
% \hline
% pcm & 8\% & 20\% \\
% kl & 14\% & 24\%\\
% sa & 9.2\% & 5.7\% \\
% \hdashline
% ja & 0.0004\% & 1\% \\
% \end{tabular}
% \caption{Percent of each data set removed after applying specialized filters. We see that the monolingual web crowded theater generally exhibited these problems to a lesser degree than the synthetic text generated by the teacher model.
%  \label{tab:error_magnification}}
% \end{wraptable}
% % https://b.corp.google.com/issues/205888441

==> Next Thousand Languages/table_errors_shortinput.tex <==


\newcommand{\inserterrorssinglewordslong}{
\begin{table}[H]
\centering
\small
\begin{tabular}{l| llll}
\hline
\hline
sl    & tl & source     & translation \\
\hline
en & ff & devices & ka\AS{\m{b}}ir\AS{\m{d}}e (dispositifs) \\
en & ff & lenses & lensuuji (lenses) \\
en & ff & flexibility & mbaydi (flexibilit{\'e}) \\
en & ff & admire & yi\AS{\m{d}}de (yi\AS{\m{d}}de) \\
en & ee & smartphones & smartphones (telefon siwo \AS{\m{n}}u wow\AS{\m{o}}a d\AS{\m{o}} le) \\
en & kl & stanford & stanford-imi ilinniartoq (student at stanford) \\
en & kl & amber & rav , qaqortoq, \\
en & kl & triangle & trekant , s. trekant \\
en & qu & attempting & attempting (to -) ruwayta munaspa \\
en & om & coupling & walqabsiisaa (coupling) \\
en & lus &  shield & r{\^ a}lthuam (shield) \\
en & lus &  fragile & hring hring (fragile) \\
\hline \\
en & pcm & removes & dey remove  \\
en & pcm & blame  & blame wetin?  \\
en & pcm & ethics & ethics wey dey  \\
en & pcm & partnerships   & partnerships wey dey  \\
en & pcm & organizing     & organizing dey  \\
\hdashline \\
en & lus & four   & pali a awm a  \\
en & lus & lawrence       & lawrence chuan a ti a  \\
en & lus & theory & theory a ni a  \\
en & lus & carpet & carpet a khuh a, a khuh lohna tur  \\
en & lus & dodge  & dodge tih a ni  \\
en & lus & freedom& zalenna a awm  \\
\hdashline \\
en & quc & solved & xsol rij ri  \\
en & quc & impress& kqak’aq b’i ri uq’ab’  \\
en & quc & flagship & ri b’inel ja’  \\
en & quc & mercury& ri mercurio  \\
en & quc & dam  & ri k'o pa ri cho  \\
\hdashline \\
en & kri & juvenile & \AS{pikin we n\m{o} rich 18 ia yet} \\
en & kri & reliable & \AS{p\m{o}sin we d\m{e}n kin abop pan} \\
en & kri & barriers & \AS{di tin d\m{e}n we de amb\m{o}g am} \\
en & kri & notorious & \AS{pipul d\m{e}n we g\m{e}t badnem} \\
en & kri & seniors  & \AS{di wan d\m{e}n we d\m{o}n ol} \\
en & kri & continued & \AS{k\m{o}ntinyu f\m{o}} \\
en & kri & wise & \AS{g\m{e}t s\m{e}ns} \\
en & kri & genome  & \AS{di j\m{e}n\m{e}tiks we de insay di b\m{o}di} \\
en & kri & runners &  \AS{di wan d\m{e}n we de r\m{o}n} \\
\hline
\end{tabular}

\caption{Our models frequently displayed exceeding verbosity with single-word inputs. In some cases they would add extra definitions for words in parentheses or commas afterwards (top half of table). In other instances they appended frequent tokens from that language after the translation, or gave whole definitions, as with Krio.}
\label{tab:errors_singlewords_long}
\end{table}
}

% https://docs.google.com/document/d/1rFpb2RIzpmUtbak4_4NWOrCvx5A7q4L_pDhyw-r0C_A/edit#




\newcommand{\insertsinglewordserrorcats}{
\begin{table}[H]
\centering
\small
\begin{tabular}{ll| lllll}
\hline
\hline
direction & 	model & 	copies & 	multi-word & 	duplicate & 	repeats & 	other \\
% \hline
% teach full & enxx &	0.5 & 	75 & 	24.7 & 	3.4 & 	13.2 \\ 
% teach full & enxx. &	0.1 & 	75.9 & 	29.6 & 	0.9 & 	9.0 \\ 
% \hdashline
% teach full & xxen &	72.4 & 	3.7 & 	14.4 & 	0.3 & 	7.0 \\ 
% teach full & xxen. &	53.1 & 	14.7 & 	19.7 & 	0.2 & 	10.6 \\ 

\hline
\enxx & 	teacher & 	1.28 & 	66.23 & 	26.48 & 	5.55 & 	17.43 \\ 
\enxx & 	teacher. & 	0.85 & 	71.71 & 	31.66 & 	2.79 & 	13.87 \\ 
\hdashline
\enxx & 	student & 	1.15 & 	48.21 & 	37.16 & 	1.43 & 	27.38 \\ 
\enxx & 	student. & 	8.28 & 	45.53 & 	36.18 & 	2.05 & 	22.73 \\
\hline
\xxen & 	teacher & 	61.87 & 	6.19 & 	21.11 & 	0.74 & 	14.74 \\
\xxen & 	teacher. & 	47.3 & 	17.02 & 	24.8 & 	0.47 & 	18.21 \\
\hdashline
\xxen & 	student & 	18.33 & 	28.54 & 	43.23 & 	2.65 & 	22.65 \\
\xxen & 	student. & 	20.1 & 	35.14 & 	40.41 & 	0.27 & 	21.70 \\

\hline
\end{tabular}
\caption{Statistics for single-token translation on the top ten thousand most common tokens from the monolingual datasets, compared for 48 language pairs, for the fine-tuned teacher model. Metrics shown are 1) percent of outputs that copy the source; 2) percent of input that is multi-word; 3) percent of outputs that are identical to other outputs, suggesting incorrect translation; 4) percent of outputs with low character diversity, suggesting repeats; and 5) percent of outputs with none of those features. The entries with full-stops (.) after them use the ``period trick'' (Section \ref{sec:period}). Single word translation is a particularly tricky task as the model needs to solve translation and LangID simultaneously, which can be undefined for short queries. 
}
\label{tab:singlewordserrorcats}
\end{table}
}

% https://docs.google.com/document/d/1rFpb2RIzpmUtbak4_4NWOrCvx5A7q4L_pDhyw-r0C_A/edit#































\newcommand{\inserterrorssinglewordsshort}{
\begin{table}[H]
\centering
\small
\begin{tabular}{ll|lll}
\hline
\hline
sl    & tl & source     & translation \\
\hline
en & ff & devices & ka\AS{\m{b}}ir\AS{\m{d}}e (dispositifs) \\
en & lus &  fragile & hring hring (fragile) \\
en & pcm & removes & \textbf{dey} remove  \\
en & pcm & blame  & blame wetin?  \\
en & lus & four   & pali \textbf{a awm a}  \\
en & lus & freedom& zalenna \textbf{a awm}  \\
en & quc & solved & xsol rij \textbf{ri}  \\
en & quc & dam  & \textbf{ri} k'o pa \textbf{ri} cho  \\
en & kri & juvenile & \AS{pikin we n\m{o} rich 18 ia yet} \\
en & kri & notorious & \AS{pipul d\m{e}n we g\m{e}t badnem} \\
\hline
\end{tabular}

\caption{Our models frequently displayed exceeding verbosity with single-word inputs. In some cases they would add extra definitions for words in parentheses or commas afterwards (top half of table). In other instances they added function words from that language after the translation (\textbf{boldface}), or gave whole definitions, as with Krio.}
\label{tab:errors_singlewords_short}
\end{table}
}


==> Next Thousand Languages/table_flores.tex <==


\begin{table*}[t]
\centering
\small
\begin{tabular}{c|cc||c|cc}
\hline
\hline
LP & this method  & M2M-100 & LP & this method  & M2M-100    \\
\hline


en$\rightarrow$as &\textbf{29.1} & 1.22 & as$\rightarrow$en & \textbf{34.5} & 3.76\\
en$\rightarrow$ckb & \textbf{28.5} & 0.23 & ckb$\rightarrow$en & \textbf{37.5} & 7.65 \\
en$\rightarrow$ff & \textbf{2.5} & 0.68 & ff$\rightarrow$en & \textbf{11.2} & 2.4 \\
en$\rightarrow$lg & \textbf{17.3} & 0.61 & lg$\rightarrow$en & \textbf{29.3} & 4.45\\
en$\rightarrow$ln & \textbf{24.7} & 1.03 & ln$\rightarrow$en & \textbf{30.2} & 4.57\\
en$\rightarrow$nso & \textbf{32.5} & 1.54 & nso$\rightarrow$en & \textbf{45.0} & 6.76\\
en$\rightarrow$om & \textbf{17.2} & 0.4 & om$\rightarrow$en & \textbf{30.8} & 3.33\\
\hline
\end{tabular}
\caption{Flores dev-test: comparing \textsc{spBleu} between this method and \citet{goyal2021flores}.
 \label{tab:flores}}
\end{table*}


==> Next Thousand Languages/table_glyphs.tex <==

\begin{table*}[ht]
\small
\centering
\begin{tabular}{lr}
Unicode character name &	Percent of Data \\
\hline
LATIN CAPITAL LETTER I &	33.6\% \\
DIGIT ONE &	30.4\% \\
\textbf{CYRILLIC LETTER PALOCHKA} &	3.8\% \\
CYRILLIC CAPITAL LETTER BYELORUSSIAN-UKRAINIAN I &	4.2\% \\
LATIN SMALL LETTER L &	2.8\% \\
GREEK CAPITAL LETTER IOTA &	0.4\% \\
\hdashline
LATIN SMALL LETTER A WITH BREVE	&	52.4\% \\
LATIN SMALL LETTER E WITH BREVE	&	55.0\% \\
LATIN SMALL LETTER C WITH CEDILLA	&	43.4\% \\
\textbf{CYRILLIC SMALL LETTER IE WITH BREVE}	&	10.2\% \\
\textbf{CYRILLIC SMALL LETTER A WITH BREVE}	&	9.4\% \\
\textbf{CYRILLIC SMALL LETTER ES WITH DESCENDER}	&	8.8\% \\
\end{tabular}
\caption{Examples of the different Unicode points used to encode the Palochka character in the Chechen language (above) and letters with diacritics in the Chuvash language (below), along with their prevalence on web-crawled data. In both cases, the ``correct'' Unicode point (\textbf{bolded}) is much less common.
 \label{tab:chechen}}
\end{table*}


\begin{table*}[ht]
\small
\centering
\begin{tabular}{llr}
Unicode point & 	name & 	avg. \chrf{} \\ 
\hline		
\multicolumn{3}{c}{}\\		
\multicolumn{3}{c}{gn, luo, quc, yua $\rightarrow$ en}\\		
\hdashline		
U+2019 & 	Right quote & 	25.7 \\ 
U+0060 & 	Grave accent & 	25.5 \\ 
U+0027 & 	Apostrophe & 	25.5 \\ 
U+02BB & 	'Okina & 	25.5 \\ 
U+00B4 & 	Acute accent & 	25.4 \\ 
 & 	None & 	24.5 \\ 
 
\multicolumn{3}{c}{}\\		
\multicolumn{3}{c}{ady, av, ce $\rightarrow$ en}\\		
\hdashline		
U+04C0 & 	Palochka & 	49.6 \\ 
U+0031 & 	ASCII 1 & 	49.4 \\ 
U+0399 & 	Greek Iota & 	49.4 \\ 
U+0406 & 	Byelorusian/Ukrainian I & 	49.3 \\ 
		
\multicolumn{3}{c}{}\\		
\multicolumn{3}{c}{ak, bm, dyu, ee $\rightarrow$ en}\\		
\hdashline		
U+025B, U+0254 & 	Latin open e/o & 	33.6 \\ 
U+03B5, U+1D10 & 	Greek epsilon; small capital O & 	25.8 \\ 
U+0033, U+0029 & 	3 and ) (chatspeak) & 	25.3 \\ 
\multicolumn{3}{c}{}\\		
\multicolumn{3}{c}{cv $\rightarrow$ en}\\		
\hdashline		
U+04D7, U+04D1, U+04AB & 	Cyrillic codepoints & 	42.3 \\ 
U+0115, U+0103, U+00E7 & 	Latin Codepoints & 	43.0 \\ 
 \end{tabular}
\caption{\chrf{} score where the source uses different versions of common Unicode points. The top line of each bloc represents the ``correct'' codepoints, whereas the lower lines are other ways of representing the same letter. In many cases there is very little difference in performance, but the African languages are affected by nonstandard \AS{\m{o}} and \AS{\m{e}}. When the apostrophe is removed entirely, the performance also drops noticeably.
 \label{tab:glyph_bleu}}
\end{table*}



==> Next Thousand Languages/table_grounding_tokens.tex <==
\newcommand{\inserttablegroundingtokens}{\begin{table*}
\centering
\scriptsize
\begin{tabular}{lllllllllllllll}
\hline
\hline
sents&	pts&	lb&	ub&	metric &	bew &	mzn &	as &	lus &	dv &	sa &	om &	ti &	cv &	ilo \\
\hline										
&       &       &       &       N mono &   33M &   12M &   9M &    8M &    8M &    6M &    6M &    4M &    3M &    3M \\
&       &       &       &       \chrf &   51.5 &  54.6 &  59.1 &  34.5 &  45.1 &  46.6 &  38 &    43.8 &  46.6 &  43.5 \\
\hline
1191&   9682&   0&      125&    $\Xi$ &       \cellcolor{scale8} 64 & \cellcolor{scale8} 65 & \cellcolor{scale9} 73 & \cellcolor{scale5} 43 & \cellcolor{scale7} 58 & \cellcolor{scale8} 64 & \cellcolor{scale7} 55 & \cellcolor{scale8} 60 & \cellcolor{scale8} 62 & \cellcolor{scale5} 41 \\
994&    2537&   125&    500&    $\Xi$ &       \cellcolor{scale7} 56 & \cellcolor{scale7} 60 & \cellcolor{scale8} 65 & \cellcolor{scale4} 32 & \cellcolor{scale6} 49 & \cellcolor{scale6} 51 & \cellcolor{scale5} 42 & \cellcolor{scale6} 52 & \cellcolor{scale6} 51 & \cellcolor{scale5} 39 \\
1034&   3102&   500&    2k&     $\Xi$ &       \cellcolor{scale7} 55 & \cellcolor{scale8} 61 & \cellcolor{scale8} 66 & \cellcolor{scale4} 31 & \cellcolor{scale6} 48 & \cellcolor{scale6} 50 & \cellcolor{scale5} 39 & \cellcolor{scale6} 45 & \cellcolor{scale6} 49 & \cellcolor{scale5} 42 \\
958&    2420&   2k&     8k&     $\Xi$ &       \cellcolor{scale6} 51 & \cellcolor{scale7} 56 & \cellcolor{scale7} 56 & \cellcolor{scale3} 27 & \cellcolor{scale6} 44 & \cellcolor{scale5} 42 & \cellcolor{scale4} 28 & \cellcolor{scale5} 38 & \cellcolor{scale5} 43 & \cellcolor{scale5} 41 \\
% 332&    402&    8k&     13k&    $\Xi$ &       \cellcolor{scale6} 47 & \cellcolor{scale6} 51 & \cellcolor{scale7} 53 & \cellcolor{scale3} 26 & \cellcolor{scale6} 44 & \cellcolor{scale4} 34 & \cellcolor{scale2} 20 & \cellcolor{scale3} 27 & \cellcolor{scale5} 39 & \cellcolor{scale5} 38 \\



\multicolumn{15}{c}{}\\
\hline
\hline
metric &        nso &   pcm &   ce &    mai &   ts &    ak &    skr &   bbc &   gn &    qu &    min &   yua &   iso &   gom \\
\hline

N mono &   2M &    2M &    1M &    1M &    1M &    1M &    974k &  932k &  861k &  842k &  533k &  419k &  409k &  311k \\
\chrf &   51.1 &  52.3 &  45.2 &  61.4 &  43.6 &  36.1 &  47.8 &  44.2 &  38.2 &  32.2 &  62.2 &  40.8 &  29.1 &  54.9 \\

\hline
$\Xi$ &       \cellcolor{scale9} 73 & \cellcolor{scale8} 61 & \cellcolor{scale7} 55 & \cellcolor{scale9} 68 & \cellcolor{scale8} 61 & \cellcolor{scale7} 57 & \cellcolor{scale8} 64 & \cellcolor{scale7} 56 & \cellcolor{scale7} 57 & \cellcolor{scale5} 40 & \cellcolor{scale9} 72 & \cellcolor{scale7} 58 & \cellcolor{scale6} 45 & \cellcolor{scale9} 69 \\
$\Xi$ &       \cellcolor{scale7} 57 & \cellcolor{scale7} 53 & \cellcolor{scale6} 47 & \cellcolor{scale8} 66 & \cellcolor{scale6} 45 & \cellcolor{scale4} 34 & \cellcolor{scale7} 53 & \cellcolor{scale6} 47 & \cellcolor{scale4} 35 & \cellcolor{scale4} 28 & \cellcolor{scale8} 66 & \cellcolor{scale5} 40 & \cellcolor{scale3} 23 & \cellcolor{scale7} 59 \\
$\Xi$ &       \cellcolor{scale6} 51 & \cellcolor{scale7} 54 & \cellcolor{scale6} 45 & \cellcolor{scale8} 67 & \cellcolor{scale5} 42 & \cellcolor{scale4} 30 & \cellcolor{scale7} 53 & \cellcolor{scale6} 46 & \cellcolor{scale4} 32 & \cellcolor{scale4} 30 & \cellcolor{scale8} 67 & \cellcolor{scale5} 39 & \cellcolor{scale2} 20 & \cellcolor{scale7} 59 \\
$\Xi$ &       \cellcolor{scale5} 41 & \cellcolor{scale7} 53 & \cellcolor{scale5} 43 & \cellcolor{scale8} 62 & \cellcolor{scale5} 38 & \cellcolor{scale3} 24 & \cellcolor{scale6} 47 & \cellcolor{scale5} 39 & \cellcolor{scale4} 28 & \cellcolor{scale4} 29 & \cellcolor{scale8} 63 & \cellcolor{scale4} 31 & \cellcolor{scale2} 17 & \cellcolor{scale6} 52 \\
% $\Xi$ &       \cellcolor{scale4} 35 & \cellcolor{scale6} 50 & \cellcolor{scale5} 39 & \cellcolor{scale7} 57 & \cellcolor{scale4} 31 & \cellcolor{scale3} 23 & \cellcolor{scale5} 40 & \cellcolor{scale4} 34 & \cellcolor{scale3} 25 & \cellcolor{scale4} 30 & \cellcolor{scale7} 56 & \cellcolor{scale4} 29 & \cellcolor{scale2} 17 & \cellcolor{scale5} 44 \\



\multicolumn{15}{c}{}\\
\hline
\hline
metric &        av &    ady &   quc &   ban &   bm &    doi &   mad &   kri &   mni &   ff &    mfa \\
\hline

N mono &   301k &  296k &  250k &  188k &  187k &  179k &  138k &  129k &  106k &  86k &   7k \\
\chrf &   48.4 &  55.2 &  27 &    35.4 &  35.8 &  62.8 &  50.1 &  56.1 &  56.2 &  40.7 &  65.1 \\
\hline
$\Xi$ &       \cellcolor{scale7} 55 & \cellcolor{scale7} 56 & \cellcolor{scale5} 42 & \cellcolor{scale6} 48 & \cellcolor{scale7} 57 & \cellcolor{scale10} 77 &        \cellcolor{scale8} 61 & \cellcolor{scale8} 65 & \cellcolor{scale9} 71 & \cellcolor{scale8} 66 & \cellcolor{scale10} 77 \\
$\Xi$ &       \cellcolor{scale7} 53 & \cellcolor{scale8} 63 & \cellcolor{scale3} 20 & \cellcolor{scale4} 33 & \cellcolor{scale4} 34 & \cellcolor{scale9} 68 & \cellcolor{scale6} 50 & \cellcolor{scale7} 58 & \cellcolor{scale8} 61 & \cellcolor{scale5} 41 & \cellcolor{scale9} 71 \\
$\Xi$ &       \cellcolor{scale7} 57 & \cellcolor{scale8} 67 & \cellcolor{scale2} 19 & \cellcolor{scale4} 33 & \cellcolor{scale4} 30 & \cellcolor{scale9} 69 & \cellcolor{scale6} 49 & \cellcolor{scale7} 59 & \cellcolor{scale7} 59 & \cellcolor{scale4} 33 & \cellcolor{scale9} 69 \\
$\Xi$ &       \cellcolor{scale7} 55 & \cellcolor{scale8} 65 & \cellcolor{scale2} 16 & \cellcolor{scale4} 29 & \cellcolor{scale3} 22 & \cellcolor{scale8} 62 & \cellcolor{scale6} 45 & \cellcolor{scale6} 50 & \cellcolor{scale6} 51 & \cellcolor{scale3} 26 & \cellcolor{scale8} 62 \\
% $\Xi$ &       \cellcolor{scale6} 51 & \cellcolor{scale7} 60 & \cellcolor{scale2} 15 & \cellcolor{scale4} 29 & \cellcolor{scale2} 20 & \cellcolor{scale7} 56 & \cellcolor{scale5} 40 & \cellcolor{scale5} 41 & \cellcolor{scale6} 46 & \cellcolor{scale2} 19 & \cellcolor{scale6} 51 \\

\end{tabular}
% \vspace{-0.6em}
\caption{Token hit-rate ($\Xi$) for different sets of tokens, binned by frequency. The lower and upper bound of the token frequency rank per bin are given in the \texttt{lb} and \texttt{ub} columns; thus, the top row is the hit-rate on the 125 most frequent tokens, and the bottom row is on the 6,000 least frequent tokens. Columns \texttt{sents} and \texttt{pts} give the number of sentences in each bin-specific eval set and the number of tokens in that bin occurring in those references, respectively. The \chrf{} score and number of monolingual training sentences is also given. 
 The interesting results are on the languages, like Fulfulde (\texttt{ff}), that have a high hit-rate on more frequent tokens and a lower hit-rate on rarer tokens. All results are only in the \xxen direction.}
\label{table:grounding_tokens}
% \vspace{-0.6em}
\end{table*}
}

==> Next Thousand Languages/table_inflecting.tex <==
\newcommand{\insertinflecting}{
\begin{table*}
\centering
% \scriptsize % \tiny \scriptsize \footnotesize \small
\fontsize{8.5pt}{9pt}\selectfont
% \fontsize{6.5pt}{8pt}\selectfont
\begin{tabular}{p{0.42\linewidth} | p{0.52\linewidth}}
\hline
source     & translation \\
\hline
I can't sing so well so I don't want to be a singer. & Erinangippallaannginnama erinarsortartunngorusunngilanga.\\
Without my car, I wouldn't be able to get to work.	& Biileqanngikkuma suliartorsinnaanavianngilanga.\\
I would like to raise a dog instead of a cat	 & Qimmiuteqarusunnerussangaluarpunga qitsuuteqarnissannit.\\
I have a cat who is lazy. &	Qitsuuteqarpunga eqiasuttuuvoq. \\
\hline
\end{tabular}

\caption{Example translations from English to Kalaallisut from our evaluation set. A token-based metric like \bleu{} is unsuitable for such a highly inflecting language, as exact match is very unlikely. Character-based metrics, like \chrf{}, are more appropriate. }
\label{tab:inflecting}
\end{table*}
}



	

% I would ask my cat some questions about what he's always trying to tell him by meowing.	Qitsuutinga apeqqutinik apeqquteqarfigerusussinnaavara miaarveertuinnaleraangami suna oqaatigerusuttaraluarneraa.

==> Next Thousand Languages/table_ntlv3_audit.tex <==

% \small
% \centering
% \begin{longtable}{l|lr:rrrrrr}
\newcommand{\insertntlaudit}{
\begin{longtable}{lrrrrrrr}

Language Name (BCP-47) &         score &         cc &    cb &    ca &    wl &    nl &    wd \\
\hline
Northeastern Dinka (dip) &      100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Zarma (dje) &   100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Dombe (dov) &   100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Dyula (dyu) &   100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Wayuu (guc) &   100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Kalenjin (kln) &        100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Wolaytta (wal) &        100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Assyrian Neo-Aramaic (aii) &        100 &   100 &   0 &     0 &     0 &     0 &     0 \\
Igbo (ig) &     99 &    98 &    2 &     0 &     0 &     0 &     0 \\ 
Balinese (ban) &        98 &    96 &    4 &     0 &     0 &     0 &     0 \\ 
Latinized Hindi (hi-Latn) &       98 &    98 &    0 &     0 &     2 &     0 &     0 \\ 
Twi (ak) &     97 &    94 &    6 &     0 &     0 &     0 &     0 \\ 
Luyia (luy) &   97 &    97 &    0 &     0 &     0 &     0 &     3 \\ 
Ewe (ee) &      96 &    91 &    9 &     0 &     0 &     0 &     0 \\ 
Seselwa Creole French (crs) &   94 &    92 &    4 &     1 &     3 &     0 &     0 \\ 
Bhojpuri (bho) &        94 &    94 &    0 &     0 &     6 &     0 &     0 \\ 
Ilocano (ilo) &   94 &    88 &    12 &    0 &     0 &     0 &     0 \\ 
Caribbean Javanese (jvn) &      94 &    87 &    13 &    0 &     0 &     0 &     0 \\ 
Meiteilon (Manipuri) (mni) &        93 &    87 &    12 &    0 &     0 &     1 &     0 \\ 
Luba-Katanga (lu) &     92 &    83 &    17 &    0 &     0 &     0 &     0 \\ 
Krio (kri) &    92 &    89 &    5 &     0 &     6 &     0 &     0 \\ 
Latinized Tamil (ta-Latn) &       91 &    81 &    19 &    0 &     0 &     0 &     0 \\ 
Lingala (ln) &  90 &    80 &    19 &    0 &     1 &     0 &     0 \\ 
Maharasthra Konkani (knn) &     89 &    85 &    8 &     1 &     6 &     0 &     0 \\ 
Northern Sami (se) &    89 &    86 &    5 &     0 &     9 &     0 &     0 \\ 
Cherokee (chr) &        88 &    78 &    20 &    0 &     1 &     1 &     0 \\ 
Latinized Malayalam (ml-Latn) &   87 &    76 &    21 &    1 &     2 &     0 &     0 \\ 
Latinized Bengali (bn-Latn) &     86 &    72 &    28 &    0 &     0 &     0 &     0 \\ 
Maithili (mai) &        86 &    83 &    5 &     1 &     11 &    0 &     0 \\ 
Hiligaynon (hil) &      84 &    80 &    8 &     0 &     9 &     3 &     0 \\ 
Tok Pisin (tpi) &       84 &    83 &    2 &     0 &     15 &    0 &     0 \\ 
Latinized Chinese	(zh-Latn)     & 84 &80 &	7 &	0 &	13 &	0 &	0 \\
Gulf Arabic (afb) &     83 &    74 &    17 &    1 &     8 &     0 &     0 \\ 
Minangkabau (min) &     81 &    64 &    34 &    0 &     2 &     0 &     0 \\ 
Chuvash (cv) &  80 &    78 &    4 &     0 &     2 &     2 &     14 \\ 
Tamazight (ber-Latn) &  79 &    69 &    20 &    0 &     10 &    1 &     0 \\ 
Latinized Telugu (te-Latn) &      79 &    74 &    10 &    0 &     0 &     16 &    0 \\ 
Libyan Arabic (ayl) &   78 &    68 &    14 &    10 &    7 &     1 &     0 \\ 
Newari (new) &  78 &    76 &    3 &     0 &     21 &    0 &     0 \\ 
Pangasinan (pag) &      75 &    67 &    17 &    0 &     0 &     17 &    0 \\ 
Waray (war) &     75 &    67 &    17 &    0 &     17 &    0 &     0 \\ 
Goan Konkani (gom) &    73 &    67 &    5 &     13 &    13 &    2 &     0 \\ 
Sanskrit (sa) &         73 &    66 &    14 &    0 &     15 &    5 &     0 \\ 
North Levantine Arabic (apc) &  73 &    62 &    21 &    0 &     16 &    1 &     0 \\ 
Sudanese Arabic (apd-SD) &      72 &    60 &    4 &     34 &    2 &     0 &     0 \\ 
Ibibio (ibb) &  72 &    63 &    17 &    0 &     20 &    0 &     0 \\ 
Shona (sn) &    72 &    43 &    57 &    0 &     0 &     0 &     0 \\ 
Sena (seh) &    71 &    71 &    0 &     0 &     29 &    0 &     0 \\ 
Latinized Marathi (mr-Latn) &     67 &    36 &    62 &    0 &     1 &     1 &     0 \\ 
Ancient Greek (grc) &         67 &    67 &    0 &     0 &     29 &    4 &     0 \\ 
Makhuwa-Meetto (mgh) &  67 &    67 &    0 &     0 &     33 &    0 &     0 \\ 
Algerian Arabic (arq) &         64 &    47 &    6 &     47 &    0 &     0 &     0 \\ 
Latinized Goan Konkani (gom-Latn) &       64 &    63 &    0 &     2 &     28 &    7 &     0 \\ 
Ga (gaa) &      58 &    58 &    0 &     0 &     0 &     0 &     41 \\ 
Wolof (wo) &    57 &    16 &    81 &    0 &     1 &     2 &     0 \\ 
Nigerian Pidgin (pcm) &         51 &    43 &    14 &    3 &     40 &    0 &     0 \\ 
Saint Lucian Creole French (acf) &      50 &    50 &    0 &     0 &     50 &    0 &     0 \\ 
Kashmiri (ks-Deva) &    48 &    47 &    1 &     2 &     17 &    33 &    0 \\ 
Latinized Arabic (ar-Latn) &      47 &    33 &    15 &    21 &    6 &     24 &    0 \\ 
Kuanyama (kj) &         43 &    43 &    0 &     0 &     57 &    0 &     0 \\ 
Adangme (ada) &         42 &    42 &    0 &     0 &     0 &     0 &     58 \\ 
Anaang (anw) &  36 &    26 &    19 &    0 &     54 &    1 &     0 \\ 
Mesopotamian Arabic (acm) &     34 &    6 &     0 &     93 &    1 &     0 &     0 \\ 
North Ndebele (nd) &    25 &    25 &    0 &     0 &     50 &    25 &    0 \\ 
Moroccan Arabic (ar-MA) &       16 &    1 &     24 &    9 &     59 &    7 &     0 \\ 
Baluchi (bal) &         10 &    10 &    0 &     0 &     90 &    0 &     0 \\ 
Saidi Arabic (aec) &    0 &     0 &     0 &     0 &     100 &   0 &     0 \\ 
Eastern Baluchi (bgp) &         0 &     0 &     0 &     0 &     100 &   0 &     0 \\ 
Eastern Baluchi (bgp-Arab) &    0 &     0 &     0 &     0 &     100 &   0 &     0 \\ 
\hdashline
mean &     74 &    68 &    10 &    3 &     15 &    2 &     2 \\ 
median &    80 &    74 &    5 &     0 &     3 &     0 &     0 \\ 
\caption{Results of an audit of the datasets we collected, conducted on sampled of 100 sentences each by a mix of native speakers and non-native speakers. The values are the percent of the audited sample that head each label. The ``score'' metric combines these numbers for an approximate notion of the percent of the data that is usable, and is described in Section \ref{sec:audit}.
 \label{tab:audit}}
\end{longtable}
}

==> Next Thousand Languages/table_period.tex <==


\newcommand{\insertmagnification}{
\begin{table*}
{
\centering
\begin{tabular}{c|ccc}
\hline
\hline
language  & \% mono & \% synth (clean)  & \% synth (noisy)  \\
\hline
pcm & 8\% & 20\% & - \\
kl & 14\% & 18\% & 30\%\\
sa & 13\% & 16\% &  37\% \\
% \hdashline
ja & 0.0004\% & - &  1\% \\
\hline
\end{tabular}
\caption{Percent of each data set removed after applying specialized filters. mono refers to the monolingual data from the corpus mined in Section~\ref{sec:data:data}. synth(clean) refers to synthetic data generated by forward translating a clean English monolingual corpus and synth (noisy) refers to synthetic data generated from a noisy web-scraped English corpus. We see that the synthetic text generated by the teacher model exhibited these problems to a greater degree than the monolingual web-sourced data, and that these problems intensified on noisier data.
 \label{tab:error_magnification}}
}
\end{table*}
}



\newcommand{\insertperiod}{
\begin{table*}{
\centering
\begin{tabular}{l| llll}
\hline
\hline
direction &	no TP. & TP & 	$\Delta$ & 	W/L  \\
\hline
\enxx & 	39.32 &	\textbf{39.56} &	+0.24 &	0.77 \\
\xxen & 	48.54 &	\textbf{49.23} &	+0.69 &	1.0 \\

\hline
\end{tabular}

\caption{Comparing \chrf{} on versions of the evaluation sets with and without terminal punctuation (TP) on 26-language distilled models. The Win/Loss ratio is also reported, meaning the fraction of language pairs that saw an increase in \chrf{} by applying the terminal punctuation.  \label{tab:period}
%The average \chrf increases robustly, especially in the \xxen direction, where 100\% of the language pairs see a score increase.
% dev + test
}
}
\end{table*}
}

==> Next Thousand Languages/table_teacher_vs_student.tex <==


\newcommand{\inserteachervsstudentold}{
\begin{table*}[b]
% \small
\centering
\begin{tabular}{l|rrr}
LP & teacher & student & $\Delta$ \\
\hline
en$\rightarrow$doi & 37.2 & 41.3 & +4.1 \\
en$\rightarrow$ay & 31.6 & 34.5 & +2.9 \\
en$\rightarrow$gom & 40.8 & 42.9 & +2.1 \\
en$\rightarrow$sa & 31.5 & 33.4 & +1.9 \\
en$\rightarrow$bm & 35.0 & 36.4 & +1.4 \\
en$\rightarrow$ee & 39.8 & 41.1 & +1.3 \\
en$\rightarrow$ff & 36.3 & 37.4 & +1.1 \\
en$\rightarrow$ilo & 54.1 & 55.1 & +1.0 \\
en$\rightarrow$lus & 40.3 & 41.3 & +1.0 \\
en$\rightarrow$mai & 39.5 & 40.5 & +1.0 \\
en$\rightarrow$lg & 39.3 & 40.2 & +0.9 \\
en$\rightarrow$nso & 46.9 & 47.7 & +0.8 \\
en$\rightarrow$as & 39.9 & 40.7 & +0.7 \\
en$\rightarrow$dv & 45.0 & 45.6 & +0.6 \\
en$\rightarrow$ti & 21.5 & 22.1 & +0.6 \\
en$\rightarrow$ts & 46.7 & 46.6 & -0.1 \\
en$\rightarrow$om & 40.2 & 40.0 & -0.2 \\
en$\rightarrow$qu & 36.2 & 36.0 & -0.2 \\
en$\rightarrow$gn & 32.3 & 32.0 & -0.3 \\
en$\rightarrow$ak & 34.7 & 34.0 & -0.7 \\
en$\rightarrow$ln & 35.3 & 34.6 & -0.7 \\
en$\rightarrow$kri & 36.8 & 35.1 & -1.7 \\
\hdashline
mean & 38.2 & 39.0 & +0.8 \\
median & 38.3 & 40.1 & +0.9 \\
\end{tabular}
\caption{Performance of the distilled student model versus the teacher model, in \chrf{}.
 \label{tab:teacher_vs_student_old}}
\end{table*}
}



\newcommand{\inserteachervsstudent}{\begin{table}[t]	
\centering	
\begin{tabular}{lcccccccccc}	
\toprule	
 & \multicolumn{2}{c}{en-ff}  & \multicolumn{2}{c}{en-kri}  & \multicolumn{2}{c}{en-doi}  & \multicolumn{2}{c}{en-bm}  & \multicolumn{2}{c}{en-ay}  \\	
Mono Size          &\multicolumn{2}{c}{86k}   & \multicolumn{2}{c}{129k}   & \multicolumn{2}{c}{179k}   & \multicolumn{2}{c}{187k}   & \multicolumn{2}{c}{267k}   \\	
	
Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\	
\midrule	
Teacher &	
45.3 &	35.3 &
64.2 &	35.4 &
65.5 &	36.9 &
38.4 &	34.7 &
39.8 &	28.6 \\
Student &	
45.5 &	37.2 &
64.6 &	36.1&
65.7 &	40.5&
38.6 &	36.4&
40.1 &	34.2 \\
$\Delta$ &	
+0.2 &	+1.9 &
+0.4 &	+0.7 &
+0.2 &	+3.6 &
+0.2 &	+1.7 &
+0.4 &	+5.6 \\
\midrule	
\midrule	
	
 & \multicolumn{2}{c}{en-gom}  & \multicolumn{2}{c}{en-bho}  & \multicolumn{2}{c}{en-kl}  & \multicolumn{2}{c}{en-ee}  & \multicolumn{2}{c}{en-qu}  \\	
Mono Size          &\multicolumn{2}{c}{311k}   & \multicolumn{2}{c}{734k}   & \multicolumn{2}{c}{741k}   & \multicolumn{2}{c}{796k}   & \multicolumn{2}{c}{842k}   \\	
	
Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\	
\midrule	
Teacher &	
57.9 &	40.8 &  
60.9&	41.2&
39.0&	35.8 &
37.0 &	40.2 &
35.3 &	35.7 \\
Student &	
57.4 &	42 &
61.3 &	42.7&
39.5 &	41.0 &
37.5 &	40.7 &
35.1 &	36.1 \\
$\Delta$ &	
-0.4 &	+1.2 &
+0.4 &	+1.5 &
+0.5 &	+5.2 &
+0.5 &	+0.4 &
-0.1 &	+0.4 \\
	
\midrule	
\midrule	
 & \multicolumn{2}{c}{en-gn}  & \multicolumn{2}{c}{en-ak}  & \multicolumn{2}{c}{en-ts}  & \multicolumn{2}{c}{en-mai}  & \multicolumn{2}{c}{en-ln}  \\	
Mono Size          &\multicolumn{2}{c}{861k}   & \multicolumn{2}{c}{1.3m}   & \multicolumn{2}{c}{1.3m}   & \multicolumn{2}{c}{1.3m}   & \multicolumn{2}{c}{1.4m}   \\	
	
Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\	
\midrule	
	
Teacher &	
43.0 &	32.1 &
38.6 &	34.3 &
47.5 &	46.5 &
65.5 &	39.2 &
31.7 &	34.6 \\
Student &	
43.4 &	31.9 &
38.9 &	34.4 &
47.7 &	46.8 &
65.5 &	40.0 &
32.1 &	34.6 \\
$\Delta$ &	
+0.4 &	-0.2 &
+0.4 &	+0.1 &
+0.2 &	+0.3 &
0.0 &	+0.8 &
+0.4 &	0.0 \\
\midrule	
\midrule	
	
 & \multicolumn{2}{c}{en-nso}  & \multicolumn{2}{c}{en-lg}  & \multicolumn{2}{c}{en-ilo}  & \multicolumn{2}{c}{en-ti}  & \multicolumn{2}{c}{en-om}  \\	
Mono Size          &\multicolumn{2}{c}{1.9m}   & \multicolumn{2}{c}{2m}   & \multicolumn{2}{c}{2.6m}   & \multicolumn{2}{c}{3.9m}   & \multicolumn{2}{c}{5.6m}   \\	
	
Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\	
\midrule	
	
Teacher &	
52.5 &	47.1 &
40.5 &	39.3 &
62.7 &	54.1 &
46.1 &	21.5 &
40.7 &	40.0 \\
Student &	
52.8 &	48.2 &
41.0 &	39.8&
62.9 &	54.8&
46.0 &	21.9&
41.5 &	40.1 \\
$\Delta$ &	
+0.3 &	+1.1 &
+0.5 &	+0.5 &
+0.2 &	+0.8 &
0.0 &	+0.5 &
+0.8 &	+0.2 \\
\midrule	
\midrule	
 & \multicolumn{2}{c}{en-sa}  & \multicolumn{2}{c}{en-dv}  & \multicolumn{2}{c}{en-lus}  & \multicolumn{2}{c}{en-as}  & \multicolumn{2}{c}{en-ckb}  \\	
Mono Size          &\multicolumn{2}{c}{6.2m}   & \multicolumn{2}{c}{7.9m}   & \multicolumn{2}{c}{8.3m}   & \multicolumn{2}{c}{9.3m}   & \multicolumn{2}{c}{25.1m}   \\	
	
Direction       & $\leftarrow$ & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$  & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ & $\leftarrow$ & $\rightarrow$ \\	
\midrule	
	
Teacher &	
49.2 &	31.0 &
48.4 &	45.0 &
42.1 &	39.7 &
60.6 &	39.6 &
55.3&	42.6 \\
Student &	
49.2 &	33.3 &
48.4 &	45.3&
41.9 &	41.3&
61.1 &	40.3&
56.4 &	44.3 \\
$\Delta$ &	
0.0 &	+2.3 &
0.0 &	+0.3 &
-0.1 &	+1.6 &
+0.6 &	+0.7 &
+1.1 &	+1.7 \\
% \midrule	
% \midrule	
	
\bottomrule	
\end{tabular}	
\caption{Performance of teacher model versus student model in \chrf{}.}	
 \label{tab:teacher_vs_student}	
\end{table}	
}	

==> Next Thousand Languages/table_unmt_outtakes.tex <==



\begin{table*}
\centering
\begin{tabular}{l p{0.80\linewidth}}
\hline
\hline
sl & translation      \\
\hline
% source: মই ভাৱো, বিলাহীসমূহ শাক-পাঁচলি
as & I think carrots are \textbf{vegetables}. \\
% source: हमरा विचार से टमाटर एक सब्जी ह। 
bho & In my opinion, tomatoes are a \textbf{vegetable}. \\
% source: मिगी लगदा ऐ जे टमाटर इक सब्जी 
doi & I think tomatoes are a \textbf{vegetable}. \\
% source: އަހަރެން ދެކޭގޮތުގައި ޓޮމާޓޯ ތަރުކާރީއެކެވެ. \\
dv & I think tomatoes are a \textbf{vegetable}. \\
% source: तोमाट भाजी आसा अशें म्हाका 
gom & I think zucchini is a \textbf{vegetable}. \\
% source: Ti panagkunak ket dagiti kamatis ket maysa a nateng. \\
ilo & I think tomatoes are a \textbf{vegetable}. \\
% source: a tink se tamatis na vegetebul. \\
kri & I think tomatoes are \textbf{vegetables}. \\
% source: Tomato te hi thlai an nih ka ring. \\
lus & I believe tomatoes are \textbf{vegetables}. \\
% source: हमरा लागय छै की टमाटर एक तरकारी 
mai & I think tomatoes are a \textbf{vegetable}. \\
% source: Ke nagana gore ditamati ke merogo. \\
nso & I think tomatoes are \textbf{vegetables}. \\
% source: akka yaadakootti timatimin muduraadha \\
om & in my opinion tomatoes are \textbf{vegetables} \\
% source: I dey think say tomatoes na \textbf{vegetable}. \\
pcm & I think tomatoes are \textbf{vegetables}. \\
% source: TOmatikunaqa waq vegetalkunachuna \\
qu & TOmatoes are other \textbf{vegetables} \\
% source: ndzi ehleketa leswaku tamatisi i tsavu \\
ts & i think tomatoes are \textbf{vegetables} \\
% source: in wa'alike' le p'aako' ma' vegetali' \\
yua & i think the tomato is not a \textbf{vegetable} \\
% source: 我認為蕃茄係一種蔬菜。 \\
yue & I consider tomatoes a \textbf{vegetable}. \\
\hdashline
% source: Ne fɛ tomati ye jiriden kɛnɛye. \\
bm & For me tomatoes are healthy \textbf{fruits}. \\
% source: খামেন অশিনবশিং মনা-মশিং অমনি হায়বা 
mni & I think Khamen Ashin is a \textbf{fruit}. \\
% source: 546.रक्तफलं एकं फलमस्ति इति अहं चिन्तयाम
sa & 546. I think that the red \textbf{fruit} is a \textbf{fruit}. \\
\hdashline
% source: Tomatenakaxa jakasiphiwa machijayukaspawa. \\
ay & Tomatoes can be \textbf{drunk alive}. \\
% source: Mebu be tomatowo nye agblemenuku. \\
ee & I think tomatoes are a \textbf{crop}. \\
% source: Cikkumi tamaate ko legimaaji. \\
ff & I thought tomatoes were \textbf{legumes}. \\
% source: Che ha'e pe tomate ha'eha ka'a. \\
gn & I say the tomato is \textbf{coffee}. \\
% source: Uanga isumaqarpunga tomaatit naatitaasut. \\
kl & I think tomatoes are \textbf{seeds}. \\
% source: ኣነ ከምዝመስለኒ ኮሚደር ተክልታት እዮም። \\
ti & I think tomatoes are \textbf{plants}. \\
% source: Me gyedi sɛ ntoosi yɛ atosodeɛ. \\
ak & I believe that \textbf{toothpaste} is an \textbf{attack}. \\
\hline
\end{tabular}

\caption{Different languages disagree about whether a tomato is a fruit, vegetable, or something else.}
\label{tab:unmt_mistakes_fruit}
\end{table*}



\begin{table*}
\centering
\begin{tabular}{l p{0.80\linewidth}}
\hline
\hline
sl & translation      \\
\hline

% source: ahosuo mmiɛnsa a ɛdikan yɛ kɔkɔɔ, ankaa, ne akokɔsradeɛ. \\
ak & the first three colors are red, \textbf{blue}, and orange. \\
% source: এই প্ৰথম তিনিটা ৰং ৰঙা, কমলা আৰু হালধীয়া হয় | \\
as & These first three colors are red, orange and yellow. \\
% source: nayriri kimsa colorunakaxa wila, chupika, qillu \\
ay & the first three colors are red, \textbf{purple}, and yellow \\
% source: पहिला तीन रंग लाल, नारंगी आ पीयर बा। \\
bho & The first three colors are red, orange and yellow. \\
% source: kulɛri saba-fɔlɔ ye bilenman, neburu ani nɛrɛma ye. \\
bm & the three-primary colors are red, \textbf{negro}, and \textbf{black}. \\
% source: पैह्ले त्रै रंग लाल, संतरी ते पीले ऐ। \\
doi & The first three colors are red, orange and yellow. \\
% source: ފުރަތަމަ ތިން ކުލައަކީ ރަތާއި އޮރެންޖާއި ރީނދުލެވެ. \\
dv & The first three colors are red, orange and yellow. \\
% source: amadede gbãtɔwoe nye dzĩ, dzohẽ kple aŋutiɖiɖi. \\
ee & the primary colors are red, \textbf{purple} and \textbf{orange}. \\
% source: goobuuji tati gadani ko boɗeejo, oraans, e oolo. \\
ff & the first three colors are \textbf{white}, orange, and \textbf{green}. \\
% source: umi mbohapy sa'y kuéra hina ha'e pytã, pytã'yju ha sa'yju. \\
gn & the three colors are red, \textbf{purple} and \textbf{blue}. \\
% source: पयले तीन रंग तांबडे, नारंगी आनी हळदुवे आसात. \\
gom & The first three colors are red, orange and yellow. \\
% source: dagiti immuna a tallo a maris ket nalabbaga, dalandan, ken duyaw. \\
ilo & the first three colors are red, \textbf{dalandan}, and yellow. \\
% source: Qalipaatit siulliit pingasuupput aappaluttoq, orange aamma sungaartoq. \\
kl & The first three colors are blue, orange and \textbf{blue}. \\
% source: di fosn tri kolo dem na red, orinj, en yelo. \\
kri & the first three colors are red, orange, and yellow. \\
% source: Rawng pawimawh leh hmasa pathum te chu a sen, serthlum rawng leh a eng te an ni. \\
lus & The first three colors are red, \textbf{purple} and \textbf{bright}. \\
% source: पहिल तीन रंग ललका, नारंगी आर पीला छै| \\
mai & The first three colors are red, orange and yellow. \\
% source: অহানবা মচু অহুম অদুদি অঙাংবা, কোমলা মচু, অমসুং নাপু। \\
mni & The first three colors are red, \textbf{yellow}, and \textbf{blue}. \\
% source: Mebala ya mathome ye meraro ke khubedu, orentitše le sorolwana. \\
nso & The first three colors are red, orange and \textbf{purple}. \\
% source: Halluuwwan jalqabaa sadan kunninis:Diimaa,Burtukaana fi keellodha. \\
om & These three primary colors are:Red,Orange and yellow. \\
% source: the first three colors na red, orange, and yellow. \\
pcm & the first three colors are red, orange, and yellow. \\
% source: Ñawpaq kimsa llimpikuna puka, nina puka, q'illu.  \\
qu & The first three colors are red, \textbf{fire red}, and yellow. \\
% source: प्रथमवर्णत्रयम् रक्त- पित - केशरी च अस्ति । \\
sa & The first three colors are red, \textbf{yellow} and \textbf{saffron}. \\
% source: ኣቶም ናይ መጀምርያ ሰለስተ ቀለማት ቀይሕ፣ቡርቱካን ና ብጫ እዮም። \\
ti & Those first three colors are red,orange and yellow. \\
% source: mihlovo yi nharhu yo sungula i tshwuka, tshopi na xitshopana \\
ts & the first three colors are red, \textbf{purple} and \textbf{pink} \\
% source: la yáax boono'obo' chaktako'ob,chakk'aank'an yéetel k'aank'an. \\
yua & the first colors are red,\textbf{red} and yellow. \\
% source: 頭三隻顏色係紅色、橙色同黃色。 \\
yue & The first three colors are red, orange and yellow. \\

\hline
\end{tabular}

\caption{Translations from various languages for the sentence meaning "the first three colors are red, orange, and yellow." Note that some of these languages don't have words for all these colors, especially orange.}
\label{tab:unmt_mistakes_colors}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{l p{0.80\linewidth}}
\hline
\hline
sl & translation      \\
\hline
% source: daytoy ti makagapo no apay nga agbalin a maris dapo ti buok kas umad-adu ti edad. \\
ilo & this is the reason why \textbf{hair} turns \textbf{gray} as age increases. \\
% source: this na why hair dey change go grey color as person dey old. \\
pcm & this is why \textbf{hair} changes to \textbf{gray} color as a person ages. \\
% source: ምስ ዕድመ ፀጉሪ ናብ ስይበት ዝቅየረሉ ምክንያት እዚ እዩ። \\
ti & This is why \textbf{hair} turns to \textbf{gray} with age. \\
% source: le óolale u tso'otsel u pool máake' ku p'átal  grisi kée ch'íijik. \\
yua & therefore the \textbf{hair} turns \textbf{gray} as it gets older. \\

\hdashline

% source: wei ne deɛ nti a tirinwii dane nsonso wɔ mfeɛ bi akyiri. \\
ak & this is why \textbf{hair} turns \textbf{discolored} after a few years. \\
% source: এই কাৰণতে বয়স হোৱাৰ লগে লগে চুলি ধোঁৱা বৰণীয়া হৈ যায় | \\
as & This is why \textbf{hair} turns \textbf{smoky} with age. \\
% source: एही से उमिर बढ़ला के साथे केस सफेद होखे लागेला। \\
bho & This is why the \textbf{hair} starts to turn \textbf{white} with age. \\
% source: o dela kunsigi bin jɛ. \\
bm & so the \textbf{hair} fell \textbf{white}. \\
% source: އުމުރާއެކު އިސްތަށި ހުދު ކުލައަށް ބަދަލުވަނީ މިހެންވެގެންނެވެ. \\
dv & This is why \textbf{hair} turns \textbf{white} with age. \\
% source: ha upévare ñande akã rague morotĩ pe ñande tujavo. \\
gn & and therefore our \textbf{hair} grows \textbf{white} in old age. \\
% source: na dis mek iya de ton ashis kolo we posin ol. \\
kri & this is why \textbf{hair} turns \textbf{ash color} when old. \\
% source: Hevang hi alawm kan lo upat hnu hian sam a truah thin. \\
lus & This is why \textbf{hair loss} occurs when we grow old. \\
% source: यहां कारन छै की बाल उम्र के साथ सफेद भौ जाय छै | \\
mai & Here is the reason why \textbf{hair} turns \textbf{white} with age. \\
% source: মরম অসিননি চহী য়াম্লকপগা লোয়ননা শম উৎ মচু ওল্লক্লিবা। \\
mni & That is why the \textbf{hair} \textbf{changes color} with age. \\
% source: Ke ka lebaka leo moriri o fetoga go ba o mošweu ge motho a gola. \\
nso & That is why \textbf{hair} turns \textbf{white} with age. \\
% source: Rifeensi kanaaf umurii faana dalaachaaya. \\
om & The \textbf{hair} therefore becomes \textbf{dull} with age. \\
% source: Watakuna pasaqtin  chuqchaqa uqhi kutipun  \\
qu & Over the years, the \textbf{hair} turns \textbf{white} \\
% source: 211. अतः केशाः आयुः बर्धने शुभ्रवर्णाः भवन्ति। \\
sa & Therefore the \textbf{hair} becomes \textbf{white} with increasing age. \\
% source: hikwalaho ka leswi misisi yi hundzuka yo basa loko munhu a kula \\
ts & because \textbf{hair} turns \textbf{white} with age \\
% source: 呢個就係點解老咗頭髮會變白嘅原因。 \\
yue & This is why \textbf{hair} turns \textbf{white} with age. \\

\hdashline

% source: Ukatpi ñik´utax qaqptiwa sinti jiliri jaqisanxa \\
ay & Therefore the \textbf{hair} \textbf{falls out} in a very old person \\
% source: ऐह् बजह ऐ जे बाल बरेस दे कन्ने चिटटे होई जंदे ऐ। \\
doi & This is the reason why \textbf{hair} becomes \textbf{sticky} with age. \\
% source: esia tae woƒoa wɔ ne wotsi. \\
ee & that is why \textbf{they} beat \textbf{flour} when they grow up. \\
% source: ko ɗum tagi hoore ina ranwa e manggu. \\
ff & that is why the \textbf{head} is \textbf{ranked in the manger}. \\
% source: हाका लागून वय वाडटा तशें केंस पिकूंक लागतात. \\
gom & This causes \textbf{hair} to \textbf{grow out} with age. \\
% source: Taamaammat nutsakka ukiunnik qaqortikkaluttuinnarput. \\
kl & That’s why \textbf{my nuts} are getting \textbf{brighter} with age. \\
\hline
\end{tabular}

\caption{Translations from various languages for the sentence meaning "this is why hair turns grey with age."}
\label{tab:unmt_mistakes_hair}
\end{table*}




\begin{table}[!htb]
\footnotesize % \tiny \scriptsize \footnotesize \small
    \caption{Global caption}
    \begin{minipage}{.5\linewidth}
      \caption{}
      \centering
        \begin{tabular}{l p{0.85\linewidth}}
\hline
\hline
sl & translation      \\
\hline
yue & I believe \textbf{lions} are stronger than \textbf{tigers}. \\
bho & In my opinion, a \textbf{lion} is much stronger than a \textbf{tiger}. \\
bm & I believe that the \textbf{lion} is stronger than the \textbf{lion's mane}. \\
gom & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
ilo & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
kl & I think the \textbf{lion} is more violent than the \textbf{tiger}. \\
kri & I believe in forcing a \textbf{lion}'s throne rather than a \textbf{tiger}. \\
lus & I think the \textbf{lion} is stronger than the \textbf{tiger}. \\
mai & I believe that \textbf{lions} are stronger than \textbf{tigers}. \\
nso & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
pcm & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
qu & Is the \textbf{lion} stronger than the \textbf{tiger} \\\
sa & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
ti & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
ts & i believe the \textbf{lion} is stronger than the \textbf{tiger} \\
\hdashline
ak & I believe that a \textbf{lion} is stronger than a \textbf{leopard}. \\
dv & I believe a \textbf{lion} would be stronger than a \textbf{miniature crocodile}. \\
ee & I am convinced that a \textbf{lion} is stronger than a \textbf{wolf}. \\
gn & I believe that the \textbf{lion} is stronger than the \textbf{jackal}. \\
om & I believe that a \textbf{lion} is stronger than a \textbf{young man}. \\
\hdashline
ay & The true captain of the \textbf{liwuna} is still chacmani and the \textbf{tiger} is a cat. \\
\hdashline
doi & I believe that \textbf{seizures} are more severe than \textbf{epilepsy}. \\
ff & I think a \textbf{rabbit} is stronger than a \textbf{squirrel}. \\
mni & I believe a \textbf{snake} is stronger than a \textbf{crocodile}. \\
yua & it seems to me a \textbf{chakmo'ole} is more powerful than an \textbf{elephant} \\

\hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        \caption{}
        \begin{tabular}{lp{0.85\linewidth}}
\hline
\hline
sl & translation      \\
\hline\\
as & There are more \textbf{tigers} in the pen than there are \textbf{sharks}. \\
ilo & there are more \textbf{tigers} in captivity than \textbf{sharks}. \\
kri & more \textbf{tigers} have been captured than \textbf{sharks}. \\
lus & There are more \textbf{tigers} than \textbf{sharks}. \\
nso & There are more \textbf{tigers} to catch than \textbf{sharks}. \\
pcm & \textbf{tigers} caught out of the bush are more numerous than \textbf{sharks}. \\
ti & There are many more captured \textbf{tigers} than \textbf{sharks}. \\
yue & More stranded \textbf{tigers} than \textbf{sharks}. \\
\hdashline
ay & Many \textbf{otters} are closed and not \textbf{sharks} \\
bho & There are more \textbf{lions} in captivity than \textbf{sharks}. \\
doi & More \textbf{seals} are in captivity than \textbf{sharks}. \\ިނައެވެ. \\
dv & There are more \textbf{miniature crocodiles} in captivity than \textbf{sharks}. \\
mni & They catch more \textbf{cats} than \textbf{sharks}. \\
om & There are more \textbf{sharks} than \textbf{sharks}. \\
yua & more \textbf{red} prisoners than \textbf{sharks}. \\
\hdashline
gom & More \textbf{tigers} have been captured than \textbf{peacocks}. \\
kl & More \textbf{tigers} than \textbf{eagles} are in the wild. \\
mai & There were more \textbf{tigers} in captivity than \textbf{SAARC}. \\
sa & There are more \textbf{tigers} of captivity than \textbf{crocodiles}. \\
qu & There are more \textbf{tigers} in Ch'achana than in \textbf{Tinurunquna} \\
ts & \textbf{tigers} are more confined than \textbf{squirrels} \\
\hdashline
ak & more \textbf{deer} have been caught in caves than in \textbf{dense water}. \\
bm & I do catch more \textbf{lion cubs} than \textbf{raccoons}. \\
ee & some \textbf{sheep} are in prison more than \textbf{wolves}. \\
ff & \textbf{cewnguuji} is more common in \textbf{tiwaande} and rekee. \\
gn & there are more in the \textbf{jackal} pen than in the \textbf{fish}. \\
\hline
        \end{tabular}
    \end{minipage} 
    % % \caption{Translations of the sentence meaning "I believe that a lion is stronger than a tiger" from various languages into English. Those above the dashed line get these two nouns correct; those below substitute other animal names in.}
% % \label{tab:unmt_mistakes_lion}
\caption{Translations from various languages for the sentence meaning "there are more tigers in captivity than sharks." This sentence exhibited among the most errors of any that we looked at. Note that the translation sin to be similar is that from Tabor X, for instance with \textit{tigers} being translated as \textit{miniature crocodiles} from Dhivehi.}
\label{tab:unmt_mistakes_sharks}
\end{table}




% \begin{table}
% % \footnotesize % \tiny \scriptsize \footnotesize \small
% % \centering
% \begin{minipage}{.5\linewidth}
% \begin{tabular}{l  p{0.8\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline

% % source: 我相信獅子比老虎強壯。 \\
% yue & I believe \textbf{lions} are stronger than \textbf{tigers}. \\
% % source: हमार समझ में शेर, बाघ से बहुते ताकतवर होला। \\
% bho & In my opinion, a \textbf{lion} is much stronger than a \textbf{tiger}. \\
% % source: Ne dalenb'a la ko waraba barikalendo ni waraninkala ye. \\
% bm & I believe that the \textbf{lion} is stronger than the \textbf{lion's mane}. \\
% % source: शींव वाघापरस बळिश्ठ आसा असो म्हजो विस्वास आसा. \\
% gom & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: Mamatiak a ti maysa a leon ket napigpigsa ngem ti maysa a tigre. \\
% ilo & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: Isumaqarpunga løveq tigerimit nakuunerusoq. \\
% kl & I think the \textbf{lion} is more violent than the \textbf{tiger}. \\
% % source: a biliv fose layon tron pas tayga. \\
% kri & I believe in forcing a \textbf{lion}'s throne rather than a \textbf{tiger}. \\
% % source: Sakeibaknei hi sakei ai chuan a chawk zawk ka ring. \\
% lus & I think the \textbf{lion} is stronger than the \textbf{tiger}. \\
% % source: हमर मानब छै की शेर बाघ से बेसी मजबूत होए छै| \\
% mai & I believe that \textbf{lions} are stronger than \textbf{tigers}. \\
% % source: Ke dumela gore tau e tiile go feta nkwe. \\
% nso & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: I believe say lion strong pass tiger. \\
% pcm & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: Leonmataqa tigrechuñam astwan kallpayuk  \\
% qu & Is the \textbf{lion} stronger than the \textbf{tiger} \\
% % source: 506.एक व्याघ्रात् एक सिंह: शक्तिशाली अस्ति इति अहं विस्वसिमि। \\
% sa & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: ኣነ ኣንበሳ ካብ ነብሪ ከምዝጥንክር ያምን። \\
% ti & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: ndzi tshemba leswaku nghala yi tiyile ku tlula tiger \\
% ts & i believe the \textbf{lion} is stronger than the \textbf{tiger} \\
% \hdashline
% % source: Me gyedi sɛ gyata ho yɛ den sene ɔsebɔ. \\
% ak & I believe that a \textbf{lion} is stronger than a \textbf{leopard}. \\
% % % source: Chiq'as kapuniwa liwunaxa wali chacmani ukasti tigruxa phisichawa. \\
% % source: މިނިކާވަގަކަށްވުރެ ސިންގާއެއް މާ ވަރުގަދަވާނެކަމަށް އަހަރެން ޤަބޫލުކުރަމެވެ. \\
% dv & I believe a \textbf{lion} would be stronger than a \textbf{miniature crocodile}. \\
% % source: Meka ɖe edzi be ŋusẽ le dzata ŋu wu kpɔ̃. \\
% ee & I am convinced that a \textbf{lion} is stronger than a \textbf{wolf}. \\
% % source: Che aguerovia pe leõ imbareteveha pe jaguarete gui. \\
% gn & I believe that the \textbf{lion} is stronger than the \textbf{jackal}. \\
% % source: Nan amana leenci qeerrensarra cimaa ta'uu. \\
% om & I believe that a \textbf{lion} is stronger than a \textbf{young man}. \\
% \hdashline
% ay & The true captain of the \textbf{liwuna} is still chacmani and the \textbf{tiger} is a cat. \\
% \hdashline
% % source: मेरा मानना ऐ जे सीह् मिरग थमां जादा जोरदार हुंदा ऐ। \\
% doi & I believe that \textbf{seizures} are more severe than \textbf{epilepsy}. \\
% % source: Cikkumi mbaroodi ɓuri heewde doole e cewngu. \\
% ff & I think a \textbf{rabbit} is stronger than a \textbf{squirrel}. \\
% % source: নোংশা অমনা কৈ অমদগী হেন্না মপাঙ্গল কল্লি হায়বা ঐহাক থাজৈ। \\
% mni & I believe a \textbf{snake} is stronger than a \textbf{crocodile}. \\
% % source: bey tin wóol juntúul chakmo'ole' maas ya'ab u muuk' kéet juntúul baalamo' \\
% yua & it seems to me a \textbf{chakmo'ole} is more powerful than an \textbf{elephant} \\

% \hline
% \end{tabular}
% \end{minipage}

% % \end{table*}


% % \begin{table*}
% % \small
% % \centering
% \begin{minipage}{.5\linewidth}
% \begin{tabular}{l p{0.45\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline

% % source: ইয়াত চাৰ্ক যিমান আছে তাতকৈ অধিক গৰালৰ ভিতৰত বাঘ আছে | \\
% as & There are more \textbf{tigers} in the pen than there are \textbf{sharks}. \\
% % source: ad-adu ti tigre a nakabalod ngem pating. \\
% ilo & there are more \textbf{tigers} in captivity than \textbf{sharks}. \\
% % source: dem don kapcho boku tayga dem pas shak. \\
% kri & more \textbf{tigers} have been captured than \textbf{sharks}. \\
% % source: Sangha liantak, shark aiin sakei khungbeh an tam zawk. \\
% lus & There are more \textbf{tigers} than \textbf{sharks}. \\
% % source: Go na le dinkwe tše dintši tšeo di ka swerwego go feta dishaka. \\
% nso & There are more \textbf{tigers} to catch than \textbf{sharks}. \\
% % source: tigers wey dem catch comot from bush plenty pass sharks. \\
% pcm & \textbf{tigers} caught out of the bush are more numerous than \textbf{sharks}. \\
% % source: ካብ ሻርክ ብዝበለጸ ቡዙሓት ዝተማረኩ ነብሪ ኣለዉ። \\
% ti & There are many more captured \textbf{tigers} than \textbf{sharks}. \\
% % source: 比人困住嘅老虎比鯊魚多。 \\
% yue & More stranded \textbf{tigers} than \textbf{sharks}. \\
% \hdashline
% % source: Walja uturunkunakawa jist´antata janirakiwa tiburones \\
% ay & Many \textbf{otters} are closed and not \textbf{sharks} \\
% % source: शार्क के तुलना में ढेर शेर कैद में बा। \\
% bho & There are more \textbf{lions} in captivity than \textbf{sharks}. \\
% % source: शार्क दी तुलना च मते सीह् कैद च ऐ। \\
% doi & More \textbf{seals} are in captivity than \textbf{sharks}. \\
% % source: މިޔަރަށްވުރެ ގިނައިން މިނިކާވަގު ބަންދުކޮށްފައިވާ މިންވަރު މާގިނައެވެ. \\
% dv & There are more \textbf{miniature crocodiles} in captivity than \textbf{sharks}. \\
% % source: শার্কশিংদগী কৈশিংনা হেন্না ফারগা থম্মি। \\
% mni & They catch more \textbf{cats} than \textbf{sharks}. \\
% % source: Qurxummii shaarkii caalaa qeerransootatuu baaji'amee argama. \\
% om & There are more \textbf{sharks} than \textbf{sharks}. \\
% % source: más ya'an chakmo'ol k'ala'ano'ob kéen tiburoono'ob. \\
% yua & more \textbf{red} prisoners than \textbf{sharks}. \\
% \hdashline
% % source: मोरयां परस चड वाघांक धरल्यात. \\
% gom & More \textbf{tigers} have been captured than \textbf{peacocks}. \\
% % source: Eqalussuarniit tigerit amerlanerit uumasuusivissuarniipput. \\
% kl & More \textbf{tigers} than \textbf{eagles} are in the wild. \\
% % source: कैद में सार्क से बेसी बाघ रहै | \\
% mai & There were more \textbf{tigers} in captivity than \textbf{SAARC}. \\
% % source: 283. तत्र अधिकांशाः बन्धनस्य व्याघ्राः सन्ति ग्राहस्य तुलनात्। \\
% sa & There are more \textbf{tigers} of captivity than \textbf{crocodiles}. \\
% % source: Ch'achanapiqa kanmi astawan tigrikuna tinurunqunamantaqa \\
% qu & There are more \textbf{tigers} in Ch'achana than in \textbf{Tinurunquna} \\
% % source: ti tiger ti pfaleriwile ku tlula tinyakwave \\
% ts & \textbf{tigers} are more confined than \textbf{squirrels} \\
% \hdashline
% % source: wɔakyere asebɔ bebree agugu buo mu kyɛn densu. \\
% ak & more \textbf{deer} have been caught in caves than in \textbf{dense water}. \\
% % source: waraninkalan camanw minɛ ne do ka tɛmɛ rekɛnw ka. \\
% bm & I do catch more \textbf{lion cubs} than \textbf{raccoons}. \\
% % source: kpɔ̃ ɖewo le gakpɔ me wu agblɔwo. \\
% ee & some \textbf{sheep} are in prison more than \textbf{wolves}. \\
% % source: ko cewnguuji ɓuri heewde e tiwaande e rekeeji. \\
% ff & \textbf{cewnguuji} is more common in \textbf{tiwaande} and rekee. \\
% % source: hetave oĩ jaguarete kuéra korápe upe pirarotogui. \\
% gn & there are more in the \textbf{jackal} pen than in the \textbf{fish}. \\
% \hline
% \end{tabular}
% \end{minipage}


% % \caption{Translations of the sentence meaning "I believe that a lion is stronger than a tiger" from various languages into English. Those above the dashed line get these two nouns correct; those below substitute other animal names in.}
% % \label{tab:unmt_mistakes_lion}
% \caption{Translations from various languages for the sentence meaning "there are more tigers in captivity than sharks." This sentence exhibited among the most errors of any that we looked at. Note that the translation sin to be similar is that from Tabor X, for instance with \textit{tigers} being translated as \textit{miniature crocodiles} from Dhivehi.}
% \label{tab:unmt_mistakes_sharks}
% \end{table}





% \begin{table*}
% \centering
% \begin{tabular}{l p{0.40\linewidth} p{0.40\linewidth} l}
% \hline
% \hline
% sl & source & translation & correct word     \\
% \hline
% kl & Taamaammat \textbf{nutsakka} ukiunnik qaqortikkaluttuinnarput. & That’s why my \textbf{nuts} are getting brighter with age. & \textbf{hair} \\
% kl & Zebrat qaqortuupput qernertunik \textbf{titarnillit}. & Zebras are white with green \textbf{tits}. & \textbf{stripes} \\
% kl & Uummatinga \textbf{assanniippoq}. & My heart is in my \textbf{ass}. & \textbf{sleeve} \\
% \hline
% \end{tabular}

% \caption{examples of the model trying to guess an unknown noun based on textual similarity to the English.}
% \label{tab:unmt_mistakes_stripes}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline
% % source: Wɔ wei mu no, mede “capsicum”, ntoosi, gyeene, galik, “green chillies”, “olivies” ne ade na mamfa “cheese” ne sradeɛ anka ho. \\
% ak & In this, I added “capsicum”, onions, ginger, garlic, “green chillies”, “olivies” and stuff and didn’t add “cheese” and fat. \\
% % source: ইয়াত মই কেপছিকাম, বিলাহী, পিয়াঁজ, নহৰু, কেঁচা জলকীয়া, জলফাই আদি ব্যৱহাৰ কৰোঁ আৰু ইয়াত পনীৰ আৰু মাখন ব্যৱহাৰ নকৰোঁ। \\
% as & Here I use capsicum, \textbf{celery}, onion, garlic, raw pepper, olives, etc. and do not use cheese and butter. \\
% % source: akanja usktwa pimiento, cebolla, ajo, chojjña wayk´a, asiytuna yakhanakampi, janiw akan uskti qisumpi mantiqillampi  \\
% ay & here I put pepper, onion, garlic, chojjña wayk ́a, asiytuna with others, I didn ́t put here the onion and butter \\
% % source: एह में हम शिमला मिर्च, टमाटर, प्याज, लहसुन, हरियर मरिचा, ओलिव वगैरह इस्तेमाल करेलीं, लेकिन पनीर व मक्खन इस्तेमाल ना करेलीं। \\
% bho & I use capsicum, tomatoes, onions, garlic, green chillies, olives, etc., but I don't use cheese and butter. \\
% % source: Nin na, ne bɛ baara kɛ ni tomatiw, jabaw, layiw, foronto binkɛnɛ, olivuw n'u ɲɔgɔnaw de ye, n'tɛ cizi ni bɛɛri k'a la. \\
% bm & Here, I use tomatoes, \textbf{lettuce}, garlic, spring greens, olives and the like, not \textbf{cider vinegar} and \textbf{berries}. \\
% % source: इसदे च आऊं शमला मर्च, टमाटर, गंढा, थोम, सैली मर्च, जैतन ते होर दा बरतून करना ऐ ते इसदे च पनीर ते मक्खन दा बरतून नई करदा। \\
% doi & I use shallot peppers, tomatoes, garlic, \textbf{thyme}, salt peppers, olives and others and I don’t use cheese or butter. \\
% % source: މީގައި އަހަރެން ބޭނުންކުރީ ކެޕްސިކަމް، ޓޮމާޓޯ، ފިޔަޔާއި، ލޮނުމެދާއި، ފެހިމިރުހާއި، ޒައިތޫނި، މިފަދައެއްޗިއްސެވެ. އަދި އެޔަށް ޗީޒް އާއި ބަޓަރ ބޭނުންނުކުރަމެވެ. \\
% dv & I used capsicum, tomatoes, onions, \textbf{salt}, green peppers, olives, etc. And I didn't use cheese or butter. \\
% % source: Le esia me la, mezãa atadi, tomato, sabala, ayo, "chiles" gbogbo, "olive", kpbb. Eye nyemezãa kesu kple bɔta le eme o. \\
% ee & In this, I use peppers, tomatoes, \textbf{lettuce}, ayo, lots of "chiles", "olive", etc. And I don't use cheese and butter in it. \\
% % source: E ɗum mbiɗa huutoro kapsiyom, tamaate, basalle, laaÿ, siliiji werte, olivaaji, egɗ kadi mi huutortaako formaas kadi mi waɗata heen boor. \\
% ff & And I say use capsicum, tomatoes, \textbf{basil}, \textbf{lettuce}, green chilies, olives, etc. And I don’t use \textbf{formaldehyde} and I \textbf{make a bowl of it}. \\
% % source: Peape che aipuru ky'ỹi, tomate, sevoi, ajo, ky'ỹi hovy ha aceituna, ha ndaipurúi kesu tera kambyrova ipype. \\
% gn & Here I use onions, tomatoes, \textbf{sevoi}, garlic, green onions and olives, and I don't use cheese or \textbf{milk} in it. \\
% % source: हातूंत हांव ढब्बु मिरसांग, तोमाटां, कांदे, लसूण, हरव्यो मिरसांगो, ऑलिव्ह इत्यादी वापरता आनी चिज आनी बटर तातूंत घालिना. \\
% gom & I use dubbed chillies, tomatoes, onions, garlic, green chillies, olives, etc. and do not add cheese and butter. \\
% % source: Nangusarak ditoy iti sili, kamatis, sibuyas, bawang, berde a sili, olibo, ken dadduma pay ken saankayo a mangusar iti keso ken mantikilya ditoy. \\
% ilo & I used peppers, tomatoes, onions, garlic, green peppers, olives, etc. here and you do not use cheese and butter here. \\
% % source: Uani akoraakka paprikkat, tomatit, uanitsut, hvidløgit, chilit qorsorpaluttut olivennit il. il. punnilinngilakka immussualernangillu. \\
% kl & Here I am mixing peppers, tomatoes, onions, garlic, chilies, green olives, etc. I am not \textbf{punching} or \textbf{immussual}. \\
% % source: pa dis a yus pepe, tamatis, yabas, galik, grin chilis, oliv dem, etc. en no yus chis en bota de. \\
% kri & on this I use peppers, tomatoes, \textbf{yabas}, garlic, green chilies, olives, etc. and don't use cheese and butter there. \\
% % source: Hemi atan hi chuan capsicum, tomato, purun sen, purun var, hmarcha hring, leh olive te ka hmang a, mahse butter leh cheese ka hmang tello. \\
% lus & I used capsicum, tomatoes, red onion, \textbf{white onion}, green chilies, and olives, but I didn't use butter or cheese. \\
% % source: एकरा में शिमला मिर्च, टमाटर, प्याज, लहसुन, हरी मिर्च, जैतून इ सब के प्रयोग करै छिये आर एकरा में पनीर आर मखहनके उपयोग नै करे छिये | \\
% mai & It uses capsicum, tomatoes, onion, garlic, green chillies, olives and does not use cheese and butter. \\
% % source: মসিদা ঐহাক কেপ্সিকম, খামেন অশিনবশিং, তিলহৌশিং, চনম, মোরোক অতেকপশিং, চোরফোনশিং, অসিনচিংবা শিজিন্নৈ অমসুং মদুদা ঘীথী অমসুং মখন শিজিন্নদে। \\
% mni & In this I use capsicum, \textbf{khamen ashinbas}, \textbf{sesame seeds}, \textbf{chanam}, \textbf{morocco atakpas}, \textbf{chorfon}, etc. and do not use \textbf{ghee} and butter. \\
% % source: Ka gare ga se ke šomiša capsicum, tomati, eie, kaliki, pherefere ye tala, olifi bjalo le bjolo ebile ga ke šomiše tšhese le potoro ka gare. \\
% nso & In this I use capsicum, tomato, onion, garlic, green pepper, olives and so on and I don't use cheese and butter in it. \\
% % source: Kan keessatti qaaraa, timaatimii,qullubbii,baala zayitaa fikkf fayyadama.dabalataniis baaduu fi dhadhaa hin fayyadamu. \\
% om & In which he uses \textbf{curry}, tomatoes, \textbf{coconut}, olive \textbf{oil} etc. plus he does not use \textbf{bacon} and butter. \\
% % source: For this one, I use capsicum, tomatoes, onions, garlic, green pepper, olives, etc. and I no dey use cheese and butter for inside. \\
% pcm & For this one, I use capsicum, tomatoes, onions, garlic, green pepper, olives, etc. and I don’t use cheese and butter in it. \\
% % source: Kaypiqa curasun pimiento, tomates, cebollas, ajo, chiles verdes, aceitunas, etc. ichaqa manan churasunchu quesutpas nipas matequillata. \\
% qu & Here we will cure peppers, tomatoes, onions, garlic, green chilies, olives, etc. but we will not add cheese or \textbf{matequilla}. \\
% % source: अत्र अहं महामरीचिका,रक्तफलं,पलाण्डुः,लशुनं,हरीमरीचिका,जितवृक्ष इत्यादयः व्यवहारं करोमि अपि च दधिक एवं नवनीतम् अत्र व्यवहारं न करोमि। \\
% sa & Here I deal with great pepper, \textbf{red fruit}, \textbf{eggplant}, garlic, green pepper, olive \textbf{tree} etc. and I don't deal with yogurt and \textbf{fresh} here. \\
% % source: ኣብዚ ከም ካፕሲካም፥ ኮመደረ፥ ሽንጉርቲ፥ ጻዕዳ ሽንጉርቲ፥ ግሪንችሊ፥ፍረ ወይራ ወዘተ ይጥቀም። ኣጅቦን ጠስምን ከይትጥቀም። \\
% ti & Use ingredients like capsicum, tomato, \textbf{mushroom}, w\textbf{hite mushroom}, \textbf{grinchly}, \textbf{grapefruit} etc. Do not use \textbf{ajbon} and \textbf{sour cream}. \\
% % source: Eka leswi ndzi tirhisile capsium, matamatisi, tinyala, xinyalani, viriviri ra rihlaza, ntlhwari na swo fana na swonaa. naswona unga tirhisi chizi na botere u nga swi tirhisi \\
% ts & For this I used \textbf{capsium}, tomatoes, \textbf{lettuce}, \textbf{lentils}, green chilies, olives and the like.and don't use cheese and butter don't use them \\
% % source: te' je'ela' ku meyajten xa'ak', p'aak,cebolla,ajo, ya'ax iik,aceitunas,etc,ma' tu meyajten queso mix mantequilla. \\
% yua & here i use \textbf{mixture}, tomato,onion,garlic, \textbf{green beans},olives,etc,no cheese or butter. \\
% % source: 我加咗甜椒、蕃茄、洋蔥、大蒜、綠辣椒同橄欖等等，冇用到芝士同牛油。 \\
% yue & I added bell peppers, tomatoes, onions, garlic, green peppers and olives, etc., no cheese and butter. \\

% \hline
% \end{tabular}

% \caption{Translations of the sentence meaning "In this I use capsicum, tomatoes, onions, garlic, green chilies, olives, etc. and do not use cheese and butter in it." from various languages into English.}
% \label{tab:unmt_mistakes_capsicum}
% \end{table*}


% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline
% % source: Mepɛ sɛ meyɛ aboa kraman dakoro pɛ. \\
% ak & I want to be an animal dog for one day. \\
% % source: এদিনৰ বাবে মই কুকুৰ হ’ব বিচাৰো | \\
% as & I want to be a dog for one day. \\
% % source: Mallitua ma urupacha anuña  \\
% ay & Mallitua is a day dog \\
% % source: हम एक दिन खातिर कुत्ता बने के चाहत बाटीं। \\
% bho & I want to be a dog for a day. \\
% % source: A tun bɛ diya ne ye ka kɛ wulu he tile kelen. \\
% bm & I would love to be a dog he day. \\
% % source: आऊं इक ध्याड़े दे लेई कुत्ता बनना चैहंग। \\
% doi & I want to be a dog for a day. \\
% % source: އަހަރެން އެއްދުވަހަށް ކުއްތާއަކަށް ވާންބޭނުމެވެ. \\
% dv & I want to be a dog for a day. \\
% % source: Madi be manye avu ŋkeke ɖeka ko. \\
% ee & I would like to be a dog for just one day. \\
% % source: Aikosetene pe jaguarõ peteĩ ára pe. \\
% gn & I want to be the dog one day. \\
% % source: म्हाका एका दिसाखातीर कुत्रो जावचें आसा. \\
% gom & I want to be a dog for a day. \\
% % source: Kayatko ti agbalin nga aso iti maysa nga aldaw. \\
% ilo & I want to be a dog one day. \\
% % source: Ulloq ataaseq qimmiorusussinnaavunga. \\
% kl & I might want to be a dog one day. \\
% % source: a go want fo bi dog fo wan de. \\
% kri & I'd want to be a dog for a day. \\
% % source: Ni khat atan ui nih chhin ka chak. \\
% lus & I want to be a dog for a day. \\
% % source: होम एक दिन ले कुकुर बनब चाहिबै| \\
% mai & Home wants to be a dog for a day. \\
% % source: Nka rata go ba mpša letšatši le tee fela. \\
% nso & I would like to be a dog for just one day. \\
% % source: Guyyaa tokkof sareen ta'uu barbaada. \\
% om & I want to be a dog for a day. \\
% % source: I go like to be dog for 1 day. \\
% pcm & I would like to be a dog for 1 day. \\
% % source: Huk punchawllas allquman kutiyta munayman  \\
% qu & I wish I could go back to the dog one day \\
% % source: ንሓደ መዓልቲ ከልቢ ምኻን ይደሊ እየ። \\
% ti & I want to be a dog for a day. \\
% % source: ndzi nga lava ku va mbyana siku rin'we \\
% ts & i would like to be a dog one day \\
% % source: ust tin t'aan ka peek'aken jump'éel k'iin. \\
% yua & ust I liked it when I was a dog one day. \\
% % source: 我都想做一日狗仔。 \\
% yue & I want to be a day dog. \\
% \hdashline
% % source: Mbiɗa yiɗatno wonnde rawaandu fodde ñalawma gooto. \\
% ff & I would like to be a \textbf{raven} for a day. \\
% % source: ঐহাক নুমিৎ অমগী ওইনা হুই অমা ওইবা পাম্মি। \\
% mni & I want to be a \textbf{horse} for a \textbf{week}. \\
% % source: 595.अहं एकस्मिन् दिवसस्य कृते कुक्कुरः भवितुं इच्छामि। \\
% sa & I want to be a \textbf{puppy} for a day. \\
% \hline
% \end{tabular}

% \caption{Translations of the sentence meaning "I would want to be a dog for a day" from various languages into English.}
% \label{tab:unmt_mistakes_dogday}
% \end{table*}




% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline
% % source: Mɛbisa me kra no nsɛm bi fa nea ɔpɛsɛ ɔka kyerɛ no nti a dabiara ɔsu meaaw no. \\
% ak & I will ask my \textbf{soul} some questions about what she wants to tell her why every day she cries meaaw. \\
% % source: মই মোৰ মেকুৰীজনীক কিছুমান প্ৰশ্ন সুধিব বিচাৰো যে, সি মিয়াউৰ দ্বাৰা সদায় কি কৈ থাকিব খোঁজে | \\
% as & I want to ask my cat some questions about what he always wants to say by meow. \\
% % source: Nayaxa jist'asiristwa phisitujaruxa kunsañaj manpachituxa mararaw sasinxa \\
% ay & I would ask my cat what he wanted me \textbf{to do in the year} \\
% % source: हम आपन बिलाई से कुछ सवाल पूछे के चाहत बानी के ऊ हमेशा मियाऊँ करके हमरा से का कहे के कोशिश करेले। \\
% bho & I want to ask my cat a few questions about what he always tries to tell me by meowing. \\
% % source: Nbi na n'ka jakuma ɲininka a b'a fɛ ka min fɔ n'a ka ŋɛwu ye. \\
% bm & Nbi will ask my \textbf{jackal} what he means with his \textbf{scythe}. \\
% % source: आऊं अपनी बिल्ली थमां किश सोआल पूछगा जे ओह् म्हेशा मिआउ करिए कैह् आक्खने दी कोशश करदी ऐ। \\
% doi & I’ll ask my cat a few questions about what she’s always trying to say by meowing. \\
% % source: އަހަރެންގެ ބުޅާ މިއާއުކުރަމުން ބުނަންއުޅެނީ ކީކޭތޯ ދެނެގަތުމަށްޓަކައި ސުވާލުތަކެއް ކުރަމެވެ. \\
% dv & I ask questions to find out what my \textbf{dog} is saying. \\
% % source: Mabia nya aɖewo ku ɖe nu si wòdina be yeagblɔ hafi nɔ xɔxlɔ̃m ɣe sia ɣi ŋu. \\
% ee & I would ask some questions about what he meant before he was always hanging out. \\
% % source: Ma mi naamdo ulluundu am yoga e naamde batte hol ko o heewi etaade wiide mi e ŋeewaali \\
% ff & I will ask my \textbf{ulcer} some of the questions behind what he often tries to tell me \textbf{in a smile} \\
% % source: Che aporanduse che mbarakajape umi ñeporandu mba'epa ha'e he'ise chupe pe imbarakajarasẽpe. \\
% gn & I want to ask my \textbf{dog} questions about what he means to him \textbf{in his music}. \\
% % source: म्हाका म्हज्या माजराक कांय प्रस्न विचारचे आसात ते म्हणल्यार सद्दां मियाँव म्हूण तें म्हाका किदें सांगूक सोदता. \\
% gom & I want to ask my cat some questions about what he means to me by always being a meow. \\
% % source: Saludsudek ti pusak maipapan iti banag a kanayon a kayatna nga ibaga kenkuana babaen iti panagmeow. \\
% ilo & I ask my cat about something she always wants to tell her by meowing. \\
% % source: Qitsuutinga apeqqutinik apeqquteqarfigerusussinnaavara miaarveertuinnaleraangami suna oqaatigerusuttaraluarneraa. \\
% kl & I would like to ask my \textbf{husband} questions about what he meant when he was in the \textbf{miaarveer}. \\
% % source: a go aks mi pus bot wetin in bin de tray fo tel am wit in miowin. \\
% kri & I'll ask my cat about what he was trying to tell her with his \textbf{miowin}. \\
% % source: Ka zawhte hi a ngiau chang apianga a sawitum hi ka zawt thin. \\
% lus & I ask him what he means whenever he asks me. \\
% % source: होम आपन बिलाई से किछो सवाल पुछ्बैं की ओ हरदम हमरा मियांउ करके की बताबय के कोशिश कराइ छै| \\
% mai & Home ask your cat some questions about what he is always trying to tell me by meowing. \\
% % source: মিয়াও খোংলগা মহাক্না মঙোন্দা মতম চুপ্পদা করিগী মরমদা হায়নবা হোৎনরিবনো হায়না ঐহাক ঐহাক্কি হৌদোংদা ৱাহং খরা হংগনি। \\
% mni & I will ask \textbf{myself} a few questions about what he is always trying to tell me. \\
% % source: Ke tla botšiša katse yaka dipotšišo ka ga seo ka mehla e lekago go mmotša sona ka go lla. \\
% nso & I will ask my cat questions about what it always tries to tell her by \textbf{crying}. \\
% % source: Adurre koo hasofsiisu nan barbaada kan isheen yeroo hunda na sagalessitu maal akka jedhuu barbaadde. \\
% om & I want to talk to my \textbf{dog} about what she always wants to say when she \textbf{calls me}. \\
% % source: I go ask my cat question about wetin he dey always dey try to tell me when e dey meow. \\
% pcm & I will ask my cat a question about what he is always trying to tell me when he meows. \\
% % source: Misiyta tapuyta munayman imarayku ch'aqwan ima niwaytataq munan \\
% qu & I would like to ask my cat why he is \textbf{fighting} and what he means \\
% % source: 513.अहं मम मार्जारं केचित् प्रश्ना: पृच्छामि यत् स: सर्वदा मियाऊ मियाँऊ उक्त्वा किं वक्तुम् इच्छति। \\
% sa & I ask my cat some questions about what he always means when he says meow meow. \\
% % source: ናተይ ድሙ ኩሉግዜ ብክእለት ንዕኡ ንምንጋር ዝሙክሮ ነገር ሓደሓደ ጥያቀታት ይጥይቅ። \\
% ti & My cat always asks some questions about what I'm trying to tell him \textbf{skillfully}. \\
% % source: ndzi nga vutisa ximanga xa mina swivutiso swa leswaku xi ringeta ku vula ku yini loko xi ku meow \\
% ts & i can ask my cat questions about what he is trying to say when he meows at you \\
% % source: jéel in meyajtik wa jayp'éel k'áatchi' ti' in walak' miis yóosal le ba'ax u k'áat u ya'al chen jo'ok u t'aano'.  \\
% yua & I'll use a few questions on my cat about what he just started talking about. \\
% % source: 我會問我隻貓到底佢啲喵喵聲係想表達啲咩。 \\
% yue & I would ask my cat what his meows meant. \\

% \hline
% \end{tabular}

% \caption{....}
% \label{tab:unmt_mistakes_meow}
% \end{table*}



% mkdir /tmp/unmt

% copy TEST
%  for f in ` fu ls /cns/vz-d/home/translate-train/nmt_train/m4-ntl/data/ntl_eval_sets/rkv/decoded/aqtxl_glompitqafkkbdmanagedbystscy_en_fg3fm3mb4_spm_20211209-1657_productionized_00590000/*_m4_ntl_eval_set-test_rkv/output.rkv ` ; do lp=$(dirname $f | bsnm | sed 's/_m4.*//g'); echo $lp ; fu cp $f /tmp/unmt/${lp}_test.rkv; done

% copy DEV
%  for f in ` fu ls /cns/vz-d/home/translate-train/nmt_train/m4-ntl/data/ntl_eval_sets/rkv/decoded/aqtxl_glompitqafkkbdmanagedbystscy_en_fg3fm3mb4_spm_20211209-1657_productionized_00590000/*_m4_ntl_eval_set-dev_rkv/output.rkv ` ; do lp=$(dirname $f | bsnm | sed 's/_m4.*//g'); echo $lp ; fu cp $f /tmp/unmt/${lp}_dev.rkv; done

% function table_with_src () { ref="$1"; for f in `ls /tmp/unmt/*` ; do cat $f | sed "s/[a-z]\+=//g" | grep "$ref" | awk -v FS="\t" '{printf "%s & %s & %s \\\\\n\\hdashline\n", $4, $2, $1}'; done; }
% 
% function table_only_output () { ref="$1"; for f in `ls /tmp/unmt/*` ; do cat $f | sed "s/[a-z]\+=//g" | grep "$ref" | awk -v FS="\t" '{printf "%% source: %s \\\\\n%s & %s \\\\\n", $2, $4, $1}'; done; }


% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline

% \hline
% \end{tabular}

% \caption{....}
% \label{tab:unmt_mistakes_lion}
% \end{table*}




==> Next Thousand Languages/table_unmterrors_main.tex <==
\newcommand{\insertunmterrorsmain}{
\begin{table*}
\centering
% \scriptsize
\fontsize{7.0pt}{9pt}\selectfont
\begin{tabular}{l| p{0.45\linewidth}  p{0.45\linewidth}}
\hline
\hline
sl    & reference     & translation \\
\hline
ak & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & 
I think the \mistake{hyena}'s \mistake{hotter} than the \mistake{elephant}. \\
% \hdashline
dv & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}.& I believe a \correct{lion} would be \correct{stronger} than a \mistake{miniature crocodile}. \\
% \hdashline
% source: নোংশা অমনা কৈ অমদগী হেন্না মপাঙ্গল কল্লি হায়বা ঐহাক থাজৈ। \\
mni & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}.& I believe a \mistake{snake} is \correct{stronger} than a \mistake{crocodile}. \\
% \hdashline
% source: मेरा मानना ऐ जे सीह् मिरग थमां जादा जोरदार हुंदा ऐ। \\
doi & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & I believe \mistake{seizures} are \correct{more severe} than \mistake{epilepsy}. \\
% \hdashline
% source: Cikkumi mbaroodi ɓuri heewde doole e cewngu. \\
ff & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & I think a \mistake{rabbit} is \correct{stronger} than a \mistake{squirrel}. \\
\hline
% source: অহানবা মচু অহুম অদুদি অঙাংবা, কোমলা মচু, অমসুং নাপু। \\
mni & The first three colors are \textbf{red}, \textbf{orange},and \textbf{yellow}. & The first three colors are \correct{red}, \mistake{yellow}, and \mistake{blue}. \\
% \hdashline

% source: Ñawpaq kimsa llimpikuna puka, nina puka, q'illu.  \\
qu &  The first three colors are \textbf{red}, \textbf{orange},and \textbf{yellow}. &The first three colors are \correct{red}, \mistake{fire red}, and \correct{yellow}. \\
% \hdashline
% source: प्रथमवर्णत्रयम् रक्त- पित - केशरी च अस्ति ।
sa &  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & The first three colors are \correct{red}, \mistake{yellow} and \mistake{saffron}. \\
% \hdashline

% source: mihlovo yi nharhu yo sungula i tshwuka, tshopi na xitshopana \\
ts &  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & the first three colors are \correct{red}, \mistake{purple} and \mistake{pink} \\
% \hdashline
% source: la yáax boono'obo' chaktako'ob,chakk'aank'an yéetel k'aank'an. \\
yua &  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & the first colors are \correct{red}, \mistake{red} and \correct{yellow}. \\
\hline
sa & In this I use \textbf{capsicum, tomatoes, onions, garlic, green chilies, olives}, etc. and do not use \textbf{cheese} and \textbf{butter} in it.  & Here I deal with \mistake{ greater marjoram, blood fruit, plantain, lassi, green marjoram, jujube}, etc., but I do not deal with \mistake{curd} and \mistake{yogurt}. \\

% \hdashline
\hline

ak & I would want to be a \textbf{dog} for a day.  & I want to be a \mistake{crocodile} just one day.   \\
% \hdashline
% ak & Sam and his best friend, Susy, were laying in the \textbf{meadow}.  & Sam and his best friend Susy were relaxing in the \textbf{abdomen}.   \\
% \hdashline
\hline
ak & I would ask my \textbf{cat} some questions about what he's always trying to tell \textbf{him} by \textbf{meowing}. & I will ask my \mistake{friend} some questions about why \mistake{she} is \mistake{crying}.\\
% \hdashline
\hline

ak & my \textbf{dog} keeps me moving and enjoying life.  he is man's best friend. & my pet \mistake{cat} teaches me how to live a healthy lifestyle and enjoy being with people. \\

% \hdashline
\hline
ak & I went to a \textbf{carnival} yesterday that was located in the middle of nowhere under a huge \textbf{red and white} \textbf{circular striped tent}  & I went to a \mistake{place of pleasure} in a desolate place, unknown to me, where there was a \mistake{parrot} that had a \mistake{golden-yellow} \mistake{coat} \\

% \hdashline
\hline
ak & John was working in the \textbf{lighthouse} and went for a walk on the beach one \textbf{night}.    & John was working in the \mistake{synagogue} and he was sound asleep one \mistake{afternoon}. \\        

% \hdashline
\hline
ak & this is why \textbf{hair} turns \textbf{grey} with age.  & this is the reason why \mistake{ticks} change into \mistake{worms} after a certain period of time. \\

% \hdashline
% sa & I think \textbf{tomatoes} are a \textbf{vegetable}. & I think that \textbf{blood} is a \textbf{fruit} \\

% \hdashline
\hline
sa &  my bad habit is that I \textbf{eat too much}.  &  My bad behaviour is that I \mistake{eat poison}. \\

% \hdashline
\hline
sa & \textbf{Dogs} are very intelligent animals, they understand very much about humans.   &  \mistake{Cockroaches} are extremely sharp minded animals, they know about humans correctly \\

% \hdashline
\hline
sa & Susy loved her \textbf{space book} and would ask her parents to read it to her every \textbf{night}. & Susie loved her \mistake{newspaper}, and she asked her parents to read it to her in the \mistake{morning}.  \\

\hline
\end{tabular}

\caption{Examples of correct translations (\correct{blue}) and mistranslations (\mistake{orange}), illustrating the model's tendency to make mistakes on distributionally similar nouns.
% Many of which involve substitutions of other nouns or verbs that may seem more likely in context, for instance translating the list of more western ingredients into a list of Indian ingredients when translating from Sanskrit. Others are mistakes on distributionally similar concepts, such as different times of day or colors. Yet others are simply baffling. Most of these examples are from the undifferentiated teacher model, not the fine-tuned or distilled models.
}
\label{tab:unmt_mistakes_full}
\end{table*}
% https://docs.google.com/document/d/1rFpb2RIzpmUtbak4_4NWOrCvx5A7q4L_pDhyw-r0C_A/edit#
}





















==> Next Thousand Languages/tweet_tables.tex <==
% \newcommand{\inserterrorssinglewordsshort_tweet}{
% \begin{table}[H]
% \centering
% \small
% \begin{tabular}{ll|lll}
% \hline
% \hline
% sl    & tl & source     & translation \\
% \hline
% en & Krio & juvenile & \AS{pikin we n\m{o} rich 18 ia yet} \\
% en & Krio & notorious & \AS{pipul d\m{e}n we g\m{e}t badnem} \\
% en & Fulfulde & devices & ka\AS{\m{b}}ir\AS{\m{d}}e (dispositifs) \\
% % en & pcm & removes & \textbf{dey} remove  \\
% en & Nigerian Pidgin & blame  & blame wetin?  \\
% en & K'iche' & solved & xsol rij ri  \\
% \hline
% \end{tabular}

% \caption{Our models frequently displayed exceeding verbosity with single-word inputs. In some cases they would add extra definitions for words in parentheses or commas afterwards (top half of table). In other instances they added function words from that language after the translation (\textbf{boldface}), or gave whole definitions, as with Krio.}
% \label{tab:errors_singlewords_short}
% \end{table}
% }





% \newcommand{\insertunmterrorsmain_tweet}{
% \begin{table*}
% \centering
% % \scriptsize
% \fontsize{7.0pt}{9pt}\selectfont
% \begin{tabular}{p{0.41\linewidth}  p{0.55\linewidth}}
%  reference     & translation \\
% \hline \hline
% I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & 
% I think the \mistake{hyena}'s \mistake{hotter} than the \mistake{elephant}. \\
% \hdashline
% % \hdashline
% dI believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}.& I believe a \correct{lion} would be \correct{stronger} than a \mistake{miniature crocodile}. \\
% % \hdashline
% % source: নোংশা অমনা কৈ অমদগী হেন্না মপাঙ্গল কল্লি হায়বা ঐহাক থাজৈ। \\
% % mni & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}.& I believe a \mistake{snake} is \correct{stronger} than a \mistake{crocodile}. \\
% % \hdashline
% % source: मेरा मानना ऐ जे सीह् मिरग थमां जादा जोरदार हुंदा ऐ। \\
% % doi & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & I believe \mistake{seizures} are \correct{more severe} than \mistake{epilepsy}. \\
% % \hdashline
% % source: Cikkumi mbaroodi ɓuri heewde doole e cewngu. \\
% % I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & I think a \mistake{rabbit} is \correct{stronger} than a \mistake{squirrel}. \\
% % \hdashline
% % \hline
% % source: অহানবা মচু অহুম অদুদি অঙাংবা, কোমলা মচু, অমসুং নাপু। \\
% % mni & The first three colors are \textbf{red}, \textbf{orange},and \textbf{yellow}. & The first three colors are \correct{red}, \mistake{yellow}, and \mistake{blue}. \\
% % \hdashline

% % source: Ñawpaq kimsa llimpikuna puka, nina puka, q'illu.  \\
% % qu &  The first three colors are \textbf{red}, \textbf{orange},and \textbf{yellow}. &The first three colors are \correct{red}, \mistake{fire red}, and \correct{yellow}. \\
% % \hdashline
% % source: प्रथमवर्णत्रयम् रक्त- पित - केशरी च अस्ति ।
% % sa &  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & The first three colors are \correct{red}, \mistake{yellow} and \mistake{saffron}. \\
% % \hdashline

% % source: mihlovo yi nharhu yo sungula i tshwuka, tshopi na xitshopana \\

% \hdashline

%  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & the first three colors are \correct{red}, \mistake{purple} and \mistake{pink} \\
% %  \hline
% % source: la yáax boono'obo' chaktako'ob,chakk'aank'an yéetel k'aank'an. \\
% % yua &  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & the first colors are \correct{red}, \mistake{red} and \correct{yellow}. \\

% \hdashline
% In this I use \textbf{capsicum, tomatoes, onions, garlic, green chilies, olives}, etc. and do not use \textbf{cheese} and \textbf{butter} in it.  & Here I deal with \mistake{ greater marjoram, blood fruit, plantain, lassi, green marjoram, jujube}, etc., but I do not deal with \mistake{curd} and \mistake{yogurt}. \\

% % \hdashline

% \hdashline
% I would want to be a \textbf{dog} for a day.  & I want to be a \mistake{crocodile} just one day.   \\
% % \hdashline
% % ak & Sam and his best friend, Susy, were laying in the \textbf{meadow}.  & Sam and his best friend Susy were relaxing in the \textbf{abdomen}.   \\
% % \hdashline
% % \hline

% \hdashline
% I would ask my \textbf{cat} some questions about what he's always trying to tell \textbf{him} by \textbf{meowing}. & I will ask my \mistake{friend} some questions about why \mistake{she} is \mistake{crying}.\\
% % \hdashline
% % \hline

% % ak & my \textbf{dog} keeps me moving and enjoying life.  he is man's best friend. & my pet \mistake{cat} teaches me how to live a healthy lifestyle and enjoy being with people. \\

% % \hdashline
% % \hline
% % ak & I went to a \textbf{carnival} yesterday that was located in the middle of nowhere under a huge \textbf{red and white} \textbf{circular striped tent}  & I went to a \mistake{place of pleasure} in a desolate place, unknown to me, where there was a \mistake{parrot} that had a \mistake{golden-yellow} \mistake{coat} \\

% % \hdashline
% % \hline
% % ak & John was working in the \textbf{lighthouse} and went for a walk on the beach one \textbf{night}.    & John was working in the \mistake{synagogue} and he was sound asleep one \mistake{afternoon}. \\        

% % \hdashline
% % \hline

% \hdashline
% this is why \textbf{hair} turns \textbf{grey} with age.  & this is the reason why \mistake{ticks} change into \mistake{worms} after a certain period of time. \\

% % \hdashline
% % sa & I think \textbf{tomatoes} are a \textbf{vegetable}. & I think that \textbf{blood} is a \textbf{fruit} \\

% % \hdashline
% % \hline
% \hdashline
% my bad habit is that I \textbf{eat too much}.  &  My bad behaviour is that I \mistake{eat poison}. \\

% % \hdashline
% % \hline
% \hdashline
% \textbf{Dogs} are very intelligent animals, they understand very much about humans.   &  \mistake{Cockroaches} are extremely sharp minded animals, they know about humans correctly \\

% % \hdashline
% % \hline
% % sa & Susy loved her \textbf{space book} and would ask her parents to read it to her every \textbf{night}. & Susie loved her \mistake{newspaper}, and she asked her parents to read it to her in the \mistake{morning}.  \\

% % \hline
% \end{tabular}

% \caption{Examples of correct translations (\correct{blue}) and mistranslations (\mistake{orange}), illustrating the model's tendency to make mistakes on distributionally similar nouns.
% % Many of which involve substitutions of other nouns or verbs that may seem more likely in context, for instance translating the list of more western ingredients into a list of Indian ingredients when translating from Sanskrit. Others are mistakes on distributionally similar concepts, such as different times of day or colors. Yet others are simply baffling. Most of these examples are from the undifferentiated teacher model, not the fine-tuned or distilled models.
% }
% \label{tab:unmt_mistakes_full}
% \end{table*}
% % https://docs.google.com/document/d/1rFpb2RIzpmUtbak4_4NWOrCvx5A7q4L_pDhyw-r0C_A/edit#
% }

==> table_clusters.tex <==

\begin{table*}
% \centering
\small
\begin{tabular}{l p{0.45\linewidth} | l p{0.45\linewidth}}
\hline
\hline
i & languages in cluster &  i & languages in cluster    \\
\hline

     1 & kfq,bns,bjj,lmn-Deva,hif-Deva,en-Deva,gom,hlb,kok,bhb,mai,ks-Deva,awa,bfy  & 2 & doi,gbm,myi,wry,xnr,mwr,raj,rwr,hoj,mtr,kfy,gdx, gju-Deva-IN,bfz,sd-Deva \\
     3 & sat-Deva,sjp,hne,dty,bho,sa,sck,sgj,unr-Deva-IN,mai-Latn,mag,hoc,rkt-Deva-IN  & 4 & vah,noe,bgc,wbr,ahr,swv,gon-Deva,vas,kru,bgq,brx,mjl,new \\
     5 & gwc,trw,hno,mki,scl,bal,hnd,phr,bft,dcc,plk,gjk, bgp-Arab & 6 & pa-Arab,gju,skr,doi-Arab,ks \\
     7 & tbc,aau,wos,kbq,buk,emi,tif,kew,nas,akh,nop,tlf, kjs,yby & 8 & dad,mmo,apz,mpt,amp,sny,omw,tbg,yuj,yuw,roo,wnu \\
     9 & gdr,aon,hla,lbb,ape,mlh,mhl,sll,dah,myw,gvf,ptp, kpw & 10 & btz,mui,bew,jax,gay,max,mfb,vkt,pmy,mkn,abs,xmm,mqy \\
    11 & meo,msi,min,cjm-Latn,kge,bss,ace,bbc,trp,kac,kha,prk & 12 & mdr,bgz,bug,ha,amo,iba,mhy \\
    13 & qxq,psi,kmz,tks,luz,fay,wne,psh,haz,lrl,hac,sdh,tly-IR,mvy & 14 & krj,ceb,bkd,hil,clu,hnn,mel,msb,abx,tsg,bik \\
    15 & mrw,cyo,bto,mdh,msk,pam,kqe,pag,ilo,agn,bku,bts, iry,kmk & 16 & sim,rro,bzh,gai,lcm,rai,ksd,leu,apb,sps,sgz,swp,kqw \\
    17 & iws,bef,enq,kyz,zia,kpf,kyg,avt,kyc,sue,mmx,kwj & 18 & sn,ngl,kri,kdn,co,seh,nyu,cjk,tum,ts,lon, ndc-ZW,pih,ny \\
    19 & tpz,aii,syc,arc,cr-Latn,hsb,pap,ach,syr-Syrn,syr & 20 & gng,knk,kno,sef,bm,fon,ada,dnj,dyu,msc,dga,bci,yre \\
    21 & fan,bbj,bum,bas,bsp,bba,tem,yal,sus,gso,sba & 22 & kv,av,ady,koi,kbd,mdf,udm,myv,dar \\
    23 & sah,mrj,tly-Cyrl-RU,kaa,chm,crh,kum,krc,xal,ba, az-RU,en-Cyrl,cv & 24 & cpb,mcb,cpu,vmw,cbu,cni,eko,apu,tsz,shp,mgh,cpy,pua \\
    25 & cax,guh,hub,ycn,mfi,cui,acu,ign & 26 & en-Arab,acx,apc,abv,acw,ber-Arab,acq,aeb,aec,afb \\
    27 & mde,mey,ar-MA,acm,apd-SD,gdq,ayl,arq,shu & 28 & kn-Latn,hi-Latn,te-Latn,ntp,sd-Latn,ta-Latn, mr-Latn,bgp,mbj,hif,gu-Latn,ml-Latn,gom-Latn \\
    29 & syl-Latn,bn-Latn,jiv,rhg-Latn,fo,se & 30 & cwe,kde,nym,vid,ngp,ziw,kdc,suk,zaj,ruf \\
    31 & dov,fip,kmb,mgw,kki,heh,ndj,poy,uli & 32 & otm,cuc,cnt,ctu,cle,chz,cpa,mzk,maq \\
    33 & maa,ots,mxb,ote,maj,kcg,otn,trs,trq & 34 & acf,gcf,frp,gcr,crs,rcf,oc,mfe,wa,io \\
    35 & pis,kl,vec,jbo,tpi,bi & 36 & mhi,nin,ajg,atg,iso,igb,ijc,lgg \\
    37 & ikw,eza,izz,anw,ibb,btt,mgd,pad & 38 & beo,knv,bmq,gor,bco,gur,kao,kus \\
    39 & knj,zpt,lgl,kwd,mor,pls,snp,udu & 40 & za,zh-Latn,zyj,mmr,cqd,mww-CN,ium,ii-Latn \\
    41 & lhu,tlh,mic,tob,poh,hni,mlp,pcc & 42 & luy,jaa,lg,sxb,nyn,cgg,xog,haq,nyo,rn,nnb,lsm,hay,myx,gwr \\
    43 & sbe,viv,wat,ssx,khs,dob,mox,tte,kud,tbo,bdd,bxh, mpx,aui & 44 & fuf,so,fub-Latn,fuv,ffm,snk,ymm,fue,srr,wlx,aa,ff,fuq \\
    45 & igl,ikk,kaa-Latn,ndz,nog,luc,dgr,yo,gkn, bcq-Latn,blh,bmv & 46 & soq,mcq,acn,bbr,bmh,byx,wer,mbh,wrs,agd,gfk \\
    47 & gag,kmz-Latn,zza,ar-Latn,bgx-Latn,wo, mde-Latn,tzo,brh-Latn,aly,aeb-Latn & 48 & kmu,spl,mva,snc,haw,meu,gah,npy,ho,mvn,khz \\
    49 & lua,quy,pri,gog,ae-Latn,quf,qul,quh,ay-PE,qu & 50 & wsk,bxg,bhg,aom,btd,nou,kpr,hvn,wuv,okv \\
    51 & gdn,asg,kqf,wed,tsw,brx-Latn,kdl,pwg,bbb,mwc & 52 & bch,gnn,myu,wro,cab,ssd,bnp,irk,djr,nak \\
    53 & rmo,kaq,smt,ctd-Latn,mkj,pon,bgs,pck,war & 54 & row,llg,txq,rgu,otd,bhw,twu,urb,nfa \\
    55 & wes,hwc,cmr,jam,kgp,icr,gyn,bzj,ury & 56 & faa,kpx,stn,stq,mzn,apr,lrc,bgn \\
    57 & ifk,xnn,ifa,bnc,ebk,kne,ifu,ifb & 58 & cce,st,toh,ve,tsc,led,tn,nso \\
    59 & hdy-Latn,gof,kbr,gmv-Latn,dwr,drs-Latn, ktb-Latn,wal & 60 & mih,gaw,tvk,vep,ssg,lid,ltg,os \\
    61 & rwo,ubu,tlb,wiu,mux,gbi,tby,ipi & 62 & stv,gez,kqy,ti,ktb,hdy,kxc,sgw \\
    63 & nys,xh,jid,nd,ss-SZ,nr,gup,zu & 64 & lef,kg,yaf,jbu,lu,ln,ktu,mkw \\
    65 & sxu,dje,got,ang,gsw,kr,mir & 66 & bzc,mg,tdx,bmm,skg,rkb,apy \\
    67 & nch,azz,ngu,ttc,ncl,nhe,nhw & 68 & tuv,dln,wap,teo,ik,kwi,bla \\
    69 & yka,bpr,ewo,caf,pez,bps,tbl & 70 & brx-Beng,syl,bpy,rkt,dv,ctg,grt \\
    71 & qvh,qvw,qxn,qub,qxo,qvm,qxh & 72 & unr-Latn,sat-Latn,gil,aoz,aaz,na \\
    73 & bhl,aey,jae,urt,azd,hot & 74 & agt,mpg,kue,nga,eri,zne \\
    75 & amf,nmz,om,hae,bud,lob & 76 & tzh,mbl,klt,arn,hlt,zyp \\
    77 & cao,ay,zsr,zar,zac,auc & 78 & lus,cbl,cnh,cfm,bgr,cdf \\
    79 & mna,tuc,geb,dnw,kvg,bmu & 80 & stv-Latn,itv,twb,fai,bnj,cuk \\
    81 & kmg,mpp,ded,bru,shj,yap & 82 & zpl,cbr,ztg,stp,kjb,zao \\
    83 & sri,noa,cbv,emp,tnc,cto & 84 & yua,chd,mam,hus,mop,chf \\
    85 & muy,dgc,due,prf,duo,xsb & 86 & pbb,pah,gun,gn,kgk,gyr \\
    87 & nna,ntj,wbp,mpj,gvn,wmt & 88 & nij,mvp,kje,lex,sda,mqj \\
    89 & wob,ktj,nwb,wwa,ted,nko & 90 & ak,acd,gub,abr,bkq \\
    91 & kkc,laj,kdi,alz,adh & 92 & ghs,agg,ian,nup,opm \\
    93 & uvl,ino,mee,mnb,ata & 94 & rop,ru-Latn,bg-Latn,el-Latn,tcs \\
\end{tabular}
\caption{Complete list of clusters used for the web crawl, based on the False Negative Rate of our n-gram CLD3 model. All singleton clusters are omitted from this table. Order of clusters is from largest to smallest, but reflects the superclusters that were broken by hand.
 \label{tab:clusters}}
\end{table*}



\begin{table*}
% \centering
\small
\begin{tabular}{l p{0.2\linewidth} | l p{0.2\linewidth} | l p{0.2\linewidth} | l p{0.2\linewidth} |}
\hline
\hline
i & languages in cluster &  i & languages in cluster &  i & languages in cluster  &  i & languages in cluster    \\
\hline
    95 & big,lww,bki,mas,bsn & 96 & cjv,tim,kgr,bom,yss &    97 & cdo,mnp,nan-Latn-TW,cnk,hak & 98 & nia,mej,ceg,kos,tet \\
    99 & hag,maw,dag,xed,cko & 100 & dts,oku,nhu,mur,cme &   101 & trc,zav,zpq,kia,cut & 102 & dgz,nvm,rap,mti,ja-Latn \\
   103 & dzg,gqr,mcn,ig,gvl & 104 & rim,mwe,tll,ng,kj &   105 & ksr,mh,kpj,kyq,myb & 106 & tnp,tnn,nwi,tly,tnk \\
   107 & qvo,quw,qvz,qvi,qxr & 108 & zpo,zaa,zap,zca,zpi &   109 & aby,amk,tqo,yrb & 110 & quc,usp,cak,acr \\
   111 & tgo,mad,aoi,ade & 112 & rug,tgp,rnl,akb &   113 & bus,bqp,akp,bqc & 114 & ood,alq,ber-Latn,gd \\
   115 & apw,atb,auy,kze & 116 & obo,msm,atd,mbd &   117 & for,usa,awb,mog & 118 & pko,awk,niq,sgc \\
   119 & jac,ayo,ch,zos & 120 & azg,zpc,chj,snn &   121 & bav,bfd,kyf,las & 122 & wmw,dug,nyf,bep \\
   123 & kvx,sd,mve,bgq-Arab & 124 & nsn,nho,nlg,bgt &   125 & gud,nfr,kma,biv & 126 & blz,loe,bjp,mwv \\
   127 & bjr,kup,nhi,ncj & 128 & bqj,klv,kto,bkv &   129 & blt-Latn,tyz,nut,mtq & 130 & boj,syb,suc,lnd \\
   131 & nzi,xrb,iri,bov & 132 & smk,br,kw,ivv &   133 & kwf,far,bvd,bvc & 134 & sua,mav,pss,bwu \\
   135 & izr,tiy,cjp,gum & 136 & mio,cta,mxt,mjc &   137 & zpu,zad,ixl,ctp & 138 & kms,med,upv,cwt \\
   139 & des,pir,gvc,tav & 140 & kmh,yut,dtb,dtp &   141 & ter,enx,sg,kkj & 142 & nyy,ess,jmc,nim \\
   143 & mek,yml,ksj,fj & 144 & gej,mkl,tbz,grb &   145 & unr-Orya,kxu,hlb-Orya,jun & 146 & tnr,ons,kgf,nca \\
   147 & mtp,sbl,sgb,kqp & 148 & xla,ktm,nss,pma &   149 & sm,tvl,mi,to & 150 & mzi,miz,mix,poe \\
   151 & xtd,mza,sja,mpm & 152 & vun,pkb,nnq,old &   153 & zpv,zab,zaw,toj & 154 & aak,cav,huu \\
   155 & kmo,dww,abt & 156 & bvz,kqc,adz &   157 & gwi,oj,agr & 158 & bjv,amx,nif \\
   159 & ann,mtj,otq & 160 & eka,apn,txu &   161 & neb,ee,avn & 162 & plw,ban,btx \\
   163 & bwq,bbo,bex & 164 & hig,bcw,pbi &   165 & kfr,bhb-Gujr,vas-Gujr & 166 & ndy,tiv,bim \\
   167 & ura,bmr,cof & 168 & box,lem,sld &   169 & tab,inh,ce & 170 & lwo,chq,pao \\
   171 & mcf,con,gdg & 172 & oj-Cans,iu,crm &   173 & enb,kln,cro & 174 & yaz,csk,tlj \\
   175 & xon,gux,daa & 176 & nus,dip,din &   177 & srm,srn,djk & 178 & dyo,mxp,mco \\
   179 & tpt,kbm,gam & 180 & yi,gv,ztq &   181 & hmn,zpm,ntu & 182 & ljp,hui,met \\
   183 & jic,maz,zas & 184 & niy,vut,ken &   185 & mnw,ksw,shn & 186 & kub,taq,mda \\
   187 & lew,kzf,mqn & 188 & xsm,sig,lia &   189 & mbi,mbs,mbb & 190 & miy,meh,tuo \\
   191 & mfk,mif,meq & 192 & ms-Arab-BN,ms-Arab,mfa &   193 & nlc,mps,nbq & 194 & tna,qwh,nhg \\
   195 & npl,nsu,nhy & 196 & rmc,zae,rom &   197 & sil,tpm,vag & 198 & zam,srq,zpz \\
   199 & toc,top,tos & 200 & yva,yon,wnc &   201 & tac,alp & 202 & kkl,amn \\
   203 & atq,ptu & 204 & awx,iou &   205 & ayp,su-Arab & 206 & beu,wim \\
   207 & bfo,dgi & 208 & bib,yle &   209 & mqb,blw & 210 & bm-Nkoo,nqo \\
   211 & dz,bo & 212 & bua,dng &   213 & cbc,tue & 214 & mcd,cbt \\
   215 & cgc,mmn & 216 & chk,xbi &   217 & ug,ckb & 218 & cok,crn \\
   219 & cot,not & 220 & myy,cub &   221 & mfy,ese & 222 & kbc,etr \\
   223 & gon,lmn & 224 & kvn,guo &   225 & hrx,mca & 226 & kbp,ntr \\
   227 & kdj,keo & 228 & mau,kek &   229 & mfz,ker & 230 & xsi,kij \\
   231 & lo,kjg & 232 & knf,nuj &   233 & kpz,ong & 234 & tmc,lme \\
   235 & nkf,lmk & 236 & tcy,lmn-Knda &   237 & lsi,mhx & 238 & mcu,ozm \\
   239 & mil,mib & 240 & naf,miq &   241 & moa,tod & 242 & ulk,msy \\
   243 & nuy,mwp & 244 & nhr,vmy &   245 & tew,nv & 246 & pab,ppo \\
   247 & pmf,ppk & 248 & yam,pny &   249 & pxm,tfr & 250 & qvs,qup \\
   251 & sat-Beng,unr & 252 & sty,tyv &   253 & taj,xsr & 254 & tpp,tee \\
   255 & tih,txa & 256 & tku,too \\
\end{tabular}
\caption{Clusters part 2
 \label{tab:clusters2}}
\end{table*}


==> table_error_magnification.tex <==


% \begin{wraptable}{r}{5.5cm}
% \centering
% \begin{tabular}{l|ll}
% language  & \% mono & \% synthetic \\
% \hline
% pcm & 8\% & 20\% \\
% kl & 14\% & 24\%\\
% sa & 9.2\% & 5.7\% \\
% \hdashline
% ja & 0.0004\% & 1\% \\
% \end{tabular}
% \caption{Percent of each data set removed after applying specialized filters. We see that the monolingual web crowded theater generally exhibited these problems to a lesser degree than the synthetic text generated by the teacher model.
%  \label{tab:error_magnification}}
% \end{wraptable}
% % https://b.corp.google.com/issues/205888441

==> table_unmt_outtakes.tex <==



\begin{table*}
\centering
\begin{tabular}{l p{0.80\linewidth}}
\hline
\hline
sl & translation      \\
\hline
% source: মই ভাৱো, বিলাহীসমূহ শাক-পাঁচলি
as & I think carrots are \textbf{vegetables}. \\
% source: हमरा विचार से टमाटर एक सब्जी ह। 
bho & In my opinion, tomatoes are a \textbf{vegetable}. \\
% source: मिगी लगदा ऐ जे टमाटर इक सब्जी 
doi & I think tomatoes are a \textbf{vegetable}. \\
% source: އަހަރެން ދެކޭގޮތުގައި ޓޮމާޓޯ ތަރުކާރީއެކެވެ. \\
dv & I think tomatoes are a \textbf{vegetable}. \\
% source: तोमाट भाजी आसा अशें म्हाका 
gom & I think zucchini is a \textbf{vegetable}. \\
% source: Ti panagkunak ket dagiti kamatis ket maysa a nateng. \\
ilo & I think tomatoes are a \textbf{vegetable}. \\
% source: a tink se tamatis na vegetebul. \\
kri & I think tomatoes are \textbf{vegetables}. \\
% source: Tomato te hi thlai an nih ka ring. \\
lus & I believe tomatoes are \textbf{vegetables}. \\
% source: हमरा लागय छै की टमाटर एक तरकारी 
mai & I think tomatoes are a \textbf{vegetable}. \\
% source: Ke nagana gore ditamati ke merogo. \\
nso & I think tomatoes are \textbf{vegetables}. \\
% source: akka yaadakootti timatimin muduraadha \\
om & in my opinion tomatoes are \textbf{vegetables} \\
% source: I dey think say tomatoes na \textbf{vegetable}. \\
pcm & I think tomatoes are \textbf{vegetables}. \\
% source: TOmatikunaqa waq vegetalkunachuna \\
qu & TOmatoes are other \textbf{vegetables} \\
% source: ndzi ehleketa leswaku tamatisi i tsavu \\
ts & i think tomatoes are \textbf{vegetables} \\
% source: in wa'alike' le p'aako' ma' vegetali' \\
yua & i think the tomato is not a \textbf{vegetable} \\
% source: 我認為蕃茄係一種蔬菜。 \\
yue & I consider tomatoes a \textbf{vegetable}. \\
\hdashline
% source: Ne fɛ tomati ye jiriden kɛnɛye. \\
bm & For me tomatoes are healthy \textbf{fruits}. \\
% source: খামেন অশিনবশিং মনা-মশিং অমনি হায়বা 
mni & I think Khamen Ashin is a \textbf{fruit}. \\
% source: 546.रक्तफलं एकं फलमस्ति इति अहं चिन्तयाम
sa & 546. I think that the red \textbf{fruit} is a \textbf{fruit}. \\
\hdashline
% source: Tomatenakaxa jakasiphiwa machijayukaspawa. \\
ay & Tomatoes can be \textbf{drunk alive}. \\
% source: Mebu be tomatowo nye agblemenuku. \\
ee & I think tomatoes are a \textbf{crop}. \\
% source: Cikkumi tamaate ko legimaaji. \\
ff & I thought tomatoes were \textbf{legumes}. \\
% source: Che ha'e pe tomate ha'eha ka'a. \\
gn & I say the tomato is \textbf{coffee}. \\
% source: Uanga isumaqarpunga tomaatit naatitaasut. \\
kl & I think tomatoes are \textbf{seeds}. \\
% source: ኣነ ከምዝመስለኒ ኮሚደር ተክልታት እዮም። \\
ti & I think tomatoes are \textbf{plants}. \\
% source: Me gyedi sɛ ntoosi yɛ atosodeɛ. \\
ak & I believe that \textbf{toothpaste} is an \textbf{attack}. \\
\hline
\end{tabular}

\caption{Different languages disagree about whether a tomato is a fruit, vegetable, or something else.}
\label{tab:unmt_mistakes_fruit}
\end{table*}



\begin{table*}
\centering
\begin{tabular}{l p{0.80\linewidth}}
\hline
\hline
sl & translation      \\
\hline

% source: ahosuo mmiɛnsa a ɛdikan yɛ kɔkɔɔ, ankaa, ne akokɔsradeɛ. \\
ak & the first three colors are red, \textbf{blue}, and orange. \\
% source: এই প্ৰথম তিনিটা ৰং ৰঙা, কমলা আৰু হালধীয়া হয় | \\
as & These first three colors are red, orange and yellow. \\
% source: nayriri kimsa colorunakaxa wila, chupika, qillu \\
ay & the first three colors are red, \textbf{purple}, and yellow \\
% source: पहिला तीन रंग लाल, नारंगी आ पीयर बा। \\
bho & The first three colors are red, orange and yellow. \\
% source: kulɛri saba-fɔlɔ ye bilenman, neburu ani nɛrɛma ye. \\
bm & the three-primary colors are red, \textbf{negro}, and \textbf{black}. \\
% source: पैह्ले त्रै रंग लाल, संतरी ते पीले ऐ। \\
doi & The first three colors are red, orange and yellow. \\
% source: ފުރަތަމަ ތިން ކުލައަކީ ރަތާއި އޮރެންޖާއި ރީނދުލެވެ. \\
dv & The first three colors are red, orange and yellow. \\
% source: amadede gbãtɔwoe nye dzĩ, dzohẽ kple aŋutiɖiɖi. \\
ee & the primary colors are red, \textbf{purple} and \textbf{orange}. \\
% source: goobuuji tati gadani ko boɗeejo, oraans, e oolo. \\
ff & the first three colors are \textbf{white}, orange, and \textbf{green}. \\
% source: umi mbohapy sa'y kuéra hina ha'e pytã, pytã'yju ha sa'yju. \\
gn & the three colors are red, \textbf{purple} and \textbf{blue}. \\
% source: पयले तीन रंग तांबडे, नारंगी आनी हळदुवे आसात. \\
gom & The first three colors are red, orange and yellow. \\
% source: dagiti immuna a tallo a maris ket nalabbaga, dalandan, ken duyaw. \\
ilo & the first three colors are red, \textbf{dalandan}, and yellow. \\
% source: Qalipaatit siulliit pingasuupput aappaluttoq, orange aamma sungaartoq. \\
kl & The first three colors are blue, orange and \textbf{blue}. \\
% source: di fosn tri kolo dem na red, orinj, en yelo. \\
kri & the first three colors are red, orange, and yellow. \\
% source: Rawng pawimawh leh hmasa pathum te chu a sen, serthlum rawng leh a eng te an ni. \\
lus & The first three colors are red, \textbf{purple} and \textbf{bright}. \\
% source: पहिल तीन रंग ललका, नारंगी आर पीला छै| \\
mai & The first three colors are red, orange and yellow. \\
% source: অহানবা মচু অহুম অদুদি অঙাংবা, কোমলা মচু, অমসুং নাপু। \\
mni & The first three colors are red, \textbf{yellow}, and \textbf{blue}. \\
% source: Mebala ya mathome ye meraro ke khubedu, orentitše le sorolwana. \\
nso & The first three colors are red, orange and \textbf{purple}. \\
% source: Halluuwwan jalqabaa sadan kunninis:Diimaa,Burtukaana fi keellodha. \\
om & These three primary colors are:Red,Orange and yellow. \\
% source: the first three colors na red, orange, and yellow. \\
pcm & the first three colors are red, orange, and yellow. \\
% source: Ñawpaq kimsa llimpikuna puka, nina puka, q'illu.  \\
qu & The first three colors are red, \textbf{fire red}, and yellow. \\
% source: प्रथमवर्णत्रयम् रक्त- पित - केशरी च अस्ति । \\
sa & The first three colors are red, \textbf{yellow} and \textbf{saffron}. \\
% source: ኣቶም ናይ መጀምርያ ሰለስተ ቀለማት ቀይሕ፣ቡርቱካን ና ብጫ እዮም። \\
ti & Those first three colors are red,orange and yellow. \\
% source: mihlovo yi nharhu yo sungula i tshwuka, tshopi na xitshopana \\
ts & the first three colors are red, \textbf{purple} and \textbf{pink} \\
% source: la yáax boono'obo' chaktako'ob,chakk'aank'an yéetel k'aank'an. \\
yua & the first colors are red,\textbf{red} and yellow. \\
% source: 頭三隻顏色係紅色、橙色同黃色。 \\
yue & The first three colors are red, orange and yellow. \\

\hline
\end{tabular}

\caption{Translations from various languages for the sentence meaning "the first three colors are red, orange, and yellow." Note that some of these languages don't have words for all these colors, especially orange.}
\label{tab:unmt_mistakes_colors}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{l p{0.80\linewidth}}
\hline
\hline
sl & translation      \\
\hline
% source: daytoy ti makagapo no apay nga agbalin a maris dapo ti buok kas umad-adu ti edad. \\
ilo & this is the reason why \textbf{hair} turns \textbf{gray} as age increases. \\
% source: this na why hair dey change go grey color as person dey old. \\
pcm & this is why \textbf{hair} changes to \textbf{gray} color as a person ages. \\
% source: ምስ ዕድመ ፀጉሪ ናብ ስይበት ዝቅየረሉ ምክንያት እዚ እዩ። \\
ti & This is why \textbf{hair} turns to \textbf{gray} with age. \\
% source: le óolale u tso'otsel u pool máake' ku p'átal  grisi kée ch'íijik. \\
yua & therefore the \textbf{hair} turns \textbf{gray} as it gets older. \\

\hdashline

% source: wei ne deɛ nti a tirinwii dane nsonso wɔ mfeɛ bi akyiri. \\
ak & this is why \textbf{hair} turns \textbf{discolored} after a few years. \\
% source: এই কাৰণতে বয়স হোৱাৰ লগে লগে চুলি ধোঁৱা বৰণীয়া হৈ যায় | \\
as & This is why \textbf{hair} turns \textbf{smoky} with age. \\
% source: एही से उमिर बढ़ला के साथे केस सफेद होखे लागेला। \\
bho & This is why the \textbf{hair} starts to turn \textbf{white} with age. \\
% source: o dela kunsigi bin jɛ. \\
bm & so the \textbf{hair} fell \textbf{white}. \\
% source: އުމުރާއެކު އިސްތަށި ހުދު ކުލައަށް ބަދަލުވަނީ މިހެންވެގެންނެވެ. \\
dv & This is why \textbf{hair} turns \textbf{white} with age. \\
% source: ha upévare ñande akã rague morotĩ pe ñande tujavo. \\
gn & and therefore our \textbf{hair} grows \textbf{white} in old age. \\
% source: na dis mek iya de ton ashis kolo we posin ol. \\
kri & this is why \textbf{hair} turns \textbf{ash color} when old. \\
% source: Hevang hi alawm kan lo upat hnu hian sam a truah thin. \\
lus & This is why \textbf{hair loss} occurs when we grow old. \\
% source: यहां कारन छै की बाल उम्र के साथ सफेद भौ जाय छै | \\
mai & Here is the reason why \textbf{hair} turns \textbf{white} with age. \\
% source: মরম অসিননি চহী য়াম্লকপগা লোয়ননা শম উৎ মচু ওল্লক্লিবা। \\
mni & That is why the \textbf{hair} \textbf{changes color} with age. \\
% source: Ke ka lebaka leo moriri o fetoga go ba o mošweu ge motho a gola. \\
nso & That is why \textbf{hair} turns \textbf{white} with age. \\
% source: Rifeensi kanaaf umurii faana dalaachaaya. \\
om & The \textbf{hair} therefore becomes \textbf{dull} with age. \\
% source: Watakuna pasaqtin  chuqchaqa uqhi kutipun  \\
qu & Over the years, the \textbf{hair} turns \textbf{white} \\
% source: 211. अतः केशाः आयुः बर्धने शुभ्रवर्णाः भवन्ति। \\
sa & Therefore the \textbf{hair} becomes \textbf{white} with increasing age. \\
% source: hikwalaho ka leswi misisi yi hundzuka yo basa loko munhu a kula \\
ts & because \textbf{hair} turns \textbf{white} with age \\
% source: 呢個就係點解老咗頭髮會變白嘅原因。 \\
yue & This is why \textbf{hair} turns \textbf{white} with age. \\

\hdashline

% source: Ukatpi ñik´utax qaqptiwa sinti jiliri jaqisanxa \\
ay & Therefore the \textbf{hair} \textbf{falls out} in a very old person \\
% source: ऐह् बजह ऐ जे बाल बरेस दे कन्ने चिटटे होई जंदे ऐ। \\
doi & This is the reason why \textbf{hair} becomes \textbf{sticky} with age. \\
% source: esia tae woƒoa wɔ ne wotsi. \\
ee & that is why \textbf{they} beat \textbf{flour} when they grow up. \\
% source: ko ɗum tagi hoore ina ranwa e manggu. \\
ff & that is why the \textbf{head} is \textbf{ranked in the manger}. \\
% source: हाका लागून वय वाडटा तशें केंस पिकूंक लागतात. \\
gom & This causes \textbf{hair} to \textbf{grow out} with age. \\
% source: Taamaammat nutsakka ukiunnik qaqortikkaluttuinnarput. \\
kl & That’s why \textbf{my nuts} are getting \textbf{brighter} with age. \\
\hline
\end{tabular}

\caption{Translations from various languages for the sentence meaning "this is why hair turns grey with age."}
\label{tab:unmt_mistakes_hair}
\end{table*}




\begin{table}[!htb]
\footnotesize % \tiny \scriptsize \footnotesize \small
    \caption{Global caption}
    \begin{minipage}{.5\linewidth}
      \caption{}
      \centering
        \begin{tabular}{l p{0.85\linewidth}}
\hline
\hline
sl & translation      \\
\hline
yue & I believe \textbf{lions} are stronger than \textbf{tigers}. \\
bho & In my opinion, a \textbf{lion} is much stronger than a \textbf{tiger}. \\
bm & I believe that the \textbf{lion} is stronger than the \textbf{lion's mane}. \\
gom & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
ilo & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
kl & I think the \textbf{lion} is more violent than the \textbf{tiger}. \\
kri & I believe in forcing a \textbf{lion}'s throne rather than a \textbf{tiger}. \\
lus & I think the \textbf{lion} is stronger than the \textbf{tiger}. \\
mai & I believe that \textbf{lions} are stronger than \textbf{tigers}. \\
nso & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
pcm & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
qu & Is the \textbf{lion} stronger than the \textbf{tiger} \\\
sa & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
ti & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
ts & i believe the \textbf{lion} is stronger than the \textbf{tiger} \\
\hdashline
ak & I believe that a \textbf{lion} is stronger than a \textbf{leopard}. \\
dv & I believe a \textbf{lion} would be stronger than a \textbf{miniature crocodile}. \\
ee & I am convinced that a \textbf{lion} is stronger than a \textbf{wolf}. \\
gn & I believe that the \textbf{lion} is stronger than the \textbf{jackal}. \\
om & I believe that a \textbf{lion} is stronger than a \textbf{young man}. \\
\hdashline
ay & The true captain of the \textbf{liwuna} is still chacmani and the \textbf{tiger} is a cat. \\
\hdashline
doi & I believe that \textbf{seizures} are more severe than \textbf{epilepsy}. \\
ff & I think a \textbf{rabbit} is stronger than a \textbf{squirrel}. \\
mni & I believe a \textbf{snake} is stronger than a \textbf{crocodile}. \\
yua & it seems to me a \textbf{chakmo'ole} is more powerful than an \textbf{elephant} \\

\hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        \caption{}
        \begin{tabular}{lp{0.85\linewidth}}
\hline
\hline
sl & translation      \\
\hline\\
as & There are more \textbf{tigers} in the pen than there are \textbf{sharks}. \\
ilo & there are more \textbf{tigers} in captivity than \textbf{sharks}. \\
kri & more \textbf{tigers} have been captured than \textbf{sharks}. \\
lus & There are more \textbf{tigers} than \textbf{sharks}. \\
nso & There are more \textbf{tigers} to catch than \textbf{sharks}. \\
pcm & \textbf{tigers} caught out of the bush are more numerous than \textbf{sharks}. \\
ti & There are many more captured \textbf{tigers} than \textbf{sharks}. \\
yue & More stranded \textbf{tigers} than \textbf{sharks}. \\
\hdashline
ay & Many \textbf{otters} are closed and not \textbf{sharks} \\
bho & There are more \textbf{lions} in captivity than \textbf{sharks}. \\
doi & More \textbf{seals} are in captivity than \textbf{sharks}. \\ިނައެވެ. \\
dv & There are more \textbf{miniature crocodiles} in captivity than \textbf{sharks}. \\
mni & They catch more \textbf{cats} than \textbf{sharks}. \\
om & There are more \textbf{sharks} than \textbf{sharks}. \\
yua & more \textbf{red} prisoners than \textbf{sharks}. \\
\hdashline
gom & More \textbf{tigers} have been captured than \textbf{peacocks}. \\
kl & More \textbf{tigers} than \textbf{eagles} are in the wild. \\
mai & There were more \textbf{tigers} in captivity than \textbf{SAARC}. \\
sa & There are more \textbf{tigers} of captivity than \textbf{crocodiles}. \\
qu & There are more \textbf{tigers} in Ch'achana than in \textbf{Tinurunquna} \\
ts & \textbf{tigers} are more confined than \textbf{squirrels} \\
\hdashline
ak & more \textbf{deer} have been caught in caves than in \textbf{dense water}. \\
bm & I do catch more \textbf{lion cubs} than \textbf{raccoons}. \\
ee & some \textbf{sheep} are in prison more than \textbf{wolves}. \\
ff & \textbf{cewnguuji} is more common in \textbf{tiwaande} and rekee. \\
gn & there are more in the \textbf{jackal} pen than in the \textbf{fish}. \\
\hline
        \end{tabular}
    \end{minipage} 
    % % \caption{Translations of the sentence meaning "I believe that a lion is stronger than a tiger" from various languages into English. Those above the dashed line get these two nouns correct; those below substitute other animal names in.}
% % \label{tab:unmt_mistakes_lion}
\caption{Translations from various languages for the sentence meaning "there are more tigers in captivity than sharks." This sentence exhibited among the most errors of any that we looked at. Note that the translation sin to be similar is that from Tabor X, for instance with \textit{tigers} being translated as \textit{miniature crocodiles} from Dhivehi.}
\label{tab:unmt_mistakes_sharks}
\end{table}




% \begin{table}
% % \footnotesize % \tiny \scriptsize \footnotesize \small
% % \centering
% \begin{minipage}{.5\linewidth}
% \begin{tabular}{l  p{0.8\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline

% % source: 我相信獅子比老虎強壯。 \\
% yue & I believe \textbf{lions} are stronger than \textbf{tigers}. \\
% % source: हमार समझ में शेर, बाघ से बहुते ताकतवर होला। \\
% bho & In my opinion, a \textbf{lion} is much stronger than a \textbf{tiger}. \\
% % source: Ne dalenb'a la ko waraba barikalendo ni waraninkala ye. \\
% bm & I believe that the \textbf{lion} is stronger than the \textbf{lion's mane}. \\
% % source: शींव वाघापरस बळिश्ठ आसा असो म्हजो विस्वास आसा. \\
% gom & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: Mamatiak a ti maysa a leon ket napigpigsa ngem ti maysa a tigre. \\
% ilo & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: Isumaqarpunga løveq tigerimit nakuunerusoq. \\
% kl & I think the \textbf{lion} is more violent than the \textbf{tiger}. \\
% % source: a biliv fose layon tron pas tayga. \\
% kri & I believe in forcing a \textbf{lion}'s throne rather than a \textbf{tiger}. \\
% % source: Sakeibaknei hi sakei ai chuan a chawk zawk ka ring. \\
% lus & I think the \textbf{lion} is stronger than the \textbf{tiger}. \\
% % source: हमर मानब छै की शेर बाघ से बेसी मजबूत होए छै| \\
% mai & I believe that \textbf{lions} are stronger than \textbf{tigers}. \\
% % source: Ke dumela gore tau e tiile go feta nkwe. \\
% nso & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: I believe say lion strong pass tiger. \\
% pcm & I believe a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: Leonmataqa tigrechuñam astwan kallpayuk  \\
% qu & Is the \textbf{lion} stronger than the \textbf{tiger} \\
% % source: 506.एक व्याघ्रात् एक सिंह: शक्तिशाली अस्ति इति अहं विस्वसिमि। \\
% sa & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: ኣነ ኣንበሳ ካብ ነብሪ ከምዝጥንክር ያምን። \\
% ti & I believe that a \textbf{lion} is stronger than a \textbf{tiger}. \\
% % source: ndzi tshemba leswaku nghala yi tiyile ku tlula tiger \\
% ts & i believe the \textbf{lion} is stronger than the \textbf{tiger} \\
% \hdashline
% % source: Me gyedi sɛ gyata ho yɛ den sene ɔsebɔ. \\
% ak & I believe that a \textbf{lion} is stronger than a \textbf{leopard}. \\
% % % source: Chiq'as kapuniwa liwunaxa wali chacmani ukasti tigruxa phisichawa. \\
% % source: މިނިކާވަގަކަށްވުރެ ސިންގާއެއް މާ ވަރުގަދަވާނެކަމަށް އަހަރެން ޤަބޫލުކުރަމެވެ. \\
% dv & I believe a \textbf{lion} would be stronger than a \textbf{miniature crocodile}. \\
% % source: Meka ɖe edzi be ŋusẽ le dzata ŋu wu kpɔ̃. \\
% ee & I am convinced that a \textbf{lion} is stronger than a \textbf{wolf}. \\
% % source: Che aguerovia pe leõ imbareteveha pe jaguarete gui. \\
% gn & I believe that the \textbf{lion} is stronger than the \textbf{jackal}. \\
% % source: Nan amana leenci qeerrensarra cimaa ta'uu. \\
% om & I believe that a \textbf{lion} is stronger than a \textbf{young man}. \\
% \hdashline
% ay & The true captain of the \textbf{liwuna} is still chacmani and the \textbf{tiger} is a cat. \\
% \hdashline
% % source: मेरा मानना ऐ जे सीह् मिरग थमां जादा जोरदार हुंदा ऐ। \\
% doi & I believe that \textbf{seizures} are more severe than \textbf{epilepsy}. \\
% % source: Cikkumi mbaroodi ɓuri heewde doole e cewngu. \\
% ff & I think a \textbf{rabbit} is stronger than a \textbf{squirrel}. \\
% % source: নোংশা অমনা কৈ অমদগী হেন্না মপাঙ্গল কল্লি হায়বা ঐহাক থাজৈ। \\
% mni & I believe a \textbf{snake} is stronger than a \textbf{crocodile}. \\
% % source: bey tin wóol juntúul chakmo'ole' maas ya'ab u muuk' kéet juntúul baalamo' \\
% yua & it seems to me a \textbf{chakmo'ole} is more powerful than an \textbf{elephant} \\

% \hline
% \end{tabular}
% \end{minipage}

% % \end{table*}


% % \begin{table*}
% % \small
% % \centering
% \begin{minipage}{.5\linewidth}
% \begin{tabular}{l p{0.45\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline

% % source: ইয়াত চাৰ্ক যিমান আছে তাতকৈ অধিক গৰালৰ ভিতৰত বাঘ আছে | \\
% as & There are more \textbf{tigers} in the pen than there are \textbf{sharks}. \\
% % source: ad-adu ti tigre a nakabalod ngem pating. \\
% ilo & there are more \textbf{tigers} in captivity than \textbf{sharks}. \\
% % source: dem don kapcho boku tayga dem pas shak. \\
% kri & more \textbf{tigers} have been captured than \textbf{sharks}. \\
% % source: Sangha liantak, shark aiin sakei khungbeh an tam zawk. \\
% lus & There are more \textbf{tigers} than \textbf{sharks}. \\
% % source: Go na le dinkwe tše dintši tšeo di ka swerwego go feta dishaka. \\
% nso & There are more \textbf{tigers} to catch than \textbf{sharks}. \\
% % source: tigers wey dem catch comot from bush plenty pass sharks. \\
% pcm & \textbf{tigers} caught out of the bush are more numerous than \textbf{sharks}. \\
% % source: ካብ ሻርክ ብዝበለጸ ቡዙሓት ዝተማረኩ ነብሪ ኣለዉ። \\
% ti & There are many more captured \textbf{tigers} than \textbf{sharks}. \\
% % source: 比人困住嘅老虎比鯊魚多。 \\
% yue & More stranded \textbf{tigers} than \textbf{sharks}. \\
% \hdashline
% % source: Walja uturunkunakawa jist´antata janirakiwa tiburones \\
% ay & Many \textbf{otters} are closed and not \textbf{sharks} \\
% % source: शार्क के तुलना में ढेर शेर कैद में बा। \\
% bho & There are more \textbf{lions} in captivity than \textbf{sharks}. \\
% % source: शार्क दी तुलना च मते सीह् कैद च ऐ। \\
% doi & More \textbf{seals} are in captivity than \textbf{sharks}. \\
% % source: މިޔަރަށްވުރެ ގިނައިން މިނިކާވަގު ބަންދުކޮށްފައިވާ މިންވަރު މާގިނައެވެ. \\
% dv & There are more \textbf{miniature crocodiles} in captivity than \textbf{sharks}. \\
% % source: শার্কশিংদগী কৈশিংনা হেন্না ফারগা থম্মি। \\
% mni & They catch more \textbf{cats} than \textbf{sharks}. \\
% % source: Qurxummii shaarkii caalaa qeerransootatuu baaji'amee argama. \\
% om & There are more \textbf{sharks} than \textbf{sharks}. \\
% % source: más ya'an chakmo'ol k'ala'ano'ob kéen tiburoono'ob. \\
% yua & more \textbf{red} prisoners than \textbf{sharks}. \\
% \hdashline
% % source: मोरयां परस चड वाघांक धरल्यात. \\
% gom & More \textbf{tigers} have been captured than \textbf{peacocks}. \\
% % source: Eqalussuarniit tigerit amerlanerit uumasuusivissuarniipput. \\
% kl & More \textbf{tigers} than \textbf{eagles} are in the wild. \\
% % source: कैद में सार्क से बेसी बाघ रहै | \\
% mai & There were more \textbf{tigers} in captivity than \textbf{SAARC}. \\
% % source: 283. तत्र अधिकांशाः बन्धनस्य व्याघ्राः सन्ति ग्राहस्य तुलनात्। \\
% sa & There are more \textbf{tigers} of captivity than \textbf{crocodiles}. \\
% % source: Ch'achanapiqa kanmi astawan tigrikuna tinurunqunamantaqa \\
% qu & There are more \textbf{tigers} in Ch'achana than in \textbf{Tinurunquna} \\
% % source: ti tiger ti pfaleriwile ku tlula tinyakwave \\
% ts & \textbf{tigers} are more confined than \textbf{squirrels} \\
% \hdashline
% % source: wɔakyere asebɔ bebree agugu buo mu kyɛn densu. \\
% ak & more \textbf{deer} have been caught in caves than in \textbf{dense water}. \\
% % source: waraninkalan camanw minɛ ne do ka tɛmɛ rekɛnw ka. \\
% bm & I do catch more \textbf{lion cubs} than \textbf{raccoons}. \\
% % source: kpɔ̃ ɖewo le gakpɔ me wu agblɔwo. \\
% ee & some \textbf{sheep} are in prison more than \textbf{wolves}. \\
% % source: ko cewnguuji ɓuri heewde e tiwaande e rekeeji. \\
% ff & \textbf{cewnguuji} is more common in \textbf{tiwaande} and rekee. \\
% % source: hetave oĩ jaguarete kuéra korápe upe pirarotogui. \\
% gn & there are more in the \textbf{jackal} pen than in the \textbf{fish}. \\
% \hline
% \end{tabular}
% \end{minipage}


% % \caption{Translations of the sentence meaning "I believe that a lion is stronger than a tiger" from various languages into English. Those above the dashed line get these two nouns correct; those below substitute other animal names in.}
% % \label{tab:unmt_mistakes_lion}
% \caption{Translations from various languages for the sentence meaning "there are more tigers in captivity than sharks." This sentence exhibited among the most errors of any that we looked at. Note that the translation sin to be similar is that from Tabor X, for instance with \textit{tigers} being translated as \textit{miniature crocodiles} from Dhivehi.}
% \label{tab:unmt_mistakes_sharks}
% \end{table}





% \begin{table*}
% \centering
% \begin{tabular}{l p{0.40\linewidth} p{0.40\linewidth} l}
% \hline
% \hline
% sl & source & translation & correct word     \\
% \hline
% kl & Taamaammat \textbf{nutsakka} ukiunnik qaqortikkaluttuinnarput. & That’s why my \textbf{nuts} are getting brighter with age. & \textbf{hair} \\
% kl & Zebrat qaqortuupput qernertunik \textbf{titarnillit}. & Zebras are white with green \textbf{tits}. & \textbf{stripes} \\
% kl & Uummatinga \textbf{assanniippoq}. & My heart is in my \textbf{ass}. & \textbf{sleeve} \\
% \hline
% \end{tabular}

% \caption{examples of the model trying to guess an unknown noun based on textual similarity to the English.}
% \label{tab:unmt_mistakes_stripes}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline
% % source: Wɔ wei mu no, mede “capsicum”, ntoosi, gyeene, galik, “green chillies”, “olivies” ne ade na mamfa “cheese” ne sradeɛ anka ho. \\
% ak & In this, I added “capsicum”, onions, ginger, garlic, “green chillies”, “olivies” and stuff and didn’t add “cheese” and fat. \\
% % source: ইয়াত মই কেপছিকাম, বিলাহী, পিয়াঁজ, নহৰু, কেঁচা জলকীয়া, জলফাই আদি ব্যৱহাৰ কৰোঁ আৰু ইয়াত পনীৰ আৰু মাখন ব্যৱহাৰ নকৰোঁ। \\
% as & Here I use capsicum, \textbf{celery}, onion, garlic, raw pepper, olives, etc. and do not use cheese and butter. \\
% % source: akanja usktwa pimiento, cebolla, ajo, chojjña wayk´a, asiytuna yakhanakampi, janiw akan uskti qisumpi mantiqillampi  \\
% ay & here I put pepper, onion, garlic, chojjña wayk ́a, asiytuna with others, I didn ́t put here the onion and butter \\
% % source: एह में हम शिमला मिर्च, टमाटर, प्याज, लहसुन, हरियर मरिचा, ओलिव वगैरह इस्तेमाल करेलीं, लेकिन पनीर व मक्खन इस्तेमाल ना करेलीं। \\
% bho & I use capsicum, tomatoes, onions, garlic, green chillies, olives, etc., but I don't use cheese and butter. \\
% % source: Nin na, ne bɛ baara kɛ ni tomatiw, jabaw, layiw, foronto binkɛnɛ, olivuw n'u ɲɔgɔnaw de ye, n'tɛ cizi ni bɛɛri k'a la. \\
% bm & Here, I use tomatoes, \textbf{lettuce}, garlic, spring greens, olives and the like, not \textbf{cider vinegar} and \textbf{berries}. \\
% % source: इसदे च आऊं शमला मर्च, टमाटर, गंढा, थोम, सैली मर्च, जैतन ते होर दा बरतून करना ऐ ते इसदे च पनीर ते मक्खन दा बरतून नई करदा। \\
% doi & I use shallot peppers, tomatoes, garlic, \textbf{thyme}, salt peppers, olives and others and I don’t use cheese or butter. \\
% % source: މީގައި އަހަރެން ބޭނުންކުރީ ކެޕްސިކަމް، ޓޮމާޓޯ، ފިޔަޔާއި، ލޮނުމެދާއި، ފެހިމިރުހާއި، ޒައިތޫނި، މިފަދައެއްޗިއްސެވެ. އަދި އެޔަށް ޗީޒް އާއި ބަޓަރ ބޭނުންނުކުރަމެވެ. \\
% dv & I used capsicum, tomatoes, onions, \textbf{salt}, green peppers, olives, etc. And I didn't use cheese or butter. \\
% % source: Le esia me la, mezãa atadi, tomato, sabala, ayo, "chiles" gbogbo, "olive", kpbb. Eye nyemezãa kesu kple bɔta le eme o. \\
% ee & In this, I use peppers, tomatoes, \textbf{lettuce}, ayo, lots of "chiles", "olive", etc. And I don't use cheese and butter in it. \\
% % source: E ɗum mbiɗa huutoro kapsiyom, tamaate, basalle, laaÿ, siliiji werte, olivaaji, egɗ kadi mi huutortaako formaas kadi mi waɗata heen boor. \\
% ff & And I say use capsicum, tomatoes, \textbf{basil}, \textbf{lettuce}, green chilies, olives, etc. And I don’t use \textbf{formaldehyde} and I \textbf{make a bowl of it}. \\
% % source: Peape che aipuru ky'ỹi, tomate, sevoi, ajo, ky'ỹi hovy ha aceituna, ha ndaipurúi kesu tera kambyrova ipype. \\
% gn & Here I use onions, tomatoes, \textbf{sevoi}, garlic, green onions and olives, and I don't use cheese or \textbf{milk} in it. \\
% % source: हातूंत हांव ढब्बु मिरसांग, तोमाटां, कांदे, लसूण, हरव्यो मिरसांगो, ऑलिव्ह इत्यादी वापरता आनी चिज आनी बटर तातूंत घालिना. \\
% gom & I use dubbed chillies, tomatoes, onions, garlic, green chillies, olives, etc. and do not add cheese and butter. \\
% % source: Nangusarak ditoy iti sili, kamatis, sibuyas, bawang, berde a sili, olibo, ken dadduma pay ken saankayo a mangusar iti keso ken mantikilya ditoy. \\
% ilo & I used peppers, tomatoes, onions, garlic, green peppers, olives, etc. here and you do not use cheese and butter here. \\
% % source: Uani akoraakka paprikkat, tomatit, uanitsut, hvidløgit, chilit qorsorpaluttut olivennit il. il. punnilinngilakka immussualernangillu. \\
% kl & Here I am mixing peppers, tomatoes, onions, garlic, chilies, green olives, etc. I am not \textbf{punching} or \textbf{immussual}. \\
% % source: pa dis a yus pepe, tamatis, yabas, galik, grin chilis, oliv dem, etc. en no yus chis en bota de. \\
% kri & on this I use peppers, tomatoes, \textbf{yabas}, garlic, green chilies, olives, etc. and don't use cheese and butter there. \\
% % source: Hemi atan hi chuan capsicum, tomato, purun sen, purun var, hmarcha hring, leh olive te ka hmang a, mahse butter leh cheese ka hmang tello. \\
% lus & I used capsicum, tomatoes, red onion, \textbf{white onion}, green chilies, and olives, but I didn't use butter or cheese. \\
% % source: एकरा में शिमला मिर्च, टमाटर, प्याज, लहसुन, हरी मिर्च, जैतून इ सब के प्रयोग करै छिये आर एकरा में पनीर आर मखहनके उपयोग नै करे छिये | \\
% mai & It uses capsicum, tomatoes, onion, garlic, green chillies, olives and does not use cheese and butter. \\
% % source: মসিদা ঐহাক কেপ্সিকম, খামেন অশিনবশিং, তিলহৌশিং, চনম, মোরোক অতেকপশিং, চোরফোনশিং, অসিনচিংবা শিজিন্নৈ অমসুং মদুদা ঘীথী অমসুং মখন শিজিন্নদে। \\
% mni & In this I use capsicum, \textbf{khamen ashinbas}, \textbf{sesame seeds}, \textbf{chanam}, \textbf{morocco atakpas}, \textbf{chorfon}, etc. and do not use \textbf{ghee} and butter. \\
% % source: Ka gare ga se ke šomiša capsicum, tomati, eie, kaliki, pherefere ye tala, olifi bjalo le bjolo ebile ga ke šomiše tšhese le potoro ka gare. \\
% nso & In this I use capsicum, tomato, onion, garlic, green pepper, olives and so on and I don't use cheese and butter in it. \\
% % source: Kan keessatti qaaraa, timaatimii,qullubbii,baala zayitaa fikkf fayyadama.dabalataniis baaduu fi dhadhaa hin fayyadamu. \\
% om & In which he uses \textbf{curry}, tomatoes, \textbf{coconut}, olive \textbf{oil} etc. plus he does not use \textbf{bacon} and butter. \\
% % source: For this one, I use capsicum, tomatoes, onions, garlic, green pepper, olives, etc. and I no dey use cheese and butter for inside. \\
% pcm & For this one, I use capsicum, tomatoes, onions, garlic, green pepper, olives, etc. and I don’t use cheese and butter in it. \\
% % source: Kaypiqa curasun pimiento, tomates, cebollas, ajo, chiles verdes, aceitunas, etc. ichaqa manan churasunchu quesutpas nipas matequillata. \\
% qu & Here we will cure peppers, tomatoes, onions, garlic, green chilies, olives, etc. but we will not add cheese or \textbf{matequilla}. \\
% % source: अत्र अहं महामरीचिका,रक्तफलं,पलाण्डुः,लशुनं,हरीमरीचिका,जितवृक्ष इत्यादयः व्यवहारं करोमि अपि च दधिक एवं नवनीतम् अत्र व्यवहारं न करोमि। \\
% sa & Here I deal with great pepper, \textbf{red fruit}, \textbf{eggplant}, garlic, green pepper, olive \textbf{tree} etc. and I don't deal with yogurt and \textbf{fresh} here. \\
% % source: ኣብዚ ከም ካፕሲካም፥ ኮመደረ፥ ሽንጉርቲ፥ ጻዕዳ ሽንጉርቲ፥ ግሪንችሊ፥ፍረ ወይራ ወዘተ ይጥቀም። ኣጅቦን ጠስምን ከይትጥቀም። \\
% ti & Use ingredients like capsicum, tomato, \textbf{mushroom}, w\textbf{hite mushroom}, \textbf{grinchly}, \textbf{grapefruit} etc. Do not use \textbf{ajbon} and \textbf{sour cream}. \\
% % source: Eka leswi ndzi tirhisile capsium, matamatisi, tinyala, xinyalani, viriviri ra rihlaza, ntlhwari na swo fana na swonaa. naswona unga tirhisi chizi na botere u nga swi tirhisi \\
% ts & For this I used \textbf{capsium}, tomatoes, \textbf{lettuce}, \textbf{lentils}, green chilies, olives and the like.and don't use cheese and butter don't use them \\
% % source: te' je'ela' ku meyajten xa'ak', p'aak,cebolla,ajo, ya'ax iik,aceitunas,etc,ma' tu meyajten queso mix mantequilla. \\
% yua & here i use \textbf{mixture}, tomato,onion,garlic, \textbf{green beans},olives,etc,no cheese or butter. \\
% % source: 我加咗甜椒、蕃茄、洋蔥、大蒜、綠辣椒同橄欖等等，冇用到芝士同牛油。 \\
% yue & I added bell peppers, tomatoes, onions, garlic, green peppers and olives, etc., no cheese and butter. \\

% \hline
% \end{tabular}

% \caption{Translations of the sentence meaning "In this I use capsicum, tomatoes, onions, garlic, green chilies, olives, etc. and do not use cheese and butter in it." from various languages into English.}
% \label{tab:unmt_mistakes_capsicum}
% \end{table*}


% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline
% % source: Mepɛ sɛ meyɛ aboa kraman dakoro pɛ. \\
% ak & I want to be an animal dog for one day. \\
% % source: এদিনৰ বাবে মই কুকুৰ হ’ব বিচাৰো | \\
% as & I want to be a dog for one day. \\
% % source: Mallitua ma urupacha anuña  \\
% ay & Mallitua is a day dog \\
% % source: हम एक दिन खातिर कुत्ता बने के चाहत बाटीं। \\
% bho & I want to be a dog for a day. \\
% % source: A tun bɛ diya ne ye ka kɛ wulu he tile kelen. \\
% bm & I would love to be a dog he day. \\
% % source: आऊं इक ध्याड़े दे लेई कुत्ता बनना चैहंग। \\
% doi & I want to be a dog for a day. \\
% % source: އަހަރެން އެއްދުވަހަށް ކުއްތާއަކަށް ވާންބޭނުމެވެ. \\
% dv & I want to be a dog for a day. \\
% % source: Madi be manye avu ŋkeke ɖeka ko. \\
% ee & I would like to be a dog for just one day. \\
% % source: Aikosetene pe jaguarõ peteĩ ára pe. \\
% gn & I want to be the dog one day. \\
% % source: म्हाका एका दिसाखातीर कुत्रो जावचें आसा. \\
% gom & I want to be a dog for a day. \\
% % source: Kayatko ti agbalin nga aso iti maysa nga aldaw. \\
% ilo & I want to be a dog one day. \\
% % source: Ulloq ataaseq qimmiorusussinnaavunga. \\
% kl & I might want to be a dog one day. \\
% % source: a go want fo bi dog fo wan de. \\
% kri & I'd want to be a dog for a day. \\
% % source: Ni khat atan ui nih chhin ka chak. \\
% lus & I want to be a dog for a day. \\
% % source: होम एक दिन ले कुकुर बनब चाहिबै| \\
% mai & Home wants to be a dog for a day. \\
% % source: Nka rata go ba mpša letšatši le tee fela. \\
% nso & I would like to be a dog for just one day. \\
% % source: Guyyaa tokkof sareen ta'uu barbaada. \\
% om & I want to be a dog for a day. \\
% % source: I go like to be dog for 1 day. \\
% pcm & I would like to be a dog for 1 day. \\
% % source: Huk punchawllas allquman kutiyta munayman  \\
% qu & I wish I could go back to the dog one day \\
% % source: ንሓደ መዓልቲ ከልቢ ምኻን ይደሊ እየ። \\
% ti & I want to be a dog for a day. \\
% % source: ndzi nga lava ku va mbyana siku rin'we \\
% ts & i would like to be a dog one day \\
% % source: ust tin t'aan ka peek'aken jump'éel k'iin. \\
% yua & ust I liked it when I was a dog one day. \\
% % source: 我都想做一日狗仔。 \\
% yue & I want to be a day dog. \\
% \hdashline
% % source: Mbiɗa yiɗatno wonnde rawaandu fodde ñalawma gooto. \\
% ff & I would like to be a \textbf{raven} for a day. \\
% % source: ঐহাক নুমিৎ অমগী ওইনা হুই অমা ওইবা পাম্মি। \\
% mni & I want to be a \textbf{horse} for a \textbf{week}. \\
% % source: 595.अहं एकस्मिन् दिवसस्य कृते कुक्कुरः भवितुं इच्छामि। \\
% sa & I want to be a \textbf{puppy} for a day. \\
% \hline
% \end{tabular}

% \caption{Translations of the sentence meaning "I would want to be a dog for a day" from various languages into English.}
% \label{tab:unmt_mistakes_dogday}
% \end{table*}




% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline
% % source: Mɛbisa me kra no nsɛm bi fa nea ɔpɛsɛ ɔka kyerɛ no nti a dabiara ɔsu meaaw no. \\
% ak & I will ask my \textbf{soul} some questions about what she wants to tell her why every day she cries meaaw. \\
% % source: মই মোৰ মেকুৰীজনীক কিছুমান প্ৰশ্ন সুধিব বিচাৰো যে, সি মিয়াউৰ দ্বাৰা সদায় কি কৈ থাকিব খোঁজে | \\
% as & I want to ask my cat some questions about what he always wants to say by meow. \\
% % source: Nayaxa jist'asiristwa phisitujaruxa kunsañaj manpachituxa mararaw sasinxa \\
% ay & I would ask my cat what he wanted me \textbf{to do in the year} \\
% % source: हम आपन बिलाई से कुछ सवाल पूछे के चाहत बानी के ऊ हमेशा मियाऊँ करके हमरा से का कहे के कोशिश करेले। \\
% bho & I want to ask my cat a few questions about what he always tries to tell me by meowing. \\
% % source: Nbi na n'ka jakuma ɲininka a b'a fɛ ka min fɔ n'a ka ŋɛwu ye. \\
% bm & Nbi will ask my \textbf{jackal} what he means with his \textbf{scythe}. \\
% % source: आऊं अपनी बिल्ली थमां किश सोआल पूछगा जे ओह् म्हेशा मिआउ करिए कैह् आक्खने दी कोशश करदी ऐ। \\
% doi & I’ll ask my cat a few questions about what she’s always trying to say by meowing. \\
% % source: އަހަރެންގެ ބުޅާ މިއާއުކުރަމުން ބުނަންއުޅެނީ ކީކޭތޯ ދެނެގަތުމަށްޓަކައި ސުވާލުތަކެއް ކުރަމެވެ. \\
% dv & I ask questions to find out what my \textbf{dog} is saying. \\
% % source: Mabia nya aɖewo ku ɖe nu si wòdina be yeagblɔ hafi nɔ xɔxlɔ̃m ɣe sia ɣi ŋu. \\
% ee & I would ask some questions about what he meant before he was always hanging out. \\
% % source: Ma mi naamdo ulluundu am yoga e naamde batte hol ko o heewi etaade wiide mi e ŋeewaali \\
% ff & I will ask my \textbf{ulcer} some of the questions behind what he often tries to tell me \textbf{in a smile} \\
% % source: Che aporanduse che mbarakajape umi ñeporandu mba'epa ha'e he'ise chupe pe imbarakajarasẽpe. \\
% gn & I want to ask my \textbf{dog} questions about what he means to him \textbf{in his music}. \\
% % source: म्हाका म्हज्या माजराक कांय प्रस्न विचारचे आसात ते म्हणल्यार सद्दां मियाँव म्हूण तें म्हाका किदें सांगूक सोदता. \\
% gom & I want to ask my cat some questions about what he means to me by always being a meow. \\
% % source: Saludsudek ti pusak maipapan iti banag a kanayon a kayatna nga ibaga kenkuana babaen iti panagmeow. \\
% ilo & I ask my cat about something she always wants to tell her by meowing. \\
% % source: Qitsuutinga apeqqutinik apeqquteqarfigerusussinnaavara miaarveertuinnaleraangami suna oqaatigerusuttaraluarneraa. \\
% kl & I would like to ask my \textbf{husband} questions about what he meant when he was in the \textbf{miaarveer}. \\
% % source: a go aks mi pus bot wetin in bin de tray fo tel am wit in miowin. \\
% kri & I'll ask my cat about what he was trying to tell her with his \textbf{miowin}. \\
% % source: Ka zawhte hi a ngiau chang apianga a sawitum hi ka zawt thin. \\
% lus & I ask him what he means whenever he asks me. \\
% % source: होम आपन बिलाई से किछो सवाल पुछ्बैं की ओ हरदम हमरा मियांउ करके की बताबय के कोशिश कराइ छै| \\
% mai & Home ask your cat some questions about what he is always trying to tell me by meowing. \\
% % source: মিয়াও খোংলগা মহাক্না মঙোন্দা মতম চুপ্পদা করিগী মরমদা হায়নবা হোৎনরিবনো হায়না ঐহাক ঐহাক্কি হৌদোংদা ৱাহং খরা হংগনি। \\
% mni & I will ask \textbf{myself} a few questions about what he is always trying to tell me. \\
% % source: Ke tla botšiša katse yaka dipotšišo ka ga seo ka mehla e lekago go mmotša sona ka go lla. \\
% nso & I will ask my cat questions about what it always tries to tell her by \textbf{crying}. \\
% % source: Adurre koo hasofsiisu nan barbaada kan isheen yeroo hunda na sagalessitu maal akka jedhuu barbaadde. \\
% om & I want to talk to my \textbf{dog} about what she always wants to say when she \textbf{calls me}. \\
% % source: I go ask my cat question about wetin he dey always dey try to tell me when e dey meow. \\
% pcm & I will ask my cat a question about what he is always trying to tell me when he meows. \\
% % source: Misiyta tapuyta munayman imarayku ch'aqwan ima niwaytataq munan \\
% qu & I would like to ask my cat why he is \textbf{fighting} and what he means \\
% % source: 513.अहं मम मार्जारं केचित् प्रश्ना: पृच्छामि यत् स: सर्वदा मियाऊ मियाँऊ उक्त्वा किं वक्तुम् इच्छति। \\
% sa & I ask my cat some questions about what he always means when he says meow meow. \\
% % source: ናተይ ድሙ ኩሉግዜ ብክእለት ንዕኡ ንምንጋር ዝሙክሮ ነገር ሓደሓደ ጥያቀታት ይጥይቅ። \\
% ti & My cat always asks some questions about what I'm trying to tell him \textbf{skillfully}. \\
% % source: ndzi nga vutisa ximanga xa mina swivutiso swa leswaku xi ringeta ku vula ku yini loko xi ku meow \\
% ts & i can ask my cat questions about what he is trying to say when he meows at you \\
% % source: jéel in meyajtik wa jayp'éel k'áatchi' ti' in walak' miis yóosal le ba'ax u k'áat u ya'al chen jo'ok u t'aano'.  \\
% yua & I'll use a few questions on my cat about what he just started talking about. \\
% % source: 我會問我隻貓到底佢啲喵喵聲係想表達啲咩。 \\
% yue & I would ask my cat what his meows meant. \\

% \hline
% \end{tabular}

% \caption{....}
% \label{tab:unmt_mistakes_meow}
% \end{table*}



% mkdir /tmp/unmt

% copy TEST
%  for f in ` fu ls /cns/vz-d/home/translate-train/nmt_train/m4-ntl/data/ntl_eval_sets/rkv/decoded/aqtxl_glompitqafkkbdmanagedbystscy_en_fg3fm3mb4_spm_20211209-1657_productionized_00590000/*_m4_ntl_eval_set-test_rkv/output.rkv ` ; do lp=$(dirname $f | bsnm | sed 's/_m4.*//g'); echo $lp ; fu cp $f /tmp/unmt/${lp}_test.rkv; done

% copy DEV
%  for f in ` fu ls /cns/vz-d/home/translate-train/nmt_train/m4-ntl/data/ntl_eval_sets/rkv/decoded/aqtxl_glompitqafkkbdmanagedbystscy_en_fg3fm3mb4_spm_20211209-1657_productionized_00590000/*_m4_ntl_eval_set-dev_rkv/output.rkv ` ; do lp=$(dirname $f | bsnm | sed 's/_m4.*//g'); echo $lp ; fu cp $f /tmp/unmt/${lp}_dev.rkv; done

% function table_with_src () { ref="$1"; for f in `ls /tmp/unmt/*` ; do cat $f | sed "s/[a-z]\+=//g" | grep "$ref" | awk -v FS="\t" '{printf "%s & %s & %s \\\\\n\\hdashline\n", $4, $2, $1}'; done; }
% 
% function table_only_output () { ref="$1"; for f in `ls /tmp/unmt/*` ; do cat $f | sed "s/[a-z]\+=//g" | grep "$ref" | awk -v FS="\t" '{printf "%% source: %s \\\\\n%s & %s \\\\\n", $2, $4, $1}'; done; }


% \begin{table*}
% \centering
% \begin{tabular}{l p{0.80\linewidth}}
% \hline
% \hline
% sl & translation      \\
% \hline

% \hline
% \end{tabular}

% \caption{....}
% \label{tab:unmt_mistakes_lion}
% \end{table*}




==> tweet_tables.tex <==
% \newcommand{\inserterrorssinglewordsshort_tweet}{
% \begin{table}[H]
% \centering
% \small
% \begin{tabular}{ll|lll}
% \hline
% \hline
% sl    & tl & source     & translation \\
% \hline
% en & Krio & juvenile & \AS{pikin we n\m{o} rich 18 ia yet} \\
% en & Krio & notorious & \AS{pipul d\m{e}n we g\m{e}t badnem} \\
% en & Fulfulde & devices & ka\AS{\m{b}}ir\AS{\m{d}}e (dispositifs) \\
% % en & pcm & removes & \textbf{dey} remove  \\
% en & Nigerian Pidgin & blame  & blame wetin?  \\
% en & K'iche' & solved & xsol rij ri  \\
% \hline
% \end{tabular}

% \caption{Our models frequently displayed exceeding verbosity with single-word inputs. In some cases they would add extra definitions for words in parentheses or commas afterwards (top half of table). In other instances they added function words from that language after the translation (\textbf{boldface}), or gave whole definitions, as with Krio.}
% \label{tab:errors_singlewords_short}
% \end{table}
% }





% \newcommand{\insertunmterrorsmain_tweet}{
% \begin{table*}
% \centering
% % \scriptsize
% \fontsize{7.0pt}{9pt}\selectfont
% \begin{tabular}{p{0.41\linewidth}  p{0.55\linewidth}}
%  reference     & translation \\
% \hline \hline
% I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & 
% I think the \mistake{hyena}'s \mistake{hotter} than the \mistake{elephant}. \\
% \hdashline
% % \hdashline
% dI believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}.& I believe a \correct{lion} would be \correct{stronger} than a \mistake{miniature crocodile}. \\
% % \hdashline
% % source: নোংশা অমনা কৈ অমদগী হেন্না মপাঙ্গল কল্লি হায়বা ঐহাক থাজৈ। \\
% % mni & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}.& I believe a \mistake{snake} is \correct{stronger} than a \mistake{crocodile}. \\
% % \hdashline
% % source: मेरा मानना ऐ जे सीह् मिरग थमां जादा जोरदार हुंदा ऐ। \\
% % doi & I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & I believe \mistake{seizures} are \correct{more severe} than \mistake{epilepsy}. \\
% % \hdashline
% % source: Cikkumi mbaroodi ɓuri heewde doole e cewngu. \\
% % I believe a \textbf{lion} is \textbf{stronger} than a \textbf{tiger}. & I think a \mistake{rabbit} is \correct{stronger} than a \mistake{squirrel}. \\
% % \hdashline
% % \hline
% % source: অহানবা মচু অহুম অদুদি অঙাংবা, কোমলা মচু, অমসুং নাপু। \\
% % mni & The first three colors are \textbf{red}, \textbf{orange},and \textbf{yellow}. & The first three colors are \correct{red}, \mistake{yellow}, and \mistake{blue}. \\
% % \hdashline

% % source: Ñawpaq kimsa llimpikuna puka, nina puka, q'illu.  \\
% % qu &  The first three colors are \textbf{red}, \textbf{orange},and \textbf{yellow}. &The first three colors are \correct{red}, \mistake{fire red}, and \correct{yellow}. \\
% % \hdashline
% % source: प्रथमवर्णत्रयम् रक्त- पित - केशरी च अस्ति ।
% % sa &  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & The first three colors are \correct{red}, \mistake{yellow} and \mistake{saffron}. \\
% % \hdashline

% % source: mihlovo yi nharhu yo sungula i tshwuka, tshopi na xitshopana \\

% \hdashline

%  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & the first three colors are \correct{red}, \mistake{purple} and \mistake{pink} \\
% %  \hline
% % source: la yáax boono'obo' chaktako'ob,chakk'aank'an yéetel k'aank'an. \\
% % yua &  The first three colors are \textbf{red}, \textbf{orange}, and \textbf{yellow}. & the first colors are \correct{red}, \mistake{red} and \correct{yellow}. \\

% \hdashline
% In this I use \textbf{capsicum, tomatoes, onions, garlic, green chilies, olives}, etc. and do not use \textbf{cheese} and \textbf{butter} in it.  & Here I deal with \mistake{ greater marjoram, blood fruit, plantain, lassi, green marjoram, jujube}, etc., but I do not deal with \mistake{curd} and \mistake{yogurt}. \\

% % \hdashline

% \hdashline
% I would want to be a \textbf{dog} for a day.  & I want to be a \mistake{crocodile} just one day.   \\
% % \hdashline
% % ak & Sam and his best friend, Susy, were laying in the \textbf{meadow}.  & Sam and his best friend Susy were relaxing in the \textbf{abdomen}.   \\
% % \hdashline
% % \hline

% \hdashline
% I would ask my \textbf{cat} some questions about what he's always trying to tell \textbf{him} by \textbf{meowing}. & I will ask my \mistake{friend} some questions about why \mistake{she} is \mistake{crying}.\\
% % \hdashline
% % \hline

% % ak & my \textbf{dog} keeps me moving and enjoying life.  he is man's best friend. & my pet \mistake{cat} teaches me how to live a healthy lifestyle and enjoy being with people. \\

% % \hdashline
% % \hline
% % ak & I went to a \textbf{carnival} yesterday that was located in the middle of nowhere under a huge \textbf{red and white} \textbf{circular striped tent}  & I went to a \mistake{place of pleasure} in a desolate place, unknown to me, where there was a \mistake{parrot} that had a \mistake{golden-yellow} \mistake{coat} \\

% % \hdashline
% % \hline
% % ak & John was working in the \textbf{lighthouse} and went for a walk on the beach one \textbf{night}.    & John was working in the \mistake{synagogue} and he was sound asleep one \mistake{afternoon}. \\        

% % \hdashline
% % \hline

% \hdashline
% this is why \textbf{hair} turns \textbf{grey} with age.  & this is the reason why \mistake{ticks} change into \mistake{worms} after a certain period of time. \\

% % \hdashline
% % sa & I think \textbf{tomatoes} are a \textbf{vegetable}. & I think that \textbf{blood} is a \textbf{fruit} \\

% % \hdashline
% % \hline
% \hdashline
% my bad habit is that I \textbf{eat too much}.  &  My bad behaviour is that I \mistake{eat poison}. \\

% % \hdashline
% % \hline
% \hdashline
% \textbf{Dogs} are very intelligent animals, they understand very much about humans.   &  \mistake{Cockroaches} are extremely sharp minded animals, they know about humans correctly \\

% % \hdashline
% % \hline
% % sa & Susy loved her \textbf{space book} and would ask her parents to read it to her every \textbf{night}. & Susie loved her \mistake{newspaper}, and she asked her parents to read it to her in the \mistake{morning}.  \\

% % \hline
% \end{tabular}

% \caption{Examples of correct translations (\correct{blue}) and mistranslations (\mistake{orange}), illustrating the model's tendency to make mistakes on distributionally similar nouns.
% % Many of which involve substitutions of other nouns or verbs that may seem more likely in context, for instance translating the list of more western ingredients into a list of Indian ingredients when translating from Sanskrit. Others are mistakes on distributionally similar concepts, such as different times of day or colors. Yet others are simply baffling. Most of these examples are from the undifferentiated teacher model, not the fine-tuned or distilled models.
% }
% \label{tab:unmt_mistakes_full}
% \end{table*}
% % https://docs.google.com/document/d/1rFpb2RIzpmUtbak4_4NWOrCvx5A7q4L_pDhyw-r0C_A/edit#
% }
